Maximum Bipartite Matching in $n^{2+o(1)}$ Time via a Combinatorial Algorithm

Maximum bipartite matching (MBM) is a fundamental problem in combinatorial optimization with a long and rich history. A classic result of Hopcroft and Karp (1973) provides an $O(m \sqrt{n})$-time algorithm for the problem, where $n$ and $m$ are the number of vertices and edges in the input graph, respectively. For dense graphs, an approach based on fast matrix multiplication achieves a running time of $O(n^{2.371})$. For several decades, these results represented state-of-the-art algorithms, until, in 2013, Madry introduced a powerful new approach for solving MBM using continuous optimization techniques. This line of research led to several spectacular results, culminating in a breakthrough $m^{1+o(1)}$-time algorithm for min-cost flow, that implies an $m^{1+o(1)}$-time algorithm for MBM as well. These striking advances naturally raise the question of whether combinatorial algorithms can match the performance of the algorithms that are based on continuous techniques for MBM. A recent work of the authors (2024) made progress on this question by giving a combinatorial $\tilde{O}(m^{1/3}n^{5/3})$-time algorithm for MBM, thus outperforming both the Hopcroft-Karp algorithm and matrix multiplication based approaches, on sufficiently dense graphs. Still, a large gap remains between the running time of their algorithm and the almost linear-time achievable by algorithms based on continuous techniques. In this work, we take another step towards narrowing this gap, and present a randomized $n^{2+o(1)}$-time combinatorial algorithm for MBM. Thus in dense graphs, our algorithm essentially matches the performance of algorithms that are based on continuous methods. We also obtain a randomized $n^{2+o(1)}$-time combinatorial algorithm for maximum vertex-capacitated $s$-$t$ flow in directed graphs when all vertex capacities are identical, using a standard reduction from this problem to MBM.

==> APPX-almost-DAG.tex <==

\newpage
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
\section{Proof of \Cref{thm: almost DAG routing}}
\label{subsec: proof of DAG-like SSSP}
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------

\iffalse
\paragraph{Initial Transformation of  Edge Lengths.} We start by performing a simple transformation of the lengths of edges, whose goal is to ensure that $\Gamma\cdot \log n\leq d\leq \max\set{4n/\eps,4\Gamma\cdot \log n}$.
 
We perform the transformation in two steps. The first step is only performed if $d>\ceil{n/\eps}$. For every edge $e\in E(G)$, we let the new length  $\tilde \ell(e)$ be obtained by rounding the length $\ell(e)$ up to the next integral multiple of $\ceil{\eps d/n}$, and we set $\tilde d=(1+2\eps)d$. Consider any simple $s$-$t$ path $P$ in $G$. Since $|E(P)|\leq n$, we get that $\sum_{e\in E(P)}\ell(e)\leq \sum_{e\in E(P)}\tilde \ell(e)\leq 2\eps d+\sum_{e\in E(P)}\ell(e)$. Notice that, if $P$ is a simple $s$-$t$ path in $G$, with $\sum_{e\in E(P)}\tilde \ell(e)\leq (1+6\eps)\tilde d$, then $\sum_{e\in E(P)} \ell(e)\leq (1+10\eps)d$.
Moreover, if $G'$ is a subgraph that is obtained from $G$ by deleting some edges from it, and $G'$ does not contain an $s$-$t$ path $P$  with $\sum_{e\in E(P)}\tilde \ell(e)\leq \tilde d$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$, then $G$ may not contain an $s$-$t$ path $P$  with $\sum_{e\in E(P)}\ell(e)\leq d$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$. Therefore, we can now replace the lengths $\ell(e)$ of edges $e\in E(G)$ with new  lengths $\tilde \ell(e)$. The problem remains unchanged, except that now, in response to  $\pquery$, the algorithm needs to return a simple $s$-$t$ path $P$ of length at most $(1+6\eps)\td$. 

Since all edge lengths are now integral multiples of $\ceil{\frac {\eps d}{n}}$, we can divide the length of every edge $e$ by $\ceil{\frac {\eps d}{n}}$, obtaining a new length, that we still denote by $\ell(e)$, which remains an integer. We also update $\td$ by dividing its value by $\ceil{\frac {\eps d}{n}}$. This scaling of the lengths of edges and of parameter $d$ do not change the problem, but now we are guaranteed that $\td\leq 4n/\eps$. For convenience, we will call $\tilde d$ by $d$ from now on.

If $d\geq \Gamma\cdot \log n$ now holds, no further transformations are necessary, since we are now guaranteed that $\Gamma\cdot \log n\leq d\leq \max\set{4n/\eps,4\Gamma\cdot \log n}$. Assume now that $d<\Gamma\cdot \log n$.
Then we multiply the lengths of all edges by factor $\ceil{\frac{\Gamma\log n}{d}}$, and replace $d$ with value $d\cdot \ceil{\frac{\Gamma\log n}{d}}$; this transformation does not change the problem, but it ensures that $\Gamma\cdot \log n\leq d\leq 4\Gamma\cdot \log n$. From now on we assume that $\Gamma\cdot \log n\leq d\leq \max\set{4n/\eps,4\Gamma\cdot \log n}$ holds. The problem remains the same, except that now, in response to  $\pquery$, the algorithm needs to return a simple $s$-$t$ path $P$ of length at most $(1+6\eps)d$. 
\fi

\mynote{unlike the version of this theorem from SODA submission, we no longer assume that $d>\Gamma\cdot \log n$. This is because we don't want to scale edge lengths at the beginning of the algorithm, because it's convenient to preserve lengths of edges incident to $s$ as being $1$. Should recheck carefully that all calculations work without this assumption. The main reason I preferred to have $d>\Gamma\log n$ in the SODA version is because of the ceiling that we take e.g. in $\ell'(e)=\ell(e)+\eps\cdot \ceil{\frac{d}{\Gamma\cdot \log n}\cdot w(e)}$. If $d\ll \Gamma$, then this ceiling can be much larger than $d/\Gamma$.}

\paragraph{Modified Edge Lengths.}
We define, for every edge $e=(u,v)\in E(G)$, a \emph{modified edge length} $\ell'(e)$, as follows: $ {\ell'(e)=\ell(e)+\eps\cdot \ceil{\frac{d}{\Gamma\cdot \log n}\cdot w(e)}}$. Notice that, since $1/\eps$ is an integer, for every edge $e\in E(G)$, its modified length $\ell'(e)$ is an integral multiple of $\eps$. 
Additionally, if $e$ is an edge that is incident to $s$, then, since $w(e)=0$, $\ell'(e)=\ell(e)$ holds.
Throughout, for a pair of vertices $u,v$ in $G$, we denote by $\dist'(u,v)$ the distance from $u$ to $v$ in the current graph $G$, with respect to edge lengths $\ell'(\cdot)$. We need the following simple observation.

\begin{observation}\label{obs: short path translation}
	Assume that at time $\tau\in \tset$,  there is an $s$-$t$ path $P$ in $G$ with $\sum_{e\in E(P)}\ell(e)\leq d$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$. Then at time $\tau$, $\dist'(s,t)\leq (1+3\eps)\cdot d$.
\end{observation}
\begin{proof}
	For all $0\leq i\leq \ceil{\log n}$, let $E_i$ be the set of all edges $e\in E(P)$ with $w(e)=2^i$. Since $\sum_{e\in E(P)}w(e)\leq \Gamma$, for all such $i$, $|E_i|\leq \frac{\Gamma}{2^i}$. We now get that:
	
	\[\begin{split}
	\sum_{e\in E(P)}\ell'(e)&\leq \sum_{e\in E(P)}\left(\ell(e)+\frac{\eps\cdot d}{\Gamma\cdot \log n}\cdot w(e)+\eps\right )\\
	&\leq \sum_{e\in E(P)}(1+\eps)\ell(e)+\sum_{i=0}^{\ceil{\log n}}\sum_{e\in E_i}\frac{\eps\cdot d}{\Gamma\cdot \log n}\cdot 2^i\\
		&\leq (1+\eps) d+\sum_{i=0}^{\ceil{\log n}} |E_i|\cdot \frac{\eps\cdot d}{\Gamma\cdot \log n}\cdot 2^i\\
			&\leq  (1+\eps)\cdot d+\sum_{i=0}^{\ceil{\log n}} \frac{\Gamma}{2^i}\cdot \frac{\eps\cdot d}{\Gamma\cdot \log n}\cdot 2^i\\
			&\leq (1+3\eps)d.
	\end{split}\]
	(we have used the fact that $\ell(e)\geq 1$ for every edge $e\in E(G)$).
\end{proof}


Throughout the algorithm, we maintain, for every vertex $v\in V(G)$, an estimate $\tdist(v)$ on $\dist'(s,v)$. If $\tdist(v)>2d$ holds, we replace $\tdist(v)$ with $\infty$. Additionally, for every edge $e=(v,u)$, vertex $u$ is given an estimate $\tdist_u(v)$ on $\dist'(s,v)$ (that may be outdated). More specifically, if $w(e)=2^i$, then vertex $v$ only communicates its estimate $\tdist(v)$ to $u$ in increments of ${\eps^2\cdot \ceil{\frac{d\cdot 2^i}{\Gamma\cdot \log n}}}$ (it is this modification of the standard Even-Shiloach tree algorithm that leads to the faster total update time). In other words, every time $\tdist(v)$ passes a threshold of $ {z\cdot \eps^2\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}}$ for some integer $z$, vertex $v$ communicates its current estimate $\tdist(v)$ to $u$, and $\tdist_u(v)$ is replaced with this amount. 
Additionally, we maintain a directed tree $T\subseteq G$, that is rooted at vertex $s$, with all edges directed away from the root. The tree contains all vertices $v\in V(G)$ with $\tdist(v)\neq\infty$. Whenever we refer to lengths of paths or distances in the tree $T$, it is with respect to edge lengths $\ell'(e)$ for $e\in E(T)$.


\paragraph{Additional Data Structures.} In addition to the tree $T$, the estimates $\tdist(v)$ for vertices $v\in V$, and estimates $\tdist_u(v)$ for edges $(v,u)\in E$, we maintain the following data structures. For every vertex $v\in V$, we maintain a heap $H(v)$ that contains all vertices of $\set{u\in V\mid (u,v)\in E}$, with the key associated with each such vertex $u$ being $\tdist_v(u)+\ell'(u,v)$. Additionally, for all $0\leq i\leq \ceil{\log n}$, we maintain a set $U_i(v)$ of vertices, that contains every vertex $u\in V(G)$, such that there is an edge  $e=(v,u)$ with $w(e)=2^i$ in $G$.



\paragraph{Invariants.}
We ensure that, throughout the algorithm, the following invariants hold.

\begin{properties}{I}
	\item For every vertex $v$, the value $\tdist(v)$ is an integral multiple of $\eps$, and it may only grow over the course of the algorithm; the same holds for values $\tdist_u(v)$ for all edges $e=(v,u)$; \label{inv: estimates grow}
	\item If $e=(x,y)$ is an edge in the tree $T$, then vertex $x$ is the vertex with the lowest key $\tdist_y(x)+\ell'(x,y)$ in $H(y)$, and moreover $\tdist(y)=\tdist_y(x)+\ell'(x,y)$; \label{inv: keys via tree}
	\item For every edge $e=(u,v)$, if $w(e)=2^i$, then $\tdist(u)-\eps^2\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}\leq \tdist_v(u)\leq \tdist(u)$; \label{inv: updates of neighbors}

	\item For all $v\in V(G)$, if $\dist'_G(s,v)\leq 2d$, then $\tdist(v)\neq \infty$ and $\tdist(v)\leq \dist'(s,v)$; and\label{inv: dist estimate upper bound}
	\item For all $v\in V(G)$, $\tdist(v)\geq (1-\eps)\cdot \dist'(s,v)$ holds at all times; moreover, if $v\in V(T)$, then the length of the $s$-$v$ path in the current tree $T$ is at most $\frac{\tdist(v)}{1-\eps}$. \label{inv: dist estimate lower bound} 
\end{properties}





\paragraph{Initialization.}
At the beginning of the algorithm, we compute a shortest-path out-tree $T$ rooted at vertex $s$, with respect to edge lengths $\ell'(\cdot)$. For every vertex $v\in V$, we then set $\tdist(v)=\dist'(s,v)$ -- the distance from $s$ to $v$ in the tree $T$.
Next, we scan all vertices in the bottom-up order in the tree $T$. For each such vertex $v$, if $\tdist(v)>2d$, then we set $\tdist(v)=\infty$, and delete $v$ from the tree. For every edge $e=(v,u)\in E$, we  set $\tdist_u(v)=\tdist(v)$. Lastly, for every vertex $v\in V$, we initialize the heap $H(v)$ with the vertices of $\set{u\in V\mid (u,v)\in E}$, and the sets $\set{U_i(v)}_{0\leq i\leq \ceil{\log n}}$ of its out-neighbors.  It is easy to verify that the initialization can be performed in time $O(m\log m)$, and that all invariants hold at the end of initialization.


Recall that a vertex $v\in V(G)$ is considered uninteresting iff there is an edge $e=(s,v)$ in graph $G$. From the definition of the problem, in such a case, $w(e)=0$ and $\ell'(e)=\ell(e)=1$ must hold. 
At the beginning of the algorithm, if $v$ is an uninteresting vertex, then, since the length of every edge in $G$ is at least $1$, edge $(s,v)$ must lie in the tree $T$, and $\tdist(v)=1$ must hold. Moreover, for every edge $(u,v)\in E$ with $u\neq s$, $\tdist_v(u)+\ell'(u,v)>1$ must hold at the beginning of the algorithm. Since the values $\tdist_v(u)$ may not decrease throughout the algorithm, it is easy to verify that, as long as $v$ remains an uninteresting vertex,  edge $(s,v)$ must lie in the tree $T$, and $\tdist(v)=1$ must hold.



Next we describe the algorithms for handling each one of the three update types.

\paragraph{Algorithm for Handling Edge Insertion.}
Consider an edge insertion operation, where an edge $e=(u,v)$ of length $\ell(e)$ and weight $w(e)$ is inserted into $G$, and recall that $v$ is an uninteresting vertex. Recall that in this case, edge $(s,v)$ of length $1$ and weight $0$ each, must be present in the tree $T$, and $\tdist(v)=1$ must hold. We set $\tdist_u(v)=\tdist(v)=1$, and insert edge $e$ into the heap $H(v)$ with the key $\tdist_u(v)+\ell'(e)$. Additionally, if $w(e)=2^i$, then we insert vertex $v$ into set $U_i(u)$, if it does not lie in that set already. All these updates can be performed in time $O(\log n)$. Since $\ell(e)\geq 1$, while $\dist_G(s,v)=1$, it is easy to verify that the insertion of the edge $e$ into graph $G$ does not change the length of the shortest $s$-$x$ path of any vertex $x\in V(G)$, and it is immediate to verify that all invariants continue to hold after this update. The total time that the algorithm spends on edge-insertion updates is then bounded by $O(m\log n)$.



\paragraph{Algorithm for Handling Vertex Splits.}
Consider now a vertex split operation, in which we are given an interesting vertex $v\in V$, and 
 a collection $U=\set{u_1,\ldots,u_k}$ of new vertices that need to be inserted into $G$. Recall that we are also given a collection $E'$ of new edges that must be inserted into $G$, and for every edge $e\in E'$, we are given a length $\ell(e)$ and a weight $w(e)$. For each such edge $e\in E'$, either both its endpoints lie in $\set{u_1,\ldots,u_k, v}$; or one endpoint lies in $\set{u_1,\ldots,u_k}$, and the other in $V(G)\setminus\set{v,u_1,\ldots,u_k}$. In the latter case, if $e=(u_i,x)$, then edge $e'=(v,x)$ must currently lie in $G$, and both $w(e')=w(e)$ and $\ell(e')=\ell(e)$ must hold, so $\ell'(e')=\ell'(e)$. Similarly, if $e=(x,u_i)$, then edge $e'=(x,v)$ must currently lie in $G$, and both $w(e')=w(e)$ and $\ell(e')=\ell(e)$ must hold, so $\ell'(e')=\ell'(e)$.
 
 If $\tdist(v)\neq \infty$, then let $e=(x,v)$ be the unique edge that is incoming into $v$ in the tree $T$. We \emph{temporarily} insert, into set $E'$, edges $e_i=(x,u_i)$ with $\ell(e_i)=\ell(e)$ and $w(e_i)=w(e)$ for all $u_i\in U$.
 
 Our algorithm consists of two steps.
 In the first step,
we set, for every vertex $u_i\in U$, $\tdist(u_i)=\tdist(v)$. We then inspect the edges of $E'$ one by one. 
Consider any such edge $e=(a,b)$.

\begin{itemize}
\item If both endpoints of $e$ lie in $U\cup\set{v}$, then we set $\tdist_b(a)=\tdist(a)$, and update the corresponding heap $H(b)$ by inserting $a$ into it.
 
\item If the second endpoint $b$ of $e$ lies in $U$ and the first endpoint $a$ lies in $V(G)\setminus (U\cup\set{v})$, then edge $e'=(a,v)$ with $\ell'(e')=\ell'(e)$ must be present in $G$. In this case, we set $\tdist_b(a)=\tdist_v(a)$, and update heap $H(b)$ by inserting $a$ into it.

\item Similarly, if the first endpoint $a$ of $e$ lies in $U$, and the second endpoint $b$ lies in $V(G)\setminus (U\cup\set{v})$, then edge $e'=(v,b)$ with $\ell'(e')=\ell'(e)$ must be present in $G$. In this case, we set $\tdist_b(a)=\tdist_b(v)$, and update heap $H(b)$ by inserting $a$ into it.
\end{itemize}

Lastly, if $w(e)=2^i$, and $b\not \in U_i(a)$, then we insert $b$ into $U_i(a)$.
We also update the graph $G$ with the insertion of the vertices of $U$ and edges of $E'$.
 Notice that all these updates can be done in time $O((|U|+|E'|)\cdot \log m)$. 
 
The second step only needs to be executed if $\tdist(v)\neq\infty$. In this step we delete from $G$ the edges $e_1,\ldots,e_k$ that were temporarily inserted. Our data structure is then updated using the algorithm that we describe below, for handling edge-deletion updates.

We now establish that all invariants hold after the first step. 
Invariant \ref{inv: estimates grow} continues to hold, as we did not update any $\tdist(a)$ or $\tdist_b(a)$ estimates except for the newly inserted vertices. 



 In order to establish Invariant \ref{inv: keys via tree}, assume that $\tdist(v)\neq \infty$, and so edge $(x,v)$ lies in tree $T$. Observe that for every vertex $u_i\in U$, all vertices in $H(u_i)$ lie in $H(v)$, except possibly for the vertices of $\left(U\cup v\right )\setminus\set{u_i}$. But for every vertex $a\in \left(U\cup v\right )\setminus\set{u_i}$,  $\tdist(a)=\tdist(v)>\tdist(x)$ currently holds, so the key of such a vertex $a$ in the heap $H(u_i)$ is greater than or equal to $\tdist_{u_i}(a)= \tdist(v)=\tdist_{v}(x)+\ell'(x,v)=\tdist_{u_i}(x)+\ell'(x,u_i)$.
Since $u_i$ is connected to $x$ in the tree $T$, we get that Invariant \ref{inv: keys via tree} holds for $u_i$. Consider now any vertex $a\not\in U$, and assume that some edge $(b,a)$ lies in tree $T$. It is possible that we have inserted new vertices into $H(a)$: if an edge $e=(u_i,a)$ for some $u_i\in U$ lies in $E'$, then $u_i$ was inserted into $H(a)$. However, in this case, edge $e'=(v,a)$ with $\ell'(e')=\ell'(e)$ belonged to $G$ before the current update, and so $v$ already lied in $H(a)$.  Since $\ell'(e)=\ell'(e')$, and $\tdist_a(u_i)=\tdist_a(v)$, the key of $u_i$ in heap $H(a)$ is equal to the key of $v$, that remained unchanged. Therefore, Invariant \ref{inv: keys via tree} continues to hold.




We now turn to prove that Invariants \ref{inv: dist estimate upper bound} and  \ref{inv: dist estimate lower bound} continue to hold. Consider any vertex $a\in V(G)$. If $a\not \in U$, then it is easy to see that $\dist'(s,a)$ did not change after the current update. This is because for any path $P$ connecting $s$ to $a$ in the current graph $G$, we can obtain a path $P'$ connecting $s$ to $a$ in the original graph $G$, whose length with respect to the modified edge lengths $\ell'(\cdot)$ is no higher than that of $P$, by replacing every vertex of $U$ on $P$ with the vertex $v$. Moreover, path $P'$ still belongs to the current graph since we did not delete any vertices or edges during the current update. Since $\tdist(a)$ did not change, and the path connecting  $s$ to $a$ in $T$ did not undergo any changes either, both invariants continue to hold for $a$.

Assume now that $a\in U$. Let $P$ be the path connecting $s$ to $v$ in the current tree $T$. Since path $P$ did not change during the current update, from Invariant \ref{inv: dist estimate lower bound} , the length of this path is at most $\frac{\tdist(v)}{1-\eps}$. Notice that the last edge on this path is $e=(x,v)$, and recall that we have inserted an edge $e'=(x,a)$ into $G$, with $\ell'(e')=\ell'(e)$. By replacing edge $e$ with $e'$ on path $P$, we obtain a path $P'$, connecting $s$ to $a$, which is the unique $s$--$a$ path in tree $T$. Moreover, the length of $P'$ is equal to the length of $P$, which, in turn, is at most $\frac{\tdist(v)}{1-\eps}=\frac{\tdist(a)}{1-\eps}$. We conclude that $\dist'(s,a)\leq \frac{\tdist(a)}{1-\eps}$, establishing Invariant \ref{inv: dist estimate lower bound}  for vertex $a$.

In order to establish Invariant \ref{inv: dist estimate upper bound} for vertex $a$, let $Q$ be the shortest $s$-$a$ path in graph $G$, with respect to edge lengths $\ell'(\cdot)$. By replacing every vertex of $U$ on this path with vertex $v$, and removing loops, we obtain an $s$-$v$ path $Q'$ in $G$, whose length is no higher than the length of $Q$. Therefore, $\dist'(s,v)\leq \dist'(s,a)$. Since we set $\tdist(a)=\tdist(v)$, we get that, if $\dist'(s,a)\neq \infty$, then $\dist'(s,v)\neq \infty$, and $\tdist(a)=\tdist(v)\leq \dist'(s,v)\leq \dist'(s,a)$. We conclude that Invariants \ref{inv: dist estimate upper bound} and \ref{inv: dist estimate lower bound}  continue to hold.

It now remains to establish Invariant \ref{inv: updates of neighbors}. 
Consider any edge $e=(a,b)$. Notice that none of the values $\tdist(a)$ of vertices $a\in V$ changed, except for the vertices of $U$ that were inserted into $G$. Similarly, value $\tdist_b(a)$ remained unchanged, except if $a$ or $b$ (or both) are vertices that were newly inserted into $G$. In other words, we only need to consider edges $e=(a,b)\in E'$.





Let $e=(a,b)$ be any such edge. As before, we need to consider three cases. The first case happens if both $a,b\in U\cup \set{v}$. In this case, we set $\tdist(a)=\tdist(b)=\tdist(v)$ and $\tdist_b(a)=\tdist(v)$, so the invariant clearly holds. Assume now that $a\in U$ and $b\not\in U\cup\set{v}$. In this case, edge $e'=(v,b)$ was present in $G$ before the current update, and we set $\tdist(a)=\tdist(v)$ and $\tdist_b(a)=\tdist_b(v)$. Since the invariant held for edge $(v,b)$ before the current update, and since $w(a,b)=w(v,b)$, the invariant holds for edge $(a,b)$ at the end of the current update. Lastly, assume
that  $a\not\in U\cup\set{v}$ and $b\in U$. In this case, edge $(a,v)$ was present in $G$ before the current update, we set $\tdist_b(a)=\tdist_v(a)$ and $\tdist(a)$ remains unchanged. Since Invariant \ref{inv: updates of neighbors} held for edge $(a,v)$ at the beginning of the current update, it now holds for edge $(a,b)$ at the end of the update.



\paragraph{Algorithm for Handling Edge Deletions.}
We now provide an algorithm for updating the data structure with the deletion of some edge $e=(x,y)$. First, we may need to update the heap $H(y)$ (by either deleting $x$ from it, or changing the key of $x$ in the heap, if another $(x,y)$ edge is present in $G$). We may also need to delete $y$ from the appropriate set $U_i(x)$; all this can be done in time $O(\log n)$. If $e\not\in E(T)$, then no further updates are needed. We assume from now on that $e\in E(T)$. We start by deleting the edge $e$ from the tree $T$. 

Throughout the algorithm, we let $S$ be the set of vertices that are not currently connected to the tree $T$. We will not maintain the set $S$ explicitly, but it will be useful  for the analysis. At the beginning of the algorithm, the set $S$ contains all vertices that lied in the original subtree of $T$ rooted at $y$.

Our algorithm maintains a heap $Q$ that contains a subset of vertices of $S$ that need to be examined. The key associated with each vertex $v$ in $Q$ is $\tdist(v)$. We will ensure that the following invariant holds throughout the update:

\begin{properties}{J}
	\item If $a$ is the vertex with minimum value $\tdist(a)$ in $S$, then $a\in Q$ holds. \label{inv: smallest key in Q}
\end{properties}





We start with the heap $Q$ containing only the vertex $y$. Then we perform iterations, as long as $Q\neq\emptyset$. In order to execute a single iteration, we let $a$ be the vertex with smallest key $\tdist(a)$ in the heap $Q$, and we let $b$ be the vertex in heap $H(a)$ with smallest key.
If $\tdist(a)>2d$, then we set $\tdist(a)$ to $\infty$ and remove it from $Q$. We then set value $\tdist(x)$ of every vertex that is currently not connected to the tree $T$ to $\infty$ and terminate the update algorithm. We assume from now on that $\tdist(a)\leq 2d$. We then consider two cases.

The first case happens if $\tdist_a(b)+\ell'(b,a)\leq \tdist(a)$. Note that from Invariant \ref{inv: smallest key in Q}, vertex $b$ is currently attached to the tree $T$. In this case, we remove $a$ from $Q$ and attach it to the tree $T$ as a child of vertex $b$, via the edge $(b,a)$. Every vertex that is currently a descendant of $a$ also becomes automatically attached to the tree $T$ and removed from the set $S$; vertex $a$ itself is removed from $S$ as well.

Consider now the second case, where $\tdist_a(b)+\ell'(b,a)> \tdist(a)$. In this case, we increase $\tdist(a)$ by (additive) $\eps$, and keep vertex $a$ in the heap $Q$. Additionally, for every integer $0\leq i\leq \ceil{\log n}$, such that, for some integer $q$, threshold $q\cdot \eps^2\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}$ lies between the old and the new value of $\tdist(a)$, we consider every vertex $z\in U_i(a)$. We set $\tdist_z(a)=\tdist(a)$ and update the key of vertex $a$ in the heap $H(z)$. Additionally, if $z$ is currently a child-vertex of $a$, then we disconnect $z$ from $a$ (so it stops being a child of $a$), and add $z$ to the heap $Q$. This finishes the algorithm for handling edge-deletion updates. 


We start by showing that Invariant \ref{inv: smallest key in Q} holds throughout the algorithm.

\begin{claim}\label{claim: update property holds}
Invariant \ref{inv: smallest key in Q} holds throughout the algorithm.
\end{claim}
\begin{proof}
 Consider any time during the execution of the update procedure, and
let $a$ be the vertex of $S$ with smallest value $\tdist(a)$. Assume for contradiction that $a\not\in Q$. Observe first that, whenever the value $\tdist(v)$ changes for any vertex of $S$, we add $v$ to $Q$. Vertex $v$ can only leave the heap $Q$ when it is connected to the tree $T$, or if we set $\tdist(v)$ to $\infty$. Therefore, if $\tdist(a)$ ever changed over the course of the current update operation, then $a\in Q$ must hold. We assume from now on that value $\tdist(a)$ did not change over the course of the current update operation. Let $b$ be the parent-vertex of $a$ at the beginning of the current update. 
From our algorithm, if value $\tdist_b(a)$ ever changed over the course of the current update operation, then vertex $a$ was immediately added to heap $Q$. Therefore, value $\tdist_b(a)$ remained unchanged throughout the current update. 

Denote the weight of edge $(b,a)$ by $2^i$.
In the next observation, we show that, at the beginning of the current update procedure, $\tdist(b)$ was significantly lower than $\tdist(a)$. We will then conclude that $\tdist(b)$ must have grown significantly over the course of the current update procedure, and so $\tdist_b(a)$ must have grown as well, leading to a contradiction.


\begin{observation}\label{obs: small tdist of b}
At the beginning of the current update procedure, $\tdist(b)\leq \tdist(a)-\frac{\eps\cdot d}{\Gamma\cdot \log n}\cdot 2^{i-1}$ held.	
\end{observation}
\begin{proof}
	From Invariant \ref{inv: keys via tree}, at the beginning of the current update procedure, $\tdist(a)=\tdist_a(b)+\ell'(b,a)$ held.
Recall that $\ell'(b,a)=\ell(b,a)+\eps\cdot \ceil{\frac{d}{\Gamma\cdot \log n}\cdot 2^i}$. Moreover, from Invariant \ref{inv: updates of neighbors}, 
$\tdist_a(b)\geq \tdist(b)-\eps^2\cdot\ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$ held at the beginning of the procedure for processing the update.
Altogether, we get that, at the beginning of the current update procedure:

\[ \begin{split}
\tdist(a)&=\tdist_a(b)+\ell'(b,a)\\
&\geq \tdist(b)-\eps^2\cdot\ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}+\ell(b,a)+\eps\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}\\
&\geq \tdist(b)+\frac{\eps}{2}\cdot \ceil{\frac{d\cdot 2^i}{\Gamma\cdot \log n}}.
\end{split} \]
 
\end{proof}



Since vertex $a$ is the vertex of $S$ with smallest value $\tdist(a)$, either vertex $b$ is currently connected to the tree $T$, or the value $\tdist(b)$ has grown to become at least $\tdist(a)$ over the course of the current update procedure. 


If vertex $b$ remained attached to the tree $T$ over the course of the entire update procedure, then $a=y$ must hold; in other words, the edge that was deleted from $G$ is $(b,a)$. In this case, $a$ must have been added to $Q$ immediately at the beginning of the update procedure.
Otherwise, if vertex $b$ became attached to tree $T$ at any time during the update procedure, then each of its children was either attached to tree $T$ together with it, or added to $Q$. Since $a$ was never added to $Q$, it must be the case that $b$ was never attached to $T$, and so $\tdist(b)$ increased over the course of the current update procedure to become at least $\tdist(a)$. We claim that in this case, value $\tdist_b(a)$ must have been updated, leading to a contradiction.


Indeed,  from the above calculations, over the course of the current update operation, value $\tdist(b)$ must have increased by at least $\frac{\eps}{2}\cdot \ceil{\frac{d\cdot 2^i}{\Gamma\cdot \log n}}>\eps^2\cdot\ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$ units, and so value $\tdist_a(b)$ must have been updated, with vertex $a$ added to $Q$, a contradiction.
\end{proof}

We now verify that Invariants \ref{inv: estimates grow}--\ref{inv: updates of neighbors} continue to hold at the end of the update procedure, assuming that they held before the procedure started.


First, it is immediate to verify that values $\tdist(v)$ for vertices $v\in V$ and values $\tdist_u(v)$ for edges $(v,u)$ are never decreased, and they only increase in integral multiples of $\eps$, so Invariant \ref{inv: estimates grow} continues to hold.





Consider now some edge $e=(v,u)$ with $w(e)=2^i$. Notice that our algorithm updates $\tdist_u(v)$ to the current value $\tdist(v)$ whenever the latter passes a threshold that is an integral multiple of $\eps^2\cdot \ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$. This ensures that  $\tdist(u)-\eps^2\ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}\leq \tdist_v(u)\leq \tdist(u)$ holds at all times and establishes Invariant \ref{inv: updates of neighbors}.






In order to establish Invariant \ref{inv: keys via tree}, we consider the time when some vertex $v\in S$ reconnects to the tree $T$ via an edge $(u,v)$. Notice that at this time, if $z$ is a descendant of $v$, and no vertex on the $v$--$z$ path in $T$ was ever added to $Q$, then $z$ becomes connected to the tree $T$ as well. If $z'$ is the parent of $z$, then $\tdist_{z}(z')$ and $\tdist(z)$ remained unchanged over the course of the current update procedure, so $\tdist(z)=\tdist_z(z')+\ell'(z',z)$ continues to hold, and $z'$ is the vertex with the lowest key $\tdist_z(z')+\ell'(z',z)$ in the heap $H(z)$. Consider now vertex $v$ itself, and recall that it reconnects to the tree $T$ via the edge $(u,v)$. From our algorithm, it must be the case that $u$ is the vertex with the smallest key $\tdist_v(u)+\ell'(u,v)$ in $H(v)$, and moreover, 
$\tdist_v(u)+\ell'(u,v)\leq \tdist(v)$. It now remains to show that 
$\tdist_v(u)+\ell'(u,v)= \tdist(v)$. If the value $\tdist(v)$ never increased over the course of the current update procedure, then, since Invariant \ref{inv: keys via tree} held at the beginning of the update procedure, and since value $\tdist_v(u)$ may only grow, it is impossible that $\tdist_v(u)+\ell'(u,v)< \tdist(v)$. Therefore, in this case, $\tdist_v(u)+\ell'(u,v)= \tdist(v)$ must hold at the end of the update procedure. Assume now that the value $\tdist(v)$ grew over the course of the current update procedure, and let $\tau$ be the time when it was increased last (recall that each increase is by exactly $\eps$ units). Then, at time $\tau$, $\tdist_v(u)+\ell'(u,v)> \tdist(v)$ held. Since value $\tdist_v(u)$ may not decrease, and since $\tdist_v(u)+\ell'(u,v)$ is an integral multiple of $\eps$, it must be the case that $\tdist_v(u)+\ell'(u,v)= \tdist(v)$ at the end of the procedure.


In order to establish Invariant \ref{inv: dist estimate lower bound}, it is enough to show that, if $v\in V(T)$, then the length of the $s$-$v$ path in the current tree $T$ is at most $\frac{\tdist(v)}{1-\eps}$. The proof is by induction on the number of edges on the path. The claim clearly holds for the root vertex $s$. Let $j>0$ be any integer. We assume that the claim holds for all vertices $v\in V(T)$ for which the $s$-$v$ path in $T$ contains at most $j-1$ edges, and prove the claim for the case where the path contains $j$ edges. Consider now some vertex $v\in V(T)$, and let $P$ be the $s$-$v$ path in tree $T$, that contains $j$ edges. Let $u$ be the penultimate vertex on the path, and let $P'$ be the subpath of $P$ from $s$ to $u$. Then $\ell'(P)=\ell'(P')+\ell'(u,v)$. Let $i$ be the integer for which $w(u,v)=2^i$. From the induction hypothesis:

\[ \ell'(P')\leq \frac{\tdist(u)}{1-\eps}. \]

From Invariant \ref{inv: keys via tree},  $\tdist(v)=\tdist_v(u)+\ell'(u,v)$, and from Invariant \ref{inv: updates of neighbors}, $\tdist_v(u)\geq \tdist(u)-\eps^2\cdot\ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$. Altogether, we get that:

\[ \tdist(v)=\tdist_v(u)+\ell'(u,v)\geq \tdist(u)-\eps^2\cdot\ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}+\ell'(u,v)\geq (1-\eps)\cdot \ell'(P)-\eps^2\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}+\ell'(u,v). \] 

Since $\ell'(u,v)=\ell(u,v)+\eps\cdot \ceil{\frac{d\cdot 2^i}{\Gamma\cdot \log n}}$, we get that $\eps^2\cdot\ceil{\frac {d \cdot 2^i}{\Gamma\cdot \log n}}\leq \eps\cdot \ell'(u,v)$.
Altogether, we get that:

\[\tdist(v)\geq (1-\eps)\cdot \ell'(P)+(1-\eps)\ell'(u,v)=(1-\eps)\ell'(P),\]
as required.






Lastly, it remains to establish Invariant \ref{inv: dist estimate upper bound}. We first prove that, for every vertex $v$ that lies in the tree $T$,  $\tdist(v)\leq \dist'(s,v)$ holds. The proof is by induction on the number of edges on the shortest path (with respect to edge lengths $\ell'(\cdot)$) connecting $s$ to $v$. Induction base is when the path consists of a single vertex and no edges, so $v=s$, in which case the claim clearly holds.  Assume now that for some integer $j>0$, the claim holds for all vertices $v'$, for which there exists a shortest $s$-$v'$ path that contains fewer than $j$ edges. Consider some vertex $v$, such that there exists a shortest $s$-$v$ path $P^*$ (with respect to edge lengths $\ell'(\cdot)$), containing exactly $j$ edges. Let $u$ be the penultimate vertex on this path. From the induction hypothesis, $\tdist(u)\leq \dist'(s,u)$.
From Invariant \ref{inv: updates of neighbors}, $\tdist_v(u)\leq \tdist(u)$ holds, and, from Invariant \ref{inv: keys via tree}, $\tdist(v)\leq \tdist_v(u)+\ell'(u,v)$. Altogether, we get that $\tdist(v)\leq \tdist(u)+\ell'(u,v)\leq \dist'(s,u)+\ell'(u,v)=\dist'(s,v)$.
From the analysis of the algorithm it is easy to verify that, once $\tdist(v)$ reaches $2d$, it must be the case that $\dist'_G(s,v)\geq 2d$. This establishes Invariant \ref{inv: dist estimate upper bound}.


\paragraph{The Remainder of the Algorithm.} 
We continue the algorithm as long as $\tdist(t)\leq (1+3\eps)\cdot d$ holds. Once  $\tdist(t)> (1+3\eps)\cdot d$, we terminate the algorithm and return ``FAIL''. From Invariant  \ref{inv: dist estimate upper bound}, at this time $\dist'_G(s,t)>(1+3\eps)\cdot d$ must hold, and, from  \Cref{obs: short path translation}, graph $G$ may no longer contain an $s$-$t$ path $P$ with 
$\sum_{e\in E(P)}\ell(e)\leq d$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$.

Whenever a \pathquery arrives, we simply return the unique $s$-$t$ path $P$ in the current tree $T$, in time $O(|E(P)|)$. Since we are guaranteed that $\tdist(t)\leq (1+3\eps)\cdot d$, from Invariant \ref{inv: dist estimate lower bound}, $\sum_{e\in E(P)}\ell'(e)\leq 
\frac{\tdist(t)}{1-\eps}\leq (1+6\eps)d$, and so $\sum_{e\in E(P)}\ell(e)\leq \sum_{e\in E(P)}\ell'(e)\leq (1+6\eps)d$.




\paragraph{Analysis of Total Update Time.}
From the discussion above, the initialization takes time $O(m\log m)$, and the total time spent on edge-insertion and vertex-splitting updates (excluding the time spent on edge-deletion updates generated by vertex-splitting) is bounded by $O(m\log m)$.

We now turn to analyze the total time spent on edge-deletion updates. Consider the algorithm for processing the deletion of some edge $e=(x,y)$, that lies in the tree $T$. Initially, we add vertex $y$ to the heap $Q$, and then inspect this vertex. Whenever any vertex $v\in Q$ is inspected, we spend time $O(\log n)$ in order to decide whether it needs to be reconnected to the tree $T$, and, if $\tdist(v)$ increases, to calculate all indices $0\leq i\leq \ceil{\log n}$ for which an integral multiple of  $\eps^2\cdot \ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$ lies between the old and the new value $\tdist(v)$. We refer to this as \emph{vertex inspection time}. Additionally, for every integer $i$, for which an integral multiple of $\eps^2\cdot \ceil{\frac{ d \cdot 2^i}{\Gamma\cdot \log n}}$ lies between the old and the new value $\tdist(v)$, we consider every vertex $u\in U_i(v)$, update $\tdist_u(v)$, and possibly insert $u$ into $Q$. We call this procedure the \emph{update of out-neighbor $u$}, and the time required to perform this update, including the possible subsequent inspection of vertex $u$ when it becomes the lowest-key vertex in $Q$, is counted as the time required to update the out-neighbor $u$. However, if such a vertex $u$ is inspected several times (in which case its value $\tdist(u)$ grows with every inspection), then only the first inspection is charged to the time that $v$ spends on updating its out-neighbors. All subsequent times are charged to the increase of value $\tdist(u)$.

To summarize, the total update time due to edge deletion updates can be bounded as follows.

\begin{itemize}
	\item Whenever an edge $e=(x,y)$ is deleted from $G$, we may spend $O(\log m)$ time on inspecting vertex $y$. In total this may contribute up to $O(m\log m)$ to total update time.
	
	\item Whenever, for some vertex $a\in V$, $\tdist(a)$ increases, we may spend $O(\log m)$ time on a subsequent inspection of $a$. Since, when $\tdist(a)$ reaches $2d$, it is set to be $\infty$, and since every increase is by $\eps$ units, there can be at most $O(d/\eps)$ such increases for each vertex $a$. Notice that, if a vertex $v$ is an uninteresting vertex throughout the algorithm, then $\tdist(v)$ remains $1$ throughout the algorithm. Therefore, each vertex $v$ that is interesting at the end of the algorithm contributes at most $O(d/\eps)$ to the total update time through this process, while all other vertices contribute $0$. Overall, the time that the algorithm spends on vertex inspections due to the increase of $\tdist(a)$ of vertices $a\in V(G)$  is bounded by $O\left(\frac{n_I\cdot d\log m}{\eps}\right )$.
	
	\item The remaining time contribution is due to out-neighbor update operations. Consider a vertex $v\in V$.
	If $v$ is an uninteresting vertex throughout the algorithm, then $\tdist(v)$ remains unchanged throughout the algorithm, and $v$ never needs to update its out-neighbors. Assume now that, at the end of the algorithm, vertex $v$ is interesting, and consider an index $0\leq i\leq \ceil{\log n}$. From Property \ref{prop: few close neighbors}, the total number of vertices that at any given time lie in $U_i(v)$ is bounded by $2^{i+2}$. Whenever $\tdist(v)$ passes a threshold that is an integral multiple of 
 $\eps^2\cdot \ceil{\frac{d \cdot 2^i}{\Gamma\cdot \log n}}$, we need to update all vertices in $U_i(v)$. Since $\tdist(v)\leq 2d$, and $\tdist(v)$ only grows throughout the algorithm, there are in total at most $O\left(\frac{\Gamma\cdot\log n}{\eps^2\cdot 2^i}\right )$ such update operations of vertices in $U_i(v)$. Since each such update operation takes time $O(|U_i(v)|\cdot \log n)\leq O(2^i\cdot \log n)$, the total time required to update all out-neighbors of $v$ in $U_i(v)$ is bounded by $	O\left(\frac{\Gamma\cdot\log^2 n}{\eps^2}\right )$. Summing this over all indices $0\leq i \leq\ceil{\log m}$, the total time required for all updates of out-neighbors of $v$ is bounded by $O\left(\frac{\Gamma\cdot\log^3 m}{\eps^2}\right )$, and the total time required for all updates of out-neighbors of all vertices is bounded by $O\left(\frac{\Gamma\cdot n_I\cdot \log^3 m}{\eps^2}\right )$.
\end{itemize}

We conclude that the total update time of the algorithm is bounded by:

\[O\left(\frac{n_I\cdot d\log m}{\eps}+ m\log m + \frac{\Gamma\cdot n_I\cdot \log^3 m}{\eps^2}\right )\leq \tilde O\left(m+\frac{\Gamma\cdot n_I}{\eps^2}\right),  \]



since $d\leq  \Gamma\cdot \log^5n$ holds, from the problem definition.


A minor point that we have ignored so far is that, during the vertex-split updates, we may temporarily insert some edges into the graph, which are then immediately deleted, and such edges are not included in the total number of edges $m$ that ever belong to $G$. However, every edge that ever lied in $G$ contributes at most one such extra edge, so the total number of edges ever present in $G$ is at most $n+m\leq 2m$, and the above asymptotic bound on total update time remains unchanged.




==> SSSP-alg-also-previous.tex <==


\newpage

\section{From the $r$-Restricted \maintaincluster Problem to $(r+1)$-Restricted \stSP: Proof of \Cref{thm: from maintaincluster to roundandcut}}
\label{sec: SSSP alg}
The proof of \Cref{thm: from maintaincluster to roundandcut} follows from the following theorem:



\begin{theorem}\label{thm: from maintaincluster to stSP}
	Suppose there exists a randomized algorithm for the $r$-restricted \maintaincluster problem, for some parameter $r\geq 1$, that, given as input  an instance
	$(G,\beta,\Delta,\eta,d,N)$ of the problem, has running time at most: 
	$c_1\cdot W^0(G)\cdot (W^0(G)-|\beta'|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$, where $\beta'$ is the set $\beta$ at the end of the algorithm.  Then there is a randomized algorithm for the $(r+1)$-restricted \stSP problem, that, given an instance
	$(G,A,B,\Delta,\eta,N)$ of the problem with $|V(G)|=n$, has running running time at most $c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}$. 
\end{theorem}

Indeed, assume that there exists  a randomized algorithm for the $r$-restricted \maintaincluster problem, for some parameter $r\geq 1$, that, on input $(G,\beta,\Delta,\eta,d,N)$, has running time at most: 
$c_1\cdot  W^0(G)\cdot (W^0(G)-|\beta'|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$, where $\beta'$ is the set $\beta$ at the end of the algorithm.  From \Cref{thm: from maintaincluster to stSP}, there exists  a randomized algorithm for the $(r+1)$-restricted \stSP problem, that, on input $(G,A,B,\Delta,\eta,N)$ with $|V(G)|=n$, has running running time at most $c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}$.  From \Cref{thm: oracle to routing}, there exists a randomized algorithm for the $(r+1)$-restricted \routeandcut problem, that, on input $(G,A,B,\Delta,\eta)$ with $|V(G)|=n$, has running time is at most: 

\[\begin{split}
&O\left(c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}\right )+O(n\cdot(n-|B|))\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \leq c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+8c_2},
\end{split}\]

since $c_2$ is a sufficiently large constant.


From now on we focus on the proof of \Cref{thm: from maintaincluster to stSP}. We denote the randomized algorithm for the $r$-restricted \maintaincluster problem from the theorem statement by $\aset$. 




We denote the input to the $(r+1)$-restricted \stSP problem by $(G,A,B,\Delta,\eta,N)$, where $G=(L,R,E)$ is an $n$-vertex  well-structured graph, $A$ and $B$ are two disjoint subsets of vertices of $G$, and $N\geq n$, $\Delta \geq 1$, and $1\leq \eta \leq \Delta$ are parameters. Recall that no regular edge of $G$ connects a vertex of $A$ to a vertex of $B$, $\Delta\leq n-|B|$, $|E|\leq O(n\cdot (n-|B|))$,  and $\frac{(n-|B|)\cdot \eta}{\Delta}\leq 2\cdot 2^{(r+1)\sqrt{\log N}}$ hold.

Recall that, as the algorithm progresses, we maintain lengths $\ell(e)$ for edges $e\in E(G)$, and, additionally, some vertices may leave the sets $A$ and $B$. Since the number of iterations is bounded by $\Delta$, at most $\Delta$ vertices may be deleted from $A$ and from $B$.
For convenience, we denote by $A^0$ and $B^0$ the initial sets $A$ and $B$, respectively, to distinguish them from the sets that are maintained during the algorithm.


Note that we can assume that $N$ is greater than a sufficiently large constant, so that, for example, $N>2^{2^{c_2}}$ holds. Indeed, if this is not the case, then, from \Cref{thm: simple stSP}, we obtain a determinisic algorithm that solves the input instance of \stSP in time:


\[
\begin{split}
O\left(n\cdot(n-|B^0|)\cdot \frac{(n-|B^0|)\cdot \eta}{\Delta}\cdot \log^6 N\right )&\leq O\left(n\cdot(n-|B^0|)\cdot N\cdot \log N\right )
\\&\le c_1\cdot n\cdot (n-|B^0|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2},
\end{split}\]

since $n\leq N\ll c_1$, and $\eta\leq \Delta$ (recall that, by definition, $c_1\gg c_2$ holds). Therefore, we assume from now on that $N$ is sufficiently large.


Throughout the algorithm, we use the parameter  $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
We let $H$ be the graph that is obtained from $G$, by adding a source vertex $s$, that connects to every vertex $a\in A$ with a length-$0$ edge, and a destination vertex $t$, to which every vertex $b\in B$ connects with a length-$0$ edge. If an edge $e\in E(G)$ is a special edge for graph $G$, then $e$ remains a special edge for $H$. All other edges of $H$, including edges incident to $s$ and $t$, are called regular edges.
For every edge $e\in E(G)$, its length in $H$ remains the same as in $G$, so for convenience, we denote the length of every edge $e\in E(H)$ by $\ell(e)$.

Recall that, at the beginning  of the algorithm, for each edge $e\in E(H)$, its length $\ell(e)$ is set as follows: if $e$ is a regular edge, then $\ell(e)=0$, and if $e$ is a special edge, then $\ell(e)=1$. 
 We start by setting $\qset=\emptyset$, and then perform at most $\Delta$ iterations. In every iteration, the algorithm must do one of the following:


\begin{properties}{R}
	\item either return FAIL;\label{outcome: fail}

	\item or return a simple $s$-$t$ path $P$ of length at most $\Lambda$ in the current graph $H$, such that $P$ contains exactly one vertex of $B$ -- the penultimate vertex on the path; \label{outcome:path}
	
		\item or compute an assignment $\ell'(e)\geq 0$ of lengths to all edges $e\in E(H)$, such that, if we denote by $E^*$ the set of all edges of $G$ with both endpoints in $B$, then $\sum_{e\in E(H)}\ell'(e)\leq \frac{\Lambda\cdot \Delta}{\eta \log^4n}+\sum_{e\in E(H)\setminus E^*}\ell(e)$; the length $\ell'(e)$ of every edge $e$ that is incident to $s$ or to $t$ is $0$; and the distance from $s$ to $t$ in $H$, with respect to edge lengths $\ell'(\cdot)$, is at least $\frac{\Lambda}{32}$;  \label{outcome: cut}
\end{properties}

Note that, if the algorithm returns assignments of lengths $\ell'(e)$ to edges $e\in E(H)$ as in Outcome \ref{outcome: cut}, then these assignments of edge lengths define a modified cut-witness for $G$ (see \Cref{def: mod cut-witness}). In this case, the algorithm terminates, and  returns the  lengths $\ell'(e)$ of all edges $e\in E(H\setminus\set{s,t})$. Slightly abusing the notation, for the sake of simplicity, we will call an assignment of lengths $\ell'(e)$ to the edges $e\in E(H)$ as  described in Outcome \ref{outcome: cut} a \emph{cut-witness}. 

If the algorithm returns an $s$-$t$ path $P$ as in Outcome \ref{outcome:path}, then $P\setminus\set{s,t}$ is a modified acceptable path for $G$ (see \Cref{def: mod acceptable path}). To simplify the notation, we say that a path $P$ described in  Outcome \ref{outcome:path} is an \emph{acceptable path}. If the algorithm returns an acceptable path $P$, then we let $P'=P\setminus\set{s,t}$, and we let $a\in A$, $b\in B$ be the endpoints of path $P'$. We remove $a$ from $A$ and $b$ from $B$, add $P'$ to $\qset$, and delete the edges $(s,a)$ and $(b,t)$ from $H$. Additionally, the lengths of some of the special edges on $P$ may be doubled; we assume that the algorithm receives the list of all such edges. 

From the problem definition, for every special edge $e\in E(H)$, the length of $e$ is doubled once $e$ participates in exactly $\eta$ paths that the algorithm returned since the last time the length of $e$ was doubled, or since the beginning of the algorithm -- whatever happened last.

Lastly, in the case of Outcome \ref{outcome: fail}, we terminate the algorithm and return ``FAIL'', but we require that the probability that the algorithm ever returns ``FAIL'' is bounded by $\frac{1}{2}$.



\subsection*{Bounding the Largest Total Length of Edges and Some Useful Inequalities}

Let $E^{\spec}$ denote the set of all special edges in graph $G$, and let $E^*\subseteq E^{\spec}$ be the subset of edges $e\in E^{\spec}$, such that, at the end of the algorithm, both endpoints of $e$ lie in $B$. For each edge $e\in E^{\spec}$, let $\ell^*(e)$ be the length of $e$ at the end of the algorithm. In the next simple observation we bound $\sum_{e\in E^{\spec}}\ell^*(e)$.



\begin{observation}\label{obs: bound edge lengths}
For every edge $e\in E^*$, $\ell^*(e)=1$, and	$\sum_{e\in E^{\spec}}\ell^*(e)\leq n+2(n-|B^0|)\log^5n$. 
\end{observation} 
\begin{proof}
In order to prove the first assertion, recall that, if $P$ is an $s$-$t$ path in graph $H$ that our algorithm ever returned as part of Outcome \ref{outcome:path}, then $P$ may only contain a single vertex of $B$, so in particular, $E^*\cap E(P)=\emptyset$. Therefore, if $e\in E^*$ is an edge whose both endpoints lie in $B$ at the end of the algorithm, then, at the beginning of the algorithm, we set $\ell(e)=1$, and the length of $e$ is never doubled over the course of the algorithm, so $\ell^*(e)=1$ holds. We now turn to prove the second assertion.
	
\iffalse
Notice that, if an edge $e\in E^{\spec}$ never belonged to $H$, then $\ell^*(e)=0$ holds. Let $E'\subseteq E^{\spec}$ be the set of edges that belong to $H$ at the end of the algorithm, and, for each edge $e\in E'$, let $\ell^0(e)$ be the length of $e$ when it was first inserted into $H$. Note that initially, $H$ may contain at most $(n-|B^0|)$ special edges, since every vertex of $G$ is incident to at most one special edge, and edges with both endpoints in $B^0$ do not lie in the initial graph $H$. The initial length of each such special edge is $1$. Additionally, over the course of $\Delta$ iterations, at most $\Delta$ new vertices are deleted from $B$, and so at most $\Delta$ new special edges are inserted into $H$. Each such edge is assigned length $\ceil{\frac{\Lambda}{\eta}}\leq \frac{2\Lambda}{\eta}$ when it is inserted. Therefore:

\[ \sum_{e\in E'}\ell^0(e)\leq (n-|B^0|)+\frac{2\Lambda\Delta}{\eta}\leq 3(n-|B^0|)\log^5n. \]

since $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
\fi


Recall that, at the beginning of the algorithm, we set the length of every special edge to $1$.
Let $E'\subseteq E^{\spec}$ denote the subset of edges $e\in E^{\spec}$ with $\ell^*(e)>1$. Clearly: 


\[\sum_{e\in E^{\spec}}\ell^*(e)\leq 	|E^{\spec}|+\sum_{e\in E'}\ell^*(e)\leq  n+\sum_{e\in E'}\ell^*(e).\]

Let $q$ be the total number of iterations Algorithm \algmwu, so $|\qset|=q$ holds, and let $\qset=\set{P_1,\ldots,P_q}$, where the paths are indexed in the order in which they were added to $\qset$. For all $1\leq i\le q$, let $C_i$ denote the length of path $P_i$ when it was added to $\qset$. Clearly, $C_i\leq \Lambda$, and $\sum_{i=1}^qC_i\leq q\cdot \Lambda$.

Consider now some edge $e\in E'$, and assume that $\ell^*(e)=z$. Recall that $\ell(e)$ was doubled at least once during the algorithm. Let $\tau$ be the last time when the length of $e$ was doubled. Then, prior to time $\tau$, there were at least $\eta$ iterations $i$, during which the path $P_i$ that was added to $\qset$ contained $e$, and the length of $e$ during the corresponding iteration was $\frac{z}{2}$. In other words, edge $e$ contributes at least $\frac{z\eta}{2}=\frac{\ell^*(e)\eta}{2}$ to $\sum_{i=1}^qC_i$.
Overall, we get that:

\[\sum_{e\in E'}\ell^*(e)\leq \frac{2\sum_{i=1}^qC_i}{\eta}\leq \frac{2q\Lambda}{\eta}\leq  \frac{2\Delta\Lambda}{\eta}\leq 2(n-|B^0|)\cdot \log^5n,\]

since $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
Altogether, we get that:

\[\sum_{e\in E^{\spec}}\ell^*(e)\leq n+\sum_{e\in E'}\ell^*(e)\leq n+2(n-|B^0|)\log^5n.\]
\end{proof}

\iffalse
	Recall that, at the beginning of the algorithm, the length $\ell(e)$ of every special edge is set to $1$, and so $\sum_{e\in E^{\spec}}\ell(e)\leq n$ holds at the beginning of the algorithm. From Requirement \ref{oracle-prop: small length growth}, the total increase in $\sum_{e\in E^{\spec}}\ell(e)$ over the course of the process described above is bounded by:
	
	\[\frac{\Delta \cdot \Lambda\cdot \log^{\hat c}n}{\eta}\leq n\cdot (\log n)^{\hat c+5},\]
	
	since $\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$. Altogether, we get that $\sum_{e\in E^{\spec}}\ell^*(e)\leq n+n\cdot (\log n)^{\hat c+5}\leq 2n\cdot (\log n)^{\hat c+5}$.
\end{proof}
\fi

Throughout the algorithm, we will use a parameter $\highlightf{N'=\max\set{N,8n\cdot \log^5n}}$. Let $\tau$ be any time in the algorithm's execution, and let $H'$ be any subgraph of $H\setminus\left (\set{s,t}\right )$ that is a perfect well-structured graph. Recall that the weight of every vertex $v\in V(H')$ is the length of the unique special edge incident to $v$. From \Cref{obs: bound edge lengths}, the total weight of all vertices of $H'$ must be bounded by $N'$. Notice also that, since $N\geq n$, we get that $N'\leq 8N\log^5n\leq N\log^6N$. It is then easy to see that: 

\begin{equation}\label{eq: bound on log n'}
\log N'\leq \log N+6\log\log N\leq \left(1+\frac{1}{64c_2r}\right)\log N,
\end{equation}

since $r\leq \sqrt{\log N}$ and $N$ is large enough. Additionally, $\sqrt{\log N'}\leq \sqrt{\log N+6\log\log N}\leq \sqrt{\log N}+\sqrt{6\log\log N}$. Therefore:

\begin{equation}
2^{\sqrt{\log N'}}\leq 2^{\sqrt{\log N}}\cdot 6\log N\leq 2^{2\sqrt{\log N}}.\label{eq: bound on N'}
\end{equation}

We will use these facts later.



The description of our algorithm for the $(r+1)$-restricted \stSP problem consists of two parts. In the first part, we provide an algorithm for maintaining an \ATO for graph $H$. This algorithm in turn exploits algorithm $\aset$ for the $r$-restricted \maintaincluster problem. In the second part, we use the algorithm from \ref{thm: almost DAG routing} for the \DLSSSP problem on the corresponding contracted graph.
\newpage



\input{SSSP-part1}
%\input{SSSP-bound-weights}
\input{SSSP-runtime-part1}
\input{SSSP-bound-bad-edges}
%\input{SSSP-previous-stuff}
\input{SSSP-part2}
\input{SSSP-completing-alg}



%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%Leftovers from here on
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================

\iffalse

\paragraph{Hidden Edges and Graph $H$.}
Our algorithm will work with a graph $H$, that we define next. Before we do so, we need to define a dynamic subset $E_{\hidden}$ of edges of $G$, that we refer to as \emph{hidden} edges: these edges will be ignored by our algorithm, in order to ensure its efficiency.

\begin{definition}[Hidden Edges]
	The set $E_{\hidden}\subseteq E(G)$ of hidden edges contains  every edge $e=(u,v)$, such that either (i) $u$ and $v$ both lie in $B$; or (ii) $v\in B$ and $e$ is a special edge of $G$.
\end{definition}

We denote by $E^0_{\hidden}$ the set $E_{\hidden}$ at the beginning of the algorithm. Clearly, as the algorithm progresses, edges may be removed from $E_{\hidden}$, but no new edges may join this set. We emphasize that our algorithm does not compute the set $E_{\hidden}$ of edges explicitly, and it is only used for the analysis.


Our algorithm explicitly maintain a graph $H$, that is obtained from $G\setminus E_{\hidden}$, by adding a source $s$, that connects to every vertex of $B$, and a destination vertex $t$, to which every vertex of $A$ are connected. If $e\in E(G)\setminus E_{\hidden}$ is a special edge for graph $G$, then we say that $e$ is a special edge for $H$; all other edges of $H$, including those incident to $s$ and $t$, are regular edges for $H$. 
We denote by $H^0$ the graph $H$ at the beginning of the algorithm.

Note that, given the input graph $G$ in the adjacency-list representation, we can construct graph $H^0$ explicitly in time $O(n\cdot (n-|B^0|))$. Subsequently, whenever a vertex $a\in A$ is deleted from set $A$, we simply delete the edge $(a,t)$ from $H$. Whenever a vertex $b\in B$ is deleted from $B$, we first insert all edges of $E^{\hidden}$ that are incident to $v$ (except for a special edge $(v,u)$ with $u\in B$, if such an edge exists). Since at most $\Delta$ vertices may be deleted from each of the sets $A$, $B$ over the course of the entire algorithm, we get that the total number of edges that are ever present in $H$ is bounded by $O(n\cdot (n-|B^0|)+n\cdot \Delta)\leq O(n\cdot(n-|B^0|))$, and graph $H$ can be maintained explicitly, throughout  the algorithm, in time $O(n\cdot (n-|B^0|))$.
%Throughout the algorithm, we denote by $E_{\hidden}\subseteq E(G)$ the set of all edges $e\in E(G)\setminus E(H)$; for each such edge $e=(u,v)$, $v\in B$ must hold, and we denote by $E^0_{\hidden}$ the initial set of such edges. We also denote by $H^0$ the graph $H$ at the beginning of the algorithm.


\paragraph{A Partition $(U,U')$ of $V(H)$.}
Throughout the algorithm, we let $U\subseteq V(H)$ be the set of vertices of $H$ that contains $s,t$, and all other vertices $v\in V(H)$, such that no special edge is incident to $v$ in $H^0$.
Notice that it is possible that a vertex $v$ lies in $U$, and yet some special edge $e$ is incident to $v$ in $G$, if $e\in E_{\hidden}$, since such an edge $e$ does not lie in $H^0$). We also denote $U'=V(H)\setminus U$. The partition $(U,U')$ of $V(H)$ remains unchanged throughout the algorithm, even though some special edges incident to vertices of $U$ may be subsequently inserted into $H$. We note that vertices of $B$ may lie in $U$ and in $U'$.
We need the following simple observation.

\begin{observation}\label{obs: properties of U}
	Throughout the algorithm, $H[U']$ is a perfect well-structured graph. Moreover, no edge with both endpoints in $U'$ is ever inserted into $G$. Lastly, $|U'|\leq 2(n-|B^0|)$ holds.
\end{observation}
\begin{proof}
	We start by proving the second assertion. The only edges that may be inserted into $H$ over the course of the algorithm are edges of $E^0_{\hidden}$. Consider any such edge $e=(u,v)$, and assume for contradiction that both $u,v\in U'$. Assume first that $e$ is a regular edge. Then, from the definition of the set $E_{\hidden}$ of edges, $u,v\in B^0$ holds. Moreover, since edge $e$ is regular, $u\in L$ and $v\in R$ holds. Since $u\in U'$, there must be a special edge $e'=(x,u)$ in graph $H^0$. But, from the definition of the set $E_{\hidden}$ of edges, $e'\in E_{\hidden}$ holds, so $e'\not\in E(H^0)$, a contradiction. Consider now the case where $e$ is a special edge. Then, since $e$ is the only special edge incident to both $u$ and $v$ in $G$, and $e\in E_{\hidden}$, it is impossible that $u,v\in U'$. 
	
	In order to prove the first assertion, observe that, throughout the algorithm, $H[U']\subseteq G$ holds, so $H[U']$ is a well-structured graph. Moreover, at the beginning of the algorithm, every vertex $v\in U'$ is incident to some special edge of $G$, whose other endpoint must also lie in $U'$. Therefore, $H^0[U']$ is a perfect well-structured graph. As the algorithm progresses, no edges may be inserted into $H[U']$, and no edges may be deleted from $H[U']$ (since the only edges that may be deleted from $H$ are the edges that are incident to $s$ and to $t$). Therefore, $H[U']$ remains a perfect well-structured graph.
	
	In order to prove the third assertion, observe that for every vertex $v\in U'$, either $v\not\in B^0$, or there is a special edge that is incident to $v$, whose other endpoints lies in $V(G)\setminus B^0$. The cardinality of each of these two sets of vertices is bounded by $n-|B^0|$, so $|U'|\leq 2(n-|B^0|)$.
\end{proof}

%Note that $H^0[U']$ is a perfect well-structured graph, and, since no special edges are ever deleted from $H$, $H[U']$ remains a perfect well-structured graph throughout the algorithm. If a vertex $v\in B$ belongs to the set $L$, and a special edge $e$ is incident to $v$ in $G$, then $e\in E^0_{\hidden}$ must hold, as edge $e$ must enter $v$. Therefore, $v\in U$ must hold. On the other hand, a vertex $v\in B\cap R$ may lie in $U$ or in $U'$.
\fi

==> SSSP-alg-previous.tex <==


\newpage

\section{From the $r$-Restricted \maintaincluster Problem to $(r+1)$-Restricted \stSP: Proof of \Cref{thm: from maintaincluster to roundandcut}}
\label{sec: SSSP alg}
The proof of \Cref{thm: from maintaincluster to roundandcut} follows from the following theorem:



\begin{theorem}\label{thm: from maintaincluster to stSP}
	Suppose there exists a randomized algorithm for the $r$-restricted \maintaincluster problem, for some parameter $r\geq 1$, that, given as input  an instance
	$(G,\beta,\Delta,\eta,d,N)$ of the problem, has running time at most: 
	$c_1\cdot W^0(G)\cdot (W^0(G)-|\beta'|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$, where $\beta'$ is the set $\beta$ at the end of the algorithm.  Then there is a randomized algorithm for the $(r+1)$-restricted \stSP problem, that, given an instance
	$(G,A,B,\Delta,\eta,N)$ of the problem with $|V(G)|=n$, has running running time at most $c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}$. 
\end{theorem}

Indeed, assume that there exists  a randomized algorithm for the $r$-restricted \maintaincluster problem, for some parameter $r\geq 1$, that, on input $(G,\beta,\Delta,\eta,d,N)$, has running time at most: 
$c_1\cdot  W^0(G)\cdot (W^0(G)-|\beta'|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$, where $\beta'$ is the set $\beta$ at the end of the algorithm.  From \Cref{thm: from maintaincluster to stSP}, there exists  a randomized algorithm for the $(r+1)$-restricted \stSP problem, that, on input $(G,A,B,\Delta,\eta,N)$ with $|V(G)|=n$, has running running time at most $c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}$.  From \Cref{thm: oracle to routing}, there exists a randomized algorithm for the $(r+1)$-restricted \routeandcut problem, that, on input $(G,A,B,\Delta,\eta)$ with $|V(G)|=n$, has running time is at most: 

\[\begin{split}
&O\left(c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2}\right )+O(n\cdot(n-|B|))\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \leq c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+8c_2},
\end{split}\]

since $c_2$ is a sufficiently large constant.


From now on we focus on the proof of \Cref{thm: from maintaincluster to stSP}. We denote the randomized algorithm for the $r$-restricted \maintaincluster problem from the theorem statement by $\aset$. 




We denote the input to the $(r+1)$-restricted \stSP problem by $(G,A,B,\Delta,\eta,N)$, where $G=(L,R,E)$ is an $n$-vertex  well-structured graph, $A$ and $B$ are two disjoint subsets of vertices of $G$, and $N\geq n$, $\Delta \geq 1$, and $1\leq \eta \leq \Delta$ are parameters. Recall that no regular edge of $G$ connects a vertex of $A$ to a vertex of $B$, $\Delta\leq n-|B|$, $|E|\leq O(n\cdot (n-|B|))$,  and $\frac{(n-|B|)\cdot \eta}{\Delta}\leq 2\cdot 2^{(r+1)\sqrt{\log N}}$ hold.

Recall that, as the algorithm progresses, we maintain lengths $\ell(e)$ for edges $e\in E(G)$, and, additionally, some vertices may leave the sets $A$ and $B$. Since the number of iterations is bounded by $\Delta$, at most $\Delta$ vertices may be deleted from $A$ and from $B$.
For convenience, we denote by $A^0$ and $B^0$ the initial sets $A$ and $B$, respectively, to distinguish them from the sets that are maintained during the algorithm.


Note that we can assume that $N$ is greater than a sufficiently large constant, so that, for example, $N>2^{2^{c_2}}$ holds. Indeed, if this is not the case, then, from \Cref{thm: simple stSP}, we obtain a determinisic algorithm that solves the input instance of \stSP in time:


\[
\begin{split}
O\left(n\cdot(n-|B^0|)\cdot \frac{(n-|B^0|)\cdot \eta}{\Delta}\cdot \log^6 N\right )&\leq O\left(n\cdot(n-|B^0|)\cdot N\cdot \log N\right )
\\&\le c_1\cdot n\cdot (n-|B^0|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+7c_2},
\end{split}\]

since $n\leq N\ll c_1$, and $\eta\leq \Delta$ (recall that, by definition, $c_1\gg c_2$ holds). Therefore, we assume from now on that $N$ is sufficiently large.


Throughout the algorithm, we use the parameter  $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
We let $H$ be the graph that is obtained from $G$, by adding a source vertex $s$, that connects to every vertex $a\in A$ with a length-$0$ edge, and a destination vertex $t$, to which every vertex $b\in B$ connects with a length-$0$ edge. If an edge $e\in E(G)$ is a special edge for graph $G$, then $e$ remains a special edge for $H$. All other edges of $H$, including edges incident to $s$ and $t$, are called regular edges.
For every edge $e\in E(G)$, its length in $H$ remains the same as in $G$, so for convenience, we denote the length of every edge $e\in E(H)$ by $\ell(e)$.

Recall that, at the beginning  of the algorithm, for each edge $e\in E(H)$, its length $\ell(e)$ is set as follows: if $e$ is a regular edge, then $\ell(e)=0$, and if $e$ is a special edge, then $\ell(e)=1$. 
 We start by setting $\qset=\emptyset$, and then perform at most $\Delta$ iterations. In every iteration, the algorithm must do one of the following:


\begin{properties}{R}
	\item either return FAIL;\label{outcome: fail}

	\item or return a simple $s$-$t$ path $P$ of length at most $\Lambda$ in the current graph $H$, such that $P$ contains exactly one vertex of $B$ -- the penultimate vertex on the path; \label{outcome:path}
	
		\item or compute an assignment $\ell'(e)\geq 0$ of lengths to all edges $e\in E(H)$, such that, if we denote by $E^*$ the set of all edges of $G$ with both endpoints in $B$, then $\sum_{e\in E(H)}\ell'(e)\leq \frac{\Lambda\cdot \Delta}{\eta \log^4n}+\sum_{e\in E(H)\setminus E^*}\ell(e)$; the length $\ell'(e)$ of every edge $e$ that is incident to $s$ or to $t$ is $0$; and the distance from $s$ to $t$ in $H$, with respect to edge lengths $\ell'(\cdot)$, is at least $\frac{\Lambda}{32}$;  \label{outcome: cut}
\end{properties}

Note that, if the algorithm returns assignments of lengths $\ell'(e)$ to edges $e\in E(H)$ as in Outcome \ref{outcome: cut}, then these assignments of edge lengths define a modified cut-witness for $G$ (see \Cref{def: mod cut-witness}). In this case, the algorithm terminates, and  returns the  lengths $\ell'(e)$ of all edges $e\in E(H\setminus\set{s,t})$. Slightly abusing the notation, for the sake of simplicity, we will call an assignment of lengths $\ell'(e)$ to the edges $e\in E(H)$ as  described in Outcome \ref{outcome: cut} a \emph{cut-witness}. 

If the algorithm returns an $s$-$t$ path $P$ as in Outcome \ref{outcome:path}, then $P\setminus\set{s,t}$ is a modified acceptable path for $G$ (see \Cref{def: mod acceptable path}). To simplify the notation, we say that a path $P$ described in  Outcome \ref{outcome:path} is an \emph{acceptable path}. If the algorithm returns an acceptable path $P$, then we let $P'=P\setminus\set{s,t}$, and we let $a\in A$, $b\in B$ be the endpoints of path $P'$. We remove $a$ from $A$ and $b$ from $B$, add $P'$ to $\qset$, and delete the edges $(s,a)$ and $(b,t)$ from $H$. Additionally, the lengths of some of the special edges on $P$ may be doubled; we assume that the algorithm receives the list of all such edges. 

From the problem definition, for every special edge $e\in E(H)$, the length of $e$ is doubled once $e$ participates in exactly $\eta$ paths that the algorithm returned since the last time the length of $e$ was doubled, or since the beginning of the algorithm -- whatever happened last.

Lastly, in the case of Outcome \ref{outcome: fail}, we terminate the algorithm and return ``FAIL'', but we require that the probability that the algorithm ever returns ``FAIL'' is bounded by $\frac{1}{2}$.



\subsection*{Bounding the Largest Total Length of Edges and Some Useful Inequalities}

Let $E^{\spec}$ denote the set of all special edges in graph $G$, and let $E^*\subseteq E^{\spec}$ be the subset of edges $e\in E^{\spec}$, such that, at the end of the algorithm, both endpoints of $e$ lie in $B$. For each edge $e\in E^{\spec}$, let $\ell^*(e)$ be the length of $e$ at the end of the algorithm. In the next simple observation we bound $\sum_{e\in E^{\spec}}\ell^*(e)$.



\begin{observation}\label{obs: bound edge lengths}
For every edge $e\in E^*$, $\ell^*(e)=1$, and	$\sum_{e\in E^{\spec}}\ell^*(e)\leq n+2(n-|B^0|)\log^5n$. 
\end{observation} 
\begin{proof}
In order to prove the first assertion, recall that, if $P$ is an $s$-$t$ path in graph $H$ that our algorithm ever returned as part of Outcome \ref{outcome:path}, then $P$ may only contain a single vertex of $B$, so in particular, $E^*\cap E(P)=\emptyset$. Therefore, if $e\in E^*$ is an edge whose both endpoints lie in $B$ at the end of the algorithm, then, at the beginning of the algorithm, we set $\ell(e)=1$, and the length of $e$ is never doubled over the course of the algorithm, so $\ell^*(e)=1$ holds. We now turn to prove the second assertion.
	
\iffalse
Notice that, if an edge $e\in E^{\spec}$ never belonged to $H$, then $\ell^*(e)=0$ holds. Let $E'\subseteq E^{\spec}$ be the set of edges that belong to $H$ at the end of the algorithm, and, for each edge $e\in E'$, let $\ell^0(e)$ be the length of $e$ when it was first inserted into $H$. Note that initially, $H$ may contain at most $(n-|B^0|)$ special edges, since every vertex of $G$ is incident to at most one special edge, and edges with both endpoints in $B^0$ do not lie in the initial graph $H$. The initial length of each such special edge is $1$. Additionally, over the course of $\Delta$ iterations, at most $\Delta$ new vertices are deleted from $B$, and so at most $\Delta$ new special edges are inserted into $H$. Each such edge is assigned length $\ceil{\frac{\Lambda}{\eta}}\leq \frac{2\Lambda}{\eta}$ when it is inserted. Therefore:

\[ \sum_{e\in E'}\ell^0(e)\leq (n-|B^0|)+\frac{2\Lambda\Delta}{\eta}\leq 3(n-|B^0|)\log^5n. \]

since $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
\fi


Recall that, at the beginning of the algorithm, we set the length of every special edge to $1$.
Let $E'\subseteq E^{\spec}$ denote the subset of edges $e\in E^{\spec}$ with $\ell^*(e)>1$. Clearly: 


\[\sum_{e\in E^{\spec}}\ell^*(e)\leq 	|E^{\spec}|+\sum_{e\in E'}\ell^*(e)\leq  n+\sum_{e\in E'}\ell^*(e).\]

Let $q$ be the total number of iterations Algorithm \algmwu, so $|\qset|=q$ holds, and let $\qset=\set{P_1,\ldots,P_q}$, where the paths are indexed in the order in which they were added to $\qset$. For all $1\leq i\le q$, let $C_i$ denote the length of path $P_i$ when it was added to $\qset$. Clearly, $C_i\leq \Lambda$, and $\sum_{i=1}^qC_i\leq q\cdot \Lambda$.

Consider now some edge $e\in E'$, and assume that $\ell^*(e)=z$. Recall that $\ell(e)$ was doubled at least once during the algorithm. Let $\tau$ be the last time when the length of $e$ was doubled. Then, prior to time $\tau$, there were at least $\eta$ iterations $i$, during which the path $P_i$ that was added to $\qset$ contained $e$, and the length of $e$ during the corresponding iteration was $\frac{z}{2}$. In other words, edge $e$ contributes at least $\frac{z\eta}{2}=\frac{\ell^*(e)\eta}{2}$ to $\sum_{i=1}^qC_i$.
Overall, we get that:

\[\sum_{e\in E'}\ell^*(e)\leq \frac{2\sum_{i=1}^qC_i}{\eta}\leq \frac{2q\Lambda}{\eta}\leq  \frac{2\Delta\Lambda}{\eta}\leq 2(n-|B^0|)\cdot \log^5n,\]

since $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
Altogether, we get that:

\[\sum_{e\in E^{\spec}}\ell^*(e)\leq n+\sum_{e\in E'}\ell^*(e)\leq n+2(n-|B^0|)\log^5n.\]
\end{proof}

\iffalse
	Recall that, at the beginning of the algorithm, the length $\ell(e)$ of every special edge is set to $1$, and so $\sum_{e\in E^{\spec}}\ell(e)\leq n$ holds at the beginning of the algorithm. From Requirement \ref{oracle-prop: small length growth}, the total increase in $\sum_{e\in E^{\spec}}\ell(e)$ over the course of the process described above is bounded by:
	
	\[\frac{\Delta \cdot \Lambda\cdot \log^{\hat c}n}{\eta}\leq n\cdot (\log n)^{\hat c+5},\]
	
	since $\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$. Altogether, we get that $\sum_{e\in E^{\spec}}\ell^*(e)\leq n+n\cdot (\log n)^{\hat c+5}\leq 2n\cdot (\log n)^{\hat c+5}$.
\end{proof}
\fi

Throughout the algorithm, we will use a parameter $\highlightf{N'=\max\set{N,8n\cdot \log^5n}}$. Let $\tau$ be any time in the algorithm's execution, and let $H'$ be any subgraph of $H\setminus\left (\set{s,t}\right )$ that is a perfect well-structured graph. Recall that the weight of every vertex $v\in V(H')$ is the length of the unique special edge incident to $v$. From \Cref{obs: bound edge lengths}, the total weight of all vertices of $H'$ must be bounded by $N'$. Notice also that, since $N\geq n$, we get that $N'\leq 8N\log^5n\leq N\log^6N$. It is then easy to see that: 

\begin{equation}\label{eq: bound on log n'}
\log N'\leq \log N+6\log\log N\leq \left(1+\frac{1}{64c_2r}\right)\log N,
\end{equation}

since $r\leq \sqrt{\log N}$ and $N$ is large enough. Additionally, $\sqrt{\log N'}\leq \sqrt{\log N+6\log\log N}\leq \sqrt{\log N}+\sqrt{6\log\log N}$. Therefore:

\begin{equation}
2^{\sqrt{\log N'}}\leq 2^{\sqrt{\log N}}\cdot 6\log N\leq 2^{2\sqrt{\log N}}.\label{eq: bound on N'}
\end{equation}

We will use these facts later.



The description of our algorithm for the $(r+1)$-restricted \stSP problem consists of two parts. In the first part, we provide an algorithm for maintaining an \ATO for graph $H$. This algorithm in turn exploits algorithm $\aset$ for the $r$-restricted \maintaincluster problem. In the second part, we use the algorithm from \ref{thm: almost DAG routing} for the \DLSSSP problem on the corresponding contracted graph.
\newpage



\input{SSSP-part1}
%\input{SSSP-bound-weights}
\input{SSSP-runtime-part1}
\input{SSSP-bound-bad-edges}
%\input{SSSP-previous-stuff}
\input{SSSP-part2}
\input{SSSP-completing-alg}



%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%Leftovers from here on
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================
%===============================

\iffalse

\paragraph{Hidden Edges and Graph $H$.}
Our algorithm will work with a graph $H$, that we define next. Before we do so, we need to define a dynamic subset $E_{\hidden}$ of edges of $G$, that we refer to as \emph{hidden} edges: these edges will be ignored by our algorithm, in order to ensure its efficiency.

\begin{definition}[Hidden Edges]
	The set $E_{\hidden}\subseteq E(G)$ of hidden edges contains  every edge $e=(u,v)$, such that either (i) $u$ and $v$ both lie in $B$; or (ii) $v\in B$ and $e$ is a special edge of $G$.
\end{definition}

We denote by $E^0_{\hidden}$ the set $E_{\hidden}$ at the beginning of the algorithm. Clearly, as the algorithm progresses, edges may be removed from $E_{\hidden}$, but no new edges may join this set. We emphasize that our algorithm does not compute the set $E_{\hidden}$ of edges explicitly, and it is only used for the analysis.


Our algorithm explicitly maintain a graph $H$, that is obtained from $G\setminus E_{\hidden}$, by adding a source $s$, that connects to every vertex of $B$, and a destination vertex $t$, to which every vertex of $A$ are connected. If $e\in E(G)\setminus E_{\hidden}$ is a special edge for graph $G$, then we say that $e$ is a special edge for $H$; all other edges of $H$, including those incident to $s$ and $t$, are regular edges for $H$. 
We denote by $H^0$ the graph $H$ at the beginning of the algorithm.

Note that, given the input graph $G$ in the adjacency-list representation, we can construct graph $H^0$ explicitly in time $O(n\cdot (n-|B^0|))$. Subsequently, whenever a vertex $a\in A$ is deleted from set $A$, we simply delete the edge $(a,t)$ from $H$. Whenever a vertex $b\in B$ is deleted from $B$, we first insert all edges of $E^{\hidden}$ that are incident to $v$ (except for a special edge $(v,u)$ with $u\in B$, if such an edge exists). Since at most $\Delta$ vertices may be deleted from each of the sets $A$, $B$ over the course of the entire algorithm, we get that the total number of edges that are ever present in $H$ is bounded by $O(n\cdot (n-|B^0|)+n\cdot \Delta)\leq O(n\cdot(n-|B^0|))$, and graph $H$ can be maintained explicitly, throughout  the algorithm, in time $O(n\cdot (n-|B^0|))$.
%Throughout the algorithm, we denote by $E_{\hidden}\subseteq E(G)$ the set of all edges $e\in E(G)\setminus E(H)$; for each such edge $e=(u,v)$, $v\in B$ must hold, and we denote by $E^0_{\hidden}$ the initial set of such edges. We also denote by $H^0$ the graph $H$ at the beginning of the algorithm.


\paragraph{A Partition $(U,U')$ of $V(H)$.}
Throughout the algorithm, we let $U\subseteq V(H)$ be the set of vertices of $H$ that contains $s,t$, and all other vertices $v\in V(H)$, such that no special edge is incident to $v$ in $H^0$.
Notice that it is possible that a vertex $v$ lies in $U$, and yet some special edge $e$ is incident to $v$ in $G$, if $e\in E_{\hidden}$, since such an edge $e$ does not lie in $H^0$). We also denote $U'=V(H)\setminus U$. The partition $(U,U')$ of $V(H)$ remains unchanged throughout the algorithm, even though some special edges incident to vertices of $U$ may be subsequently inserted into $H$. We note that vertices of $B$ may lie in $U$ and in $U'$.
We need the following simple observation.

\begin{observation}\label{obs: properties of U}
	Throughout the algorithm, $H[U']$ is a perfect well-structured graph. Moreover, no edge with both endpoints in $U'$ is ever inserted into $G$. Lastly, $|U'|\leq 2(n-|B^0|)$ holds.
\end{observation}
\begin{proof}
	We start by proving the second assertion. The only edges that may be inserted into $H$ over the course of the algorithm are edges of $E^0_{\hidden}$. Consider any such edge $e=(u,v)$, and assume for contradiction that both $u,v\in U'$. Assume first that $e$ is a regular edge. Then, from the definition of the set $E_{\hidden}$ of edges, $u,v\in B^0$ holds. Moreover, since edge $e$ is regular, $u\in L$ and $v\in R$ holds. Since $u\in U'$, there must be a special edge $e'=(x,u)$ in graph $H^0$. But, from the definition of the set $E_{\hidden}$ of edges, $e'\in E_{\hidden}$ holds, so $e'\not\in E(H^0)$, a contradiction. Consider now the case where $e$ is a special edge. Then, since $e$ is the only special edge incident to both $u$ and $v$ in $G$, and $e\in E_{\hidden}$, it is impossible that $u,v\in U'$. 
	
	In order to prove the first assertion, observe that, throughout the algorithm, $H[U']\subseteq G$ holds, so $H[U']$ is a well-structured graph. Moreover, at the beginning of the algorithm, every vertex $v\in U'$ is incident to some special edge of $G$, whose other endpoint must also lie in $U'$. Therefore, $H^0[U']$ is a perfect well-structured graph. As the algorithm progresses, no edges may be inserted into $H[U']$, and no edges may be deleted from $H[U']$ (since the only edges that may be deleted from $H$ are the edges that are incident to $s$ and to $t$). Therefore, $H[U']$ remains a perfect well-structured graph.
	
	In order to prove the third assertion, observe that for every vertex $v\in U'$, either $v\not\in B^0$, or there is a special edge that is incident to $v$, whose other endpoints lies in $V(G)\setminus B^0$. The cardinality of each of these two sets of vertices is bounded by $n-|B^0|$, so $|U'|\leq 2(n-|B^0|)$.
\end{proof}

%Note that $H^0[U']$ is a perfect well-structured graph, and, since no special edges are ever deleted from $H$, $H[U']$ remains a perfect well-structured graph throughout the algorithm. If a vertex $v\in B$ belongs to the set $L$, and a special edge $e$ is incident to $v$ in $G$, then $e\in E^0_{\hidden}$ must hold, as edge $e$ must enter $v$. Therefore, $v\in U$ must hold. On the other hand, a vertex $v\in B\cap R$ may lie in $U$ or in $U'$.
\fi

==> SSSP-bound-weights.tex <==




==> SSSP-part1-backup.tex <==

\subsection{Part 1 - Maintaining the \ATO}

In this part we describe our algorithm for maintaining the \ATO $(\xset,\rho, U, \gamma)$ for graph $H$. Notice that $|V(H)|=|V(G)|+2=n+2$. 
Throughout, we use a parameter ${d= \frac{(n-|B^0|)\cdot\eta}{4\Delta\cdot 2^{\sqrt{\log N}}}}$.
Notice that:

\begin{equation}\label{eq: two bounds on d}
2^{2\sqrt{\log N}}\leq d\leq  2^{r\sqrt{\log N}-1}.
\end{equation}

Here, the first inequality follows from Inequality \ref{eq: bound on d2}.
The second inequality follows since the input instance of \stSP is $(r+1)$-restricted, so $\frac{(n-|B^0|)\cdot\eta}{\Delta}\leq 2\cdot 2^{(r+1)\sqrt{\log N}}$ holds. 
  

 
Let $U\subseteq V(H)\setminus\set{s,t}$ be the collection of all vertices $v$, such that some special edge of $E^{\spec}$ is incident to $v$, and let $U'=V(H)\setminus U$. Notice that $H[U]$ is a perfect well-structured graph  (see \Cref{def: well structured graphs}).
We let the initial collection $\xset$ of vertex subsets contain the set $U$, and, for every vertex $v\in U'$, a set $X_v=\set{v}$. For convenience, we denote $S=\set{s}$ and $T=\set{t}$. 
We distinguish between two cases. Case 1 happens when $|U|>2(n-|B^0|)\cdot (\log N)^{128}$. In this case, we let $U$ be the special cluster of the \ATO, and we set $\gamma=|U|-128(n-|B^0|)(\log N)^{64}$. 
%(n-|B^0|)\cdot (\log N)^{128}$. 
Otherwise, Case 2 happens, the special cluster of the \ATO is undefined, and we set $\gamma=1$.



Next, we assign, to every resulting set $X\in \xset$, an interval $I_X\subseteq \set{1,\ldots,|V(H)|-\gamma+1}$, so that, for each regular cluster $X\in \xset$, $|I_X|=|X|$, and, if the special cluster is defined, then $|I_U|=|U|-\gamma+1$. In order to do so, it is sufficient to define an ordering $\sigma$ of the sets in $\xset$. We let $S$ appear first in the ordering, followed by the sets in $\set{X_v\mid v\in U'\cap L}$ in an arbitrary order, followed by set $U$, which is followed by the sets  in $\set{X_v\mid v\in U'\cap R}$ in an arbitrary order, followed by $T$. Since vertices of $U'$ are not incident to special edges, it is easy to verify that  no edge of $H$ is a right-to-left edge with respect to this initial \ATO.
Throughout the algorithm, we refer to each set $X\in \xset$ of vertices as a \emph{cluster}. If $|X|=1$, then we say that $X$ is a \emph{singleton} cluster. 
As the algorithm progresses, cluster $U$ may be partitioned into smaller and smaller clusters, with each such cluster assigned an interval that is contained in the initial interval $I_{U}$, but the clusters in $\set{X_v\mid v\in U'}$, together with their corresponding intervals $I_{X_v}$, remain unchanged. For convenience, we denote the initial set $U$ by $U^0$.
We will ensure that, throughout the algorithm, the following invariants hold:

\begin{properties}{I}
	
	\item If $X\in \xset$ is a non-singleton cluster, then $H[X]$ is a perfect well-structured graph; \label{inv: perfect well structured} 
	
	\item If the special cluster is defined, then $U\in \xset$ holds throughout the algorithm, and moreover, $|U|\geq \gamma$ always holds; and \label{inv: special cluster}
	
	\item  If $e=(x,y)$ is a right-to-left edge with respect to the current \ATO, and $X,Y\in \xset$ are the clusters that contain $x$ and $y$, respectively, so that $Y$ appears before $X$ in the ordering $\sigma$ of clusters of $\xset$ defined by the \ATO, then $e$ must be a special edge, and moreover, $X=\set{x}$ and $Y=\set{y}$ must hold; in other words, $X$ and $Y$ are both singleton clusters. \label{inv: backward edges}
\end{properties}

It is easy to verify that the invariant holds for the initial \ATO.

For each cluster $X$ that is ever added to $\xset$, we denote by $X^0$ the set $X$ when it was just added to $\xset$. If $|X^0|>1$ (that is, $X$ is not a singleton cluster when it is added to $\xset$), then, from Invariant \ref{inv: perfect well structured}, $H[X]$ is a perfect well-structured graph, so weights of vertices of $X$ are well defined. In such a case, we denote by $W^0(X)$ the  total weight of all vertices of $X$ when $X$ is added to $\xset$. Whenever a non-singleton regular cluster $X$ is added to set $\xset$, we define the parameter ${d_X=\min\set{\frac{|X^0|\cdot \eta}{\Delta},d}}$. We may sometimes refer to $d_X$ as $d_{X^0}$.
Next, we partition all clusters that are ever added to $\xset$ into \emph{leaf} and \emph{non-leaf} clusters.

\begin{definition}[Leaf and Non-Leaf Clusters]\label{def: leaf}
	Let $X$ be a cluster that was just added to $\xset$. We say that $X$ is a \emph{leaf cluster}, if $|X^0| \leq \frac{\Delta\cdot (\log N)^{128}}{\eta}$.
If $X$ is not a leaf cluster, then we call it a \emph{non-leaf} cluster.
\end{definition}

Recall that, if $U$ is a special cluster, then $|U^0|>2(n-|B^0|)\cdot (\log N)^{128}$. Since $\Delta\leq n-|B^0|$ from the definition of the \stSP problem, we get that a special cluster may not be a leaf cluster. 

Recall that in general, once a cluster $X$ is added to the collection $\xset$ of clusters of an \ATO, it must remain in $\xset$ throughout the algorithm, though we may delete some vertices from $X$. A new cluster $Y$ may only be added to the set $\xset$ if it is a subset of some cluster $X$ that currently lies in $\xset$. When we describe our algorithm for maintaining the \ATO, it will be convenient for us to sometimes remove a cluster $X$ from the set $\xset$, and then  immediately reinsert it into $\xset$. This is only done for clarity of exposition and convenience of analysis, and we do not need to do so in order to maintain the \ATO. Additionally, we will sometimes replace a cluster $X\in \xset$ with a new collection of clusters, each of which contains a single vertex of $X$. In such a case we could simply identify $X$ with one of the new clusters and implement this update to $\xset$ via a sequence of cluster splitting operations, though for clarity of exposition we will treat all newly inserted clusters as new clusters, and we will think of $X$ as being removed from $\xset$.


Next, we describe an algorithm for maintaining each cluster $X$ that is added to $\xset$. We employ different algorithms for leaf clusters, non-leaf regular clusters, and the special cluster, if it is defined. We now describe each of the three algorithms in turn.


\subsubsection{Leaf Clusters}

Let $X$ be a leaf cluster that was just added to $\xset$. If $X$ is a singleton cluster, then no further processing of this cluster is needed. Assume now that $X$ is a non-singleton cluster.
We immediately remove $X$ from $\xset$, and instead add, for every vertex $v\in X$, a new singleton cluster $\set{v}$ to $\xset$. We assign, to each such new cluster $\set{v}$, an interval $I_{\set{v}}\subseteq I_{X}$ of length $1$, so that all intervals corresponding to the vertices of $X\cap L$ appear before all intervals corresponding to the vertices of $X\cap R$. Notice that the only new right-to-left edges that are introduced by this transformation are the edges of $E_H(X\cap R,X\cap L)$, which are all special edges. The number of such edges is $|X\cap R|=|X\cap L|\leq |X|$. We say that these new right-to-left edges are \emph{bad edges}, and that they are \emph{owned} by the leaf cluster $X$. We denote the set of these edges by $E^{\bad}(X)$. From the above discussion, $|E^{\bad}(X)|\leq |X|$, and each edge $e\in E^{\bad}(X)$ has $\spann(e)\leq |X|$.




\subsubsection{Non-Leaf Regular Clusters}

Whenever a new non-leaf regular cluster $X$ is added to $\xset$, we  initialize Algorithm $\aset$ for the $r$-restricted \maintaincluster problem on graph $H[X^0]$, with parameters $\Delta$ and $\eta$ that remain unchanged, parameter $d$ replaced with $d_X$, and parameter $N$ replaced with $N'$. We denote this instantiation of Algorithm $\aset$ by $\aset(X)$. We now verify that $(H[X^0],\Delta,\eta,d_X,N')$ is indeed a valid input instance for the $r$-restricted \maintaincluster problem, in the following simple but technical observation, whose proof is deferred to Section \ref{subsec: appx: proof valid instance} of Appendix.

\begin{observation}\label{obs: valid instance}
	$(H[X^0],\Delta,\eta,d_X,N')$ is a valid input instance for the $r$-restricted \maintaincluster problem.
\end{observation}



Recall that Algorithm $\aset(X)$ may, at any time, 
produce a strongly well-structured cut $(Y,Z)$ in $H[X]$ of sparsity $\Phi_{H[X]}(Y,Z)\leq \frac{(\log N')^{64}}{d_X}$. 
Below, we provide an algorithm for processing such a cut.
But before we do so, we provide the remaining details for processing cluster $X$.



Recall that the algorithm for the \stSP problem consists of at most $\Delta$ iterations. At the beginning of every iteration $i$, we will compute, for every non-leaf regular cluster $X\in \xset$, a pair $x,y\in V(X)$ of vertices (where possibly $x=y$). The corresponding algorithm $\aset(X)$ is then required to compute a simple path $P_X$ connecting $x$ to $y$ in graph $H[X]$, whose length is at most $d_X$. We will then process the resulting paths $P_X$ for all non-leaf clusters $X\in \xset$, in order to obtain a short $s$-$t$ path $P_i$ in $H$, as required. For each non-leaf cluster $X\in \xset$, we will ensure that $E(P_i)\cap E(H[X])\subseteq E(P_X)$. Following that, the lengths of some special edges on path $P_i$ may be doubled; we assume that our algorithm is given the list of all such edges. In particular, for each non-leaf regular cluster $X\in \xset$, we are given a subset of the special edges on path $P_X$, whose lengths must be doubled. 
From the definition of the \stSP problem, we are guaranteed that, for every non-leaf regular cluster $X\in \xset$, for every special edge $e\in E(H[X])$, if  $\tau'>\tau$ are two times at which the length of $e$ is doubled, then the number of paths $P_X$ that Algorithm $\aset(X)$ returned  in response to queries during the time interval $(\tau,\tau']$, which contain $e$, is at least $\eta$, so Property \ref{maintaincluster-prop: edge congestion} holds for the instance of the \maintaincluster problem associated with $X$. If Algorithm $\aset(X)$ ever returns ``FAIL'', then we terminate our algorithm for the \stSP problem, and return ``FAIL'' as well.


Lastly, whenever, for a non-leaf regular cluster $X\in \xset$, $|X|$ falls below $\frac{|X^0|}{2}$, we terminate Algorithm $\aset(X)$, and we say that cluster $X$ is \emph{destroyed}. We then think of the resulting set $X$ of vertices as a new cluster that was just added to $\xset$, and treat it as such (so we think that, once cluster $X$ is destroyed, it is deleted from $\xset$, and instead a new cluster, that is identical to $X$, is inserted into $\xset$).
It now remains to describe the algorithm to process sparse cuts produced by Algorithm $\aset(X)$ for non-leaf regular clusters $X\in \xset$.



\subsubsection*{Processing a Cut $(Y,Z)$ in Cluster $X$}

We assume that we are given a non-leaf regular cluster $X\in \xset$, and a strongly well-structured cut $(Y,Z)$ in $H[X]$ of sparsity $\Phi_{H[X]}(Y,Z)\leq \frac{(\log N')^{64}}{d_X}$. 
We denote by $J\subseteq Y$ and $J'\subseteq Z$ the sets of vertices that serve as endpoints of the edges of $E_H(Y,Z)$. Since the edges of $E_H(Y,Z)$ are special edges, it must be the case that $J\subseteq R$ and $J'\subseteq L$. Denote $Y'=Y\setminus J$ and $Z'=Z\setminus J'$.
We start with the following simple observation, whose proof is deferred to Section \ref{subsec: appx: proof of both graphs are perfect well-str} of Appendix.

\begin{observation}\label{obs: both graphs are perfect well-structured}
Each of the graphs $H[Y'],H[Z']$ is a perfect well-structured graph.
\end{observation}


Assume first that $w(Y)\leq w(Z)$.
We update the set $X$ of vertices, by deleting the vertices of $Y\cup J'$ from it; in other words, we set $X=Z'$. We then add $Y'$ as a new cluster to $\xset$, and additionally, for every vertex $v\in J\cup J'$, we add a new singleton cluster $\set{v}$ to $\xset$.  We define the intervals associated with the new clusters, as follows. We assign, to every vertex $v\in J'\cup J$ an interval $I_{\set{v}}\subseteq I_X$ of length $1$, and additionally we define two intervals: $I_{Y'}\subseteq I_X$ of length $|Y'|$ and $I_{Z'}\subseteq I_X$ of length $|Z'|$, so that all resulting intervals $I_{Y'},I_{Z'},\set{I_{\set{v}}}_{v\in J\cup J'}$ are mutually disjoint, and the intervals are ordered as follows: we place the intervals corresponding to the vertices of $J'$ first, followed by interval $I_{Z'}$, then $I_{Y'}$, and lastly the intervals corresponding to the vertices of $J$. Since we have set $X=Z'$, we let $I_X=I_{Z'}$.  From \Cref{obs: both graphs are perfect well-structured}, Invariant \ref{inv: perfect well structured} continues to hold.
We now show that Invariant \ref{inv: backward edges} continues to hold, in the following observation, whose proof is deferred to Section \ref{subsec: appx: proof of obs new right to left} of Appendix. 

\begin{observation}\label{obs: new right to left}
	If $e=(u,v)$ is a right-to-left edge that was added due to the above transformation of \ATO, then $u\in J$ and $v\in J'$ holds, and so $e\in E_H(Y,Z)$, and $e$ is a special edge.
\end{observation}



Since we have defined a separate singleton cluster for every vertex of $J\cup J'$, from \Cref{obs: new right to left}, Invariant  \ref{inv: backward edges} continues to hold. Moreover, the only right-to-left edges that we have introduced during this update are the edges of $E_{H}(Y,Z)$. Notice that the $\spann(e)$ value of each such edge is at most $|X|$. We call all edges of $E_{H}(Y,Z)$ \emph{bad edges}, and we say that they are \emph{owned} by cluster $X$. 

Recall that so far we have assumed that $w(Y)\leq w(Z)$. If $w(Y)>w(Z)$, then the algorithm remains the same, except that at the end we update cluster $X$ by deleting the vertices of $Z\cup J$ from it; or equivalently, we set $X=Y'$. We also set $I_X=I_{Y'}$. This concludes the algorithm for processing the cut $(Y,Z)$ of a non-leaf regular cluster $X\in \xset$.


\subsubsection{The Special Cluster}

Recall that Case 1 happens if
$|U^0|>2(n-|B^0|)\cdot (\log N)^{128}$ holds. In this case, we let $U$ be the special cluster of the \ATO, and we set $\gamma=|U^0|-128(n-|B^0|)(\log N)^{64}$. 
We now show an algorithm for processing the special cluster $U$ if Case 1 happened. We initialize Algorithm $\aset'$ for the $r$-restricted \maintainspeccluster problem on graph $H[U^0]$, with parameters $\Delta$ and $\eta$ that remain unchanged, parameter $d$ replaced by parameter $d_U= \max\set{(\log N')^{64},\left (|U^0\setminus B^0|+\Delta\right )\frac{\eta}{2\Delta\cdot 2^{\sqrt{\log N}}}}$, and parameter $N$ replaced with $N'$. We also initially set $\beta=B^0\cap U^0$, and we ensure that, throughout the algorithm, $\beta=B\cap U$ holds. In other words, whenever a vertex of $\beta$ is deleted from $B$ or from $U$, it is also deleted from $\beta$.

We denote this instantiation of Algorithm $\aset'$ by $\aset'(U)$. We now verify that $(H[U^0],\beta,\Delta,\eta,d,N')$ is indeed a valid input instance for the $r$-restricted \maintainspeccluster problem, in the following simple observation, whose proof is deferred to Section \ref{subsec: appx: proof valid spec instance} of Appendix.

\begin{observation}\label{obs: valid spec instance}
	$(H[U^0],\beta,\Delta,\eta,d_U,N')$ is a valid input instance for the $r$-restricted \maintainspeccluster problem.
\end{observation}


Recall that Algorithm $\aset'(U)$ may, at any time, 
produce a strongly well-structured cut $(Y,Z)$ in $H[U]$ of sparsity $\Phi_{H[U]}(Y,Z)\leq \frac{(\log N')^{64}}{d_U}$, such that $w(Y)\geq 2|\beta\cap Y|$ holds. 
Below, we provide an algorithm for processing such a cut.
But before we do so, we provide the remaining details for processing cluster $U$.




Recall that the algorithm for the \stSP problem consists of at most $\Delta$ iterations. At the beginning of every iteration $i$, we may compute a single vertex $x\in U$, that is sent as a query to Algorithm $\aset'(U)$. Algorithm $\aset'(U)$ is then required to compute a simple path $P(x)$ connecting $x$ to some vertex $y\in \beta$ in graph $H[U]$, whose length is at most $d_U$, such that no inner vertex of $P(x)$ lies in $\beta$ (if $x\in \beta$, then we require that path $P(x)$ only consists of the vertex $x$). 
Our algorithm will then compute a short $s$-$t$ path $P_i$ in $H$, as required, so that $E(P_i)\cap E(H[U])\subseteq E(P(x))$. Following that, the lengths of some special edges on path $P_i$ may be doubled; we assume that our algorithm is given the list of all such edges. In particular, we are given a subset of the special edges on path $P(x)$, whose lengths must be doubled. Additionally, vertex $y$ that serves as an endpoint of path $P(x)$ is deleted from set $B$ and from set $\beta$. This ensures that the lengths of the special edges that are incident to vertices of $\beta$ always remain $1$. We note that in some of the iterations the algorithm for the \stSP problem may not ask any queries to algorithm $\aset'(U)$, and in such iterations the lengths of the special edges of $H[U]$ are not doubled. 
From the definition of the \stSP problem, we are guaranteed that, for every special edge $e\in E(H[U])$, if  $\tau'>\tau$ are two times at which the length of $e$ is doubled, then the number of paths $P(x)$ that Algorithm $\aset'(U)$ returned  in response to queries during the time interval $(\tau,\tau']$, which contain $e$, is at least $\eta$, so Property \ref{maintaincluster-prop: edge congestion} holds for the instance of the \maintainspeccluster problem associated with $U$. If Algorithm $\aset'(U)$ ever returns ``FAIL'', then we terminate our algorithm for the \stSP problem, and return ``FAIL'' as well.


Finally, we provide an algorithm for processing the sparse cuts that Algorithm $\aset'(U)$ may produce. Suppose Algorithm $\aset'(U)$ returns  a strongly well-structured cut $(Y,Z)$ in $H[U]$ of sparsity $\Phi_{H[U]}(Y,Z)\leq \frac{(\log N')^{64}}{d_U}$, such that $w(Y)\geq 2|\beta\cap Y|$ holds.  
We denote by $J\subseteq Y$ and $J'\subseteq Z$ the sets of vertices that serve as endpoints of the edges of $E_H(Y,Z)$, and we let $Y'=Y\setminus J$ and $Z'=Z\setminus J'$.
 Using the same reasoning as in the proof of \Cref{obs: both graphs are perfect well-structured}, 
each of the graphs $H[Y'],H[Z']$ is a perfect well-structured graph.
We will show below that $|Z'|\geq \gamma$ must hold. We delete the vertices of $Y\cup J'$ from $U$, so that $U=Z'$ now holds, and we add $Y'$ as a new cluster to $\xset$. Additionally, for every vertex $v\in J\cup J'$, we add a new singleton cluster $\set{v}$ to $\xset$.  We define the intervals associated with the new clusters as follows. We assign, to every vertex $v\in J'\cup J$ an interval $I_{\set{v}}\subseteq I_U$ of length $1$, and additionally we define two intervals: $I_{Y'}\subseteq I_U$ of length $|Y'|$ and $I_{Z'}\subseteq I_U$ of length $|Z'|-\gamma+1$, so that all resulting intervals $I_{Y'},I_{Z'},\set{I_{\set{v}}}_{v\in J\cup J'}$ are mutually disjoint, and the intervals are ordered as follows: we place the intervals corresponding to the vertices of $J'$ first, followed by interval $I_{Z'}$, then $I_{Y'}$, and lastly the intervals corresponding to the vertices of $J$. Since we have set $U=Z'$, we let $I_U=I_{Z'}$.  As before, Invariant \ref{inv: perfect well structured} continues to hold. Using the same reasoning as in the proof of \Cref{obs: new right to left}, 	if $e=(u,v)$ is a right-to-left edge that was added due to the above transformation of \ATO, then $u\in J$ and $v\in J'$ holds, and so $e\in E_H(Y,Z)$, and $e$ is a special edge. In particular, Invariant \ref{inv: backward edges} continues to hold.
 Moreover, the only right-to-left edges that we have introduced during this update are the edges of $E_{H}(Y,Z)$. Notice that the $\spann(e)$ value of each such edge is at most $|U^0|-\gamma+1$. We call all edges of $E_{H}(Y,Z)$ \emph{bad edges}, and we say that they are \emph{owned} by cluster $U$. 
We denote by $E^{\bad}(U)$ the set of all bad edges that are owned by cluster $U$ over the course of the algorithm. In the following observation we show that $|U|\geq \gamma$ holds throughout the algorithm, and we bound $|E^{\bad}(U)|$.


\begin{observation}\label{obs: large size of U}
	Over the course of the algorithm, at most $ 16|U^0\setminus B^0|+64\Delta\cdot(\log N)^{64}\leq 128(n-|B^0|)(\log N)^{64}$ vertices are deleted from $U$, and so throughout  the algorithm, $|U|\geq \gamma$ holds. Moreover, $|E^{\bad}(U)|\leq \frac{\Delta\cdot 2^{6\sqrt{\log N}}}{\eta}$.
\end{observation}
\begin{proof}
	Recall that we denoted by $E^*\subseteq E^{\spec}$ the set of all special edges $e=(u,v)$, such that $u,v\in B$ holds at the end of the algorithm. Let $B^*\subseteq B$ the set of vertices containing all endpoints of the edges in $E^*$, and let $\tilde U=U^0\setminus B^*$. For every vertex $v\in U^0$, we define a weight $\tilde w(v)$ as follows: if, at the end of the algorithm, $v\in U$, then $\tilde w(v)$ is the weight of $v$ at the end of the algorithm; otherwise, $\tilde w(v)$ is the weight of $v$ just before it is deleted from $U$. We use the following observation, whose proof is very similar to the proof of  \Cref{obs: bound edge lengths}, and deferred to Section \ref{subsec: appx: proof of bound on final weights in U} of Appendix.
	
	
	\begin{observation}\label{obs: bound final weights in U}
	$\sum_{v\in \tilde U}\tilde w(v)\leq  8|U^0\setminus B^0|+8\Delta\cdot (\log N')^{64}$.
	\end{observation}

	
	
	Consider now some cut $(Y,Z)$ of $U$ that Algorithm $\aset'(U)$ produced. Recall that $|E_H(Y,Z)|\leq \frac{(\log N')^{64}}{d_U}\cdot w(Y)$, and that $w(Y)\geq 2|\beta\cap Y|$ holds. Since $B^*\cap Y\subseteq \beta\cap Y$, we get that $w(Y)\geq 2|B^*\cap Y|$. Since the weight of every vertex in $B^*$ remains $1$ throughout the algorithm, we get that $w(Y\setminus B^*)= w(Y)-|B^*\cap Y|\geq w(Y)/2$. Moreover, $|Y|\leq w(Y)=w(Y\setminus B^*)+|Y\cap B^*|\leq 2w(Y\setminus B^*)$ holds. Recall that all vertices of $Y$, and also the endpoints of the special edges in $E_H(Y,Z)$ are deleted from cluster $U$ following the cut $(Y,Z)$. Therefore, the total number of vertices deleted from $U$ following the cut $(Y,Z)$ is at most $2|Y|\le 4w(Y\setminus B^*)\leq 4\sum_{v\in Y\cap \tilde U}\tilde w(v)$. Lastly: 
	
	
	\[|E_H(Y,Z)|\leq \frac{(\log N')^{64}}{d_U}\cdot w(Y)\le\frac{(\log N')^{64}}{d_U}\cdot 2w(Y\setminus B^*)\leq \frac{2\cdot (\log N')^{64}}{d_U}\cdot \sum_{v\in Y\cap \tilde U}\tilde w(v).\]
	
	
	Consider now all cuts $(Y_1,Z_1),\ldots,(Y_r,Z_r)$ that Algorithm $\aset'(U)$ ever produced, in the order in which they were produced. For all $1\leq i\leq r$, following the cut $(Y_i,Z_i)$, the vertices of $Y_i$, along with some additional vertices, were deleted from $U$. From the above discussion, the total number of vertices deleted from $U$ following the cut is bounded by $4\sum_{v\in Y_i\cap \tilde U}\tilde w(v)$, and $|E_H(Y_i,Z_i)|\leq \frac{2\cdot (\log N')^{64}}{d_U}\cdot \sum_{v\in Y\cap \tilde U}\cdot \sum_{v\in Y_i\cap \tilde U}\tilde w(v)$. We conclude that the total number of vertices deleted from $U$ over the course of the algorithm is bounded by:
	
	
	\[\begin{split}
	4\sum_{i=1}^r\sum_{v\in Y_i\cap \tilde U}\tilde w(v)&\leq 4\sum_{v\in \tilde U}\tilde w(v)\\
	&\leq  16|U^0\setminus B^0|+32\Delta\cdot(\log N')^{64}\\
	&\leq 16|U^0\setminus B^0|+64\Delta\cdot(\log N)^{64}\\
	&\leq 128(n-|B^0|)(\log N)^{64},\end{split} \]
	
	from Inequality \ref{eq: bound on log n'}.
	Since, at the beginning of the algorithm, $|U|>2(n-|B^0|)\cdot (\log N)^{128}$ holds, and since
	$\gamma=|U^0|-128(n-|B^0|)(\log N)^{64}$,  we get that $|U|\geq \gamma$ holds throughout the algorithm.
	Lastly, we get that:
	
	\[
	\begin{split}
	|E^{\bad}(U)|&\leq \sum_{i=1}^r|E_H(Y_i,Z_i)|\\
	&\leq \frac{2\cdot (\log N')^{64}}{d_U}\cdot \sum_{i=1}^r\sum_{v\in Y\cap \tilde U}\tilde w(v)\\
&\leq  \frac{\Delta\cdot 2^{2\sqrt{\log N'}}}{\left (|U^0\setminus B^0|+\Delta \right )\cdot\eta}\cdot \sum_{v\in \tilde U}\tilde w(v)\\
&\leq \frac{\Delta\cdot 2^{2\sqrt{\log N'}}}{\left (|U^0\setminus B^0|+\Delta \right )\cdot\eta}\cdot \left( 4|U^0\setminus B^0|+8\Delta (\log N')^{64}\right )\\
&\leq  \frac{\Delta\cdot 2^{6\sqrt{\log N}}}{\eta},
	\end{split}\]
	
	since $d_U= \max\set{(\log N')^{64},\left (|U^0\setminus B^0|+\Delta\right )\frac{\eta}{2\Delta\cdot 2^{\sqrt{\log N}}}}\geq \left (|U^0\setminus B^0|+\Delta\right )\frac{\eta}{2\Delta\cdot 2^{\sqrt{\log N}}}$; we have also used Inequality \ref{eq: bound on N'}.
\end{proof}


\subsubsection{Child Clusters, Descendant Clusters, and a Useful Bound}

%Recall that $E^*\subseteq E^{\spec}$ denote the set of all special edges $e=(u,v)$, such that, at the end of the algorithm, $u,v\in B$ holds.

Let $\tilde \xset$ denote the set of all clusters that ever belonged to $\xset$ over the course of the algorithm. We partition $\tilde \xset$ into three subsets: set  $\tilde \xset_0$ contains all singleton clusters, set $\tilde \xset_1$ contains all non-singleton leaf clusters, and set $\tilde \xset_2$ contains all non-leaf clusters. If the special cluster is defined, then we set $\tilde \xset_2'=\tilde \xset_2\setminus\set{U}$, and otherwise we let $\tilde \xset_2'=\tilde \xset_2$.

Let $E^{\bad}$ be the set of all edges of $G$ that ever served as right-to-left edges of the \ATO. For every cluster $X\in \tilde\xset_1\cup \tilde \xset_2$, we denote by $E^{\bad}(X)$ the set of all bad edges that cluster $X$ owns. Recall that, once an edge $e=(x,y)$ is added to the set $E^{\bad}(X)$ of edges, its initial value $\spann(e)$ is bounded by $|X|$. From Invariant \ref{inv: backward edges}, 
once edge $e$ was added to set $E^{\bad}$, if $Y,Y'$ were the clusters of $\xset$ containing $x$ and $y$ respectively, then $Y=\set{x}$ and $Y'=\set{y}$ holds. In other words, when $e$ was added to $E^{\bad}$, $Y$ and $Y'$ were singleton clusters. Therefore, these clusters, and their corresponding intervals $I_Y$ and $I_{Y'}$, remain unchanged for the remainder of the algorithm. In particular, the value $\spann(e)$ also remains unchanged for the remainder of the algorithm.



Recall that, from Invariant \ref{inv: perfect well structured}, for every cluster $X\in \tilde \xset_2'$, graph $H[X]$ remains a perfect well-structured graph for as long as $X$ lies in $\xset$. Recall also that we have defined weights of vertices for such graphs: for every vertex $v\in X$, its weight $w(v)$ is the length of the unique special edge incident to $v$ in $H[X]$. As the algorithm progresses, the lengths of some special edges grow, and so do the weights of the vertices in $H[X]$. 
For every vertex $v\in X^0$, we denote by $w^0_X(v)$ the weight of $v$ when cluster $X$ was first added to set $\xset$, and algorithm $\aset(X)$ was initialized. If $v$ belongs to set $X$ when algorithm $\aset(X)$ is terminated (e.g. because $|X|$ fell below $|X^0|/2$), then we let $w^*_X(v)$ denote the weight of $v$ in graph $H[X]$ when algorithm $\aset(X)$ terminated. Otherwise, we denote by $w^*_X(v)$ the weight of $v$ just before it was deleted from $X$. 
We also denote $W^0(X)=\sum_{v\in X^0}w^0_X(v)$, and $W^*(X)=\sum_{v\in X^0}w^*_X(v)$. 
From \Cref{obs: bound edge lengths}, the total length of all edges in $E^{\spec}$ at the end of the algorithm is bounded by $|E^{\spec}|+2(n-|B^0|)\log^5n\leq 4n\log^5n$, and so, for every cluster $X\in \tilde \xset_2$: 

\begin{equation}\label{eq: final weight of a cluster}
W^0(X)\leq W^*(X)\leq 8n\log^5n. 
\end{equation}

Recall that, at the beginning of the algorithm, $\xset$ may contain at most one non-leaf cluster -- the cluster $U$. A new non-leaf cluster $X'$ may only be inserted into $\xset$ in one of the following two cases: (i) there is some existing non-leaf cluster $X\in \xset$, for which $|X|$ fell below $|X^0|/2$, and $X'=X$; or (ii) there is some existing non-leaf cluster $X\in \xset$, for which Algorithm $\aset(X)$ or $\aset'(X)$ just computed a sparse well-structured cut $(Y,Z)$, and $X'$ is contained in one of the sets $Y$ or $Z$. %Recall that, in the latter case, we are guaranteed that $\sum_{v\in X'}w(v)\leq \frac{\sum_{v\in X}w(v)}2$ holds at the time when $X'$ is added to $\xset$, and moreover, 
In the latter case, the vertices of $X'$ (along, possibly, with some additional vertices) are deleted from $X$. In either one of the above two cases, we say that $X$ is the \emph{parent-cluster} of $X'$, and $X'$ is the \emph{child-cluster} of $X$. We can now naturally define a descendant-ancestor relationship between clusters: Cluster $X'$ is a descendant-cluster of another cluster $X$, iff there is a sequence $X'=X_1,X_2,\ldots,X_r=X$ of $r\geq 1$ clusters, such that, for all $1\leq i<r$, $X_i$ is a child-cluster of $X_{i+1}$. If $X'$ is a descendant-cluster of $X$, then $X$ is the ancestor-cluster of $X'$. It is easy to verify that, for every pair $X_1,X_2\in \tilde \xset_2$ of clusters, either $X^0_1\cap X^0_2=\emptyset$, or $X_1^0\subseteq X^0_2$ (in which case $X_1$ is a descendant cluster of $X_2$), or $X_2^0\subseteq X^0_1$ (in which case $X_2$ is a descendant cluster of $X_1$).
From the above discussion, if $X_1$ is a child-cluster of some cluster $X_2\in \xset'_2$, then either $|X_1^0|<|X_2^0|/2$; or, at the time when $X_1$ was created, $\sum_{v\in X_1}w(v)\leq \sum_{v\in X_2}w(v)/2$ held, following which the vertices of $X_1$ were deleted from $X_2$.


Consider now a pair $X_1,X_2\in \tilde \xset_2'$ of clusters, where $X_2$ is a descendant cluster of $X_1$. We say that $X_2$ is a \emph{close descendant of $X_1$} iff $|X_2^0|>|X_1^0|/2$. In the following claim, we bound the number of close descendants of every cluster in $\tilde X_2'$. The proof is somewhat technical and deferred to Section \ref{subsec: proof of close descendant} of Appendix.

\begin{claim}\label{claim: close descendant}
	Every cluster $X\in \tilde X_2'$ has at most $64\ceil{\log n}$ close descendants.
\end{claim}


%\subsubsection{Additional Useful Bounds}


%Whenever, for any non-leaf non-singleton cluster $X\in \xset$, $|X|$ falls below $n_{X_0}/2$, we terminate algorithm $\aset(X)$, and we think of $X$ as a cluster that was just added to $\xset$. Therefore, if $|X|\leq \frac{2n\cdot 2^{2\sqrt{\log N}}}{d}$, then it is processed as a leaf cluster, and otherwise we recompute the value $d_X=\frac{|X|}{2n}\cdot d$, and initialize a new instance of Algorithm $\aset$ for the new cluster $X$.

%Throughout, we denote by $\xset'\subseteq \xset$ the set of all singleton clusters, and we let $\xset''=\xset\setminus \xset'$.





%Recall that the algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration $i$, we will compute, for every cluster $X\in \xset''$, a pair $x,y\in V(X)$ of vertices (where possibly $x=y$). The corresponding algorithm $\aset(X)$ is then required to compute a simple path $P_X$ connecting $x$ to a vertex $y'\in \set{y}\cup \beta_X=\set{y}\cup (X\cap B)$ in $H[X]$, whose length is at most $d_X$. We will then process the resulting paths $P_X$ for clusters $X\in \xset''$ in order to obtain a short $s$-$t$ path $P_i$ in $H$, as required, with $E(P_i)\subseteq \bigcup_{X\in \xset''}E(P_X)$. Following that, the lengths of some edges on path $P_i$ may be doubled; we assume that our algorithm is given the list of all such edges. In particular, for each a cluster $X\in \xset''$, we are given a subset of the special edges on path $P_X$, whose lengths must be doubled. Additionally, if Algorithm $\aset(X)$ returned a path $P_X$ that terminates at a vertex $y'\in \beta_X=B\cap X$, then vertex $y'$ may be deleted from set $B$ and from set $\beta_X$.
%From the definition of the \routeandcut problem, we are guaranteed that, for every cluster $X\in \xset''$, for every special edge $e\in E(H[X])$, if  $\tau'>\tau$ are two times at which the length of $e$ is doubled, then the number of paths $P_X$ that Algorithm $\aset(X)$ returned  in response to queries during the time interval $(\tau,\tau']$, which contain $e$, is at least $\eta$, so Property \ref{maintaincluster-prop: edge congestion} holds for the instance of the \maintaincluster problem associated with $X$.




%For every cluster $X\in \tilde \xset_2$, we denote by $\beta'_X\subseteq \beta_X$ the set of all important vertices at the end of Algorithm $\aset(X)$. In other words, $\beta'_X$ contains all vertices that lie in $B\cap X$ at the end of Algorithm $\aset(X)$, and whose weight at the end of that algorithm is $1$.
For the sake of analysis, we need to bound $\sum_{X\in \tilde \xset_2'}W^*(X)$. This bound will later be used both in order to bound the running time of the algorithm, and in order to bound $\sum_{e\in E^{\bad}}\spann(e)$.




\begin{observation}\label{obs: weights of clusters}
%	For all $0\leq i<\ceil{\log n}$  and $0\leq j\leq 4\ceil{\log n}$, 
%	$\sum_{X\in \xset_{i,j}}W^*(X)\leq 128(n-|B^0|)\cdot (\log N)^{130}$.
	$\sum_{X\in \tilde \xset_2'}W^*(X)\leq (n-|B^0|)\cdot (\log N)^{133}$.
\end{observation}
\begin{proof}
	Recall that for every cluster $X\in \tilde \xset'_2$, $W^0(X)\leq 8n\log^5n$ holds (see Inequality \ref{eq: final weight of a cluster}). 
	For all $0\leq i<\ceil{\log n}$ and $0\leq j\leq 4\ceil{\log n}$, we denote by $\xset_{i,j}$ the set of all clusters $X\in \tilde \xset'_2$ with $2^i\leq |X^0|<2^{i+1}$ and $2^j\leq W^0(X)<2^{j+1}$. 
	
	Fix a pair  $0\leq i<\ceil{\log n}$   and $0\leq j\leq 4\ceil{\log n}$ of indices, and consider the collection $\xset_{i,j}$ of clusters. Notice that, if $X,X'\in \xset_{i,j}$, and $X'$ is a descendant-cluster of $X$, then $X'$ is a close descendant of $X$. From \Cref{claim: close descendant}, for every cluster $X\in \xset_{i,j}$, at most $64\ceil{\log n}$ descendant clusters of $X$ lie in $\xset_{i,j}$. Using a simple greedy algorithm, we can then paratition the clusters in $\xset_{i,j}$ into $z=64\ceil{\log n}+1$ subsets $\yset_1,\ldots,\yset_z$, such that, for all $1\leq z'\leq z$, for every pair $X,X'\in \yset_{z'}$ of clusters, neither of the two clusters is a descendant of the other. In order to do so, we consider the clusters $X\in \xset_{i,j}$ one by one, in the non-decreasing order of $|X^0|$, breaking ties arbitrarily. When cluster $X$ is considered, there must be some index $1\leq z'\leq z$, such that no descendant of $X$ lies in $\yset_{z'}$, and we add $X$ to such a set $\yset_{z'}$.
	For all $1\leq z'\leq z$, we now bound $\sum_{X\in \yset_{z'}}W^*(X)$ separately.
	
	Fix any index $1\leq z'\leq z$, and denote $\yset'=\set{X^0\mid X\in \yset_{z'}}$. Since, for every pair $X,X'$ of clusters in $\yset_{z'}$, neither is the descendant of the other, all sets in $\yset'$ are mutually disjoint. 
	
	Assume first that Case 2 happened, so the special cluster is undefined, and $|U^0|\leq 2(n-|B^0|)\cdot  (\log N)^{128}$ holds. From the construction of the set $U$ of vertices at the beginning of the algorithm, for every special edge $e\in E^{\spec}$, both endpoints of $e$ lie in $U^0$. Therefore, $|E^{\spec}|\leq \frac{|U^0|}{2}\leq (n-|B^0|)\cdot  (\log N)^{128}$. From \Cref{obs: bound edge lengths}, the total length of all edges in $E^{\spec}$ at the end of the algorithm is bounded by $|E^{\spec}|+2(n-|B^0|)\log^5n\leq (n-|B^0|)\cdot  (\log N)^{129}$. Since the clusters in $\yset'$ are mutually disjoint, it is easy to verify that $\sum_{X\in \yset_{z'}}W^*(X)\leq 2(n-|B^0|)\cdot  (\log N)^{129}$.
	
	Next, we consider Case 1, where the special cluster is defined. Let $U^*$ denote the set $U$ of vertices at the end of the algorithm. Notice that $U^*$ is disjoint from all sets of vertices in $\yset'$. For every vertex $v\in U^*$, let $w^*(v)$ be the weight of $v$ at the end of the algorithm, and let $W^*(U)=\sum_{v\in U^*}w^*(v)$. From \Cref{obs: bound edge lengths}, the total length of all edges in $E^{\spec}$ at the end of the algorithm is bounded by $|E^{\spec}|+2(n-|B^0|)\log^5n$, and so: 
	
	\begin{equation}\label{eq: total weight at the end}
	\sum_{X\in \yset_{z'}}W^*(X)+W^*(U)\leq 2|E^{\spec}|+4(n-|B^0|)\log^5n.
	\end{equation} 
	
	
	Recall that all vertices that serve as endpoints of the edges in $E^{\spec}$ lie in $U^0$. From \Cref{obs: large size of U}, $|U^0\setminus U^*|\leq 64(n-|B^0|)\cdot(\log N)^{64}$. Therefore, $|U^*|\ge 2|E^{\spec}|-64(n-|B^0|)\cdot(\log N)^{64}$, and $W^*(U)\geq |U^*|\geq 2|E^{\spec}|-64(n-|B^0|)\cdot(\log N)^{64}$.
Combining this with Inequality \ref{eq: total weight at the end}, we get that:
	
\[\sum_{X\in \yset_{z'}}W^*(X)\leq 2|E^{\spec}|+4(n-|B^0|)\log^5n-W^*(U) \leq 128(n-|B^0|)\cdot (\log N)^{64}\leq 2(n-|B^0|)\cdot (\log N)^{129}.\]
To conclude, we have shown that, for every index $1\leq z'\leq z$:


\[
\sum_{X\in \yset_{z'}}W^*(X)\leq 2(n-|B^0|)\cdot (\log N)^{129}.
\]

Summing this up over all indices $1\leq z'\leq z$, and recalling that $z=64\ceil{\log n}+1\leq 128\log n$, we get that:



\[
\sum_{X\in \xset_{i,j}}W^*(X)\leq 256(n-|B^0|)\cdot (\log N)^{130}.
\]

Lastly, by summing up the above inequality over all indices $0\leq i<\ceil{\log n}$   and $0\leq j\leq 4\ceil{\log n}$, we get that: 

\[\sum_{X\in \tilde \xset'_2}W^*(X)\leq 2^{12}(n-|B^0|)\cdot (\log N)^{132}\leq (n-|B^0|)\cdot (\log N)^{133}.\]
\end{proof}


We obtain the following corollary of \Cref{obs: weights of clusters}, that allows us to bound the total span of all bad edges owned by the clusters in $\tilde \xset_2'$.

\begin{corollary}\label{cor: span of bad edges type 1}
	$\sum_{X\in \tilde \xset_2'}\sum_{e\in E^{\bad}(X)}\spann(e)\leq \frac{(n-|B^0|)\cdot \Delta\cdot 2^{4\sqrt{\log N}}}{\eta}$.
\end{corollary}
\begin{proof}
	Consider a cluster $X\in \xset_2'$, and let $(Y,Z)$ be a cut that Algorithm $\aset(X)$ returned. Recall that $|E_{H}(Y,Z)|\leq \frac{(\log N')^{64}}{d_X}\cdot \min\set{w(Y),w(Z)}$. If $w(Y)\leq w(Z)$, then let $Z'=Y$, and otherwise let $Z'=Z$. Then $|E_{H}(Y,Z)|\leq \frac{(\log N')^{64}}{d_X}\cdot w(Z')\leq \frac{(\log N')^{64}}{d_X}\cdot\sum_{v\in Z'}w^*_X(v)$ holds. Moreover, all vertices of $Z'$ are deleted from $X$ following the cut $(Y,Z)$, and the edges of $E_H(Y,Z)$ are added to the set $E^{\bad}(X)$ of bad edges that $X$ owns. We assign to every vertex $v\in Z'$ a \emph{charge} of $\frac{(\log N')^{64}}{d_X}\cdot w^*_X(v)$ units, so that the total charge assigned to the vertices of $Z'$ is at least $|E_H(Y,Z)|$. It is then easy to see that, at the end of Algorithm $\aset(X)$, the total number of edges in $E^{\bad}(X)$ is bounded by the total charge to all vertices of $X^0$, which, in turn, is bounded by:
	\[ \frac{(\log N')^{64}}{d_X}\cdot \sum_{v\in X^0}w^*_X(v)=\frac{(\log N')^{64}}{d_X}\cdot W^*(X).\]
	
	
	Next, we show that $d_X\geq \frac{|X^0|\cdot \eta}{\Delta\cdot 2^{2\sqrt{\log N}}}$. Indeed, recall that $d= \frac{(n-|B^0|)\cdot\eta}{4\Delta\cdot 2^{\sqrt{\log N}}}$ and so:
	
	\begin{equation}\label{eq: bound on dx}
	d_X=\min\set{\frac{|X^0|\cdot \eta}{\Delta},d}=\min\set{\frac{|X^0|\cdot \eta}{\Delta}, \frac{(n-|B^0|)\cdot\eta}{4\Delta\cdot 2^{\sqrt{\log N}}}}.
	\end{equation}
	
	If Case 2 happened, then $|U^0|\leq 2(n-|B^0|)\cdot (\log N)^{128}$, and, since $X^0\subseteq U^0$, we get that $|X^0|\leq 2(n-|B^0|)\cdot (\log N)^{128}$. If Case 1 happened, then, from \Cref{obs: large size of U}, $|X^0|\leq 128(n-|B^0|)(\log N)^{64}$. Therefore, in any case, $|X^0|\leq 2(n-|B^0|)\cdot (\log N)^{128}$ must hold. Substituting the bound $n-|B^0|\geq \frac{|X^0|}{2(\log N)^{128}}$ into Inequality \ref{eq: bound on dx}, we get that $d_X\geq \frac{|X^0|\cdot \eta}{\Delta\cdot 2^{2\sqrt{\log N}}}$. Altogether, we get that:
	
	\[|E^{\bad}(X)|\leq \frac{(\log N')^{64}}{d_X}\cdot W^*(X)\leq \frac{\Delta\cdot 2^{2\sqrt{\log N}}\cdot  (\log N')^{64}}{|X^0|\cdot \eta} \cdot W^*(X)\leq \frac{\Delta\cdot 2^{3\sqrt{\log N}}}{|X^0|\cdot \eta} \cdot W^*(X).\]
	
	Since for every edge $e\in E^{\bad}(X)$, $\spann(e)\leq |X^0|$, we get that:
	
	\[\sum_{e\in E^{\bad}(X)}\spann(e)\leq |X^0|\cdot |E^{\bad}(X)|\leq \frac{\Delta\cdot 2^{3\sqrt{\log N}}}{\eta} \cdot W^*(X).\]

Finally, from \Cref{obs: weights of clusters}:

\[
\begin{split}
 \sum_{X\in \tilde \xset_2'}\sum_{e\in E^{\bad}(X)}\spann(e)& \leq \frac{\Delta\cdot 2^{3\sqrt{\log N}}}{\eta} \cdot\sum_{X\in \tilde \xset_2'}W^*(X)\\
 &\leq \frac{(n-|B^0|)\cdot \Delta\cdot 2^{3\sqrt{\log N}}\cdot (\log N)^{133}}{\eta}\\
 &\leq \frac{(n-|B^0|)\cdot \Delta\cdot 2^{4\sqrt{\log N}}}{\eta}. 
 \end{split}
 \]
\end{proof}

%========================================
%========================================
%========================================
%========================================
%Old proof below
%========================================
%========================================
%========================================
%========================================


\iffalse
\begin{proof}
	Fix a pair  $0\leq i<\ceil{\log n}$   and $0\leq j\leq \ceil{2\log n}$ of indices, and consider the collection $\xset_{i,j}$ of clusters. Notice that, if $X,X'\in \xset_{i,j}$, and $X'$ is a descendant-cluster of $X$, then $X'$ is a close descendant of $X$. From \Cref{claim: close descendant}, for every cluster $X\in \xset_{i,j}$, at most $32\ceil{\log n}$ descendant clusters of $X$ lie in $\xset_{i,j}$. Using a simple greedy algorithm, we can then paratition the clusters in $\xset_{i,j}$ into $z=32\ceil{\log n}+1$ subsets $\yset_1,\ldots,\yset_z$, such that, for all $1\leq z'\leq z$, for every pair $X,X'\in \yset_{z'}$ of clusters, neither of the two clusters is a descendant of the other. In order to do so, we consider the clusters $X\in \xset_{i,j}$ one by one, in the increasing order of $|X^0|$, breaking ties arbitrarily. When cluster $X$ is considered, there must be some index $1\leq z'\leq z$, such that no descendant cluster of $X$ lies in $\yset_{z'}$, and we add $X$ to such a set $\yset_{z'}$.
	For all $1\leq z'\leq z$, we now bound $\sum_{X\in \yset_{z'}}W^*(X)$ and $\sum_{X\in \yset_{z'}}\left(W^*(X)-|\beta'_X|\right)$ separately.
	
	Fix any index $1\leq z'\leq z$, and denote $\yset'=\set{X^0\mid X\in \yset_{z'}}$. Since, for every pair $X,X'$ of clusters in $\yset_{z'}$, neither is the descendant of the other, all sets in $\yset'$ are mutually disjoint. For convenience, denote $\yset'=\set{Y_1,\ldots,Y_r}$.
	Note that,  for every special edge $e=(u,v)\in E^{\spec}$, either both endpoints of $e$ lie in some cluster of $\yset'$, or no endpoint of $e$ lies in $\bigcup_{a=1}^rY_{a}$. Let $E'\subseteq E^{\spec}$ be the set of all special edges $e=(u,v)$, such that both endpoints of $e$ lie in some set of $\yset'$, and let $E''=E^{\spec}\setminus E'$. Let $Y_{r+1}$ be the set of vertices of $G$ that contains the endpoints of every special edge in $E''$. Finally, let $\yset''=\yset'\cup \set{Y_{r+1}}$. From our discussion, all vertex sets in $\yset''$ are mutually disjoint, and, for every special edge $e=(u,v)\in E^{\spec}$, both endpoints of $e$ lie in the same cluster of $\yset''$. 
	
	Consider now some cluster $Y_a\in \yset''$. For every vertex $v\in Y_a$, let $\hat w(v)$ be the weight of $v$ at the end of the algorithm; that is, $\hat w(v)$ is the final length $\ell^*(e)$ of the unique special edge $e$ that is incident to $v$ in $G$. Let $\hat W(Y_a)=\sum_{v\in Y_a}\hat w(v)$.
	Clearly, $\sum_{a=1}^{r+1}\hat W(Y_a)\leq 2\sum_{e\in E^{\spec}}\ell^*(e)\leq 2|E^{\spec}|+2(n-|B^0|)\log^5n$,
	from \Cref{obs: bound edge lengths}.
	In particular: 
	
	\[
	\sum_{a=1}^{r}W^*(Y_a)\leq \sum_{a=1}^r\hat W(Y_a)\leq 	 2|E^{\spec}|+2(n-|B^0|)\log^5n.
	\]
	
	
	Recall that, at the end of the algorithm, for every edge $e\in E^*$, $\ell^*(e)=1$ holds. Therefore, $\hat W(Y_{r+1})\geq 2|E^*\cap E''|$. At the same time, every edge $e\in E^*\cap E'$ has both its endpoints in $\bigcup_{a=1}^r\beta'_{Y_a}$. Therefore, altogether, the endpoints of the edges of $E^*$ contribute at least $2|E^*|$ to $\sum_{a=1}^{r+1}\hat W(Y_a)$, but their contribution to $\sum_{a=1}^{r}(W^*(Y_a)-|\beta'_{Y_a}|)$ is $0$. We then get that:
	
	
	\[\begin{split}
	\sum_{a=1}^{r}\left(W^*(Y_a)-|\beta'_{Y_a}|\right )&\leq \sum_{a=1}^{r}\left(\hat W(Y_a)-|\beta'_{Y_a}|\right )\\
	&\leq \sum_{a=1}^{r}\hat W(Y_a)-2|E^*\cap E'|\\
	&\leq \sum_{a=1}^{r+1}\hat W(Y_a)-2|E^*\cap E'|-2|E^*\cap E''|\\
	&\leq 2|E^{\spec}|+2(n-|B^0|)\log^5n-2|E^*|.
	\end{split}  \]
	
	
		
	Next, we show that $|E^{\spec}|-|E^*|=|E^{\spec}\setminus E^*|\leq 2(n-|B^0|)$. 
	In order to do so, we partition the set $E^{\spec}\setminus E^*$ if edges into two subsets: set $E_1$ contains all edges $e$, such that at least one endpoint of $e$ lied in $V(G)\setminus B$ at the beginning of the algorithm, and set $E_2$ contains all remaining edges of $E^{\spec}\setminus E^*$. Since every edge of $E_1$ is incident to a vertex of $V(G)\setminus B^0$, and every vertex of $G$ may serve as an endpoint of at most one special edge, $|E_1|\leq n-|B^0|$ must hold. Consider now some edge $e\in E_2$. From the definition, over the course of the algorithm, at least one endpoint of $e$ was deleted from $B$. Since at most $\Delta$ vertices are deleted from $B$ over the course of the algorithm, and since each such vertex may serve as an endpoint of at most one special edge, we get that $|E_2|\leq \Delta\leq n-|B^0|$, from the definition of the \stSP problem. Altogether, we get that 
	$|E^{\spec}\setminus E^*|\leq |E_1|+|E_2|\leq 2(n-|B^0|)$, and so:
	
	\[
	\sum_{a=1}^{r}\left(W^*(Y_a)-|\beta'_{Y_a}|\right )\leq 2(n-|B^0|)\log^5n+2|E^{\spec}\setminus E^*|\leq 8(n-|B^0|)\log^5n.\]
	
	
	To conclude we showed that, for every index $1\leq z'\leq z$:
	
	
	\[
	\sum_{X\in \yset_{z'}}W^*(X)\leq 2|E^{\spec}|+2(n-|B^0|)\log^5n,
	\]
	
	and
	
	\[
	\sum_{X\in \yset_{z'}}\left(W^*(X)-|\beta'_{X}|\right )\leq 8(n-|B^0|)\log^5n.
	\]
	
	Summing up both inequalities over all indices $1\leq z'\leq z$, and recalling that $z=32\ceil{\log n}+1\leq 64\log n$, we get that:
	
	
	
	\begin{equation}\label{eq: final weigh summation}
	\sum_{X\in \xset_{i,j}}W^*(X)\leq 128|E^{\spec}|\log n+128(n-|B^0|)\log^6n,
	\end{equation}
	
	and
	
	\[
	\sum_{X\in \xset_{i,j}}\left(W^*(X)-|\beta'_{X}|\right )\leq 512(n-|B^0|)\log^5n.
	\]
	
	
	
	
	Lastly, by summing up Inequality \ref{eq: final weigh summation} for all indices $0\leq i<\ceil{\log n}$   and $0\leq j\leq \ceil{2\log n}$, we get that: $\sum_{X\in \tilde \xset_2}W^*(X)\leq 1024|E^{\spec}|\log^3+1024(n-|B^0|)\log^8n\leq 2048n\log^8n$, since $|E^{\spec}|\leq n$.
\end{proof}
\fi

==> SSSP-part1-previous.tex <==

\subsection{Part 1 - Maintaining the \ATO}



\mynote{Important: if a special edge connecting two vertices in $B$ becomes a backward edge, we give it a weight of 1. Then later when one of its endpoints is deleted from $B$, its weight becomes what it should be. But when bounding the total span of all edgs, we don't need to count edges with both endpoints in $B$ (at the end of the algorithm), because such edges will not participate in the bad paths. This should help ensure that $\Gamma$ behaves like $(n-|B|)$.}

\mynote{prove that after each cut the two clusters remain perfect well-structured}
In this part we describe our algorithm for maintaining the \ATO $(\xset,\rho)$ for graph $H$. 
Throughout, we use a parameter $\highlightf{d= \frac{(n-|B^0|)\cdot\eta}{2\Delta\cdot 2^{\sqrt{\log N}}}}$.
Recall that, since the input instance of \stSP is $(r+1)$-restricted, $\frac{(n-|B^0|)\cdot\eta}{\Delta}\leq 2\cdot 2^{(r+1)\sqrt{\log N}}$ holds. Therefore, $d\leq 2^{r\sqrt{\log N}}$. Notice also that $|V(H)|=|V(G)|+2=n+2$. 





At the beginning of the algorithm, we initialize the \ATO $(\xset,\rho)$ as follows. We let the initial collection $\xset$ of vertex subsets contain the set $U'$, and, for every vertex $v\in U$, the set $X_v=\set{v}$ containing only a single vertex $v$. Clearly, $\xset$ is a partition of $V(H)$. For convenience, we denote $S=\set{s}$ and $T=\set{t}$. For every set $X\in \xset$, we now define an interval $I_X\subseteq \set{1,\ldots,n+2}$ of size $|X|$, so that interval $I_S$ appears first, followed by the intervals in $\set{I_{X_v}\mid v\in L\cap U}$ in an arbitrary order, followed by interval $I_{U'}$, followed by the intervals in $\set{I_{X_v}\mid v\in U\cap R}$ in an arbitrary order, with the interval $I_T$ appearing last. 
Recall that, for every vertex $v\in U\setminus\set{s,t}$, no special edge in $H^0$ is incident to $v$. Therefore, if $v\in L$, then $v$ has no incoming edges (except for, possibly, the edge $(s,v)$), and, if $v\in R$, then $v$ has no outgoing edges (except for, possibly, the edge $(v,t)$). It is now easy to see that no edge of $H^0$ is a right-to-left edge with respect to this \ATO.
Throughout the algorithm, we refer to each set $X\in \xset$ of vertices as a \emph{cluster}. If $|X|=1$, then we say that $X$ is a \emph{singleton} cluster. 

As the algorithm progresses, cluster $U'$ may be partitioned into smaller and smaller clusters, with each such cluster assigned an interval that is contained in $I_{U'}$, but the clusters in $\set{X_v\mid v\in U}$, together with their corresponding intervals $I_{X_v}$, remain unchanged. Recall that, when a vertex $v\in B$ is deleted from $B$, we insert, into graph $H$, all edges  of $E_{\hidden}$ that are incident to $v$, except possibly for a special edge $(v,u)$ with $u\in B$, if such an edge exists. It is easy to verify that all newly inserted regular edges must be left-to-right edges with respect to the current \ATO (since vertices of $U\cap L$ appear before vertices of $U\cap R$ in the ordering defined by the \ATO). However, it is possible that we insert a special edge that is incident to $v$, and such an edge may turn out to be a right-to-left edge with respect to our \ATO. However, at most $\Delta$ vertices may be deleted from $B$ over the course of the algorithm, and so at most $\Delta$ such right-to-left edges may be inserted into $H$ over the course of the algorithm. 


We will ensure that, throughout the algorithm, the following invariants hold:

\begin{properties}{I}

	
	\item If $X\in \xset$ is a non-singleton cluster, then $H[X]$ is a perfect well-structured graph; \label{inv: perfect well structured} and
	
	\item  If $e=(x,y)$ is a right-to-left edge with respect to the current \ATO $(\xset,\rho)$, and $X,Y\in \xset$ are the clusters that contain $x$ and $y$, respectively, so that $Y$ appears before $X$ in the ordering $\sigma$ of clusters of $\xset$ defined by $\rho$, then $e$ must be a special edge, and moreover, $X=\set{x}$ and $Y=\set{y}$ must hold; in other words, $X$ and $Y$ are both singleton clusters. \label{inv: backward edges}
\end{properties}

It is easy to verify that the invariant holds for the initial \ATO $(\xset,\rho)$, from \Cref{obs: properties of U} and our discussion.

Whenever a non-singleton cluster $X$  with $1<|X|\leq \frac{2(n-|B^0|)\cdot 2^{2\sqrt{\log N}}}{d}$ is added to $\xset$, we call it a \emph{leaf cluster}, and process it as follows.
We immediately remove $X$ from $\xset$, and instead add, for every vertex $v\in X$, a new singleton cluster $\set{v}$ to $\xset$. We assign, to each such new cluster $\set{v}$, an interval $I_{\set{v}}\subseteq I_{X}$ of length $1$, so that all intervals corresponding to the vertices of $X\cap L$ appear before all intervals corresponding to the vertices of $X\cap R$. Notice that the only new right-to-left edges that are introduced by this transformation are the edges of $E_H(X\cap R,X\cap L)$, which are all special edges. The number of such edges is $|X\cap R|=|X\cap L|\leq |X|$. We say that these new right-to-left edges are \emph{bad edges}, and that they are \emph{owned} by the leaf cluster $X$. We denote the set of these edges by $E^{\bad}(X)$. From the above discussion, $|E^{\bad}(X)|\leq |X|$, and each edge $e\in E^{\bad}(X)$ has $\spann(e)\leq |X|$.


Whenever a new non-singleton cluster $X$ with $|X|\ge \frac{2(n-|B^0|)\cdot 2^{2\sqrt{\log N}}}{d}$ is added to $\xset$, we denote by $W^0(X)$ the total weight of all vertices of $X$ when $X$ is added to $\xset$, and we define a parameter $d_X=\frac{|X|}{2(n-|B^0|)}\cdot d$.  We denote the set $X$ when it is just added to $\xset$ by $X^0$, and we denote $n_{X^0}=|X^0|$, and $d_{X^0}=d_X$. Recall that, from \Cref{obs: bound edge lengths}, we are guaranteed that $W^0(X)\leq N'$, where $N'=\max\set{N,8(n-|B^0|)\cdot \log^5n}$ is the parameter that we have defined. Since $|X|\ge \frac{2(n-|B^0|)\cdot 2^{2\sqrt{\log N}}}{d}$, we get that $d_X\geq 2^{2\sqrt{\log N}}\geq 2^{\sqrt{\log N'}}$ from Inequality \ref{eq: bound on N'}.

Whenever a new non-singleton non-leaf cluster $X$ is added to $\xset$, we will initialize Algorithm $\aset$ for the $r$-restricted \maintaincluster problem on graph $H[X]$, with parameters $\Delta$ and $\eta$ that remain unchanged, parameter $d$ replaced with $d_X$, and parameter $N$ replaced with $N'$. We denote this instantiation of Algorithm $\aset$ by $\aset(X)$.

As observed already, we are guaranteed that $d_X\geq  2^{\sqrt{\log N'}}$ and that $N'\geq W^0(X)$. From the definition of the \stSP problem, we also get that $1\leq \eta\leq \Delta$ and $1\leq \Delta \leq (n-|B^0|)\leq N\leq N'$. Additionally: 

\[\frac{\Delta\cdot d_X}{\eta}=\frac{\Delta\cdot |X|\cdot d}{2 \eta\cdot (n-|B^0|)}\leq |X|,\]

since $d=\frac{(n-|B^0|)\cdot \eta}{2\Delta\cdot 2^{\sqrt{\log N}}}$.
Therefore, $(H[X],\Delta,\eta,d_X,N')$ is a valid input to the \maintaincluster problem.
Moreover, since $d_X\leq d\leq 2^{r\sqrt{\log N}}\leq 2^{r\sqrt{\log N'}}$ (as $|X|\leq |U'|\leq 2(n-|B^0|)$ from \Cref{obs: properties of U}), and since $r\leq \sqrt{\log N}\leq \sqrt{\log N'}$, it is an $r$-restricted instance of the problem.


Recall that Algorithm $\aset(X)$ may, at any time, 
produce a strongly well-structured cut $(A,B)$ in $H[X]$, whose sparsity $\Phi_{H[X]}(A,B)\leq \frac{2^{\sqrt{\log N'}}}{d_X}$. 
We denote by $J\subseteq A$ and $J'\subseteq B$ the sets of vertices that serve as endpoints of the edges of $E_H(A,B)$. Since the edges of $E_H(A,B)$ are special edges, it must be the case that $J\subseteq R$ and $J'\subseteq L$. %Therefore, for every vertex $v\in J$, all edges entering $v$ are regular edges, and the unique edge leaving $v$ is a special edge. Similarly, for every vertex $v'\in J'$, all edges leaving $v'$ are regular edges, and the unique edge entering $v'$ is a special edge. 
Denote $A'=A\setminus J$ and $B'=B\setminus J'$, and observe that both $G[A']$ and $G[B']$ remain perfect well-structured graphs (see \Cref{def: well structured graphs}). 

Assume first that $w(A)\leq W(B)$.
We update the set $X$ of vertices, by setting $X=B'$, add $A'$ as a new cluster to $\xset$, and additionally, for every vertex $v\in J\cup J'$, we add a new singleton cluster $\set{v}$ to $\xset$.  We define the intervals associated with the new clusters, as follows. We assign, to every vertex $v\in J'\cup J$ an interval $I_{\set{v}}\subseteq I_X$ of length $1$, and additionally we define two intervals: $I_{A'}\subseteq I_X$ of length $|A'|$ and $I_{B'}\subseteq I_X$ of length $|B'|$, so that all resulting intervals $I_{A'},I_{B'},\set{I_{\set{v}}}_{v\in J\cup J'}$ are mutually disjoint, and the intervals are ordered as follows: we place the intervals corresponding to the vertices in $J'$ first, followed by interval $I_{B'}$, then $I_{A'}$, and lastly the intervals corresponding to the vertices of $J$. Since we have set $X=B'$, we let $I_X=I_{B'}$. 
We now show that Invariant \ref{inv: backward edges} continues to hold, in the following observation. 

\begin{observation}\label{obs: new right to left}
	If $e=(u,v)$ is a right-to-left edge that was added due to the above transformation of \ATO, then $u\in J$ and $v\in J'$ holds, and so $e\in E_H(A,B)$.
\end{observation}
\begin{proof} 
	Let $e=(u,v)$ be a new right-to-left edge that was added to the \ATO as the result of the current transformation. Assume first that $v\in J'$. Since $J'\subseteq L$, edge $e$ must be the unique special edge entering $v$, and, from the definition of the set $J'$ of vertices, $e\in E_{H[X]}(A,B)=E_H(A,B)$ must hold. Therefore, $u\in J$ must hold. %We will show that the edges of $E_{G[X]}(A,B)$, that connect vertices of $J$ to vertices of $J'$, are the only right-to-left edges that were added during the current update.
	Assume next that $v\in B'$. Since edge $e$ is a right-to-left edge, it must be the case that $u\in A'\cup J=A$. However, there can be no edges connecting $A$ to $B'$ in $G[X]$, from the definition of the sets $J'$ and $B'$ of vertices. Assume now that $v\in A'$. Since edge $e$ is a right-to-left edge, $u\in J$ must hold. However, as observed already, $J\subseteq R$ must hold, and for every vertex $u\in J$, the only edge that leaves $u$ is the unique special edge incident to $u$, whose other endpoint is in $J'$. Therefore, it is impossible that $u\in J$ and $v\in A'$ holds for an edge $(v,u)$. Lastly, we need to consider the case where $v\in J$. Since $(u,v)$ is a right-to-left edge, it must be the case that $u\in J$. But since $J\subseteq R$, it is impossible that an edge of $G$ has both endpoints in $J$. 
\end{proof}

Since we have defined a separate singleton cluster for every vertex of $J\cup J'$, from \Cref{obs: new right to left}, Invariant  \ref{inv: backward edges} continues to hold. Moreover, the only right-to-left edges that we have introduced during this update are the edges of $E_{H}(A,B)$. Notice that the $\spann(e)$ value of each such edge is at most $|X|$. We call all edges of $E_{H}(A,B)$ \emph{bad edges}, and we say that they are \emph{owned} by cluster $X^0$. It is easy to verify that Invariant \ref{inv: perfect well structured} also continues to hold, as both $A'$ and $B'$ are perfect well-structured graphs.

Recall that so far we have assumed that $w(A)\leq w(B)$. If $w(A)>w(B)$, then the algorithm remains the same, except that we set at the end $X=A'$ and $I_X=I_{A'}$.


Whenever, for any non-leaf non-signleton cluster $X\in \xset$, $|X|$ falls below $n_{X_0}/2$, we terminate algorithm $\aset(X)$, and we think of $X$ as a cluster that was just added to $\xset$. Therefore, if $|X|\leq \frac{2(n-|B^0|)\cdot 2^{2\sqrt{\log N}}}{d}$, then it is processed as a leaf cluster, and otherwise we recompute the value $d_X=\frac{|X|}{2(n-|B^0|)}\cdot d$, and initialize a new instance of Algorithm $\aset$ for the new cluster $X$.
Throughout, we denote by $\xset'\subseteq \xset$ the set of all singleton clusters, and we let $\xset''=\xset\setminus \xset'$.





Recall that the algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration $i$, we will compute, for every cluster $X\in \xset''$, a pair $x,y\in V(X)$ of vertices (where possibly $x=y$). The corresponding algorithm $\aset(X)$ is then required to compute a simple path $P_X$ connecting $x$ to $y$ in $H[X]$, whose length is at most $d_X$. We will then process the resulting paths $P_X$ for clusters $X\in \xset''$ in order to obtain a short $s$-$t$ path $P_i$ in $H$, as required, with $E(P_i)\subseteq \bigcup_{X\in \xset''}E(P_X)$. Following that, the lengths of some edges on path $P_i$ may be doubled; we assume that our algorithm is given the list of all such edges. In particular, for each a cluster $X\in \xset''$, we are given a subset of the special edges on path $P_X$, whose lengths must be doubled. 
From Property \ref{maintaincluster-prop: edge congestion}, we are, however, guaranteed that, for every cluster $X\in \xset''$, for every special edge $e\in H[X]$, if  $\tau'>\tau$ are two times at which the length of $e$ is doubled, then the number of paths $P_X$ that Algorithm $\aset(X)$ returned  in response to queries during the time interval $(\tau,\tau']$, which contain $e$, is at least $\eta$.


Let $\tilde \xset$ denote the set of all leaf clusters that ever belonged to $\xset$, let  $\tilde \xset'$ be the collection of all singleton clusters that ever belonged to $\xset$, and let $\tilde \xset''$ be defined similarly for non-singleton and non-leaf clusters. Let $E^{\bad}$ be the set of all edges of $G$ that ever served as right-to-left edges. For every cluster $X\in \tilde\xset\cup \tilde \xset''$, we denote by $E^{\bad}(X)$ the set of all bad edges that cluster $X$ owns. Recall that, once an edge $e=(x,y)$ is added to set $E^{\bad}(X)$ of edges, its initial value $\spann(e)$ is bounded by $|X|$. From Invariant \ref{inv: backward edges}, 
if, at the time when $e$ was added to $E^{\bad}$, $x\in Y$, $y\in Y'$ held, then $Y=\set{x}$ and $Y'=\set{y}$ must hold. Clusters $Y$ and $Y'$, and the corresponding intervals $I_Y$ and $I_{Y'}$ remain unchanged for the remainder of the algorithm, and so the value $\spann(e)$ also remains unchanged.


Recall that, for every cluster $X\in \tilde \xset''$, graph $H[X]$ remains a perfect well-structured graph for as long as $X$ lies in $\xset$. Recall also that we have defined weights of vertices for such graphs: for every vertex $v\in X$, its weight $w(v)$ is the length of the unique special edge incident to $v$ in $H[X]$. As the algorithm progresses, the lengths of some special edges grow, and so do the weights of the vertices in $H[X]$. 
For every vertex $v\in X^0$, we denote by $w^0_X(v)$ the weight of $v$ when cluster $X$ was first added to set $\xset$, and algorithm $\aset(X)$ was initialized. If $v$ belongs to set $X$ when algorithm $\aset(X)$ is terminated (e.g. because $|X|$ fell below $n_{X^0}/2$), then we let $w^*_X(v)$ denote the weight of vertex $v$ in graph $H[X]$ when algorithm $\aset(X)$ terminated. Otherwise, we denote by $w^*_X(v)$ the weight of $v$ just before it was deleted from $X$. 
We also denote $W^0(X)=\sum_{v\in X^0}w^0_X(v)$, and $W^*(X)=\sum_{v\in X^0}w^*_X(v)$. 

For all $0\leq i<\ceil{\log n}$, we denote by $\xset_i$ the set of all clusters $X\in \tilde \xset''$ with $2^i\leq n_{X^0}<2^{i+1}$. For the sake of analysis, we need to bound, for all $i$, $\sum_{X\in \xset_i}W^*(X)$, and also $\sum_{X\in \tilde \xset''}W^*(X)$. These bounds will later be used both in order to bound the running time of the algorithm, and in order to bound $\sum_{e\in E^{\bad}}\spann(e)$.




\begin{observation}\label{obs: weights of clusters}
	For all $0\leq i<\ceil{\log n}$, $\sum_{X\in \xset_i}W^*(X)\leq 4(n-|B^0|)\log^5n$, and $\sum_{X\in \xset''}W^*(X)\leq 8(n-|B^0|)\log^6n$.
\end{observation}
\begin{proof}
	Observe that for all $0\leq i<\ceil{\log n}$, all clusters in $\set{X^0\mid X\in \xset_i}$ are mutually disjoint.
	Therefore, if we denote, for each edge $e\in E^{\spec}$ by $\ell^*(e)$ the length of edge $e$ at the end of the algorithm, then $\sum_{X\in \xset_i}W^*(X)\leq 2\sum_{e\in E^{\spec}}\ell^*(e)$ must hold. Since, from \Cref{obs: bound edge lengths},
	$\sum_{e\in E^{\spec}}\ell^*(e)\leq  4(n-|B^0|)\log^5n$, we get that $\sum_{X\in \xset_i}W^*(X)\leq  4(n-|B^0|)\log^5n$.  Summing up over all indices $0\leq i<\ceil{\log n}$, we get that $\sum_{X\in \xset''}W^*(X)\leq  8(n-|B^0|)\log^6n$.
\end{proof}

==> SSSP-part2-previous.tex <==



\newpage
\subsection{Part 2: Solving \DLSSSP on the Contracted Graph}



The second part of our algorithm maintains the contracted graph $H=G_{|\xset}$. Once this graph is intialized, it is easy to verify that all changes to this graph can be implemented via vertex-splitting and edge-deletion updates. Whenever a cluster $A$ is split off from some cluster $X\in \xset$, we perform a vertex splitting operation, in which vertex $v_A$ is split off from $v_X$. We include in the corresponding set $E'$ all edges that have one endpoint in $A$ and another outside of $A$. Notice that each such edge either connects a vertex of $A$ and a vertex of $X$; or it has one endpoint in $A$ and another in $V(G)\setminus\set{A\cup X}$. In the latter case, if $e=(a,b)$ with $a\in A$ and $b\not\in A\cup X$, then edge $(v_X,v_Y)$, where $Y$ is the cluster of $\xset$ containing $b$, was already present in $H$. After the vertex-splitting update is complete, we delete this edge from $H$ via standard edge-deletion update. Similarly, if the edge is $e=(b,a)$ with 
$a\in A$ and $b\not\in A\cup X$, then edge $(v_Y,v_X)$, where $Y$ is the cluster of $\xset$ containing $b$, was already present in $H$. After the vertex-splitting update is complete, we delete this edge from $H$ via standard edge-deletion update. Notice that this introduces a number of extra edges in graph $H$. For every edge $e$, whenever a cluster containing one endpoint $a$ of $e$ is split, if $a$ belongs to the smaller side of the partition, then a new copy of $e$ is introduced into $H$ and then the older copy is deleted from it. But it is easy to verify that for each edge $e$ of $G$, at most $\log n$ copies may be introduced, so the number of edges ever present in $H$ is still bounded by $O(m\log^2m)$.





For every edge $e$ of $H$, the weight $w(e)$ is set to be the smallest integral power of $2$ that is greater than $\skipp(e)$. Recall that the value $\skipp(e)$ of an edge may grow overtime. In order to avoid having to  insert edges into $H$ outside of the vertex-splitting updates, for every edge $e$, for every integer $\ceil{\log(\skipp(e))}\leq i\leq \ceil{\log n}$, we add a copy of $e$ whose weight is $2^i$. As the value $\skipp(e)$ grows, we simply remove copies of $e$ as needed. The total number of edges ever present in $H$ is now bounded by $O(m\log^3m)$.

Consider now some vertex $v_X\in V(H)$, and some integer $0\leq i\leq \ceil{\log n}$. Recall that we have denoted by  $U_i(v)=\set{u\in V(H)\mid \exists e=(v,u)\in E(H)\mbox{ with } w(e)=2^i}$. 
Equivalently, if we denote $v=v_X$, then set $U_i$ contains all nodes $v_Y$, such that some edge $e$ of $H$ connects a vertex of $X$ to a vertex of $Y$, and has value $\skipp(e)\leq 2^{i}$. In particular, the distance between intervals $I_X$ and $I_Y$ is at most $2^i$, and so at most $2^i$ other intervals may lie between them. Therefore, it is immediate to verify that $|U_i(v)|\leq 2^{i+1}$ always holds, establishing Property \ref{prop: few close neighbors}	

We apply the algorithm from \Cref{thm: almost DAG routing} to the resulting instance of the \DLSSSP problem, with the parameter $\Gamma$ that we defined above, distance parameter $d=\Lambda$, and $\eps=1/16$. Recall that the algorithm may only return FAIL if the current graph $H$ does not contain any $s$-$t$ path $P$  with $\sum_{e\in E(P)}\ell(e)\leq \Lambda$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$. From our discussion, this may only happen when Condition \ref{stopping condition3} is violated. Recall that the running time of the algorithm is bounded by:


\[\tilde O\left(n^2+\Gamma\cdot n\right)\leq n^2\cdot 2^{6\sqrt{\log N}},\]

since $\Gamma=n\cdot 2^{5\sqrt{\log N}}$.
The total running update time of both parts of the algorithm so far is bounded by:


\[n^2\cdot 2^{c\sqrt{\log N}}\cdot (\log n)^{16cr+5\hat c}+  n^2\cdot 2^{6\sqrt{\log N}}\leq 2n^2\cdot 2^{c\sqrt{\log N}}\cdot (\log n)^{16cr+5\hat c}.\]




===========================


\newpage


Once the algorithm for the \DLSSSP problem terminates, we are guaranteed that $\hat H$ contains no $s$-$t$ path $Q$ with $\sum_{e\in E(Q)}\ell(e)\leq \frac{\Lambda}{64}$ and $\sum_{e\in E(Q)}\skipp(e)\leq \frac{\Gamma}{4}$.
Let $A'$ be the set of all vertices $v\in V(G)$ such that edge $(s,v)$ is still present in $H$, and let $B'$ be the set of all vertices $u\in V(G)$, such that edge $(u,t)$ is stil present in $H$.
 We now define an assignment $\ell'(e)\ge 0$ of lengths to edges of $ E(H)$, such that
 the length $\ell'(e)$ of every regular edge is $0$;
 $\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta\cdot \Lambda}{2\eta\log^4n}+\sum_{e\in E(H)}\ell(e)$, and the distance from $s$ to $t$ in $H$, with respect to these new edge lengths is at least $\frac{\Lambda}{64}$.
 
 
 For every special edge $e\in E^{\spec}$, if $e\not\in E^{\bad}$, then we set $\ell'(e)=\ell(e)$. Otherwise, we set $\ell'(e)=\ell(e)+\spann(e)\cdot \frac{\eta\cdot\log n}{4\Delta\cdot 2^{4\sqrt{\log N}}}$. For every regular edge $e$, we set $\ell'(e)=0$.
 
 Observe first that:
 
 \[\begin{split} 
 \sum_{e\in E(G)}\ell'(e)& \leq \sum_{e\in E(H)}\ell(e)+\frac{\eta\cdot\log n}{4\Delta\cdot 2^{4\sqrt{\log N}}}\sum_{e\in E^{\bad}}\spann(e)\\
 &\leq\sum_{e\in E(H)}\ell(e)+\frac{\eta\cdot\log n}{4\Delta\cdot 2^{4\sqrt{\log N}}}\cdot \frac{2n\Delta\cdot 2^{4\sqrt{\log N}}}{\eta}\\
 &\leq\sum_{e\in E(H)}\ell(e)+\frac{n\log n}{2}\\
 &\leq \frac{\Delta\cdot \Lambda}{2\eta\log^4n}+\sum_{e\in E(H)}\ell(e),
 \end{split} \]
 
 since $\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$.
 
Next, we assume for contradiction that there is an $s$-$t$ path $Q$ in the current graph $G$, such that $\sum_{e\in E(Q)}\ell'(e)\leq \frac{\Lambda}{64}$. Path $Q$ naturally defines a path $Q'$ in the contracted graph $\hat H$. Clearly, $\sum_{e\in E(Q')}\ell(e)\leq \sum_{e\in E(Q)}\ell'(e)\le \frac{\Lambda}{64}$. We now claim that $\sum_{e\in E(Q')}w(e)\leq \Gamma$ must hold, leading to a contradiction.


Indeed, since $\sum_{e\in E(Q)}\ell'(e)\leq \frac{\Lambda}{64}$, we get that:

\[\sum_{e\in E(Q')\cap E^{\bad}}\spann(e)\cdot \frac{\eta\cdot\log n}{4\Delta\cdot 2^{4\sqrt{\log N}}}\leq \frac{\Lambda}{64}.  \]

Therefore:

\[ \sum_{e\in E(Q')\cap E^{\bad}}\spann(e)\leq \frac{\Lambda\cdot \Delta\cdot 2^{4\sqrt{\log N}}}{16\eta\log n}= \frac{n \cdot 2^{4\sqrt{\log N}}\cdot \log^4n}{16},\]


since $\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$. But then: 

\[\sum_{e\in E(Q')}\skipp(e)\leq n+2\sum_{e\in E(Q')}\spann(e)\leq n+\frac{n \cdot 2^{4\sqrt{\log N}}\cdot \log^4n}{8}\leq \Gamma,\]

since $\Gamma=n\cdot 2^{5\sqrt{\log N}}$, a contradiction.

\newpage

==> SSSP-previous-stuff.tex <==


\subsection{Previous Stuff, to be Deleted}



Recall that, over the course of the algorithm, the lengths of the edges in $G$ may grow, and so the weights of the vertices of $G$ may grow as well. Initially, for every vertex $v$, $w(v)=1$, since the lengths of all special edges are $1$. We denote, for every vertex $v\in V(G)$ by $w^*(v)$ the weight of $v$ at the end of the algorithm. For a subset $X$ of vertices of $G$, we denote by $w^*(X)=\sum_{x\in X}w^*(X)$, and we denote by $W^*=W^*(V(G))$. We start by showing that $W^*$ may not be too large.



\begin{observation}\label{obs: small weight gain}
	$W^*(G)\leq W^0(G) +2n\log^{\hat c}n\leq O(W^0(G)\cdot \log^{\hat c}n)$.
\end{observation}

\begin{proof}
	Recall that the weight of every vertex in $G$ is equal to the length of the unique special edge incident to this vertex. Therefore, $W^*(G)-W^0(G)$ is equal to twice the total increase in the lengths of all edges. Let $q$ denote the total number of iterations, and recall that $q\leq \Delta$. Then $W^*(G)-W^0(G)\leq 2\sum_{i=1}^qC_i$. From Requirement \ref{maintaincluster-prop: small length growth}, $\sum_{i=1}^qC_i\leq \frac{q\cdot d\cdot \log^{\hat c}n}{\eta}\leq  \frac{\Delta\cdot d\cdot \log^{\hat c}n}{\eta}\leq  n\log^{\hat c}n$, since from the definition of the \maintaincluster problem, $\frac{\Delta\cdot d}{\eta}\leq n$ must hold. We conclude that $W^*(G)\leq W^0(G)+2n\log^{\hat c}n$. Lastly, since, for every vertex $v\in V(G^0)$, $w^0(v)\geq 1$, we get that $W^0(G)\geq n$, and so $W^*(G)\leq W^0(G) +2n\log^{\hat c}n\leq O(W^0(G)\cdot \log^{\hat c}n)$ holds.
\end{proof}


Consider again a graph $G$ that serves as input to the \maintaincluster problem. We associate with this instance a collection $E^{\bad}$ of \emph{bad edges}, that $G$ \emph{owns}. At the beginning of the algorithm, $E^{\bad}=\emptyset$. Whenever the algorithm for the \maintaincluster problem produces a cut $(X,Y)$ of $G$ of sparsity $\Phi_G(X,Y)\leq \phi$, we add the edges of $E_G(X,Y)$ to the set $E^{\bad}$ of bad edges. Recall that the vertices of the smaller set of $\set{X,Y}$ are then deleted from $G$. The bad edges that arise from executing the algorithm for the \maintaincluster problem will eventually become right-to-left edges in the \ATO that our algorithm maintains. In order to ensure that the running time of our algorithm is suitably bounded, it is crucial to ensure that the number of bad edges that graph $G$ owns is bounded. We will next bound the total number of edges that belong to $E^{\bad}$ at the end of the algorithm, in terms of the total initial weight of the vertices of $G$.


For convenience, we denote by $G^0$ the graph $G$ at the beginning of the algorithm. For every vertex $v\in V(G^0)$, we denote by $w^0(v)$ the weight of $v$ at the beginning of the algorithm. If $v$ lies in $G$ at the end of the algorithm, then we denote by $w^*(v)$ the weight of $v$ at the end of the algorithm; otherwise, we let $w^*(v)$ be the weight of $v$ just before it is deleted from $G$. We denote by $W^0(G)=\sum_{v\in V(G^0)}w^0(v)$ -- the total weight of all vertices of $G$ at the beginning of the algorithm, and we denote by $W^*(G)=\sum_{v\in V(G^0)}w^*(v)$.
For a subset $S$ of vertices of $G$, we denote by $W^0(S)=\sum_{v\in S}w^0(v)$ and $W^*(S)=\sum_{v\in S}w^*(v)$
Notice that, as the algorithm progresses, as long as vertex $v$ lies in $G$, its weight may only grow. Therefore, $w^0(v)\leq w(v)\leq w^*(v)$ holds as long as $v\in V(G)$. The following observation shows that $W^*(G)$ cannot be much larger than $W^0(G)$.


\begin{observation}\label{obs: small weight gain}
	$W^*(G)\leq W^0(G) +2n\log^{\hat c}n\leq O(W^0(G)\cdot \log^{\hat c}n)$.
\end{observation}

\begin{proof}
	Recall that the weight of every vertex in $G$ is equal to the length of the unique special edge incident to this vertex. Therefore, $W^*(G)-W^0(G)$ is equal to twice the total increase in the lengths of all edges. Let $q$ denote the total number of iterations, and recall that $q\leq \Delta$. Then $W^*(G)-W^0(G)\leq 2\sum_{i=1}^qC_i$. From Requirement \ref{maintaincluster-prop: small length growth}, $\sum_{i=1}^qC_i\leq \frac{q\cdot d\cdot \log^{\hat c}n}{\eta}\leq  \frac{\Delta\cdot d\cdot \log^{\hat c}n}{\eta}\leq  n\log^{\hat c}n$, since from the definition of the \maintaincluster problem, $\frac{\Delta\cdot d}{\eta}\leq n$ must hold. We conclude that $W^*(G)\leq W^0(G)+2n\log^{\hat c}n$. Lastly, since, for every vertex $v\in V(G^0)$, $w^0(v)\geq 1$, we get that $W^0(G)\geq n$, and so $W^*(G)\leq W^0(G) +2n\log^{\hat c}n\leq O(W^0(G)\cdot \log^{\hat c}n)$ holds.
\end{proof}



\begin{claim}\label{claim: number of bad edges}
	At the end of the algorithm, $|E^{\bad}|\leq O(\phi\cdot W^0(G)\cdot \log^{\hat c+1}n)$.
\end{claim}
\begin{proof}
	Consider any time during the algorithm's execution, when it  produces a well-structured cut $(X,Y)$ of $G$ of sparsity $\Phi_G(X,Y)\leq \phi$.
	Recall that the edges of $E_G(X,Y)$ are then added to the set $E^{\bad}$ of bad edges. From the definition of sparsity, $|E_G(X,Y)|\leq \phi\cdot\min\set{w(X),w(Y)}$. Recall that for every vertex $v\in V(G)$, $w(v)\leq w^*(v)$. Therefore, $w(X)\leq w^*(X)$ and $w(Y)\leq w^*(Y)$. Let $Z$ denote the set from among $X,Y$ with smaller value $w^*(Z)$, breaking ties arbitrarily, and let $Z'$ denote the other set. Then, from our discussion, $|E_G(X,Y)|\leq \phi\cdot w^*(Z)$ must hold. We \emph{charge} every vertex $v\in Z$ for the edges in $E_G(X,Y)$, where each such vertex $v$ is charged $\phi\cdot w^*(v)$ units. This ensures that the total charge of vertices in $Z$ is at least $E_G(X,Y)$. Notice that some vertices in $Z$ may remain in $G$, and they may be charged again. However, if this happens, then $|Z'|\leq |Z|$ must hold, and the vertices of $Z'$ must be deleted from $G$. Therefore, $\sum_{v\in V(G)}w^*(v)$ must decrease by at least factor $2$. We conclude that every vertex $v\in V(G^0)$ may be charged at most $\log(W^*(G))\leq \log(4n^2)=O(\log n)$ time (we have used the fact that all edge lengths in $G^0$ are bounded by $2d$, so $W^0(G)\leq \log(4n^2)$).
	
	The total number of edges in set $E^{\bad}$ at the end of the algorithm is then bounded by the total charge to all vertices of $G$. Therefore:
	
	\[|E^{\bad}|\leq \phi\cdot W^*(G)\cdot O(\log n)\leq O(\phi\cdot W^0(G)\cdot \log^{\hat c+1}n).   \]	
\end{proof}





The proof of \Cref{thm: alg for maintain cluster} is by induction, from smaller to larger values of $d$ (which we will discretize). In order to prove the theorem for a specific value of $d$, we will need to solve several instances of maximum flow problem in the input graph $G$. For example, we will embed an expander into $G$ via the cut-matching game, and the algorithm for the matching player requires solving $O(\log n)$ instances of maximum flow in $G$. In order to solve each such instance, we use the \MWU method as before, reducing the problem to a special case of directed \SSSP. We then maintain an \ATO on the resulting graph, by maintaining a collection $\xset$ of almost-expander graphs. The latter is done by employing the algorithm for the \maintaincluster poblem for smaller values of $d$. Therefore, our algoritm needs to maintain an \ATO when given as a blackbox an algorithm for the \maintaincluster problem for small values of $d$, and we employ this method several times throughout the algorithm. In all these cases, the specific framework for maintaining at \ATO is the same, though some specific details change based on context. Below we formalize the specific framework for maintaining \ATO that we employ. We decouple this framework from the specifics of the algorithm for the \maintaincluster problem, but later when we use this framework, we will apply an algorithm for the \maintaincluster problem to each of the clusters in $\xset$.


We start by recapping the standard definition of cut sparsity in general simple unweighted directed graphs, and recalling several useful properties of this definition. We then extend this definition to the types of graph that arise in our algorithm, where edges have lengths and parallel edges may be allowed. While the specifics of this modified definition of sparsity may appear not very intuitive, they are motivated by preserving the useful properties of the standard definition of cut sparsity, and of adapting this standard definition of cut sparsity to the very specific types of graphs that arise in our algorithm.


\paragraph{Standard Sparsity.}
We start by recapping the standard definition of cut sparsity
Let $G=(V,E)$ be a directed $n$-vertex graph. Assume that $G$ contains no parallel edges, and it is unweighted, that is, we think of all edge lengths in $G$ as being unit. Recall that a \emph{cut} in $G$ is an ordered pair $(A,B)$ of subsets of vertices of $G$, with $A,B\neq \emptyset$ and $A\cup B=V$. The \emph{standard sparsity} of the cut $(A,B)$ is $\frac{|E(A,B)|}{\min\set{|A|,|B|}}$.
Note that we do not require that $|A|\leq |B|$ under this definition. We say that graph $G$ is a $\phi$-expander if the sparsity of every cut $(A,B)$ in $G$ is at most $\phi$.


\paragraph{Useful Properties of Standard Sparsity.}
We now list some well known useful properties of the standard notion of sparsity. Since we do not use them directly, we do not prove them here, we only list them as motivation.

Let us consider a simple directed bipartite graph $G=(L,R,E)$ with unit edge lengths, where the edges of $E_G(L,R)$ are called \emph{regular} and the edges of $E_G(R,L)$ are called \emph{special}. Assume further that every vertex of $G$ is incident to at most one special edge.

The first useful property is that, if we are given a parameter $d$, and a pair $x,y$ of vertices of $G$ with $\dist_G(x,y)\geq d$, then, using a variation of the standard ball-growing technique, we can compute a cut $(A,B)$ in $G$, whose sparsity is at most $\otilde(1/d)$, such that all edges of $E_G(A,B)$ are special edges.

The second useful property is that, if we are given any ordered pair $(A,B)$ of disjoint subsets of vertices of $G$ of cardinality $n/2$ each, and additional parameters $0<z\leq n/2$ and $d>0$, then either there is a cut $(X,Y)$ in $G$ with $|X|,|Y|\geq z$ and $E_G(X,Y)\leq \frac{2n}{d}$, such that all edges of $E(X,Y)$ are special edges; or there is a collection $\qset$ of at least $n/2-z$  paths, connecting vertices of $A$ to vertices of $Y$ in $G$, such that the length of every path is $\otilde(d)$; the paths cause edge-congestion $\otilde(d)$; and the endpoints of the paths are all distinct. In fact \cite{matching-old} provided an algorithm that returns either the desired collection of $A$-$B$ paths, or a cut $(X,Y)$ as above. In the typical use of this result, parameter $z$ is set to be $\Theta(n/\poly\log n)$, so, in the case a cut $(X,Y)$ is returned, its sparsity is $\otilde(1/d)$.


For the third property, we consider a process in which graph $G$ is gradually partitioned via sparse cuts. Consider the following process. We start with the graph $G$, and then proceed in iterations. In every iteration, we compute a cut $(A,B)$ in $G$ of sparsity at most $\phi$, such that all edges in $E_G(A,B)$ are special. We refer to the edges of $E_G(A,B)$ as \emph{cut edges}. If $|A|\leq |B|$ then we delete the vertices of $A$ from $G$, and otherwise we delete the vertices of $B$ from $G$, and then continue to the next iteration. Let $E'$ be the set of all cut edges that are introduced over the course of this process. By standard accounting methods it is easy to show that $|E'|\leq \phi\cdot n$ must hold.





%The first useful property of the notion of sparsity is that, if we are given a graph $G$ as above that is a $\phi$-expander, then for every ordered pair $(u,v)$ of vertices of $G$, the distance from $u$ to $v$ in $G$ is roughly bounded by $O\left(\frac{\phi}{\dmax\log n}\right )$, where $\dmax$ is the maximum vertex degree in $G$ (see \Cref{obs: ball growing}).


Graphs that arise in our algorithm are somewhat more complex: edges in such graphs may have different lengths, and parallel edges are allowed. However, the class of graphs that we may obtain is still significantly more restricted than general directed graphs with parallel edges and non-uniform edge lengths. We start by defining the types of graphs that we need to deal with, that we call \emph{well-structured graphs}. We will extend the definition of cut sparsity to such graphs in a way that allows us to obtain the analogues of the above three properties, and additional useful properties.




\paragraph{Well-Structured Graphs.}

\begin{definition}[Well-Structured Graphs]\label{def: well structured graphs} Let $G=(L,R,E)$ be a bipartite directed graph with lengths $\ell(e)\geq 0$ on its edges, and let $m^*\geq |E|$ be a parameter. We call the edges of $E_G(L,R)$ \emph{regular} and the edges of $E_G(R,L)$ \emph{special}. We say that $G$ is a \emph{well-structured graph} if the following hold:
	
	\begin{itemize}
		\item If $e$ is a regular edge, then $\ell(e)=0$, and no edges are parallel to $e$;
		
		\item If $e$ is a special edge, then $\ell(e)$ is an integral power of $2$ between $1$ and $2m^*$. There may be up to $\ceil{\log (2m^*)}$ edges parallel to $e$, and all parallel edges must have different lengths; 
		
		\item If $v$ is any vertex of $G$, then all special edges that $v$ is incident to are parallel to each other.
	\end{itemize}
\end{definition}

Notice that, if $G^*$ is the graph that serves as input to the restricted \SSSP problem, then $G^*\setminus\set{s,t}$ is a well-structured graph, with respect to parameter $m^*=|E(G^*)|$. The well-structured graphs that we will consider are all subgraphs of $G^*\setminus\set{s,t}$, and we will always use $m^*=|E(G^*)|$.

Notice also that, if $G$ is initially a well-structured graph, that undergoes an online sequence of edge deletions, then $G$ remains a well-structured graph throughout the update sequence.

For all $1\leq i\leq \ceil{\log(2m^*)}$, we define a set $E_i(G)$ of special edges of $G$ as follows: an special edge $e$ lies in $E_i(G)$ iff $\ell(e)=2^i$, and moreover, for every edge $e'$ that is parallel to $e$, $\ell(e')>2^i$. Note that, as graph $G$ undergoes an online sequence of edge deletions, edge set $E_i(G)$ evolves: an edge $e$ may be deleted from $E_i(G)$ if $e$ is deleted from $G$; and an edge $e'$ may be added to $E_i(G)$ if all edges that were parallel to $e'$ and had length less than $2^i$ were deleted from $G$. At every time $\tau$ during the time horizon, we denote by $N_i(G)$ the total number of edges that ever belonged to $E_i(G)$ up to time $\tau$.




\newpage
----------

\paragraph{Well-Structured Cuts.}
Suppose we are given a simple unweighted directed bipartite graph $H=(L,R,E)$ (with no parallel edges), such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$. We call the edges that are directed from $R$ to $L$ \emph{special edges}, and the remaining edges are \emph{regular} edges.

We say that a cut $(A,B)$ in $H$ is \emph{well-structured} iff all edges of $E(A,B)$ are special edges.



\begin{observation}\label{obs: sparse cut to structured}
	Suppose we are given a
	simple directed   bipartite graph $H=(L,R,E)$ with no isolated vertices, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$, together with and a cut $(A,B)$ in $H$ of sparsity at most $\phi\leq \frac{1}{4}$. Then there is a well-structured cut $(A',B')$ in $H$, with $A'\subseteq A$ and sparsity at most $2\phi$, such that $|A'|\geq (1-\phi)|A|$, $\vol_H(A')\geq \Omega(\vol_H(A))$ holds. % and $\vol_H(B')\geq \Omega(\vol_H(B))$ hold. %If $Z$ is the side of the cut $(A,B)$, and $Z'$ is the smaller side of the cut $(A',B')$, then $\vol_H(Z')\le 2\vol_H(Z)$.  
	Moreover, there is an algorithm, that, given cut $(A,B)$, computes such a cut  $(A',B')$, in time $O(\min\set{\vol_H(A),\vol_H(B)})$.
\end{observation}

\begin{proof}
	We start with cut $(A,B)$ and inspect every vertex in $A$. If $v$ is any such vertex, and there is an edge $(v,u)$ in $E(A,B)$ that is not a special edge, we move $v$ from $A$ to $B$. Note that the only new edge that this move introduces into the cut $(A,B)$ is a special edge that enters $v$, if such an edge exists. Vertex $v$ is removed from $A$, and we say that edge $(v,u)$ is \emph{responsible} for this move. Notice that every regular edge of $E(A,B)$ is responsible for moving at most $1$ vertex from $A$ to $B$.
	
	Let $(A',B')$ denote the final cut. For convenience, denote $R=\min\set{|A|,|B|}$. It is easy to verify that $|B'|\geq R$ continues to hold, and $|A'|\geq |A|-|E(A,B)|\geq |A|-\phi\cdot R\geq \frac{|A|}{2}$. Therefore, $\min\set{|A'|,|B'|}\geq \frac{\min\set{|A|,|B|}}{2}$.
	From the above discussion, $|A'|\geq |A|-\phi\cdot R\geq (1-\phi)|A|$ also holds.
	
	Notice also that $|E(A',B')|\leq |E(A,B)|$, since every regular edge $e\in E(A,B)$ may cause at most one additional special edge to be added to the cut. Altogether, we get that:
	
	\[\frac{|E(A',B'|)}{\min\set{|A'|,|B'|}}\leq \frac{2|E(A,B)|}{ \min\set{|A|,|B|}}\leq 2\phi.\]
	
	
	Notice that for every edge $e\in E_H(A)$, at least one endpoint of $e$ must remain in $A'$. Indeed, consider any such edge $e=(x,y)$. The only way that $x$ is moved from $A$ to $B$ is if there is a regular edge $(x,y')\in E_H(A,B)$, which, in turn may only happen if $x\in L$. Using the same reasoning, $y$ may only be moved to $B$ if $y\in L$. But since $(x,y)$ are connected by an edge, it is impossible that both vertices lie in $B$. Since $|E_H(A,B)|<|A|$, we get that:
	
	\[ \vol_H(A')\geq   \Omega(|E_H(A)|+|E_{H}(A',B')|)\geq \Omega(|E_H(A)|+|A|) \geq   \Omega(|E_H(A)|+|E_H(A,B)|)\geq 
	\Omega(\vol_H(A)).\]
	
	(we have used the fact that $H$ has no isolated vertices). 
	
	%	Since our procedure only moves vertices from $A$ to $B$, it is easy to verify that $\vol_H(B')\geq \vol_H(B)$.
	
	
	The running time of the algorithm is bounded by $O(\vol_H(A))$. If $\vol_H(B)<\vol_H(A)$, then we can instead scan all vertices of $B$, and for each such vertex $u$ try to identify a regular edge $(v,u)\in E(A,B)$. In this case, the running time is bounded by $O(\vol_H(B))$.
\end{proof}





\iffalse
Suppose we $G$ is a well-structured graph (see \Cref{def: well-structured}), and let $H$ be a subgraph of the corresponding graph $G'=G\setminus\set{s,t}$. We say that a cut $(A,B)$ in $H$ is \emph{well-structured} iff all edges of $E(A,B)$ are special edges (that is, edges that correspond to a matching.)


\begin{observation}
	Suppose we are given a well-structured graph $G$, a subgraph $H$ of $G\setminus\set{s,t}$, and a cut $(A,B)$ in $H$ of sparsity at most $\phi\leq \frac{1}{4\log m}$. Then there is a well-structured cut $(A',B)')$ in $H$, with $A'\subseteq A$ and sparsity at most $\phi\cdot 2\log m$. Moreover, there is an algorithm, that, given cut $(A,B)$, computes cut  $(A',B')$, in time $O(\min\set{\vol_H(A),\vol_H(B) })$.
\end{observation}

\begin{proof}
	We start with cut $(A,B)$ and inspect every vertex in $A$. If $v$ is any such vertex, and there is an edge $(v,u)$ in $E(A,B)$ that is not a special edge, we move $v$ from $A$ to $B$. Note that the only new edges that this move introduces into the cut $(A,B)$ are up to $\log m$ parallel special edges that enter $v$. Vertex $v$ is removed from $A$, and we say that edge $(v,u)$ is \emph{responsible} for this move. Notice that every regular edge of $E(A,B)$ is responsible for moving at most $1$ vertex from $A$ to $B$.
	
	Let $(A',B')$ denote the final cut. For convenience, denote $R=\min\set{|A|,|B|}$. It is easy to verify that $|B'|\geq R$ continues to hold, and $|A'|\geq |A|-|E(A,B)|\geq |A|-\phi\cdot R\geq |A|-\phi\cdot R\geq \frac{|A|}{2}$. Therefore, $\min\set{|A'|,|B'|}\geq \frac{\min\set{|A|,|B|}}{2}$. Notice also that $|E(A',B')|\leq |E(A,B)|\cdot \log m$, since every regular edge $e\in E(A,B)$ may cause at most $\log m$ special edges to be added to the cut. Altogether, we get that:
	
	\[\frac{|E(A',B'|)}{\min\set{|A'|,|B'|}}\leq \frac{|E(A,B)|\cdot 2\log m}{ \min\set{|A|,|B|}}\leq 2\phi\log m.\]
	
	The running time of the algorithm is bounded by $O(\vol_H(A))$. If $\vol_H(B)<\vol_H(A)$, then we can instead scan all vertices of $B$, and for each such vertex $u$ try to identify a regular edge $(v,u)\in E(A,B)$.
\end{proof}
\fi

\iffalse
\paragraph{Vertex Cuts and their Expansion.} 
Let $G$ be a directed graph. A \emph{vertex cut} in $G$ is an ordered triple $(A,S,B)$ of subsets of vertices of $G$ that partition $V(G)$, such that there is no edge connecting a vertex of $A$ to a vertex of $B$ and $A,B\neq\emptyset$. The sparsity of the cut is $\frac{|S|}{\min\set{|A|,|B|}}$.


\begin{observation}\label{obs: vertex cut to well structured}
	Suppose we are given a
	simple  bipartite graph $H=(L,R,E)$, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$,   together with a vertex cut $(A,S,B)$ in $H$ of sparsity $0<\phi<1$. Then in time $O(|S|)$ we can compute a well-structured cut $(X,Y)$ in $H$ of sparsity at most $\phi$ with $X\subseteq A\cup S$ and $Y\subseteq B\cup S$.
\end{observation}

\begin{proof}
	We start with $X=A$, $Y=B$, and then consider the vertices $v\in S$ one by one. Let $v\in S$ be any such vertex, and assume first that $v\in L$. In this case, no regular edge enters $v$, and at most one  special edge enters it. We place $v$ in $Y$ in this case, so it may only contribute a single special edge to $E(X,Y)$ and no regular edges. Similarly, if $v\in R$, then no regular edges may leave $v$, while at most one special edge leaves $v$. In this case we place $v$ in $X$, and it contributes at most $1$ special edge and no regular edges to $E(X,Y)$. Since no edges connect vertices of $A$ to vertices of $B$, it is immediate to verify that $|E(X,Y)|\leq |S|$ holds at the end of this procedure, while $|X|\geq |A|$ and $|Y|\geq |B|$. Moreover, all edges in $E(X,Y)$ are special, so the cut is well-structured, and its sparsity is at most $phi$.
\end{proof}
\fi

\subsection{\maintaincluster Problem}

We now define a new problem, called \maintaincluster problem. Intuitively, the purpose in this problem is to maintain an expander-like subgraph of a given input graph, and to support short-path queries between pairs of its vertices.


\paragraph{Definition of \maintaincluster Problem.}
The input to the problem is a 
simple  directed bipartite graph $H=(L,R,E)$, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$, together with integral parameters $d^*>0$ and $\Delta>0$. We are also given a parameter $m^*$ (the number of edges in the original graph $G$), with $|E|\leq m^*$. All edge lengths in $H$ are unit. 
%The edges of $E(L,R)$ are called \emph{regular}, and the edges of $E(R,L)$ are called \emph{special}. A cut $(X,Y)$ in $H$ is \emph{well-structured} iff all edges of $E(X,Y)$ are special. 
The algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration, the algorithm is given some pair $x,y\in V(H)$ of vertices, and it must return a simple path $P$ connecting $x$ to $y$, whose length is at most $d^*$. After that, some edges of $P$ may be deleted from $H$. If some edge of $H$ participated in $\ceil{\log m^*}$  of the paths that the algorithm returned, then such an edge is always deleted from $H$. At any time, the algorithm may provide a well-structured cut $(X,Y)$ in $H$, whose sparsity is at most $O\left(\frac{\log^4n}{d^*} \right )$. If $|X|\leq |Y|$, then the cut must be provided by listing the vertices of $X$, and otherwise it must be provided by listing the vertices of $Y$. After that the vertices of the smaller side of the cut are deleted from $H$. In other words, if $|X|\leq |Y|$, then we continue with the graph $H[Y]$, and otherwise we continue with the graph $H[X]$. Once the number of vertices in $H$ falls below half the original number, the algorithm halts, even if fewer than $\Delta$ iterations occurred.

Below is our main theorem for the \maintaincluster problem. The proof is deferred to \Cref{sec: expander algs}.

\begin{theorem}\label{thm: main for expander tools}
	There is an algorithm for the \maintaincluster problem, that, given an $n$-vertex graph $H$ as in the problem definition and parameters $c^*\log^4n\leq d^*\leq  n$, and $1\leq \Delta\leq n$, where $c^*$ is a large enough constant, has running time at most: \[\otilde(|E(H)|\cdot d^*+n^2)\cdot  \max\set{1,\frac{\Delta\cdot (d^*)^2}{n}}. \]
\end{theorem}



We note that the running time of the algorithm in the above theorem includes both the total update time of the data structure and the time needed to respond to queries.
We also note that some of the results from \cite{SCC} can be viewed as providing an algorithm for the \maintaincluster problem. In particular, by combining their Theorem 4.3 with Theorem 4.4 and Theorem 4.5, one can obtain such an algorithm (except for minor technical differences, e.g. the algorithm produces sparse vertex cuts and not edge cuts). The total update time of their algorithm is roughly $\ohat(|E(H)|\cdot (d^*)^2)$. Our algorithm achieves a better running time for the specific setting that we consider, and it is also significantly simpler.




Our algorithm consists of two parts. The first part is responsible for maintaining an \ATO $(\xset,\rho)$ of graph $G$, and the second graph essentially executes the algorithm from \Cref{thm: almost DAG routing} on the corresponding contracted graph $G_{|\xset}$. We now describe each of the two parts in turn.

\subsection{Part 1: Maintaining  the \ATO.} 
In this part we will work with a graph $\hat G$ that is obtained from $G\setminus \Elong$, by setting the length of every edge to $1$, and removing parallel edges. Notice that $\hat G$ is a dynamic graph that undergoes online edge deletions. We will maintain an \ATO  $(\xset,\rho)$ for this graph (that will naturally also define an \ATO for $G$).

We start with a partition $\xset$ of $V(\hat G)$, containing three sets: $S=\set{s},T=\set{t}$, and $X=V(\hat G)\setminus \set{s,t}$.
Their corresponding intervals are initialized to $I_S=\set{1}$, $I_T=\set{n}$, and $I_X=\set{2,\ldots,n-1}$. For convenience, we call the sets of vertices in $\xset$ \emph{clusters}.




 Whenever a new cluster $X$ joins $\xset$ (excluding the sets $S$ and $T$), we set ${d_X=\frac{|X|}{n}\cdot d}$. If $d_X\geq c^*\log^4|X|$, where $c^*$ is the constant from \Cref{thm: main for expander tools}, then we say that $X$ is a \emph{non-leaf cluster}. We then immediately initialize the algorithm for the \maintaincluster problem from \Cref{thm: main for expander tools} on the corresponding graph $\hat G[X]$, with distance parameter $d^*=d_X$, and parameter $\Delta$ remaining unchanged.
 If $d_X<c^*\log^4|X|$, then we say that $X$ is a \emph{leaf} cluster. We then replace $X$ in set $\xset$ with $|X|$ new clusters, each of which consists of a single distinct vertex of $X$. For each such new cluster $\set{v}$, we assign an interval $I_{\set{v}}\subseteq I_X$, that consists of a single integer arbitrarily, but we ensure that the intervals assigned to vertices of $L$ appear before intervals assigned to vertices of $R$. This ensures that all regular edges of $X$ are left-to-right edges, and the special edges are right-to-left edges. We call all special edges of $X$ \emph{bad edges}, and we say that $X$ is responsible for these edges. Clearly, $X$ is responsible for at most $|X|$ bad edges, and each such bad edge $e$ has $\spann(e)\leq |X|$. Observe that, since $d_X=\frac{|X|}{n}\cdot d$ and $d_X< c^*\log^4|X|\leq c^*\log^4n$, it must be the case that $|X|\leq \frac{c^*n\log^4n}{d}$.


  For convenience, for every cluster $X$, we denote by $X_0$ the set $X$ of vertices at the time when it first joined $\xset$, and we will also sometimes denote $d_{X}$ by $d_{X_0}$.
  
 Consider now some non-leaf cluster $X$. 
Recall that the algorithm from \Cref{thm: main for expander tools}, when applied to $X$,  has running time at most: 

\[\otilde(|E(\hat G[X])|\cdot d_X+|X_0|^2)\cdot  \max\set{1,\frac{\Delta\cdot (d_X)^2}{|X|}}. \]

Since $d_X=\frac{|X|}{n}\cdot d$ and $d=\sqrt{\frac{ n}{\Delta}}$, we get that  $\frac{\Delta\cdot d_X^2}{|X|}=\frac{\Delta \cdot |X| d^2}{n^2}=\frac{|X|}{n}\leq 1$. Therefore, the running time of the algorithm is bounded by:

\[\otilde(|E(\hat G[X])|\cdot d_X+|X_0|^2).\]
 
 Once the number of vertices in $X$ falls below $|X_0|/2$, the algorithm from  \Cref{thm: main for expander tools} terminates. We then terminate the algorithm from \Cref{thm: main for expander tools}, and update the distance parameter $d_X=\frac{|X|}{n}\cdot d$. If $d_X\geq c^*\log^4|X|$, then we apply the algorithm from \Cref{thm: main for expander tools} to this new cluster $X$ again, with the updated parameter $d_X$; otherwise cluster $X$ becomes a leaf cluster and is treated as such. In any case,  we will think of $X$ as a set that newly joined $\xset$. 





Whenever the algorithm for the \maintaincluster problem on graph $\hat G[X]$ produces a cut $(A,B)$ in $\hat G[X]$ of sparsity at most $O\left(\frac{\log^4n}{d_X} \right )$, we proceed as follows. 
 We partition inteval $I_X$ into two intervals: interval $I_A\subseteq I_X$ of length $|A|$ and interval $I_B\subseteq I_X$ of length $|B|$, so that $I_B$ appears to the left of $I_A$. We say that set $X_0$ \emph{owns} the edges in $E(A,B)$ and $E(B,A)$. Notice that edges of $E(B,A)$ are directed from left to right, and edges of $E(A,B)$ are directed from right to left. We will say that the edges of $E(A,B)$ are \emph{bad} edges. 
Recall that, if $|A|\leq |B|$, the algorithm for the \maintaincluster problem deletes $A$ from $X$ and continues with the new set $X=B$.
We then assign interval $I_B$ to the new set $X=B$, and we add the set $A$ to the collection $\xset$ of vertex subsets that we maintain (after which the algorithm for the \maintaincluster problem is applied to $\hat G[A]$ if it is a non-leaf cluster, or it is processed as a leaf cluster otherwise). We say that set $X$ of vertices just underwent \emph{splitting}, and that cluster $A$ was split off from it. Similarly, if $|B|<|A|$, the algorithm for the \maintaincluster problem deletes $B$ from $X$ and continues with the new set $X=A$.
We then assign interval $I_A$ to the new set $X=A$, and we add the set $B$ to the collection $\xset$ of vertex subsets that we maintain. We say that set $X$ of vertices just underwent splitting, and that cluster $B$ was split off from it.

It is easy to verify, using standard accounting methods, that the total number of bad edges that cluster $X_0$ owns at the end of the algorithm is bounded by $\otilde\left(\frac{|X_0|}{d_X}\right )$. It is also easy to verify that each such bad edge $e$ has $\spann(e)\leq |X_0|$ when it first becomes a bad edge, and from that point onward $\spann(e)$ may only decrease.
This completes the description of the first part of the algorithm. We now bound its total update time and the total span of all bad edges.

\paragraph{Bounding the Total Update Time of Part 1.}
Let $\xset^*$ be the collection of all non-leaf sets $X_0$ that were ever added to $\xset$, excluding $S$ and $T$. For all $0\leq i\leq \floor{\log n}$, let $\xset_i\subseteq \xset^*$ be the collection of all sets $X_0$ with $2^i\leq |X_0|<2^{i+1}$. It is easy to verify that all sets in the collection $\xset_i$ are mutually disjoint, and so $|\xset_i|\leq \frac{n}{2^i}$. 

Recall that for each set $X_0\in \xset_i$, the total update time of the algorithm for the \maintaincluster problem on $\hat G[X]$ from \Cref{thm: main for expander tools} is most:

\[\otilde(|E(\hat G[X_0])|\cdot d_{X_0}+|X_0|^2).\]


Since $d_{X_0}=\frac{|X_0|}{n}\cdot d$ and $|X_0|\leq 2^{i+1}$, we get that this time is bounded by: 


\[
\begin{split}
\otilde(|E(\hat G[X])|\cdot d_X+|X_0|^2)&\leq\otilde \left(|E(\hat G[X])|\cdot \frac{|X_0|}{n}\cdot d+|X_0|^2\right ) \\
%&\leq  \ohat \left(\frac{|X_0|^3}{n}\cdot d+ \frac{|X_0|^3}{n^2}\cdot d^2\right )\\
&\leq \otilde \left(\frac{2^{i}\cdot |E(\hat G[X])|}{n}\cdot d+ 2^{2i}\right )
\end{split} \]

Since $|\xset_i|\leq \frac{n}{2^i}$, the total running time for all clusters $X_0\in \xset_i$ is bounded by: 

\[\otilde  \left(\frac{2^{i}\cdot |E(G)|\cdot d}{n}+ n\cdot 2^{i}\right )\]

 Summing up over all indices $i$, we get that the total update time of all algorithms for the \maintaincluster problem is bounded by ${\otilde \left(md+n^2\right )}$.


\paragraph{Bounding the Total Span of All Bad Edges.}
We partition the set of all bad edges into two subsets. The first subset, $E_1$, contains all edges that are owned by non-leaf clusters.

Recall that for all $0\leq i\leq \floor{\log n}$, every cluster $X_0\in \xset_i$  may be responsible for at most $\otilde\left(\frac{|X_0|\cdot }{d_{X_0}}\right)$ bad edges. Initially, when an edge $e$ is added to the set of bad edges, it has $\spann(e)\leq |X_0|$, and after that  its $\spann(e)$ value may only decrease. In our calculations, for each bad edge $e$, we consider the initial value $\spann(e)$, when the edge was just added to the set of bad edges. The summation of all $\spann(e)$ values of all bad edges owned by clusters in $\xset_i$ is then bounded by:

\[
\begin{split}
\sum_{X_0\in \xset_i}\otilde \left(\frac{|X_0|^2}{d_{X_0}}\right )& \leq \sum_{X_0\in \xset_i}\frac{|X_0|\cdot\otilde(n)}{d}\\
&\leq \otilde\left(\frac{n^{2}}{d}\right ),
\end{split}
\]


since $d_{X_0}=\frac{|X_0|}{n}\cdot d$.
We conclude that  $\sum_{e\in E_1}\spann(e)\leq \otilde\left(\frac{n^{2}}{d}\right )$.

We denote by $E_2$ the set of all bad edges that are owned by leaf clusters. Recall that each leaf cluster $X$ owns at most $|X|$ bad edges, and the $\spann(e)$ value of each such edge is bounded by $|X|\leq \otilde\left(\frac{n}{d}\right )$. Since all leaf clusters that were ever added to $\xset$ are disjoint, we get that $\sum_{e\in E_2}\spann(e)\leq \otilde\left(\frac{n^2}{d}\right )$. Overall, we get that the total span value of all bad edges is bounded by $\otilde\left(\frac{n^2}{d}\right )$.


So far we viewed $(\xset,\rho)$ as an \ATO in the graph $\hat G$. It equivalently defines an $\ATO$ in the original graph $G$. However, for each right-to-left edge $e$ of $\hat G$, we may now have up to $\log m$ parallel copies of $e$ in $G$, and additionally, for every long edge $e$, it is possible that the edge is a right-to-left edge.

Observe first that, from our discussion so far, $\sum_{e\in E(G)\setminus \Elong}\spann(e)\leq \otilde\left(\frac{n^2}{d}\right )$ holds at all times (recall that $\Elong$ is the set of the long edges).

As long as Condition 
\ref{stopping conditionfinal} holds, since the paths in $\qset$ are edge-disjoint, there must be some $s$-$t$ path $Q$ whose length is at most $\Lambda$ in the current graph, and $\sum_{e\in E(Q)\setminus \Elong}\spann(e)\leq 
\otilde \left(\frac{n^{2}}{d}\cdot  \frac{512\log^2m}{\Delta}\right )=\otilde \left(\frac{n^{2}}{d\cdot \Delta}\right )$.

Since every edge $e\in \Elong$ has length at least $\frac{\Lambda}{64d\log m}$, and the length of $Q$ is at most $\Lambda$, we get that at most $64d\log m$ edges of $\Elong$ may lie in $Q$. Since for each such edge $e\in \Elong$, $\spann(e)\leq n$, we conclude that:
$\sum_{e\in E(Q)}\spann(e)\leq \otilde \left(\frac{n^{2+o(1)}}{d\cdot \Delta}+n\cdot d\right )$.


It is then immediate to verify that, for this path $Q$, $\sum_{e\in E(Q)}\skipp(e)\leq \otilde \left(\frac{n^{2}}{d\cdot \Delta}+n\cdot d\right )$. By selecting an appropriate parameter $\Gamma=\otilde \left(\frac{n^{2}}{d\cdot \Delta}+n\cdot d\right )$, we ensure that, as long as Condition \ref{stopping conditionfinal} holds, there is an $s$-$t$ path $Q$ in $G$ with $\sum_{e\in E(Q)}\skipp(e)\leq \Gamma/4$, such that the length of $Q$ is at most $\Lambda$.



\subsection{Part 2: Solving \DLSSSP on the Contracted Graph}
The second part of our algorithm maintains the contracted graph $H=G_{|\xset}$. Once this graph is intialized, it is easy to verify that all changes to this graph can be implemented via vertex-splitting and edge-deletion updates. Whenever a cluster $A$ is split off from some cluster $X\in \xset$, we perform a vertex splitting operation, in which vertex $v_A$ is split off from $v_X$. We include in the corresponding set $E'$ all edges that have one endpoint in $A$ and another outside of $A$. Notice that each such edge either connects a vertex of $A$ and a vertex of $X$; or it has one endpoint in $A$ and another in $V(G)\setminus\set{A\cup X}$. In the latter case, if $e=(a,b)$ with $a\in A$ and $b\not\in A\cup X$, then edge $(v_X,v_Y)$, where $Y$ is the cluster of $\xset$ containing $b$, was already present in $H$. After the vertex-splitting update is complete, we delete this edge from $H$ via standard edge-deletion update. Similarly, if the edge is $e=(b,a)$ with 
$a\in A$ and $b\not\in A\cup X$, then edge $(v_Y,v_X)$, where $Y$ is the cluster of $\xset$ containing $b$, was already present in $H$. After the vertex-splitting update is complete, we delete this edge from $H$ via standard edge-deletion update. Notice that this introduces a number of extra edges in graph $H$. For every edge $e$, whenever a cluster containing one endpoint $a$ of $e$ is split, if $a$ belongs to the smaller side of the partition, then a new copy of $e$ is introduced into $H$ and then the older copy is deleted from it. But it is easy to verify that for each edge $e$ of $G$, at most $\log n$ copies may be introduced, so the number of edges ever present in $H$ is still bounded by $O(m\log^2m)$.



For every edge $e$ of $H$, the weight $w(e)$ is set to be the smallest integral power of $2$ that is greater than $\skipp(e)$. Recall that the value $\skipp(e)$ of an edge may grow overtime. In order to avoid having to  insert edges into $H$ outside of the vertex-splitting updates, for every edge $e$, for every integer $\ceil{\log(\skipp(e))}\leq i\leq \ceil{\log n}$, we add a copy of $e$ whose weight is $2^i$. As the value $\skipp(e)$ grows, we simply remove copies of $e$ as needed. The total number of edges ever present in $H$ is now bounded by $O(m\log^3m)$.

Consider now some vertex $v_X\in V(H)$, and some integer $0\leq i\leq \ceil{\log n}$. Recall that we have denoted by  $U_i(v)=\set{u\in V(H)\mid \exists e=(v,u)\in E(H)\mbox{ with } w(e)=2^i}$. 
Equivalently, if we denote $v=v_X$, then set $U_i$ contains all nodes $v_Y$, such that some edge $e$ of $H$ connects a vertex of $X$ to a vertex of $Y$, and has value $\skipp(e)\leq 2^{i}$. In particular, the distance between intervals $I_X$ and $I_Y$ is at most $2^i$, and so at most $2^i$ other intervals may lie between them. Therefore, it is immediate to verify that $|U_i(v)|\leq 2^{i+1}$ always holds, establishing Property \ref{prop: few close neighbors}	

We apply the algorithm from \Cref{thm: almost DAG routing} to the resulting instance of the \DLSSSP problem, with the parameter $\Gamma$ that we defined above, distance parameter $d=\Lambda$, and $\eps=1/16$. Recall that the algorithm may only return FAIL if the current graph $H$ does not contain any $s$-$t$ path $P$  with $\sum_{e\in E(P)}\ell(e)\leq \Lambda$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$. From our discussion, this may only happen when Condition \ref{stopping conditionfinal} is violated. Recall that the running time of the algorithm is bounded by:


\[\otilde \left(n\cdot \Lambda+ m + \Gamma\cdot n\right )\leq \otilde \left(\frac{n^2}{\Delta}+ n^{2}\cdot d+\frac{n^{3}}{d\cdot \Delta}\right )\leq \otilde \left(n^2d+\frac{n^{3}}{d\cdot \Delta}\right ).\]


The total running update time of both parts of the algorithm is bounded by:


\[\otilde \left(n^{2} d+\frac{n^{3}}{d\cdot \Delta}\right ) \]


Substituting the value $d=\sqrt{n/\Delta}$, we obtain total update time:

\[{\otilde\left(\frac{n^{2.5}}{\sqrt{\Delta}}\right ) }\]





\paragraph{Completing the Algorithm.}
At the beginning of every iteration, we use the algorithm from \Cref{thm: almost DAG routing} to compute a simple $s$-$t$ path $P$ in graph $H$, whose length is at most $(1+6\eps)\Lambda\leq 1.5\Lambda$. Let $(v_S=v_{X_1},v_{X_2},\ldots,v_{X_k}=v_T)$ be the  sequence of supernodes on this path. For all $1\leq j<k$, let $e=(x_j,y_j)$ be the corresponding edge in graph $G$, with $x_j\in X_j$ and $y_j\in X_{j+1}$.

For all $1< j< k$, we use the data structure from the MaintainCluster problem on graph $G[X_j]$ in order to compute a path $Q_j$, connecting $y_j$ to $x_{j+1}$. Recall that the path contains at most $d_{X_j}$ edges, and, since each such edge is short, the length of the path in $G$ is bounded by $d_{X_j}\cdot \frac{\Lambda}{64d\log m}$.

We let $P'$ be the path obtained by concatenating $e_0,Q_1,e_1,\ldots,Q_k,e_k$. It is easy to see that $P'$ is an $s$-$t$ path in the current graph $G$. Next, we bound its length. Recall that the length of the original path $P$ was at most $1.5\Lambda$. The total lengths of all paths in $\set{Q_1,\ldots,Q_k}$ can be bounded by:

\[ 
\begin{split}
 \frac{\Lambda}{64d\log m}\cdot \sum_{j=1}^k d_{X_j}&\leq \frac{\Lambda}{64d\log m}\cdot \sum_{X_0\in \xset^*}d_{X_0}\\
&\leq \frac{\Lambda}{64d\log m}\cdot \sum_{i=0}^{\floor{\log n}}\sum_{X_0\in \xset_i}d_{X_0}\\
&=\frac{\Lambda}{64d\log m}\cdot \sum_{i=0}^{\floor{\log n}}\sum_{X_0\in \xset_i}\frac{|X_0|}{n}\cdot d\\
&\leq \frac{\Lambda}{64d\log m} \cdot d\log m\\
&\leq \frac{\Lambda}{16},
\end{split}
 \]


since for all $X_0\in \xset$, $d_{X_0}=\frac{|X_0|}{n}\cdot d$, and for all $0\leq i\leq \floor{\log n}$, $\sum_{X_0\in \xset_i}|X_0|\leq n$.
Altogether, the length of the final path $P'$ is bounded by $2\Lambda$ as required. In time $O(\Lambda)$, we turn path $P'$ into a simple path that the algorithm then returns.

After our algorithm returns a path $Q$, it is given a batch of edge deletions, with all deleted edges lying on $Q$. It will then update the \maintaincluster algorithms for clusters $X\in \xset$ with the edges that were deleted from $\hat G[X]$, and then update graph $H=G_{|\xset}$ with edge deletions and any vertex splits that may have resulted from splitting of clusters of $\xset$.

Recall that the algorithm has at most $\Delta$ iterations. In every iteration, the time required to compute the initial path $P$ in graph $H$ is bounded by $O(|E(P)|)\leq O(\Lambda)$. The time that is required to respond to \shortpath queries within the clusters $X_j$ is already accounted for as part of total running time of the \maintaincluster algorithm on $\hat G[X_j]$. We may spend up to $O(\Lambda)$ additional time in order to transform the resulting path into a simple one. Therefore, the additional time required to compute the paths is bounded by $O(\Delta\cdot \Lambda)\leq \otilde(n)$. The total running time of the algorithm is bounded by ${\otilde \left(\frac{n^{2.5}}{\sqrt{\Delta}}\right ) }$.




\iffalse

\subsection{Quick Run Time Calculations}

\begin{itemize}
	\item total: $T(m,n,\Delta)+n^{1.5}+m\Delta$.
	
	\item Threshold for paths lengts: $n/\Delta$.
	\item with parameter $d<n/\Delta$:
	
	\begin{itemize}
		\item short paths: $O(md)$
		\item expanders (best case): $n^2d$.
		\item ATO calculations: add $n/d$ edges of span $n$, so total span $n^2/d$. This is distributed among $\Delta$ paths, with overhead $n$ get time: $\frac{n^3}{\Delta d}$. This adds unweighted length $d$ to each path. Because we allow path lengths $n/\Delta$, we can handle edges of length up to $\frac{n}{\Delta d}$ (short edges).
		
		\item long edges: edges of length more than $\frac{n}{\Delta d}$: at most $d$ of them in one path. Each adds span $n$ to the path. so $n^2d$ total?
		
		Final: $n^{1.5}+m\Delta+n^2d+\frac{n^3}{\Delta d}$
		
		\item to equalize $n^2d$ with $n^3/(\Delta d)$, we need to choose $d=\sqrt{n/\Delta}$. Both terms become $n^{2.5}/\sqrt{\Delta}$.
		
		\item final bound is $O(m\Delta+n^{2.5}/\sqrt{\Delta})$. 
		
		\item let's assume that $m=n^{1.5}$. Then we get $n^{1.5}\Delta+n^{2.5}/\sqrt{\Delta}$. $\Delta^{3/2}=n$, $\Delta=n^{2/3}$. Bound becomes $n^{2.1}$.
		
		\item if we want to beat $m\sqrt{n}$, should set $\Delta=n^{1/2-\eps}$. Then we get $mn^{1/2-\eps}+n^{2.5-1/4+2\eps}=mn^{1/2-\eps}+n^{2.25+2\eps}=mn^{1/2-\eps}+n^{1/2-\eps}\cdot n^{1.75+3\eps}$.
		
		\item for $m=n^2$, we get $n^2\Delta=n^{2.5}/\sqrt{\Delta}$, so $\Delta^{3/2}=n^{1/2}$ and $\Delta=n^{1/3}$. Bound is $n^{2.333}$
	\end{itemize}

\item ES-tree isue in expanders: total number of edges ever deleted from $H$ is $\Delta\cdot d$. In the above calculations we used $d=\sqrt{n/\Delta}$, so $\Delta=\frac{n}{d^2}$. So total number of edge ever deleted from $H$ is at most $\frac{n}{d}$. Each edge deletion may force the deletion of $d$ edges from the expander. But then we only have $n^{o(1)}$ recomputations of expanders.

\item calculations for smaller graphs: $d_X=\frac{|X|}{n}\cdot d$. now total number of edges ever deleted is $\Delta\cdot d_X=\frac{|X|}{n}\cdot\Delta d\leq \frac{|X|}{n}\cdot\frac{n}{d}=\frac{|X|}{d}$, because $\Delta d=\frac{n}{d}$. So total number of edges ever deleted from expander: $\frac{|X|\cdot d_X}{d}<|X|$, because $d_X<d$.

\end{itemize}
\fi



\iffalse
\subsection{Discussion and Overview}

Currently, \cite{SCC} provide a proof of the above theorem with running time roughly $\ohat(|E(H)|(d^*)^2$. Our hope is to achieve the running time stated in the theorem, but with $\delta$ close to $0$. Below is a quick overview of the proof of \cite{SCC}, issues with it, how to adapt/improve it, etc.

The proof of the theorem consists of two parts.

\paragraph{Part 1.} This is a stand-alone part, that I'll call \APSP on expanders. Here, we are given an expander graph $G$ (with pretty good expansion, low vertex degrees etc, but the graph is directed), and it undergoes a sequence of edge deletions. Our goal is to maintain a sufficiently large \emph{core} $C\subseteq V(G)$ that is decremental (so we can delete vertices from $C$ but can't add them to $C$), and support short-path queries between {\bf vertices of $C$ only}. Given two such vertices $x,y$, we need to return an $x$-$y$ path $P$ in $G$, whose length is $\ohat(1)$, in time $\otilde(|E(P)|)$. The number of edge deletions that this process should be able to withstand is something like $n^{1-o(1)}$ (assuming that the expansion is $1/n^{o(1)}$, and the degrees are at least $n^{o(1)}$). A typical way to use this tool: if we have a graph $G'$ that is not quite an expander, but contains a large expander $G$, we can build an ES-tree in $G'$, that is rooted at the vertices of the core $C$ (in fact for directed graphs, two trees: an in-tree and an out-tree). If some vertex of $G'$ becomes too far from the core (distance more than some given threhsold), we can quickly compute a sparse cut. As long as no vertex is far from the core, we can support 
short-path queries between any pair of vertices of $G$: given two vertices $x,y$, we first use the ES-trees to connect both of them to/from the core, and then do short-path query in the core.

There is an algorithm in my paper with Thatchaphol for doing this, but it's in undirected graphs. In \cite{SCC} they extend this algorithm to directed graphs  (Theorem 4.5) but it's a bit messy because it needs to go through expander pruning for directed graph (which is a pain) and directed cut-matching game (which also needs a separate proof which they provide). If there is time before SODA I can try to generalize my distanced-matching game stuff to directed graphs and it should give a clean and self contained proof of this part.
But otherwise I think it's OK to just cite them for now. (but I'll need to check that their algorithm is combinatorial).

The algorithm for this part will take time $\ohat(n)$ (because the expander has low degree).

\paragraph{Part 2.}
The algorithm that proves \Cref{thm: main for expander tools} works in at most $d^*$ iterations. In every iteration, we start with current graph $H$ and embed a large expander into it (if we can't do it we'll find a sparse and balanced cut). The embedding is on paths of length at most $d^*$, and with congestion at most $d^*$. Because of this high congestion, after only $n/d^*$ edges are deleted from $H$, the expander will be destroyed. That's why we'll need $d^*$ iterations. Even just listing the embedding takes time $nd^*$, so time $n(d^*)^2$ is the minimum for this part.
Once we embed the expander, we use the $\ohat(n)$-time algorithm for \APSP in expanders. Additionally, the ES-tree rooted at the core of the expander will take time $O(md^*)$, and that will need to be recomputed every $d^*$ iterations. This is the first main bottleneck.

Expander embedding is done through the cut-matching game. The algorithm for the cut player is super efficient and not a problem (except that we'll need to check if it's combinatorial for directed graphs and the proof is not super complicated).

The second main bottleneck is the algorithm for the matching player. Given two sets $A,B$ in the input graph $G$, we should either connect many pairs with paths of lenghts $O(d^*)$, or compute a sparse balanced cut. This can be implemented by simple greedy path peeling, but that would require time $O(md^*)$, and cause higher congestion, $O((d^*)^2)$, so all this will also need to be repeated $\ohat((d^*)^2)$ times, which is not good.
Even if we use MWU, the best we could hope for would be time $O(md^*)$ per iteration (because we'd need to do SSSP up to depth $d^*$), and that again will need to be repeated $O(d^*)$ times, with total time $O(m(d^*)^2)$, which is too high.


One way to fix all this: we'll have at most $\Delta$ iterations, in every iteration at most $d^*$ edges are deleted from the graph. Using the best current balancing between $\Delta$ and $d$ (that optimizes the total running time of the algorithm while ignoring this part), total number of edges ever deleted from the graph becomes $\Delta d=n/d$, each of them gives rise to up to $d$ edge deletions in the expander, so in total at most $n$ edges are deleted from the expander. This means that instead of $d^*$ iterations we'll have $n^{0(1)}$ iterations. Now it looks like simple MWU may work for the matching player, and a simple ES-tree up to depth $d^*$ to connect the whole graph to the core of the expander. This kind of argument is OK for the current balancing of the parameters. If we will want in the future a different balancing, we'll need to do this differently (my idea in commented out part, only for the matching player, not for the ES-tree).



In this section we provide an algorithm for the restricted \SSSP problem, proving \Cref{thm: sssp main}. Recall that we are given as input a well-structured graph $G$ of size $m$ (see \Cref{def: well-structured}), where $m$ is a given parameter, together with another parameter $\Delta>0$. We denote $|V(G)|=n$ and  ${\Lambda=\frac{2^{11}n\log^2m}{\Delta}}$. For every edge $e\in E(G)$, we are also given a length $\ell(e)$, that is an integral power of $2$ between $1$ and $2\Lambda$. 



The algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration, the algorithm must compute an $s$-$t$ path $P$ in the current graph $G$ of length at most $2\Lambda$. We assume that for each edge $e\in E(P)$, edge $e$ is the shortest from among its parallel copies. Every edge on $P$ is then deleted from $G$, and the iteration ends.

The algorithm is allowed, at any time, to halt and return FAIL, but it may only do so if the  following condition is violated:


\begin{properties}[2]{C}
	\item Let $\qset$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $G$, such that the paths in $\qset$ are internally vertex-disjoint, every path has length at most  $\Lambda$  in the current graph. Then ${|\qset|\geq \frac{\Delta}{512\log^2m}}$ holds. \label{stopping conditionfinal}
\end{properties} 



We use a parameter ${d=\sqrt{n/\Delta}}$.
We say that an edge $e\in E(G)$ is \emph{long} if ${\ell(e)\geq \frac{\Lambda}{64d\log m}}$, and otherwise we say that it is short.
We denote the set of all long edges by $\Elong$.
\fi

==> STSP-oracle.tex <==
\subsubsection{From $r$-Restricted Oracle to $r$-Restricted \routeandcut}

We now show that, if we are given an algorithm for the $r$-restricted \stSP problem, then we can obtain an algorithm for $r$-restricted \routeandcut problem, with the same asymptotic running time.


\begin{theorem}\label{thm: oracle to routing} Suppose there is an algorithm for the $r$-restricted \stSP problem, that, given on an input $(G,A,B,\Delta,\eta)$ with $|V(G)|=n$, has running time at most $T(n,\Delta,\eta)$. Then there is an algorithm for the $r$-restricted \routeandcut problem, that, on input $(G,A,B,\Delta,\eta)$ei with $|V(G)|=n$, either produces a valid output to the problem, or returns ``FAIL'', such that the probability that the algorithm returns ``FAIL'' is at most $1/2$, and its running time is at most $T(n,\Delta,\eta)+O(|E(G)|)$.
\end{theorem}

\begin{proof}
Let $(G=(L,R,E),A,B,\Delta,\eta)$ be an instance of the $r$-restricted \routeandcut problem. Throughout, we denote $m=|E|$. 
As before, we
let $\qset^*$ denote the largest-cardinality routing from $A$ to $B$ in $G$ with congestion at most $\eta$.
We partition the set $\qset^*$ of paths into two subsets, as before: set $\qset^*_1$ contains all paths $Q\in \qset^*$ that consist of a single regular edge, and set $\qset^*_2$ contains all remaining paths. As before, we construct a maximal set $\qset_1$ of disjoint paths, where every path connects a distinct vertex of $A$ to a distinct vertex of $B$, and consists of a single regular edge, in time $O(m)$, so that $|\qset_1|\geq |\qset^*_1|/2$ holds, and we delete the endpoints of the paths in $\qset_1$ from $A$ and $B$, respectively, so that $G$ no longer contains a regualar edge connecting a vertex of $A$ to a vertex of $B$.

Let $\aset$ denote the algorithm for the $r$-restricted \stSP from the statement of \Cref{thm: oracle to routing}.
We then construct the graphs $\hat G$ and $H$ as described above, and we initialize  Algorithm $\aset$ on graph $G$, with parameters $\Delta$ and $\eta$ that remain unchanged, and the sets $A,B$ of vertices that no longer contain the endpoints of the paths in $\qset_1$.


Next, we apply Algorithm \algmwu to graph $\hat G$, where we use Algorithm $\aset$ as the oracle. Specifically, in every iteration, if Algorithm $\aset$ produces an $s$-$t$ path $P$ of length at most $\Lambda$ in graph $H$, together with a set $\tilde E$ of special edges in $H$, then we are guaranteed that the length of $P$ in $\hat G$ is at most $1$. We add $P\setminus\set{s,t}$ to $\pset$, double the length of every edge in $\tilde E$, set the lengths of the first and the last edge on $P$ to $1$ in $\hat G$, and continue to the next iteration. If Algorithm $\aset$ establishes that Condition \ref{stopping condition3} no longer holds in $H$, then we are guaranteed that Condition \ref{stopping condition2} is violated in $\hat G$, and we terminate the algorithm.
If Algorithm $\aset$ ever returns ``FAIL'', then we terminate our algorithm and return ``FAIL'' as well. From the definition of the \stSP problem, this may happen with probability at most $1/2$.

It is easy to verify that the running time of the algorithm is dominated by the running time of Algorithm $\aset$, except for $O(m)$ time that we spend on the construction of graph $\hat G$. Therefore, the running time of the algorithm so far is bounded by $T(n,\Delta,\eta)+O(m)$ (our algorithm does not need to update the lengths of the edges explicitly, it is sufficient that this is done by the algorithm for the \stSP problem).
We denote by $\qset_2$ the set $\pset$ that is obtained at the end of the algorithm, and we let $\qset=\qset_1\cup \qset_2$.

Let $A'\subseteq A,B'\subseteq B$ denote the sets of vertices that do not serve as endpoints of the paths in $\qset$.
It now remains to show that the paths in $\qset$ cause edge-congestion at most $O(\eta\poly\log n)$, and that, if $|\qset^*|\geq \Delta$, then $|\qset|\geq \Delta/\poly\log n$. Additionally, we need to compute a cut $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{\Delta}{\eta\log^4n}+\frac{3|\qset|}{\eta}$, such that $A'\subseteq X$ and $B'\subseteq Y$ holds.
We start by proving that the final collection $\qset$ of paths has all required properties, using the following claim.

\begin{claim}\label{claim: appox MWU}
	Let $\pset$ be the set of paths obtained at the end of Algorithm \algmwu. Then every edge of $G$ belongs to at most $8\eta\cdot \log^{\hat c+1}n$ paths of $\pset$. Moreover, if $|\qset_2|\geq \frac{\Delta}2$, then $|\pset|\geq \frac{\Delta}{2^{13}\log^{\hat c+1}n}$.
\end{claim}

\begin{proof}
	We start by proving that every special edge of $\hat G$ belongs to at most $4\eta\cdot \log^{\hat c+1}n$ paths of $\pset$. Consider any such special edge $e$. Recall that, at the beginning of the algorithm, we set $\ell(e)=\frac{1}{\Lambda}=\frac{\Delta}{n\eta \cdot \log^5n}$. Let $i_1,i_2,\ldots,i_q$ denote the indices of the iterations when $\ell(e)$ was doubled. Notice that, once $\ell(e)$ grows above $1$, it may no longer be used by any paths that are added to $\pset$, so $q\leq 2\log \Lambda\leq 4\log n$ must hold.  Property \ref{oracle-prop: edge congestion} further ensures that, for all $1\leq j<r$, the number of paths that were added to $\pset$ between iteration $i_j$ and iteration $i_{j+1}$, that contained $e$, is bounded by $\eta\cdot \log^{\hat c}n$. Therefore, altogether $e$ may belong to at most $4\eta\cdot \log^{\hat c+1}n$ paths in $\pset$.
	
	 Consider now some regular edge $e=(u,v)$. Recall that no regular edge in $G$ may connect a vertex of $A$ to a vertex of $B$. Therefore, if a path $P\in \pset$ contains $e$, then it must contain either the unique special edge that is incident to $u$ (if it exists), or the unique special edge that is incident to $v$ (if it exists). Since every special edge appears in at most $4\eta\cdot \log^{\hat c+1}n$
	  paths in $\pset$, every regular edge of $G$ belongs to at most $8\eta\cdot \log^{\hat c+1}n$ paths in $\pset$. We conclude that the paths in $\pset$ cause edge-congestion at most $8\eta\cdot \log^{\hat c+1}n$ in $G$.
	
	Next, we assume that $|\qset_2|\geq \frac{\Delta} 2$, and we prove that that $|\pset|\geq \frac{\Delta}{2^{13}\log^{\hat c+1}n}$.  
	Let $q$ be the total number of iterations in the algorithm, so $|\pset|=q$ holds. Recall that, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{n}{\Lambda}=\frac{\Delta}{\eta\cdot \log^5n}$ held, since 
	$\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$. Moreover, since the initial length of every regular edge is $0$, and the capacities of the special edges are $\eta$, we get that, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}c(e)\cdot \ell(e)\leq \frac{\Delta}{\log^5n}$ held.
	
	
	
	In every iteration $i$, we doubled the lengths of all edges in set $\tilde E_i$ (each of which has capacity $\eta$), and we also increased the lengths of the first and the last edge on $P_i$ from $0$ to $1$ (each of these edges has capacity $1$). Therefore, $\sum_{e\in E(\hat G)}c(e)\ell(e)$ grows by (additive) $2+\eta\cdot C_i$ in iteration $i$. From Property \ref{oracle-prop: small length growth} of the oracle, and since the length of every special edge in $H$ is $\Lambda$ times its length in $\hat G$, we are then guaranteed that, at the end of the algorithm: 
	
	\[\sum_{e\in E(\hat G)}c(e)\ell(e)\leq \frac{\Delta}{\log^5n}+\frac{\eta}{\Lambda}\cdot \sum_{i=1}^qC_i+2|\pset|
	\leq \frac{\Delta}{\log^5n}+q\cdot (\log n)^{\hat c}\leq \frac{\Delta}{\log^5n}+ 2|\pset|\cdot (\log n)^{\hat c}.\] 
	
	
	%	It is immediate to verify that the paths in $\pset$ cause congestion $O(\log m)$, since we set the length of every edge $e$ to be $1/m$ initially, and then double it every time a path is added to $\pset$ contains $e$. Since all paths in $\pset$ have length at most $1$, once $\ell(e)>1$ holds, the edge may no longer be used by paths that are newly added to $\pset$. Therefore, the length of $e$ may be doubled at most $O(\log m)$ times, and at most $O(\log m)$ paths in $\pset$ may use $e$.
	
	Consider now the following thought experiment. We start with the set $\pset$ of paths, and the edge lengths in graph $\hat G$ that were obtained at the end of Algorithm \algmwu. Let $G_1$ denote the resulting graph (which is identical to $\hat G$ but may have different edge lengths).
	
	Next, we will construct another set $\pset'$ of paths in $G_1$, as follows. Initially, we let $\pset'=\emptyset$, and we let $G_2$ be the copy of the graph $G_1$. %For every special edge $e\in E(G_2)$, we maintain a counter $n(e)$, that counts the number of paths containing $e$ that have been added to $\pset'$ since the last time $\ell(e)$ was doubled (or since the beginning of the thought experiment if $\ell(e)$ was never doubled yet. 
	Then we iterate, as long as there is an $s$-$t$ path in $G_2$, whose length is at most $\frac{1}{1024\log n}$. In every iteration, we select an arbitrary simple $s$-$t$ path $P$ in $G_2$ of length at most  $\frac{1}{1024\log n}$, let $P'$ be the path obtained from $P$ by deleting the first and the last vertices from it, and add $P'$ to $\pset'$. We set the lengths of the first and the last edges on $P'$ to $1$, and we increase the length of every special edge $e\in E(P')$ by factor $\left(1+\frac{1}{\eta}\right)$. %If $n(e)$ reaches $\eta$ for any such edge $e$, then we double $\ell(e)$, and we set $n(e)=0$. 
	This algorithm terminates when every $s$-$t$ path in $G_2$ has length at least $\frac{1}{1024\log n}$. We denote by $G_3$ the graph $G_2$ that is obtained at the end of this algorithm (which is identical to $\hat G$ and to $G_2$, except for the edge lengths).
	In the following observation, we show that every special edge of $G_2$ may appear in at most $O(\eta)$ paths in $\pset'$, and, if $|\qset_2^*|\geq \Delta$, then $|\pset|+|\pset'|\geq \frac{\Delta}{2^{12}\log^{\hat c+1}n}$.
	
	\begin{observation}\label{obs: many paths}
		For every special edge $e\in E(G_2)$, the number of paths in $\pset'$ that contain $e$ is at most $8\eta\log n$. Moreover, if $|\qset_2^*|\geq \Delta$, then
		$|\pset|+|\pset'|\geq \frac{\Delta}{2^{12}\log^{\hat c+1}n}$.
	\end{observation}
	\begin{proof}
		Consider any special edge $e\in E(G_2)$. Recall that, at the beginning of the thought experiment, $\ell(e)\geq \frac{1}{\Lambda}\geq \frac{\Delta}{n\eta \cdot \log^5n}\geq \frac{1}{n^2}$ holds. Let $N$ be the number of paths in $\pset'$ that contain $e$. Since every time a path containing $e$ is added to $\pset'$, we increase $\ell(e)$ by factor $\left(1+\frac{1}{\eta}\right)$, we get that the final length of edge $e$ is at least $\frac{1}{n^2}\cdot \left(1+\frac{1}{\eta}\right)^N$. Since at the end of the algorithm $\ell(e)\leq 2$ must hold, we get that $N\leq 8\eta\log n$, and so $e$ may belong to at most $8\eta\log n$ paths in $\pset'$.
		
		
		Let $C=\sum_{e\in E(G_1)}c(e)\ell(e)$, and let $C'=\sum_{e\in E(G_3)}c(e)\ell(e)-C$. As observed already, $C\leq \frac{\Delta}{\log^5n}+ 2|\pset|\cdot (\log n)^{\hat c}$. During our thought experiment, in every iteration of the algorithm, we added a single path $P$ to $\pset'$, and increased $\sum_{e\in E(G_2)}c(e)\ell(e)$ by at most (additive) $2+\frac{1}{1024\log n}$. 
		Indeed, if $P$ is the path that was added to $\pset'$ during an iteration, and $P'$ is the path that is obtained from $P$ by deleting the first and the last vertex from it, then the lengths of the first and the last edges on $P$ increased by $1$ each, and each of these edges have capacity $1$. Additionally, since the total length of all special edges on $P'$ is bounded by $\frac{1}{1024\log n}$, the total increase in the lengths of the special edges on $P'$ is at most $\frac{1}{1024\eta \log n}$. Since each such edge has capacity $\eta$, we get that their total contribution to the increase in $\sum_{e\in E(G_2)}c(e)\ell(e)$ is bounded by $\frac{1}{1024\log n}$ 
		
		Therefore, the total increase in $\sum_{e\in E(G_2)}c(e)\ell(e)$ during the thought experiment is $C'\leq |\pset'|\cdot\left(2+\frac{1}{1024\log n}\right )$. Altogether, we get that:

		\[\sum_{e\in E(G_3)}c(e)\ell(e)=C+C'\leq \frac{\Delta}{\log^5n}+ 2|\pset|\cdot (\log n)^{\hat c}+2|\pset'|+\frac{|\pset'|}{1024\log n}\leq    \frac{\Delta}{\log^5n}+(|\pset|+|\pset'|)\cdot \log^{\hat c}n.\]
		
		% $|\pset|+|\pset'|\geq \frac{C+C'}{2\log^{\hat c}n}-\frac{\Delta}{2^{12}\log^{\hat c+1}n}$.
		
		Since, at the end of the algorithm, every $s$-$t$ path has length at least $\frac{1}{1024\log n}$, by multiplying the length of every edge in $G_3$ by factor $1024\log n$, we obtain a feasible solution to the dual LP (recall that graph $G_3$ is identical to $\hat G$, except for the edge lengths). Therefore, there is a solution to the dual LP on graph $\hat G$, whose value is:
		
		 \[C^*=(C+C')\cdot 1024 \log n \leq 1024(|\pset|+|\pset'|)\cdot \log^{\hat c+1}n+\frac{1024\Delta}{\log^4n}.\]
		 
		 
		If $|\qset^*_2|\geq \Delta/2$, then the  value of the optimal solution to the primal LP is at least $\Delta/2$,  and so is the value of the optimal solution to the dual LP, and so $C^*\geq \frac{\Delta}2$. Overall, we get that $|\pset|+\pset'|\geq \frac{\Delta}{2^{12}\log^{\hat c+1}n}$.
	\end{proof}
	
	From now on we assume that $|\qset_2^*|\geq \frac{\Delta} 2$, and we prove that $|\pset|\geq \frac{\Delta}{2^{13}\log^{\hat c+1}n}$.  Indeed, assume otherwise. Then $|\pset'|\geq \frac{\Delta}{2^{13}\log^{\hat c+1}n}$ must hold. We prove that this is impossible, by showing that, if this were the case, then, when Algorithm \algmwu was terminated, Condition \ref{stopping condition2} still held, leading to a contradiction. The following observation will then finish the proof of  \Cref{claim: appox MWU}.
	
	
	\begin{observation}\label{obs: few in P'}
		If $|\pset'|\geq \frac{\Delta}{2^{13}\log^{\hat c+1}n}$, then, at the time when \algmwu terminated, Condition \ref{stopping condition2} still held.
	\end{observation}
	\begin{proof}
		Recall that each path $P\in \pset'$ had length at most $\frac{1}{1024\log n}$ in graph $G_2$, when it was added to $\pset'$. Since edge lengths only grow overtime, every path $P\in \pset'$ has length at most $\frac{1}{1024\log n}$ in $G_1$. Consider a new graph $G^*$, that is obtained by taking the union of all edges and vertices that appear on the paths in $\pset'$. The length of every edge in $G^*$ is set to be its length in $G_1$. Denote $|\pset'|=k$. 
		Since every path in $\pset'$ has length at most $\frac{1}{1024\log n}$ in $G_1$, $\sum_{e\in E(G^*)}\ell(e)\leq\frac{k}{1024\log n}$. 
		
		
		Recall that every special edge of $G_1$ may belong to at most $8\eta\log n$ paths in $\pset'$. Due to the special structure of graph $G^*$, every vertex of $G^*\setminus\set{s,t}$ belongs to at most $8\eta\log n$ paths in $\pset'$. 
	By sending $\frac{1}{8\log n}$ flow units via every path in $\pset'$, we obtain an $s$-$t$ flow in $G^*$ that obeys edge capacities, and has value at least $\frac{k}{8\log n}$. From the integrality of flow, there is a collection $\rset$ of at least $\frac{k}{8\log n}$  $s$-$t$ paths in $H^*$ that obey edge capacities. We say that a path $Q\in \rset$ is \emph{long}, if its length is greater than $\frac{1}{64}$. Since $\sum_{e\in E(H^*)}\ell(e)\leq \frac{k}{1024
	\log n}$, the number of long paths in $\rset$ is bounded by $ \frac{k}{16\log n}$, and the remaining paths are short. 
		
%		Need: $\frac{64k}{z}\leq \frac{k}{16\log n}$. So $z=2^{10}\log n$.
		
		
		But then we obtain a collection of at least $\frac{k}{16\log n}\geq \frac{\Delta}{2^{17}\log^{\hat c+2}n}\geq \frac{\Delta}{\log^{2\hat c}n}$  $s$-$t$ paths of length at most $\frac{1}{64}$ each in $G_2$, that obey edge capacities. Therefore, when Algorithm \algmwu terminated, Condition \ref{stopping condition2} still held.
	\end{proof}
\end{proof}
\end{proof}

It is easy to verify that the endpoints of the paths in $\qset$ are all disjoint. Indeed, once a path consisting of a single special edge is added to $\qset_1$, its endpoints are deleted from $A$ and $B$ respectively. Moreover, whenever a path $P'$ connecting some vertex $a\in A$ to some vertex $b\in B$ is added to set $\pset$, we set the lengths of the edges $(s,a)$ and $(b,t)$ are set to $1$, so these edges may no longer be used in the future paths that the oracle returns. In particular, if $P''$ is a path that is added to $\pset$ afterwards, it may not originate from $a$, and it may not terminate at $t$. Recall that the paths in $\qset_1$ are edge-disjoint. From \Cref{claim: appox MWU}, every special edge of $G$ may participate in at most  $8\eta\cdot \log^{\hat c+1}n$ paths of $\qset_2$. Recall that, after the preprocessing step, we have ensured that there is no path in $G$ that connects a vertex of $A$ to a vertex of $B$ and consists of a single regular edge. Therefore, if $e=(u,v)$ is a regular edge of $G$, and $e$ participates in some path $Q\in \qset_2$, then $Q$ must contain either the unique special edge that is incident to $u$, or the unique special edge that is incident to $v$. Therefore, every regular edge of $G$ participates in at most $O(\eta\cdot \log^{\hat c+1}n)$ paths of $\qset_2$, and the total congestion that the paths in $\qset$ cause in $G$ is bounded by $O(\eta\cdot \log^{\hat c+1}n)$. Notice that, if $|\qset^*|\geq \Delta$, then either $|\qset_1^*|\geq \Delta/2$, or $|\qset_2^*|\geq \Delta/2$ must hold. In the former case, we are guaranteed that $|\qset_1|\geq |\qset_1^*|/2\geq\Delta/4$, while in the latter case, from \Cref{claim: appox MWU}, $|\pset|\ge \frac{\Delta}{2^{13}\log^{\hat c+1}n}$. Therefore, if $|\qset^*|\geq \Delta$, then $|\qset|\geq\frac{\Delta}{\poly\log n}$ must hold.

Recall that so far, the running time of the algorithm is bounded by $T(n,\Delta,\eta)+O(m)$. Let $A'\subseteq A,B'\subseteq B$ be the subsets of vertices that do not serve as endpoints of the paths in $\qset$. It now remains to compute a cut $(X,Y)$ in $G$, with $|E_G(X,Y)|\leq \frac{\Delta}{\eta\cdot \eta\log^4n}+\frac{|\qset|\cdot (\log n)^{\hat c}}{\eta}$, such that $A'\subseteq X$ and $B'\subseteq Y$. Recall that, if our did not terminate with a ``FAIL'', then it terminated because the algorithm for the $r$-restricted \stSP problem established that Condition \ref{stopping condition3} no longer holds in the current graph $H$. The algorithm also must have produced an assignment $\ell'(e)$ of non-negative lengths to edges of $ E(G)$, such that the length $\ell'(e)$ of every regular edge is $0$, and $\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta\cdot \Lambda}{2\eta\log^4n}+\sum_{e\in E(H)}\ell(e)$. 
In the remainder of this section, we use $\dist'_G(\cdot,\cdot)$ to indicate the distance in graph $G$ between sets of vertices or inidivdual vertices, with respect to edge lengths $\ell'(\cdot)$. Recall that we are guaranteed that $\dist'_G(A',B')\geq \frac{\Lambda}{64}$. 


Recall that graph $H$ is identical to graph $\hat G$, except that the lengths of all edges are multiplied by factor $\Lambda$. Therefore, we get that:

\[\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta\cdot \Lambda}{2\eta\log^4n}+\Lambda\cdot \sum_{e\in E(G)}\ell(e).\]

Let $q$ be the total number of iterations in the algorithm, so $|\pset|=q$ holds. Recall that, at the beginning of the algorithm, $\sum_{e\in E(G)}\ell(e)\leq \frac{n}{\Lambda}=\frac{\Delta}{\eta\cdot \log^5n}$ held, since 
$\Lambda=\frac{n\eta \cdot \log^5n}{\Delta}$. 


In every iteration $i$, we double the lengths of all edges in set $\tilde E_i$. We also increase the lengths of the edges incident to $s$ and $t$, but, since these edges do not lie in the original graph $G$, we ignore them. Therefore, $\sum_{e\in E(G)}\ell(e)$ grows by (additive) $\frac{C_i}{\Lambda}$ in iteration $i$. From Property \ref{oracle-prop: small length growth} of the oracle, we are then guaranteed that, at the end of the algorithm: 

\[\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta\cdot \Lambda}{2\eta\log^4n}+ \frac{\Delta\cdot \Lambda}{\eta\log^5n}+ \sum_{i=1}^qC_i
\leq \frac{\Delta\cdot \Lambda}{\eta\cdot \log^4n}+\frac{q\cdot \Lambda\cdot (\log n)^{\hat c}}{\eta}\leq \Lambda\cdot\left(\frac{\Delta}{\eta\cdot \log^4n}+\frac{|\qset|\cdot (\log n)^{\hat c}}{\eta}\right ).\] 


Consider a thought experiment, where we select a threshold $\rho\in(0,\Lambda)$ uniformly at random, and then let $X$ be the set of all vertices $v\in V(G)$, such that the distance from $A'$ to $v$, with respect to the length $\ell'(\cdot)$ of edges is at most $\rho$. Let $Y=V(G)\setminus X$. It is easy to verify that, since the distance from $A'$ to $B'$ in $G$ with respect to edge lengths $\ell'(\cdot)$ is at least $\Lambda$, $A'\subseteq X$ and $B'\subseteq Y$ must hold. Moreover, the probability that an edge $e\in E(G)$ lies in $E_G(X,Y)$ is bounded by $\ell'(e)/\Lambda$. Therefore, the expectation of $|E(X,Y)|$ is bounded by $\frac{\sum_{e\in E(G)}\ell'(e)}{\Lambda}\leq \frac{\Delta}{\eta\cdot \eta\log^4n}+\frac{|\qset|\cdot (\log n)^{\hat c}}{\eta}$. By performing a standard ball-growing procedure from the set $A'$ of vertices we can compute, in time $O(m)$, a cut $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{\Delta}{\eta\cdot \eta\log^4n}+\frac{|\qset|\cdot (\log n)^{\hat c}}{\eta}$, such that $A'\subseteq X$ and $B'\subseteq Y$. From our discussion, the total running time of the algorithm is bounded by $T(n,\Delta,\eta)+O(m)$.





==> almost-DAG-previous.tex <==
\subsection{SSSP in DAG-like Graphs}
\label{sec: SSSP in almost DAGS}


In this subsection we define a problem that can be thought of as an abstraction for the types of \SSSP instances that we obtain via \ATO. We call this problem \DLSSSP, and we provide an algorithm for this problem, that is essentially identical to the algorithm of \cite{AlmostDAG2}, with very minor modifications.


\subsubsection{Problem Definition}

The input to the \DLSSSP problem consists of:

\begin{itemize}
	\item a directed graph $G=(V,E)$, that may have parallel edges but no self-loops, with two designated vertices $s$ and $t$;
	
	\item for every edge $e\in E(G)$, an integral \emph{length} $\ell(e)$, and an additional \emph{weight} $w(e)$. If $e$ is an edge that is incident to $s$, then $\ell(e)=1$ and $w(e)=0$ must hold, and otherwise $\ell(e)\geq 1$ must hold, and $w(e)$  must be an integral power of $2$ between $1$ and $2^{\ceil{\log n}}$;
		
	\item  a distance parameter $d>0$, and another parameter $\Gamma>0$, such that	$d\leq  \Gamma\cdot \log^5n$; and
	
	\item 
	a precision parameter $0<\eps\leq 1/8$, such that $1/\eps$ is an integer.
\end{itemize}
	

Graph $G$ undergoes the following three types of online updates:

\begin{itemize}
	\item {\bf Edge deletion:} given an edge $e\in E$, delete $e$ from $G$; and
	
	\item {\bf Vertex splitting:} in this operation, we are given as input a vertex $v\not\in\set{s,t}$ in the current graph, and new vertices $u_1,\ldots,u_k$ that need to be inserted into $G$; we may sometimes say that vertices $u_1,\ldots,u_k$ are \emph{split-off from $v$}. In addition to vertex $v$ and vertices $u_1,\ldots,u_k$, we are given a new collection $E'$ of edges that must be inserted into $G$, and for every edge $e\in E'$, we are given an integral length $\ell(e)>0$ and a weight $w(e)$ that must be an integral power of $2$ between $1$ and $2^{\ceil{\log n}}$. For each such edge $e\in E'$, either both endpoints of $e$ lie in $\set{u_1,\ldots,u_k, v}$; or one endpoint lies in $\set{u_1,\ldots,u_k}$, and the other in $V(G)\setminus\set{v,u_1,\ldots,u_k}$. In the latter case, if $e=(u_i,x)$, then edge $e'=(v,x)$ must currently lie in $G$, and both $w(e')=w(e)$ and $\ell(e')=\ell(e)$ must hold. Similarly, if $e=(x,u_i)$, then edge $e'=(x,v)$ must currently lie in $G$, and both $w(e')=w(e)$ and $\ell(e')=\ell(e)$ must hold. Notice that, at the end of the vertex splitting operation, $v$ must remain an iteresting vertex, and all newly inserted vertices are interesting as well.
\end{itemize}


We let $\tset$ be the \emph{time horizon} of the algorithm -- that is, the time interval during which the graph $G$ undergoes all updates. 
We denote by $n$ and by $m$ the total number of vertices and edges, respectively, that were ever present in $G$ during $\tset$, and we denote by $n_I$ the total number of interesting vertices at the end of the time interval $\tset$. We assume w.l.o.g. that for every vertex $v$ that was ever present in $G$, some edge was incident to $v$ at some time during the update sequence, so $n\leq O(m)$.

For every vertex $v\in V(G)$ and integer $0\leq i\leq \ceil{\log n}$, we define a vertex set:
 $$U_i(v)=\set{u\in V(G)\mid \exists e=(v,u)\in E(G)\mbox{ with } w(e)=2^i}.$$ 
 Note that, over the course of time interval $\tset$, each such set $U_i(v)$ may change, with vertices both leaving and joining the set. We require that
the following property holds at all times $\tau\in \tset$:

\begin{properties}{P}
	\item For every vertex $v\in V(G)\setminus\set{s}$, for every integer $0\leq i\leq \ceil{\log n}$, $|U_i(v)|\leq 2^{i+2}$.  \label{prop: few close neighbors}	
\end{properties}

As graph $G$ undergoes edge-deletion, edge-insertion, and vertex-splitting updates, at any time the algorithm may be asked a query $\pquery$. It is then required to return a {\bf simple} path $P$ connecting $s$ to $t$, whose length $\sum_{e\in E(P)}\ell(e)$ is bounded by $(1+6\eps)d$, in time $O(|E(P)|)$. 


Lastly, the algorithm may return FAIL at any time and halt. However, it may only do so if the current graph $G$ does not contain any $s$-$t$ path $P$  with $\sum_{e\in E(P)}\ell(e)\leq d$, and $\sum_{e\in E(P)}w(e)\leq \Gamma$. This completes the definition of the \DLSSSP problem.


\subsubsection{An Algorithm for \DLSSSP}

The following theorem provides an algorithm for the \DLSSSP problem; it follows almost immediately from the results of \cite{AlmostDAG2}. Specifically, Theorem 5.1 of \cite{AlmostDAG2} provides a similar result with a slightly different setting of parameters, though it does not support edge insertions. However, their arguments can be easily extended to prove the theorem below. We provide the proof for completeness in Section \ref{subsec: proof of DAG-like SSSP} of Appendix. Recall that $n_I$ denotes the number of interesting vertices in the  graph $G$ at the end of the algorithm.
 
\begin{theorem}\label{thm: almost DAG routing}
	There is a deterministic algorithm for the \DLSSSP problem with total update time $\tilde O\left(m+\frac{\Gamma\cdot n_I}{\eps^2}\right)$.
\end{theorem}





==> appx-ball-growing.tex <==

\section{Proof of \Cref{obs: ball growing}}
\label{sec: appx ball growing}
%\begin{proof}
	For all integers $i\geq 0$, let $S_i=B_G(x,i)$ be the set of all vertices $u\in V(G)$ with $\dist_G(x,u)\leq i$.
	
	Let $L=d/4$. We claim that, if $|S_L|< n/2$, then there is some index $1\leq i<L$ for which $|E_G(S_i,V\setminus S_i)|\leq  \phi\cdot |S_i|$ holds.
	
	Indeed, assume otherwise. Then for all $1\leq i<L$, $|E_G(S_i,V\setminus S_i)|\geq \phi\cdot |S_i|$. Denote $R_i=S_{i+1}\setminus S_i$. Since every edge in $E_G(S_i,V\setminus S_i)$ must enter a vertex of $R_i$, and the degree of every vertex in $G$ is at most $\dmax$, we get that $|R_i|\geq \frac{|E_G(S_i,V\setminus S_i)|}{\dmax}\geq \frac{\phi\cdot |S_i|}{\dmax}$ must hold.
	
	Therefore, for all $1\leq i<L$, $|S_{i+1}|\geq \left(1+\frac{\phi}{\dmax}\right )|S_i|$, and $|S_L|\geq \left(1+\frac{\phi}{\dmax}\right )^L\geq \left(1+\frac{\phi}{\dmax}\right )^{d/4}$.
	

Since $d=\frac{32\dmax\log n}{\phi}$, we get that $|S_L|>n$, a contradiction.

	For all integers $i\geq 0$, we also let $S'_i=\set{u\in V(G) \mid \dist(u,y)\leq i}$. Using the same reasoning, if $|S'_L|\leq n/2$, then there is some index $1\leq i<L$ for which $|E_G(V\setminus S'_i,S'_i)|\leq  \phi\cdot |S'_i|$.	
	

We are now ready to describe our algorithm. We run in parallel two processes. The first process simply performs a BFS from vertex $x$, while the second process performs a reversed BFS from vertex $y$. The first process, whenever it computes a set $S_i$, checks whether $|E_G(S_i,V\setminus S_i)|\leq \phi\cdot |S_i|$. If so, we terminate both processes and return the cut $(A,B)=(S_i,V\setminus S_i)$. Similarly, the second process, whenever it computes a set $S'_j$, checks whether $|E_G(V\setminus S'_j,S'_j)|\leq  \phi\cdot |S'_j|$ holds. If so, we terminate both processes and return the cut $(A,B)=	(V\setminus S'_j,S'_j)$. Since we set $L=d/4$, it must be the case that either $|S_L|\leq n/2$ or $|S'_L|\leq n/2$, so one of the two processes must terminate with a sparse cut. Since we run the two processes in parallel, it is easy to verify that the running time is bounded by the number of edges that the process that successfully terminated explored. Therefore, the running time of the algorithm is at most $O(\dmax\cdot \min\set{|A|,|B|})$.
%	\end{proof}



==> appx-ball-growing2.tex <==

\section{Proof of \Cref{obs: ball growing2}}
\label{sec: appx: ball growing 2}
%\begin{proof}
Let $\phi'=\frac{64\log n}{d}$.
	For all $i\geq 1$, let $S_i=B_H(v,i)=\set{u\in V(H)\mid \dist_H(v,u)\leq i}$ -- the ball of radius $i$ around $v$. Assume first that $v\in R$. Then for all odd indices $i>1$, $S_i\setminus S_{i-1}$ only contains vertices of $L$, while for all even indices $i>1$, $S_i\setminus S_{i-1}$ only contains vertices of $R$. Therefore, for every even index $i>1$, all edges in $E_H(S_i,V(H)\setminus S_i)$ are special edges. We say that an even index $i>1$ is \emph{acceptable} if $|E_H(S_i,V(H)\setminus S_i)|\leq \phi'\cdot |S_i|$. We now claim that some even index $1<i\leq d-1$ must be acceptable. Indeed, assume for contradiction that each such even index $i$ is unacceptable. Consider any such even index $i$. 
	Then $|E_H(S_i,V(H)\setminus S_i)|>\phi'\cdot |S_i|$. Since all edges in $E_H(S_i,V(H)\setminus S_i)$ are special, every vertex in $S_{i+1}\setminus S_i$ is incident to exactly one such edge, and so $|S_{i+1}\setminus S_i|\geq |E_H(S_i,V(H)\setminus S_i)|>\phi'\cdot |S_i|$. In particular, $|S_{i+2}|\geq |S_{i+1}|\geq (1+\phi')\cdot |S_i|$. Let $r$ be the largest even integer that is at most $d-1$, so $r\geq d-2\geq d/2$. Then, since 	$\phi'=\frac{64\log n}{d}$:
	
	\[|S_r|\geq (1+\phi')^{r/2}\geq (1+\phi')^{d/4}=\left(1+\frac{64\log n}{d}\right )^{d/4}>n,\]
	
	a contradiction. 
	
	Our algorithm performs a BFS starting from $v$, until it reaches the first even index $i$ for which set $S_i$ is acceptable. It then returns a cut $(A,B)$ with $S_i=A$ and $B=V(H)\setminus A$. Clearly, $|E_H(A,B)|\leq \phi'\cdot |A|\leq \phi\cdot |A|$ holds from the definition of acceptable index. Moreover, since $|E_H(A,B)|\leq \phi'\cdot n= \frac{64\log n}{d}\cdot n$, while $|B|\geq |X|\geq \frac{n}{32}$, we get that $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}|B|=\phi\cdot |B|$. Therefore, the sparsity of cut $(A,B)$ is at most $\phi$. It is immediate to verify that this cut has all other required properties. It is also immediate to verify that the running time of the algorithm is $O(\vol_H(A))$.
	
	If $v\in L$, then for all odd indices $i>1$, $S_i\setminus S_{i-1}$ only contains vertices of $R$, while for all even indices $i>1$, $S_i\setminus S_{i-1}$ only contains vertices of $L$. Therefore, for every odd index $i>1$, all edges in $E_H(S_i,V(H)\setminus S_i)$ are special edges.
	The algorithm is the same as before, except that we use odd indices $i$ instead of even indices.
%\end{proof}

%===========================
%===========================
%===========================
%===========================
%===========================
%===========================
%===========================

==> cut-player-alg.tex <==
\section{Algorithm for the Cut Player -- Proof of \Cref{thm: cut player outer}}
\label{subsec: algorithm for the cut player}


For simplicity of notation, in this proof we will denote $\hat n$ by $n$.
The proof of \Cref{thm: cut player outer} easily follows from the following slightly weaker theorem.



\begin{theorem}\label{thm: cut player inner}
	There is a deterministic algorithm, that, given an $n$-vertex directed graph $X$ with maximum vertex degree at most $O(\log n)$, returns one of the following:
	
	\begin{itemize}
		\item either a cut $(A,B)$ in $X$ with $|E_X(A,B)|\leq  \frac{\min\set{|A|,|B|}}{128}$ and $|A|,|B|\geq \frac{\alpha_0}{2^{14}}\cdot n$; or
		
		\item another directed $n$-vertex graph $X'$ with maximum vertex degree at most $18$, such that $X'$ is an $\alpha_0$-expander, together with a subset $F\subseteq E(X')$ of at most $k=\frac{\alpha_0\cdot n}{1000}$ edges of $X'$, and an embedding $\pset$ of $X'\setminus F$ into $X$ via paths of length at most $d=O(\log n)$, that cause congestion at most $\eta=O(\log n)$.
	\end{itemize}
	
	The running time of the algorithm is $\otilde(n^2)$.
\end{theorem}


We prove \Cref{thm: cut player inner} below, after we complete the proof of \Cref{thm: cut player outer} using it. We start with the graph $\hat X=G$, and then perform iterations, as long as $|V(\hat X)|\geq n/4$. We will also construct a collection $\xset$ of subsets of vertices of $\hat X$, that is initialized to $\emptyset$. In every iteration, we may add a single set $X$ to $\xset$ (that defines a sparse cut in the current graph $\hat X$), and then delete the vertices of $X$ from $\hat X$.

In order to execute a single iteration, we apply the algorithm from \Cref{thm: cut player inner} to the current graph $\hat X$. Let $n'\geq n/4$ denote the number of vertices that currently belong to $\hat X$. If the algorithm returned a directed $n'$-vertex  $\alpha_0$-expander graph $X'$ with maximum vertex degree at most $18$, together with a subset $F\subseteq E(X')$ of at most $k=\frac{\alpha_0\cdot n'}{1000}\leq \frac{\alpha_0 n}{1000}$ edges of $X'$, and an embedding $\pset$ of $X'\setminus F$ into $\hat X$ via paths of length at most $d$, that cause congestion at most $\eta$, then we terminate the algorithm and return $X'$, $F$ and $\pset$. 

Assume now that the algorithm from \Cref{thm: cut player inner}  returned a cut $(A',B')$ in $\hat X$ with $|E_{\hat X}(A',B')|\leq  \frac{\min\set{|A'|,|B'|}}{128}$ and $|A'|,|B'|\geq \frac{\alpha_0}{2^{14}}\cdot n'\geq \frac{\alpha_0}{2^{16}}n$.
Denote the sets $A',B'$ by $X$ and $Y$ respectively, where $X$ is the set of $\set{A',B'}$ of smaller cardinality, and $Y$ is the other set (if the cardinalities of the two sets are equal, break the tie arbitrarily). We then add $X$ to $\xset$, delete the vertices of $X$ from $\hat X$, and continue to the next iteration. 

If the above algorithm does not terminate with an expander $X'$ that is embedded into $G$, then it must terminate once $|V(\hat X)|\leq n/4$ holds. Let $\xset=\set{X_1,X_2,\ldots,X_r}$ be the final collection of vertex subsets, where the sets are indexed in the order in which they were added to $\xset$. We also denote by $X_{r+1}$ the set $V(\hat X)$ obtained at the end of the algorithm, and we add $X_{r+1}$ to $\xset$ as well. For all $1\leq j\leq r$, denote $X'_j=X_{j+1}\cup \cdots\cup X_{r+1}$. From our algorithm, for each such index $j$, either $|E_G(X_j,X'_j)|\leq  |X_j|/128$, or $|E_G(X'_j,X_j)|\leq |X_j|/128$. Moreover, for all $1\leq j\leq r+1$, $|X_j|\leq n/2$, while $|X_{r+1}|\geq \frac{n}{8}$. Therefore, if we let $\alpha$ be such that $\max_{X_j\in \xset}\set{|X_j|}=\alpha\cdot n$, then $\frac 1 8\leq \alpha\leq \frac 1 2$.
 

We can now use the algorithm from \Cref{obs: from many sparse to one balanced} to compute, in time $O(|E( G)|)\leq \otilde(n)$, a cut $(A,B)$ in $G$, with   $|E_{G}(A,B)|\leq n/128$, and  $|A|,|B|\geq \min \set{\frac{1-\alpha}{2}\cdot n, \frac n 4}\geq \frac{n}{10}$.

The running time of every iteration of our algorithm is $\otilde(n^2)$, and the number of iterations is bounded by a constant. The running time of the algorithm from \Cref{obs: from many sparse to one balanced}  is bounded by $\otilde(n)$, and so the total running time of our algorithm is $\otilde(n^2)$.

In order to complete the proof of \cref{thm: cut player outer}, it is now enough to prove \Cref{thm: cut player inner}.

\begin{proofof}{\Cref{thm: cut player inner}}
	Since we can afford in the proof of the theorem a running time that is as high as $\otilde(n^2)$, we can use a straightforward algorithm, that is significantly simpler than other current deterministic algorithms for the cut player (see e.g. Theorem 7.3 in \cite{SCC}, that generalizes the results of \cite{detbalanced} to directed graphs). 
	
	
We set the parameters
$d=\frac{2^{32}\log n}{\alpha_0}$ and $\eta=\frac{2^{58}\log n}{\alpha_0^2}$.
	
	

We start by using the algorithm from \Cref{thm:explicit expander} to construct, in time $O(n)$, a directed  $n$-vertex graph $X'$ that is an $\alpha_0$-expander, with maximum vertex degree at most $18$.

Next, we start with a graph $\hat X=X$, and then perform $|E(X')|$ iterations. In every iteration we will attempt to embed some edge $e\in E(X')$ into $\hat X$, and we will delete from $\hat X$ edges that participate in too many of the embedding paths. We will maintain a partition $(E',E'',F)$ of the edges of $E(X')$, where set $E'$ contains all edges $e\in E'$ for which an embedding path $P(e)$ was already computed by the algorithm; set $F$ contains all edges $e\in E'$ for which the algorithm failed to compute an embedding path; and $E''$ contains all edges of $X'$ that were not considered by the algorithm yet. We also maintain a set $\pset=\set{P(e)\mid e\in E'}$ of all embedding paths that the algorithm computed so far. For every edge $e\in E(X)$ we will maintain a counter $\mu(e)$ that counts the number of paths in $\pset$ containing $e$.

Initially, we set $E'=F=\emptyset$, $E''=E(X')$, and $\pset=\emptyset$.  We also set $\hat X=X$, and perform iterations as long as $E''\neq \emptyset$.

In order to perform an iteration, we consider any edge $e=(u,v)\in E''$. We compute the shortest path $P$ in the current graph $\hat X$ connecting $u$ to $v$, by peforming a BFS from vertex $u$, in time $O(|E(\hat X)|)\leq \otilde(n)$. If the length of $P$ is greater than $d$, then we move edge $e$ from $E''$ to $F$. Otherwise, we set $P(e)=P$, move $e$ from $E''$ to $E'$, and add path $P(e)$ to set $\pset$. Additionally, for every edge $e'\in E(P)$ we increase the counter $\mu(e')$ by $1$, and if the counter reaches $\eta$, we delete $e'$ from $\hat X$.

Once $E''=\emptyset$ holds, the algorithm terminates. 
Notice that, since the algorithm spends at most $\otilde(n)$ time on processing every edge of $X'$, its running time so far is $\otilde(n^2)$.

We now consider two cases. Assume first that, at the end of the above procedure, $|F|\leq k$ holds. In this case, we terminate the algorithm, and return the $\alpha_0$-expander $X'$, the set $F$ of its edges, and the embedding $\pset$ of $X'\setminus F$ into $X$ that our algorithm has computed. It is easy to verify that every path in $\pset$ has length at most $d$ and causes congestion at most $\eta$.



From now on we assume that $|F|>k$. We now show an algorithm to compute a cut $(A,B)$ in $X$ of sparsity at most $\frac 1 {128}$, such that $|A|,|B|\geq \frac{\alpha_0}{2^{14}}\cdot n$.




Let $E^*=E(X)\setminus E(\hat X)$. Equivalently, set $E^*$ contains all edges that participate in $\eta$ paths in $\pset$. Recall that $|\pset|\leq |E(X')|\leq 9n$, and the length of every path in $\pset$ is at most $d$. Therefore, $\sum_{P\in \pset}|E(P)|\leq 9dn$, and $|E^*|\leq\frac{\sum_{P\in \pset}|E(P)|}{\eta}\leq \frac{9dn}{\eta}$.




In the remainder of the algorithm, we will iteratively cut off sparse cuts (that may be quite small) from graph $\hat X$. We maintain a set $\xset$ of subsets of vertices of $\hat X$, that is initially empty. The algorithm is iterative, and in every iteration a single set $Z$ is added to $\xset$, with the vertices of $Z$ deleted from $\hat X$. The algorithm continues as long as $|V(\hat X)|\geq n-k/2$ holds.
We now describe the execution of a single iteration.

Since $|V(\hat X)|\geq n-k/2$, there exists an edge $e=(x,y)\in F$ with $x,y\in \hat X$. Moreover, since we were unable to embed $e$ into $\hat X$ when it was considered, and since we only deleted edges and vertices from $\hat X$ since then, it must be the case that $\dist_{\hat X}(x,y)>d$ holds right now. Let $\Delta=18$ denote the maximum vertex degree in $\hat X$. Since $d=\frac{2^{32}\log n}{\alpha_0}$, it is immediate that $d\geq 64\Delta\log n$. We now use the algorithm from \Cref{obs: ball growing} to compute a cut $(Z,Z')$ in the current graph $\hat X$, whose sparsity is at most $\phi'=\frac{32\Delta\log n}{d}\leq \frac{32\cdot 18\cdot\alpha_0\log n}{2^{32}\log n}\leq \frac{\alpha_0}{2^{22}}$. Denote the sets $Z,Z'$ by $X$ and $Y$, such that $X$ is the set of smaller cardinality, and $Y$ is the other set (if the cardinalities of the two sets are equal, break the tie arbitrarily). We then add $X$ to $\xset$, delete the vertices of $X$ from $\hat X$, and continue to the next iteration. Note that, if $X$ is the set of vertices that was added to $\xset$ during the current iteration, then from \Cref{obs: ball growing}, the running time of the iteration is bounded by $O(|X|)$.









When the above algorithm terminates, we let $\xset=\set{X_1,X_2,\ldots,X_r}$ be the final collection of vertex subsets, where the sets are indexed in the order in which they were added to $\xset$. We also denote by $X_{r+1}$ the set $V(\hat X)$ obtained at the end of the algorithm, and we add $X_{r+1}$ to $\xset$ as well. For all $1\leq j\leq r$, denote $X'_j=X_{j+1}\cup \cdots\cup X_{r+1}$. From our algorithm, for each such index $j$, either $|E_{\hat X}(X_j,X'_j)|\leq \phi'\cdot |X_j|$, or $|E_{\hat X}(X'_j,X_j)|\leq \phi'\cdot |X_j|$. 
From our discussion, the total time that the algorithm spent on constructing the sets of vertices in $\xset$ is bounded by $\sum_{j=1}^rO(|X_j|)\leq O(n)$.
Let $\alpha$ be chosen such that the cardinality of largest set of vertices in $\xset$ is $\alpha\cdot n$. From our algorithm, $\alpha\leq 1-\frac{k}{2n}\leq 1-\frac{\alpha_0}{2000}$, since $k=\frac{\alpha_0\cdot n}{1000}$. 






We can now use the algorithm from \Cref{obs: from many sparse to one balanced} to compute, in time $O(|E(\hat X)|)\leq \otilde(n)$, a cut $(A,B)$ in $\hat X$, with   $|E_{\hat X}(A,B)|\leq \phi'\cdot \sum_{i=1}^{r}|X_i|$, and  $|A|,|B|\geq \min \set{\frac{1-\alpha}{2}\cdot n, \frac n 4}\geq \frac{\alpha_0n}{4000}$.

Recall that graph $\hat X$ was obtained from $X$ by deleting the edges of $E^*$ from it, and that $|E^*|\leq \frac{9dn}{\eta}$. Subtituting $d=\frac{2^{32}\log n}{\alpha_0}$,  $\eta=\frac{2^{58}\log n}{\alpha_0^2}$, we get that:
$|E^*|\leq \frac{\alpha_0 n}{2^{22}}$.


Overall:

\[|E_X(A,B)|\leq |E_{\hat X}(A,B)|+|E^*|\leq \phi' n+\frac{\alpha_0 n}{2^{22}}\leq \frac{\alpha_0 n}{2^{21}}.\]


(we have used the fact that $\phi'\leq \frac{\alpha_0}{2^{22}}$). Lastly, since $|A|,|B|\geq \frac{\alpha_0n}{4000}\geq \frac{\alpha_0n}{2^{14}}$, we get that $ |E_X(A,B)|\leq \frac{\min\set{|A|,|B|}}{128}$, as required.


From our discussion, the running time of the entire algorithm is bounded by $\otilde(n^2)$.
\end{proofof}

==> document.tex <==
We also use a parameter $\hat d=\frac{2^{30}\log n}{\alpha_0}$, and we will ensure that at all times, for every pair $x,y$ of vertices of $W^*$, $\dist_{W^*}(x,y),\dist_{W^*}(y,x)\leq \hat d$.
 Let $D=18$, and observe that $\hat d\geq 64D\log n$. 
 From \Cref{obs: ball growing}, since graph $W^*$ is initially an $\alpha_0$-expander with maximum vertex degree at most $D$, at the beginning of Step 2, for every pair $x,y$ of vertices of $W^*$, $\dist_{W^*}(x,y),\dist_{W^*}(y,x)\leq \hat d$ holds.


We maintain two additional graphs: graph $H'$ that is obtained from $H$ by adding a source vertex $s$, and connecting it to every vertex in $V(W^*)$ with an edge of length $1$, and graph $H''$ that is obtained from $H$ by adding a vertex $s'$, connecting every vertex in $V(W^*)$ to it with an edge of length $1$, and then reversing the directions of all edges. Whenever a vertex $v$ leaves the set $V(W^*)$ of vertices, we delete the edge $(s,v)$ from $H'$, and we also delete the edge $(s',v)$ from $H''$. Additionally, whenever an edge is deleted from graph $H$ due to an update operation, we delete the corresponding edge from both $H'$ and $H''$.

We initialize the \EST data structure from \Cref{thm: directed weighted ESTree} for graph $H'$, with distance parameter $d+1$, and we similarly initialize \EST data structure for $H''$ with distance parameter $d+1$. We denote the corresponding trees by $\tau'$ and $\tau''$, respectively.

We will ensure that, throughout the algorithm, every vertex $v$ of $H$ lies in both $\tau'$ and $\tau''$, so that $\dist_H(V(W^*),v),\dist_H(v,V(W^*))\leq d$ always holds. In order to ensure this, we use the \EST data structures to identify vertices $v$ for which this no longer holds. Whenever we identify a vertex $v$ with $\dist_H(v,V(W^*))>d$, we  use the algorithm from \Cref{obs: ball growing} in order to compute a well-structured cut $(A,B)$ in $H$ with $v\in A$, $V(W^*)\subseteq B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. If $|A|\leq |B|$, then we delete the vertices of $A$ from $H$, (which includes deleting their incident edges from graphs $H,H'$, and $H''$, and both \EST data structures $\tau'$ and $\tau''$), and then continue the algorithm. If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated. Alternatively, if $|A|>|B|$, then we delete the vertices of $B$ from $H$, and terminate the current phase. Notice that in this case, at least $|V(W^*)|\geq n''/4\geq n/64$  vertices have been deleted from $H$ in the current phase.

Similarly, whenever we identify a vertex $v$ with $\dist_H(V(W^*),v)>d$, we  use the algorithm from \Cref{obs: ball growing} (but with reversed directions of edges) in order to compute a well-structured cut $(A,B)$ in $H$ with $V(W^*)\subseteq  A$, $v\in B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. As before, if $|B|\leq |A|$, then we delete the vertices of $B$ from $H$, and from both \EST data structures. If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated, and otherwise we continue the algorithm as before. Alternatively, if $|B|>|A|$, then we delete the vertices of $A$ from $H$, and terminate the current phase. In the latter case, at least $n/64$ vertices have been deleted from $H$ in the current phase.

==> expander-algs.tex <==

\section{Algorithm for the \maintaincluster Problem -- Proof of \Cref{thm: main for expander tools}}
\label{sec: expander algs}


We will use the following theorem as a subroutine. The theorem provides an efficient algorithm that either embeds a large expander into the input graph $H$, or to computes a sparse cut in $H$, with both sides of the cut being sufficiently large. The proof of the theorem uses standard techniques (namely the Cut-Matching Game), though we provide a simpler algorithm for one of the ingredients (algorithm for the Cut Player), and an algorithm achieving slightly better parameters for another ingredient (algorithm for the Matching Player). The theorem uses parameter $\alpha_0$ from \Cref{thm:explicit expander}; its proof is deferred to Section \ref{sec: embed or cut}.


\begin{theorem}\label{thm: embed expander or cut}	
	There is a deterministic algorithm, whose input consists of a directed $n$-vertex bipartite graph $G=(L,R,E)$, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$, and a parameter $d\geq 4$.
	
	The algorithm returns one of the following:
	\begin{itemize}
		\item Either a cut $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{2n}{d}+1$ and $|X|,|Y|\geq \Omega\left ( \frac{n}{\log^2 n}\right )$; or
		
		\item A directed graph $W^*$ with $|V(W^*)|\geq n/8$ and maximum vertex degree at most $18$, such that $W^*$ is an $\alpha_0$-expander, together with a subset $F\subseteq E(W^*)$ of at most $\frac{\alpha_0\cdot n}{500}$ edges of $W^*$, and an embedding $\pset^*$ of $W^*\setminus F$ into $G$ via paths of length at most $O(d\log n)$, that cause congestion at most $O(d\log^3n)$, such that every path in $\pset^*$ is simple.
	\end{itemize}
	The running time of the algorithm is $\otilde(md+n^2)$.
\end{theorem}

Note that in the above theorem we assume that all edge lengths in the input graph $G$ are unit.


We will also use the following simple observation that uses the standard ball-growing technique. The proof is deferred to Section \ref{sec: appx: ball growing 2} of Appendix.

\begin{observation}\label{obs: ball growing2}
	There is a deterministic algorithm, that receives as input a directed bipartite $n$-vertex graph $H=(L,R,E)$, where the edges in $E_H(L,R)$ are called regular and the edges in $E_H(R,L)$ are called special. Every vertex of $H$ may be incident to at most one special edge. Additionally, the algorithm is given a set $X\subseteq V(H)$ of at least $\frac{n}{32}$ vertices, and a vertex $v$, such that $\dist_H(v,X)\geq d$, for some given parameter ${d\geq 2^{11}\log n}$. The algorithm computes a  well-structured cut $(A,B)$ in $H$, with $v\in A$, $X\subseteq B$, and $|E_H(A,B)|\leq \phi\cdot\min\set{|A|,|B|}$, for 	${\phi=\frac{2^{11}\log n}{d}}$. The running time of the algorithm is $O(\vol_H(A))$.
\end{observation}





We are now ready to complete the proof of \Cref{thm: main for expander tools}. Recall that we are given as input a 
simple  bipartite $n$-vertex graph $H=(L,R,E)$, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$, together with integral parameters $c^*\log^4n\leq d^*\leq n$, where $c^*$ is a large enough constant and $1\leq \Delta\leq n$.
Recall that we refer to the edges of $E_H(R,L)$ as \emph{special}, and the edges of $E_H(L,R)$ as \emph{regular}. Recall also that a cut $(X,Y)$ in $H$ is \emph{well-structured} iff all edges in $E_H(X,Y)$ are special.

The algorithm is required to respond to at most $\Delta$ \shortpath queries: given a pair $x,y\in V(H)$ of vertices, it must return a simple path $P$ connecting $x$ to $y$ in $H$, whose length is at most $d^*$. Once the algorithm responds to a query, it receives a set of edges that need to be deleted from $H$, with all the deleted edges lying on path $P$.  At any time, the algorithm may provide a well-structured cut $(X,Y)$ of $H$, whose sparsity is at most $O\left(\frac{\log^4 n}{d^*}\right )$. 
If $|X|\leq |Y|$, then the cut must be provided by listing the vertices of $X$, and otherwise it must be provided by listing the vertices of $Y$. After that the vertices of the smaller side of the cut are deleted from $H$. 

Note that, over the course of the algorithm, vertices may be deleted from $H$. We denote by $n$ the initial number of vertices in $H$. Once $|V(H)|$ falls below $n/2$, the algorithm terminates, even if fewer than $\Delta$ queries were asked.

Throughout, we use a parameter ${d=\frac{d^*}{c'\log^2 n}}$, where $c'$ is some large enough constant, whose value we will set later. Since $d^*\geq c^*\cdot \log^4 n$ for a large enough constant $c^*$, we can ensure that $d\geq 2^{11}\log n$.

Our algorithm consists of a number of phases. 
Let $N=\frac{\alpha_0 n}{2^{20} (d^*)^2\log n}$, and let $\hat c$ be a large enough contant whose value we choose later. A phase terminates whenever one of the following two conditions are met: either (i) the number of vertices in $H$ decreased by the factor of at least ${\left( 1-\frac{1}{\hat c\log^4n}\right )}$ over the course of the current phase (in which case we say that the phase is of \emph{type 1}); or (ii) at least $N$ \shortpath queries were responded to during the current phase (in which case the phase is of \emph{type 2}). Clearly, at most $O(\log^4n)$ phases may be of type 1, and the number of type-2 phases is bounded by $\max\set{1,\frac{\Delta}{N}}\leq \max\set{1,O\left ( \frac{\Delta\cdot (d^*)^2\log n}{n}\right )}$. Overall, the number of phases in the algorithm is bounded by $O\left (\max\set{\log^4n,\frac{\Delta\cdot (d^*)^2\cdot \log^5n}{n}}\right )$.
At a high level, we follow a scheme that is by now quite standard: we embed a large $\Omega(1)$-expander $W^*$ into graph $H$, and then maintain two \EST data structures in  $H$, both of which are rooted at the vertices of $W^*$; in the first tree all edges are directed away from the root, while in the second tree the edges are directed towards the root. Given a query $(x,y)$, we then use the \EST data structures in order to connect $x$ to some vertex $x'\in V(W^*)$, and to connect some vertex $y'\in V(W^*)$ to $y$, via short paths. Lastly, we compute a short path connecting $x'$ to $y'$ in $W^*$ by performing a BFS, which is then transformed into an $x'$-$y'$ path in $H$ by exploiting the embedding of $W^*$ into $H$. At a high level, we can view each phase as consisting of two steps. In the first step, we embed an expander $W^*$ into $H$, and the second step contains the remainder of the algorithm that allows us to support \shortpath queries. We now describe each of the two steps in turn.


\subsection*{Step 1: Embedding an Expander}
During the first step of the phase,  we will attempt to embed a large expander into the current graph $H$ via \Cref{thm: embed expander or cut}. Specifically, we perform a number of iterations. In every iteration, we apply the algorithm from \Cref{thm: embed expander or cut} to the current graph $H$. 

Assume first that the algorithm returned a cut $(X,Y)$ in $H$ with $|E_H(X,Y)|\leq \frac{2n}{d}+1$ and $|X|,|Y|\geq \Omega\left ( \frac{n}{\log^2 n}\right )$. In this case, we say that the current iteration is a \emph{bad} iteration.
Clearly, $|E_H(X,Y)|\leq \frac{2n}{d}+1\leq \frac{4n}{d}\leq O\left(\frac{\log^2n}{d} \right )\cdot \min\set{|X|,|Y|}$. In other words, the sparsity of the cut $(X,Y)$ is at most $O\left(\frac{\log^2n}{d} \right )=O\left(\frac{\log^4n}{d^*} \right )$. 
Since $d^*\geq c^*\log^4n$, where $c^*$ is a large enough constant, we can ensure that the sparsity of the cut, that we denote by $\phi$, is bounded by $1/4$.
Using the algorithm from \Cref{obs: sparse cut to structured}, we compute, in time $O(|E(H)|)$, a well-structured cut $(X',Y')$ in $H$, whose sparsity remains at most $O\left(\frac{\log^2n}{d} \right )=O\left(\frac{\log^4n}{d^*} \right )$. 

Denote the sets $X',Y'$ by $Z$ and $Z'$, so that $Z$ is the smaller set of the two, breaking the tie arbitrarily. Notice that the algorithm from \Cref{obs: sparse cut to structured} ensures that $|Z|\geq (1-\phi)\cdot \min\set{|X|,|Y|}\geq \Omega\left ( \frac{n}{\log^2 n}\right )$. We then output the cut $(X,Y)$ and delete the vertices of $Z$ from graph $H$. If the number of vertices in $H$ falls below $n/2$, then we terminate the algorithm. Otherwise, we continue to the next iteration. 

Assume now that the algorithm from \Cref{thm: embed expander or cut}	 returned a directed graph $W^*$ with $|V(W^*)|\geq |V(H)|/8$ and maximum vertex degree at most $18$, such that $W^*$ is an $\alpha_0$-expander, together with a subset $F\subseteq E(W^*)$ of at most $\frac{\alpha_0\cdot |V(H)|}{500}$ edges of $W^*$, and an embedding $\pset^*$ of $W^*\setminus F$ into $G$ via paths of length at most $O(d\log n)$, that cause congestion at most $O(d\log^3n)$.
In this case, we say that the current iteration is  a \emph{good} iteration. We then terminate the first step of the current phase and continue to the second step.

Since in every bad iteration at least $\Omega\left ( \frac{n}{\log^2 n}\right )$ vertices are deleted from $H$, the total number of iterations in the first step is bounded by $O(\log^2n)$. In every iteration we apply the algorithm from \Cref{thm: embed expander or cut}, whose running time is $\otilde(|E(H)|d+n^2)$ to the current graph $H$, and then possibly use the algorithm from \Cref{obs: sparse cut to structured}, whose running time is at most $O(|E(H)|)$. Overall, the running time of Step 1 of a single phase is $\otilde(|E(H)|\cdot d+n^2)$. 





\subsection*{Step 2: Even-Shiloach Trees and Supporting Short-Path Queries}
We denote by $n'$ the number of vertices in $H$ at the beginning of Step 2. The purpose of Step 2 is to support \shortpath queries. 
Over the course of Step 2, the number of vertices in $H$ may decrease. Whenever this number falls below $n'\cdot \left(1-\frac{1}{\hat c\log^4n}\right )$, for a large enough constant $\hat c$ whose value we choose later, we terminate the algorithm for Step 2 and the current phase.

We start by defining additional data structures that we maintain.

Recall that, at the beginning of Step 2, we are given an $\alpha_0$-expander graph $W^*$ with  $|V(W^*)|\geq n'/8$ and maximum vertex degree at most $18$, together with a subset $F\subseteq E(W^*)$ of at most $\frac{\alpha_0\cdot n'}{500}$ edges of $W^*$, and an embedding $\pset^*$ of $W^*\setminus F$ into $H$ via paths of length at most $O(d\log n)$, that cause congestion at most $O(d\log^3n)$. 


We denote the number of vertices in $W^*$ at the beginning of the phase by $n''$, so $n''\geq n'/8\geq n/16$.
 Over the course of Step 2, some vertices may be deleted from $W^*$, but we will ensure that throughout the algorithm for Step 2, $|V(W^*)|\geq n''/4\geq |V(H)|/32$ holds.
 We also use a parameter $\hat d=\frac{2^{30}\log n}{\alpha_0}$, and we will ensure that at all times, for every pair $x,y$ of vertices of $W^*$, $\dist_{W^*}(x,y),\dist_{W^*}(y,x)\leq \hat d$.
 Let $D=18$, and observe that $\hat d\geq 64D\log n$. 
 From \Cref{obs: ball growing}, since graph $W^*$ is initially an $\alpha_0$-expander with maximum vertex degree at most $D$, at the beginning of Step 2, for every pair $x,y$ of vertices of $W^*$, $\dist_{W^*}(x,y),\dist_{W^*}(y,x)\leq \hat d$ holds.


We maintain two additional graphs: graph $H'$ that is obtained from $H$ by adding a source vertex $s'$, and connecting it to every vertex in $V(W^*)$ with an edge of length $1$, and graph $H''$ that is obtained from $H$ by adding a vertex $s''$, connecting every vertex in $V(W^*)$ to it with an edge of length $1$, and then reversing the directions of all edges. Whenever a vertex $v$ leaves the set $V(W^*)$ of vertices, we delete the edge $(s',v)$ from $H'$, and we also delete the edge $(s'',v)$ from $H''$. Additionally, whenever an edge is deleted from graph $H$ due to an update operation, we delete the corresponding edge from both $H'$ and $H''$. When vertices are deleted from graph $H$ (after sparse cuts are returned by the algorithm), we also update both $H'$ and $H''$ with the deletions of these vertices.

We initialize the \EST data structure from \Cref{thm: directed weighted ESTree} for graph $H'$, with source vertex $s'$ and distance parameter $d+1$, and we similarly initialize \EST data structure for $H''$ with source vertex $s''$ and distance parameter $d+1$. We denote the corresponding trees by $\tau'$ and $\tau''$, respectively.

We will ensure that, throughout the algorithm, every vertex $v$ of $H$ lies in both $\tau'$ and $\tau''$, so that $\dist_H(V(W^*),v),\dist_H(v,V(W^*))\leq d$ always holds. In order to ensure this, we use the \EST data structures to identify vertices $v$ for which this no longer holds. Whenever we identify a vertex $v$ with $\dist_H(v,V(W^*))>d$, we  use the algorithm from \Cref{obs: ball growing2} in order to compute a well-structured cut $(A,B)$ in $H$ with $v\in A$, $V(W^*)\subseteq B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. If $|A|\leq |B|$, then we delete the vertices of $A$ from $H$, (which includes deleting their incident edges from graphs $H,H'$, and $H''$, and both \EST data structures $\tau'$ and $\tau''$), and then continue the algorithm. If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated. Alternatively, if $|A|>|B|$, then we delete the vertices of $B$ from $H$, and terminate the current phase. Notice that in this case, at least $|V(W^*)|\geq n''/4\geq n/64$  vertices have been deleted from $H$ in the current phase.

Similarly, whenever we identify a vertex $v$ with $\dist_H(V(W^*),v)>d$, we  use the algorithm from \Cref{obs: ball growing2} (but with reversed directions of edges) in order to compute a well-structured cut $(A,B)$ in $H$ with $V(W^*)\subseteq  A$, $v\in B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. As before, if $|B|\leq |A|$, then we delete the vertices of $B$ from $H$, and from both \EST data structures. If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated, and otherwise we continue the algorithm as before. Alternatively, if $|B|>|A|$, then we delete the vertices of $A$ from $H$, and terminate the current phase. In the latter case, at least $n/64$ vertices have been deleted from $H$ in the current phase.


In either case, if the set of vertices that was deleted from $H$ is denoted by $Z$, then the running time of the algorithm from \Cref{obs: ball growing2}  is bounded by $O(\vol_H(Z))$. Therefore, the total time that the algorithm ever spends over the course of Step 2 to cut sparse cuts off from $H$ via \Cref{obs: ball growing2}  is bounded by $O(|E(H)|)$. Additionally, the algorithms for maintaining the two \EST data structures have total update time $O(|E(H)|\cdot d)$.
Therefore, the total update time of Step 2 of a single phase is so far bounded by $O(|E(H)|\cdot d)$.



\subsection*{Updates to the Expander $W^*$}
Recall that, at the beginning of Step 2, we are given an $\alpha_0$-expander $W^*$, with $|V(W^*)|=n''\geq n'/8$ and maximum vertex degree at most $18$, together with a subset $F\subseteq E(W^*)$ of at most $\frac{\alpha_0\cdot n'}{500}$ edges of $W^*$, and an embedding $\pset^*$ of $W^*\setminus F$ into $G$ via paths of length at most $O(d\log n)$, that cause congestion at most $O(d\log^3n)$. 

Over the course of the algorithm, we may delete some edges from $W^*$, and we may also compute sparse cuts in $W^*$ that decompose $W^*$ into smaller subgraphs. For convenience, we will maintain a collection $\xset$ of subsets of vertices of $W^*$ that partition the original set $V(W^*)$. At the beginning of the algorithm, $\xset$ contains a single set $V(W^*)$ of vertices. Over the course of the algorithm, if we identify a sparse cut $(X,Y)$ in the current graph $W^*$, we will replace $V(W^*)$ with $X$ and $Y$ in $\xset$, and we will delete the vertices of the smaller of the two sets from $W^*$. The key is to ensure that, since the cuts that we compute are sparse, and since the number of edges deleted from $W^*$ over the course of the second step is relatively small, $|V(W^*)|\geq n''/4$ continues to hold throughout the algorithm.
For every edge $e\in E(H)$, we maintain a set $S(e)$ of all edges $e'\in E(W^*)\setminus F$ whose embedding path $P(e')\in \pset^*$ contains $e$. We can initialize the sets $S(e)$ of edges for all $e\in E(H)$ by scanning every edge $e'\in E(W^*)\setminus F$ and considering all edges on path $P(e')$. Clearly, the total time required to initialize the sets $S(e)$ of edges for all $e\in E(H)$ is subsumed by the time spent on constructing the embedding $\pset^*$ of $W^*\setminus F$ into $H$ in Step 1.

There are three types of updates that expander $W^*$ may undergo over the course of the algorithm, that we describe next.


\paragraph{First Type of Updates.}
Suppose some edge $e$ was deleted from $H$, as part of the update sequence that  graph $H$ undergoes. In this case, we delete every edge $e'\in S(e)$ from $W^*$. For each such edge $e'$, we also delete $e'$ from the set $S(e'')$ of every edge $e''$ that lies on the embedding path $P(e')\in \pset^*$. Recall that, over the course of the current phase, our algorithm will need to respond to at most $N$ \shortpath queries. If $Q$ is a path that is returned in response to such a query, then $Q$ may contain at most $d^*$ edges, and the only edges that may be deleted from $H$ over the course of the current phase as part of the update sequence are edges that lie on such paths. Therefore, the total number of edges that may be deleted from $H$ as part of the update sequence during a single phase is at most $N\cdot d^*$. Since the embedding of $W^*\setminus F$ causes congestion at most $O(d\log^3n)$ in $H$, the number of corresponding edge deletions from $W^*$ is bounded by: 


\[O(N\cdot d^*\cdot d\log^3n)\leq N\cdot (d^*)^2\cdot \log n\leq \frac{\alpha_0 n}{2^{20}} \]

since $d=\frac{d^*}{c'\log^2 n}$, where $c'$ can be chosen as a large enough constant and $N=\frac{\alpha_0 n}{2^{20} (d^*)^2\log n}$.
Throughout, we denote by $E'$ the set of edges that were deleted from $W^*$ as the result of this type of updates to $W^*$, so $|E'|\leq \frac{\alpha_0 n}{2^{20}}$ always holds. The time that is required to update graph $W^*$ with this type of updates is subsumed by the time spent in Step 1 of the algorithm.


\paragraph{Second Type of Updates.} 
The second type of update happens when the algorithm for Step 2 identifies a well-structured cut $(A,B)$ in $H$ with $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}$. Denote sets $A$ and $B$ by $Z$ and $Z'$, so that $Z$ is the smaller of the two sets, breaking ties arbitrarily. Recall that our algorithm then deletes the vertices of $Z$ from $H$. If, as the result of this deletion, the number of vertices in $H$ falls below $\left (1-\frac{1}{\hat c \log^4 n}\right )n'$, then the current phase terminates. If this did not happen, then we update graph $W^*$ as follows. Let $\hat E=\bigcup_{e\in E_H(A,B)}S(e)$, that is, these are all edges $e'\in E(W^*)\setminus F$ whose embedding path contains an edge of $E_H(A,B)$. Since the embedding of $W^*\setminus F$ into $H$ causes congestion at most $O(d\log^3 n)$ in $H$, we get that $|\hat E|\leq O(d\log^3 n)\cdot |E_H(A,B)|\leq O(|Z|\cdot \log^4n)$. 



We start by deleting the edges of $\hat E$ from $W^*$. Note that, if $Z=A$ and $Z'=B$, then graph $W^*\setminus F$ no longer contains any edges connecting vertices of $Z\cap V(W^*)$ to vertices of $Z'\cap V(W^*)$. In other words, $(Z\cap V(W^*),Z'\cap V(W^*))$ is a cut of sparsity $0$ in $W^*\setminus F$. We replace the set $V(W^*)$ of vertices in $\xset$ by two sets: $Z\cap V(W^*)$ and $Z'\cap V(W^*)$. We also delete the vertices of $Z$ from $W^*$. Similarly, if $Z=B$ and $Z'=A$, then $(Z'\cap V(W^*),Z\cap V(W^*))$ is a cut of sparsity $0$ in $W^*\setminus F$. We replace the set $V(W^*)$ of vertices in $\xset$ by two sets: $Z\cap V(W^*)$ and $Z'\cap V(W^*)$, and we delete the vertices of $Z$ from $W^*$.

We denote by $E''$ the set of edges that were deleted from $W^*$ as the result of this type of transformation: in other words, for each sparse cut $(A,B)$ of $H$ that our algorithm computes, we add all edges of $\bigcup_{e\in E_H(A,B)}S(e)$ to $E''$. Recall that the number of edges added to $E''$ due to such cut $(A,B)$ is bounded by 
$O(\log^4n)\cdot\min\set{|A|,|B|}$, and that the vertices of $A$ or the vertices of $B$ are deleted from $H$. Since the total number of vertices that may be deleted from $H$ before the phase terminates is bounded by $\frac{n'}{\hat c\log^4 n}$, where $\hat c$ can be chosen to be a large enough constant, we can ensure that throughout the phase $|E''|\leq \frac{\alpha_0 n}{2^{20}}$ holds.


\paragraph{Third Type of Updates.}
The algorithm for responding to \shortpath queries, that we describe below, may sometimes identify cuts $(A,B)$ in $W^*\setminus F$, with $|E_{W^*\setminus F}(A,B)|\leq \frac{\alpha_0}{2^{20}}\cdot \min\set{|A|,|B|}$. Whenever this happens, we replace the set $V(W^*)$ of vertices in $\xset$ with $V(A)$ and $V(B)$. Denote $A$ and $B$ by $Z$ and $Z'$, where $Z$ is the smaller of the two sets, breaking ties arbitrarily. We then delete the vertices of $Z$ from graph $W^*$.
Notice that $|E_{W^*\setminus F}(A,B)|\leq \frac{\alpha_0}{2^{20}}\cdot|Z|$.

 Let $E'''$ denote the collection of all edges that participate in such cuts. In other words, for each such sparse cut $(A,B)$ of $W^*\setminus F$, we include the edges of $E_{W^*\setminus F}(A,B)$ in $E'''$. From the above discussion, throughout the algorithm, $|E'''|\leq \frac{\alpha_0}{2^{20}}\cdot n''\leq \frac{\alpha_0}{2^{20}}\cdot n$ holds.
 
 Lastly, we denote $E^*=F\cup E'\cup E''\cup E'''$. Recall that $|F|\leq \frac{\alpha_0\cdot n'}{500}\leq \frac{\alpha_0\cdot n''}{62}$, since $n''\geq n'/8$. The cardinality of each of the three sets $E',E''$ and $E'''$ is bounded by $\frac{\alpha_0\cdot n}{2^{20}}\leq \frac{\alpha_0\cdot n'}{2^{19}}\leq \frac{\alpha_0\cdot n''}{2^{14}}$.
 Overall, we get that $|E^*|\leq \frac{\alpha_0\cdot n''}{32}$ holds throughout the algorithm.
We now show that, throughout the algorithm, $|V(W^*)|\geq n''/4$ holds.

\begin{claim}\label{claim: expander remains large}
	Throughout the algorithm,  $|V(W^*)|\geq n''/4$.
\end{claim}
\begin{proof}
	Assume otherwise. Consider some time $\tau$ at which $|V(W^*)|< n''/4$ holds. For convenience, we denote by $W$ the original graph $W^*$, which is an $\alpha_0$-expander, with $n''$ vertices and we denote by $W'$ the graph $W\setminus E^*$, with respect to the set $E^*$ of edges at time $\tau$. We also consider the set $\xset$ of vertex subsets at time $\tau$. We denote the sets of $\xset$ by $X_1,X_2,\ldots,X_r$, where $X_r=V(W^*)$ at time $\tau$, and the remaining sets are indexed in the order in which they were added to $\xset$. For all $1\leq j<r$, let $X'_j=X_{j+1}\cup\cdots\cup X_r$. At the time when $X_j$ was added to $\xset$, it defined a sparse cut in graph $W^*\setminus F$. In other words, either $|E_{W'}(X_j,X'_j)|\leq \frac{\alpha_0}{2^{20}}|X_j|$, or $|E_{W'}(X'_j,X_j)|\leq \frac{\alpha_0}{2^{20}}|X_j|$ holds. Let $\alpha$ be such that $\max_{X_j\in \xset}|X_j|=\alpha\cdot n''$. Then it is easy to verify that $\alpha\leq 1/2$ must hold. From \Cref{obs: from many sparse to one balanced}, there is a cut $(A,B)$ in $W'$ with $|A|,|B|\geq n''/4$, and $|E_{W'}(A,B)|\leq \frac{\alpha_0\cdot n''}{2^{20}}$.
	
	Observe that $|E_W(A,B)|\leq |E^*|+\frac{\alpha_0\cdot n''}{2^{20}}\leq \frac{\alpha_0\cdot n''}{16}$. Since $|A|,|B|\geq n''/4$, we obtain a cut $(A,B)$ in $W$, whose sparsity is below $\alpha_0$, contradicting the fact that $W$ is an $\alpha_0$-expander.
\end{proof}



This completes the description of the data structures that we maintain over the course of Step 2. Next, we describe an algorithm for responding to a \shortpath query.

\subsection*{Responding to \shortpath queries}
In a \shortpath query, we are given a pair $x,y$ of vertices of $H$, and our goal is to compute a path connecting $x$ to $y$ in $H$ of length at most $d^*$. We note that we only need to ensure that the total time spent on responding to all $N$ queries is suitably bounded, but the time spent on responding to a specific query may be quite large. 
The algorithm for responding to a query consists of two steps. In the first step, we compute the desired path connecting $x$ to $y$ in $H$, whose length is at most $d^*$. After that, some edges may be deleted from $H$. We then execute a second, clean-up step, whose purpose is to ensure that for every pair $a,b$ of vertices that remain in the expander $W^*$,
$\dist_{W^*}(a,b),\dist_{W^*}(b,a)\leq \hat d$ holds, where  $\hat d=\frac{2^{30}\log n}{\alpha_0}$ is the parameter that we defined above. Additionally, we will need to ensure that every vertex of $H$ lies in both the trees $\tau'$ and $\tau''$.


In order to execute the first step, we use \EST $\tau''$ to compute a path $P'$ of length at most $d$, connecting $x$ to some vertex $x'\in V(W^*)$, in time $O(d)$. Similarly, we use \EST $\tau'$ in order to compute a path $P''$ of length at most $d$, connecting some vertex $y'\in V(W^*)$ to $y$, in time $O(d)$. Next, we perform a BFS in graph $W^*$, from vertex $x'$, in order to compute the shortest $x'$-$y'$ path $Q$ in $W^*$. Recall that we are guaranteed that the length of $Q$ in $W^*$ is bounded by  $\hat d=\frac{2^{30}\log n}{\alpha_0}$. We then use the embedding of $W^*$ into $H$ via paths of lengths at most $O(d\log n)$ in order to obtain a path $\hat P$ connecting $x'$ to $y'$ in $H$, whose length is at most $O(d \log^2n)$.
Let $P^*$ be the path that is obtained by concatenating  $P',\hat P$ and $P''$. Path $P^*$ connects $x$ to $y$ in graph $H$, and its length is bounded by $2d+O(d\log^2n)$. Since we have set $d=\frac{d^*}{c'\log^2 n}$, where $c'$ is a large enough constant, the length of $P^*$ is bounded by $d^*$. We transform $P^*$ into a simple path in time $O(d^*)$ and return the resulting path. This finishes the first step of the algorithm for responding to the query. Notice that its running time is bounded by $O(n+d^*)$, since a BFS search in $W^*$ can be performed in time $O(n)$, and the time required to compute paths $P'$ and $P''$ and to transform $Q$ into path $P^*$ is bounded by $O(d^*)$. 


We now proceed to describe the second, clean-up step of the algorithm for responding to a \shortpath query. Once path $P^*$ is returned by the algorithm in response to the query, some edges of $P^*$ may be deleted from $H$. As a result, it is possible that some vertices of $H$ no longer belong to one on both of the trees $\tau',\tau''$. As described already, we will compute a sparse cut in $H$ in order to fix this issue, but this may in turn affect the expander $W^*$. Additionally, the deletion of the edges from $H$ may lead to the deletion of some edges from the expander $W^*$. As a result, it is possible that its diameter grows beyond $\hat d$. In such a case, we will  compute  a sparse cut in the expander $W^*$, but this may in turn affect the trees $\tau',\tau''$. We now formally describe the clean-up step.



 At the beginning of the clean-up step, we select an arbitrary vertex  $v\in V(W^*)$, and compute two shortest-paths trees $\hat \tau'$ and $\hat \tau''$ rooted at $v$ in graph $W^*$, where the edges in $\hat \tau'$ are directed away from $v$, and the edges in $\hat \tau''$ are directed towards $v$. In other words, for every vertex $a\in V(W^*)$, the unique $s$-$a$ path in $\hat \tau'$ is a shortest $s$-$a$ path in $W^*$, and the unique $a$-$s$ path in $\hat \tau''$ is a shortest $a$-$s$ path in $W^*$. Note that both trees can be computed in time $O(n)$. We then perform a number of iterations. At the beginning of every iteration, we assume that we are given some vertex $v\in V(W^*)$, and two shortest paths trees $\hat \tau'$ and $\hat \tau''$ in $W^*$ that are both rooted at $v$, with the edges of $\hat \tau'$ directed away from $v$, and the edges of $\hat \tau'$ directed towards $v$. The iterations are executed as long as one of the following two conditions hold: (i) some vertex $u\in V(H)$ does not lie in $\tau'$ or in $\tau''$; or (ii) the depth of at least one of the trees $\hat \tau',\hat \tau''$ is greater than $\hat d$. We now describe the execution of a single iteration.
 
 
 Assume first that some vertex $u\in V(H)$ no longer lies in $\tau''$; in other words, $\dist_H(u,V(W^*))>d$ holds. As we described already, we  use the algorithm from \Cref{obs: ball growing2} in order to compute a well-structured cut $(A,B)$ in $H$ with $u\in A$, $V(W^*)\subseteq B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. If $|A|\leq |B|$, then we delete the vertices of $A$ from $H$, (which includes deleting their incident edges from graphs $H,H'$, and $H''$, and both \EST data structures $\tau'$ and $\tau''$). If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated, and otherwise we continue the algorithm. Alternatively, if $|A|>|B|$, then we delete the vertices of $B$ from $H$, and terminate the current phase.
 Similarly, if some vertex $u\in V(H)$ no longer lies in $\tau'$, then, as desribed above, we  use the algorithm from \Cref{obs: ball growing2} (but with reversed directions of edges) in order to compute a well-structured cut $(A,B)$ in $H$ with $V(W^*)\subseteq  A$, $v\in B$, and $|E_H(A,B)|\leq \frac{2^{11}\log n}{d}\cdot \min\set{|A|,|B|}\leq O\left(\frac{\log^4n}{d^*} \right )\cdot \min\set{|A|,|B|}$. As before, if $|B|\leq |A|$, then we delete the vertices of $B$ from $H$, and from both \EST data structures. If $|V(H)|$ falls below $n'\left(1-\frac{1}{\hat c\log^4n}\right )$, then the algorithm is terminated, and otherwise we continue the algorithm. Alternatively, if $|B|>|A|$, then we delete the vertices of $A$ from $H$, and terminate the current phase. In the latter case, at least $n/64$ vertices have been deleted from $H$ in the current phase.
 Let $Z$ be the set of all vertices that were deleted from $H$ in the current iteration, and let
 $\hat E=\bigcup_{e\in E_H(A,B)}S(e)$, that is, these are all edges $e'\in E(W^*)\setminus F$ whose embedding path contains an edge of $E_H(A,B)$.
 Since the embedding of $W^*\setminus F$ into $H$ causes congestion at most $O(d\log^3 n)$, we get that $|\hat E|\leq O(d\log^3 n)\cdot |E_H(A,B)|\leq O(|Z|\cdot \log^4n)$. 
  We delete the edges of $\hat E$ from graph $W^*$. If $Z\cap V(W^*)=\emptyset$, then we say that the current iteration is a \emph{type-(1a) iteration}, and we continue to the next iteration. Notice that in this case, the running time of the current iteration is $\otilde(\vol_H(Z))$, and we \emph{charge} the running time of the current iteration to the set $Z$ of vertices.
 
Assume now that $Z\cap V(W^*)\neq \emptyset$. In this case, we say that the current iteration is a \emph{type-(1b) iteration}.  Let $X=Z\cap V(W^*)$. So far the total running time of the iteration is  $\tilde O(\vol_H(Z))$, and it is charged to the set $Z$ of vertices. Next, we delete the vertices of $X$ from $W^*$. The remainder of the running time of the current iteration will be charged to set $X$. As observed already, if $Z=A$, and we denote $Z'=B$, then graph $W^*\setminus F$ no longer contains any edges connecting vertices of $Z\cap V(W^*)$ to vertices of $Z'\cap V(W^*)$. In other words, $(Z\cap V(W^*),Z'\cap V(W^*))$ is a cut of sparsity $0$ in $W^*\setminus F$.
Similarly, if $Z=B$, and we denote $Z'=A$, then cut $(Z'\cap V(W^*),Z\cap V(W^*))$ is a cut of sparsity $0$ in $W^*\setminus F$. Once the vertices of $X$ are deleted from $W^*$, we select an arbitrary vertex $v\in V(W^*)$, and compute two shortest-paths trees $\hat \tau'$ and $\hat \tau''$ rooted at $v$ in graph $W^*$, where the edges in $\hat \tau'$ are directed away from $v$, and the edges in $\hat \tau''$ are directed towards $v$. It is easy to verify that the total running time of a type-(1b) iteration is bounded by $\otilde(\vol_H(Z))+O(n)$. We charge time $\otilde(\vol_H(Z))$ to the set  $Z$ of vertices that is deleted from $H$ in the current iteration, and we charge time $O(n)$ to the set $X$ of vertices that is deleted from $W^*$ in the current iteration. 
Lastly, graphs $H'$ and $H''$ need to be updated to reflect the deletion of the vertices of $X$ from $W^*$: namely, for all $u\in X$, we delete the edge $(s',u)$ from $H'$, and we delete the edge $(s'',u)$ from $H''$. This, in turn, may require updating the \EST data structures $\tau'$ and $\tau''$. The time required to update the two trees is counted as part of the total update time of these data structures, and not as part of the running time of the current iteration.
This completes the description of a type-(1b) iteration.

If the depth of either of the trees $\hat \tau',\hat \tau''$ is greater than $\hat d$, then we say that the current iteration is a type-2 iteration. In this case, we can compute, in time $O(1)$, a pair $a,b\in V(W^*)$ of vertices with $\dist_{W^*}(a,b)>\hat d$.
Recall that  $\hat d=\frac{2^{30}\log n}{\alpha_0}$, and the maximum vertex degree in $W^*$ is bounded by $D=18$. We can now use the algorithm from \Cref{obs: ball growing} to compute, in time $O(n)$, a cut $(A,B)$ in $W^*$ of sparsity at most $\phi=\frac{32D\log n}{\hat d}\leq \frac{\alpha_0}{2^{20}}$. If $|A|\leq |B|$, then we delete from $W^*$ the vertices of $A$, and otherwise we delete from $W^*$ the vertices of $B$.
If we denote by $X$ the set of vertices deleted from $W^*$ in the current iteration, then graphs $H'$ and $H''$ need to be updated accordingly (namely, for all $u\in X$, we delete the edge $(s',u)$ from $H'$ and we delete the edge $(s'',u)$ from $H''$). This, in turn, may require updating the \EST data structures $\tau'$ and $\tau''$. The time required to update the two trees is counted as part of the total update time of these data structures, and not as part of the running time of the current iteration.
 We then select an arbitrary vertex $v\in V(W^*)$, and compute two shortest-paths trees $\hat \tau'$ and $\hat \tau''$ rooted at $v$ in graph $W^*$, where the edges in $\hat \tau'$ are directed away from $v$, and the edges in $\hat \tau''$ are directed towards $v$. Clearly, the running time of a type-2 iteration is $O(n)$, and we charge it to the set of vertices (either $A$ or $B$) that was deleted from $W^*$ over the course of the current iteration.  

The algorithm for the second clean-up step terminates once every vertex of $H$ lies in both $\tau'$ and $\tau''$, and the depths of the trees $\hat \tau'$ and $\hat \tau''$ are both bounded by $\hat d$.

We now bound the total time required to respond to \shortpath queries. The first step of the algorithm for responding to the query takes time $O(n+d^*)$. We include in this time the time required to compute the shortest-path trees $\hat \tau',\hat \tau''$ in $W^*$ for the first time at the beginning of the clean-up step. The total running time of the first step of the algorithm for responding to \shortpath queries, over all $N=O\left(\frac{n}{(d^*)^2\log n}\right )$ queries that we need to support over the course of the phase, is bounded by $O(N\cdot(n+d^*))\leq O(n^2)$.

If we denote by $Z$ the set of all vertices that are deleted over the course of the phase from graph $H$, and by $\xset$ the collection of all subsets of vertices that were deleted from $V(W^*)$ over the course of the phase, then, from our charging scheme, the remaining running time that is spent on the cleanup step can be bounded by $\otilde(\vol_H(Z))+O(|\xset|\cdot n)\leq \otilde(\vol_H(Z))+O(n^2)$. Therefore, the total time spent over the course of a single phase on responding to $\shortpath$ queries is bounded by $\otilde(\vol_H(Z))+O(n^2)$, where $Z$ is the set of vertices deleted from $H$ during the phase.



\paragraph{Final Analysis of the Running Time.}
We now bound the total running time of a single phase. Recall that the running time of Step 1 is bounded by $O(|E(H)|\cdot d+n^2)$. The total time spent on responding to queries is bounded by $\tilde O(n^2+|E(H)|)$, and the time spent on maintaining \EST data strucures $\tau'$ and $\tau''$ is bounded by $\tilde O(|E(H)|\cdot d)$. 
Additional time that is required to maintain the expander $W^*$ is bounded by the above running times, and so the running time of a single phase is bounded by $\tilde O(|E(H)|\cdot d+n^2)\leq \tilde O(|E(H)|\cdot d^*+n^2)$.

Since the number of phases is bounded by $\tilde O\left (\max\set{1,\frac{\Delta\cdot (d^*)^2}{n}}\right )$, we get that the total running time of the algorithm is bounded by:

\[\otilde(|E(H)|\cdot d^*+n^2)\cdot  \max\set{1,\frac{\Delta\cdot (d^*)^2}{n}}. \]



%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------

\subsection{Algorithm \algembedorcut: Proof of \Cref{thm: embed expander or cut}}
\label{sec: embed or cut}
We use the Cut-Matching Game -- a framework that was initially proposed by \cite{KRV}. The specific variant of the game is due to \cite{KKOV}. Its slight modification (that we also use) was proposed in \cite{detbalanced}, and later adapted to directed graphs in \cite{SCC}.
We also note that \cite{directed-CMG} extended the original cut-matching game of \cite{KRV} to directed graphs, though we do not use this variation here.
We now define the variant of the game that we use.

The game is played between two players: the Cut Player and the Matching Player. 
The game starts with a directed graph $W$ that contains $n$ vertices,  and no edges, where $n$ is an even integer, and proceeds in iterations. In the $i$th iteration, the Cut Player chooses a cut $(A_i,B_i)$ in $W$ with $|A_i|,|B_i|\geq n/10$, and $|E_W(A_i,B_i)|\leq n/100$. It then computes two arbitrary equal-cardinality sets $A_i',B_i'$ of vertices with $|A'_i|\geq n/4$, such that either $A_i\subseteq A'_i$, or $B_i\subseteq B'_i$. The matching player then needs to return two perfect matchings: a matching $M_i\subseteq A'_i\times B'_i$, and  a matching $M'_i\subseteq B'_i\times A'_i$, both of cardinality $|A'_i|$. The edges of $M_i\cup M'_i$ are added to $W$, and the iteration terminates. The following bound on the number of iterations in this variant of the Cut-Matching Game was shown in \cite{SCC}, extending a similar result of \cite{KKOV} for undirected graphs.

\begin{theorem}[Lemma 7.4 in \cite{SCC}; see also Theorem 7.3 and the following discussion]\label{thm: CMG bound}
The number of iterations in the above Cut-Matching Game is bounded by $O(\log n)$.
\end{theorem}

From the above theorem, there is an absolute constant $\cCMG>0$, such that, after $\cCMG\log n$ iterations of the above game, for every cut $(A,B)$ in $W$ with $|A|,|B|\geq n/10$, $|E_W(A_i,B_i)|>n/100$ must hold. Notice that the maximum vertex degree in the final graph $W$ is bounded by $2\cCMG\log n$.

In order to implement the Cut-Matching Game, we design two algorithms: an algorithm for the Cut Player, and an algorithm for the Matching Player. We note that previous work, such as, e.g. \cite{SCC} also designed similar algorithms, but since we focus here on a more specific setting, we believe that our algorithm for the cut player is significally simpler, while the algorithm for the Matching Player achieves better parameters.


The algorithm for the Cut Player is summarized in the following theorem, whose proof is deferred to \Cref{subsec: algorithm for the cut player}.
The theorem uses the constant $\alpha_0$ from \Cref{thm:explicit expander}.
\begin{theorem}\label{thm: cut player outer}
	There is a deterministic algorithm, that, given an $n$-vertex directed graph $G$ with maximum vertex degree at most $O(\log n)$, returns one of the following:
	
	\begin{itemize}
		\item Either a cut $(A,B)$ in $G$ with $|E_G(A,B)|\leq n/100$ and $|A|,|B|\geq n/10$; or
		
		\item another directed graph $W'$ with $|V(W')|\geq n/4$ and maximum vertex degree at most $18$, such that $W'$ is an $\alpha_0$-expander, together with a subset $F\subseteq E(W')$ of at most $\frac{\alpha_0\cdot n}{1000}$ edges of $W'$, and an embedding $\pset$ of $W'\setminus F$ into $W$ via paths of length at most $d=O(\log n)$, that cause congestion at most $\eta=O(\log n)$.
	\end{itemize}
	
	The running time of the algorithm is $\otilde(n^2)$.
\end{theorem}

We note that \cite{SCC}, generalizing the results of \cite{detbalanced} to directed graphs, provided an algorithm for the cut player with faster running time $\ohat(n)$ (see Theorem 7.3 in \cite{SCC}). We could have used their algorithm as a blackbox instead of the algorithm from \Cref{thm: cut player outer}. However, the proof of \Cref{thm: cut player outer} is significantly simpler than that of \cite{SCC} and \cite{detbalanced}, and we can afford this  slower running time since other components of our algorithm have slower running time. 



The algorithm for the Matching Player is summarized in the following theorem, whose proof is deferred to \Cref{sec: matching player alg}.

\begin{theorem}\label{thm: alg for matching player}
	There is a deterministic algorithm, whose input consists of a directed $n$-vertex bipartite graph $G=(L,R,E)$, where $n$ is an even integer, such that every vertex in $R$ has out-degree at most $1$ and every vertex in $L$ has in-degree at most $1$, together with two disjoint sets $A,B$ of vertices of $G$ of cardinality $n/2$ each, and two parameters $d\geq 4$ and $z\geq 1$.
	
	The algorithm returns one of the following:
	\begin{itemize}
		\item either a cut $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{2n}{d}$ and $|X|,|Y|\geq z$; or
		
		\item a collection $\qset$ of at least $(n/2-z)$ paths in graph $G$, with every path $Q\in \qset$ connecting some vertex of $A$ to some vertex of $B$, such that the length of every path in $\qset$ is at most $2d+1$, the paths cause congestion at most $O(d\log n)$, and the endpoints of all paths are distinct.
	\end{itemize}
	The running time of the algorithm is $\otilde(md)$.
\end{theorem}

Note that in the above theorem we assume that all edge lengths in the input graph $G$ are unit.




We are now ready to complete the algorithm for \Cref{thm: embed expander or cut}. We will assume that $n=|V(G)|$ is an even integer; otherwise, we temporarily delete an arbitrary vertex $v_0$ from $G$. 
We let $c$ be a large enough constant, so that,  
in \Cref{thm: cut player outer} the parameter $\eta\leq c\log n$. 

 We start with a graph $W$ that contains $n$ vertices and no edges, and then run the Cut-Matching game on it. Recall that the number of iterations in the game is bounded by $\cCMG\cdot \log n$. 
This ensures that the graph $W$ that is maintained over the course of the game has maximum vertex degree $O(\log n)$.
We now describe the execution of the $i$th iteration.


First, we apply the algorithm from \Cref{thm: cut player outer} to the current graph $W$. We say that the current iteration is a type-1 iteration, if the algorithm returns 
a cut $(A_i,B_i)$ in $W$ with $|E_W(A_i,B_i)|\leq n/100$ and $|A_i|,|B_i|\geq n/10$, and otherwise we say that it is a type-2 iteration. Assume first that the current iteration is a type-1 iteration. Then we compute an arbitrary partition $(A'_i,B'_i)$ of $V(W)$ into two subsets of cardinality $n/2$ each, such that either $A_i\subseteq A'_i$ or $B_i\subseteq B'_i$, and we treat $(A'_i,B'_i)$ as the move of the cut player.

Next, we twice apply the algorithm from \Cref{thm: alg for matching player} to  graph $G$, with parameter $d$ that remains unchanged, and parameter ${z=\frac{\alpha_0}{2000c\cdot \cCMG\cdot \log^2n}\cdot n}$: once for the ordered pair of sets $(A'_i,B'_i)$, and once for the ordered pair of sets $(B'_i,A'_i)$.

Assume first that in any of the two applications of the algorithm, it returns  a cut $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{2n}{d}$ and $|X|,|Y|\geq z\geq \Omega(n/\log^2 n)$. In this case, we terminate the algorithm and return the cut $(X,Y)$ as its outcome. 
If the initial value $|V(G)|$ was odd, then we add vertex $v_0$ to $X$ if $v_0\in R$, and to $Y$ otherwise. In this case, the only newly added edge to $E_G(X,Y)$ is the special edge incident to $v_0$ (if such an edge exists), and so $|E_G(X,Y)|\leq \frac{2n}{d}+1$ holds.
We also say that the current iteration is of \emph{type (1a)}. 

Otherwise, the algorithm computes a collection $\qset'_i$ of at least $(n/2-z)$ paths in graph $G$, with every path $Q\in \qset_i$ connecting a distinct vertex of $A'_i$ to a distinct vertex of $B'_i$, 
and a collection $\qset''_i$ of at least $(n/2-z)$ paths in  $G$, with every path $Q'\in \qset'_i$ connecting a distinct vertex of $B'_i$ to a distinct vertex of $A'_i$. The paths in $\qset'_i\cup \qset''_i$ have lengths at most $2d+1$ each, and they cause congestion at most $O(d\log n)$.
In this case, we say that the current iteration is of \emph{type (1b)}.
 The set $\qset'_i$ of paths naturally defines a matching $M'_i\subseteq A'_i\times B'_i$, where for every path $Q\in \qset_i$ whose endpoints are $a\in A'_i,b\in B'_i$, we add an edge $e=(a,b)$ to the matching. We also let $P(e)=Q$ be its embedding into $G$. Similarly, the set $\qset''_i$ of paths defines a matching $M''_i\subseteq B'\times A'$, together with an embedding $P(e)\in \qset''_i$ of each edge $e\in M''$. Recall that matching $M'_i$ has cardinality at least $n/2-z$, while $|A'|=|B'|=n/2$. Therefore, by adding a set $F'_i$ of at most $z$ additional edges (that we refer to as \emph{fake edges}), we can turn matching $M'_i$ into a perfect one. Similarly, we add a collection $F''_i$ of at most $z$ fake edges to $M''_i$ in order to turn it into a perfect matching. The edges of $M'_i\cup M''_i$ are then added to graph $W$, and the current iteration terminates.


Finally, assume that the current iteration $i$ is of type 2. In this case, the algorithm for the Cut Player from \Cref{thm: cut player outer} computed a graph 
$W'$ with $|V(W')|\geq n/4$ and maximum vertex degree at most $18$, such that $W'$ is an $\alpha_0$-expander, together with a subset $\hat F\subseteq E(W')$ of at most $\frac{\alpha_0\cdot n}{1000}$ edges of $W'$, and an embedding $\pset$ of $W'\setminus \hat F$ into $W^*$ via paths of length at most $O(\log n)$, that cause congestion at most $c\log n$.

Consider the current graph $W^*$. Denote $F^*=\bigcup_{i'=1}^{i-1}(F'_i\cup F''_i)$ -- the collection of the fake edges that we have computed so far. Since for all $1\leq i'<i$, $|F'_i\cup F''_i|\leq 2z$ and $i\leq \cCMG\log n$, we get that $|F^*|\leq 2\cCMG z \log n$.
We also denote $\qset^*=\bigcup_{i'=1}^{i-1}(\qset'_i\cup \qset''_i)$. Note that $\qset^*$ defines an embedding of $W^*\setminus F^*$ into $G$. All paths in $\qset^*$ have lengths at most $2d+1$. Each set $\qset'_i\cup \qset''_i$ causes congestion at most $O(d\log n)$, and so the total congestion caused by the paths in $\qset^*$ is bounded by $\eta^*=O( d\log^2n)$.

Next, we will construct a set $F\subseteq E(W')$ of fake edges, and an embedding of the remaining edges of $W'$ into $G$. We start with $F=\hat F$. Next, we process every edge $e\in E(W')\setminus \hat F$ one by one. When an edge $e=(u,v)$ is processed, we consider the path $P(e)\in \pset$, that serves as an embedding of $e$ into graph $W^*$. Recall that the length of the path is at most $O(\log n)$. Let $P(e)=(e_1,e_2,\ldots,e_k)$, where $k\leq O(\log n)$. 
If path $P(e)$ contains any edges of $F^*$, then we add $e$ to the set $F$ of fake edges. Otherwise,
for all $1\leq j\leq k$, we consider the path $Q(e_j)\in \qset^*$, that serves as the embedding of the edge $e_j$ into graph $G$. Recall that the length of $Q$ is at most $O(d)$. By concatenating the paths $Q(e_1),\ldots,Q(e_k)$, we obtain a path $P'(e)$ connecting $u$ to $v$ in $G$, whose length is at most $O(d\log n)$.  We turn $P'(e)$ into a simple path in time $O(d\log n)$, obtaining the final path $P^*(e)$, that will serve as an embedding of the edge $e$.

Once every edge of $W'\setminus \hat F$ is processed, we obtain a final set $F$ of fake edges, and, for every remaining edge $e\in E(W')\setminus F$, a simple path $P^*(e)$ of length $O(d\log n)$, that serves as the embedding of $e$ in $G$. Recall that $|V(W')|\geq n/4$. If the original value $|V(G)|$ was odd, then $|V(W')|\geq (|V(G)|-1)/4\geq |V(G)|/8$ holds. As required, graph $W'$ is an $\alpha_0$-expander with maximum vertex degree at most $18$. It remains to bound the congestion caused by the paths in set $\pset^*=\set{P^*(e)\mid e\in E(W')\setminus F}$, and the cardinality of the set $F$.


Consider any edge $e\in E(G)$. Recall that $e$ may participate in at most $\eta^*= O(d\log^2n)$ paths in set $\qset^*=\set{Q(e')\mid e'\in E(W)\setminus F^*}$. Every edge $e'\in E(W)\setminus F^*$, whose corresponding path $Q(e')$ contains the edge $e$, may in turn participate in at most $O(\log n)$ paths of $\pset$. Therefore, overall, every edge $e$ of $G$ participates in at most $O(d\log^3n)$ paths of $\pset^*$.

In order to bound the final number of the fake edges in $W'$,
 recall that $|F^*|\leq 2\cCMG z \log n$. Since the paths in $\pset$ cause congestion at most $c\log n$, we get that every edge of $F^*$ may participate in at most $c\log n$ paths of $\pset$. Therefore, $|F\setminus \hat F|\leq (2\cCMG z \log n)\cdot (c\log n)\leq 2c\cdot \cCMG\cdot z\cdot \log^2n\leq \frac{\alpha_0\cdot n}{1000}$,
since $z=\frac{\alpha_0}{2000c\cdot \cCMG\cdot \log^2n}\cdot n$.  
Since $|\hat F|\leq \frac{\alpha_0\cdot n}{1000}$, we get that $|F|\leq \frac{\alpha_0\cdot n}{500}$.

It now remains to bound the running time of the algorithm. The algorithm has $O(\log n)$ iterations. In every iteration we use the algorithm for the Cut Player from \Cref{thm: cut player outer}, whose running time is  $\otilde(n^2)$, and an algorithm for the Matching Player from \Cref{thm: alg for matching player}, whose running time is $\otilde(md+n^2)$.

Additionally, when computing the embedding of $W'\setminus F$ into $G$, we spend time at most $O(d\log n)$ per edge of $W'$, and, since $|E(W')|\le O(n)$, the computation of the embedding takes time $O(nd\log n)$.
Overall, the running time of the algorithm is $\otilde(md+n^2)$.
\input{cut-player-alg}
\input{matching-player-alg}

==> leftovers.tex <==

We now describe a primal-dual framework for computing integral $A'$-$B'$ flow in graph $G'$. This is similar in spirit to the primal-dual framework of~\cite{GK98, Fleischer00} used in proving Theorem~\ref{thm: informal max s-t flow and min s-t cut}, but it is better suited for our integral routing application (see also~\cite{AAP93}).


Let $\pset$ be the set of all paths connecting vertices of $A'$ to vertices of $B'$ in $G'$.
We use the following linear program and its dual.


\begin{tabular}[t]{|l|l|}\hline &\\
	$\begin{array}{lll}
	\text{\underline{Primal}}&&\\
	\text{Max}&\sum_{P\in \pset} f(P)&\\
	\text{s.t.}&&\\
	%&\sum_{P\in \pset(a)}f(P)\leq 1&\forall a\in A'\\
	%&\sum_{P\in \pset(b)}f(P)\leq 1&\forall b\in B'\\
	&\sum_{\stackrel{P\in\pset:}{v\in P}}f(P)\leq
	c(v)&\forall v\in V(G')\\
	&f(P)\geq 0&\forall P\in \pset\\
	\end{array}$
	&$
	\begin{array}{lll}
	\text{\underline{Dual}}&&\\
	\text{Min}&\sum_{v\in V(G')}c(v)x_v\\
	\text{s.t.}&&\\
	&\sum_{v\in P}x_v\geq 1&\forall P\in \pset\\
	&x_v\geq 0&\forall v\in V(G')\\
	&&\\
	\end{array}$\\ &\\ \hline
\end{tabular}

Recall that, if we denote by $\opt$ the value of the optimal integral solution to the primal linear program, and by $\optp$ and $\optd$ the values of the optimal (fractional) solutions to the primal and the dual LP's, respectively, then for any feasible dual solution of cost $\costd$,

\[\opt\leq \optp \leq \optd \leq \costd.\]


The algorithm starts with an infeasible dual solution, where for every vertex $v\in V'$, we set $x_v=0$, and a path set $\qset=\emptyset$. Throughout the algorithm, we increase the vertex lengths $x_v$ and add paths to $\qset$. At every point in the algorithm, for every path $P\in \pset$, we define its length to be $\sum_{v\in P}x_v$.


We assume for now that  we are given an oracle, that, in every iteration, either produces a path $P\in \pset$, whose length is less than $1$, or certifies that every path in $P\in \pset$ has length at least $(1-\eps)$ for some $\eps \in (0,1/2)$. An iteration is executed as follows. If the oracle returns a path $P\in \pset$ of length less than $1$, then we add $P$ to $\qset$. Assume that $a\in A'$ and $b\in B'$ are the endpoints of $P$. We set $x_a=x_b=1$, and, for every regular vertex $v\in V'$ that lies on $P$, we update the value $x_v$ as follows. If $x_v=0$, then we set $x_v=1/n$; otherwise, we set $x_v = (1 + \alpha)x_v$. 
Notice that in every iteration, the number of the paths we route increases by $1$, while the cost of the dual solution value increases by at most $4$ (since $\alpha\leq 1$).  Therefore, if $\qset$ if the current set of paths that we have routed, then $|\qset|\geq  (\sum_{v \in V'} c(v)x_v)/4$ holds throughout the algorithm. Notice that all paths in $\qset$ are guaranteed to have distinct endpoints. The algorithm terminates once the oracle reports that every path in $\pset$ has length at least $(1-\eps)$. We now consider two cases.

The first case happens if $|\qset|\geq |A|/100$ at the end of the algorithm. In this case, we return a set $\qset'$ of paths, obtained from the set $\qset$ of paths by deleting, for every path $Q\in \qset$, its first and last vertex. This ensures that the paths of $\qset'$ are contained in the original graph $G$. Notice that their endpoints still remain disjoint. Moreover, it is easy to see that the paths in $\qset'$ cause vertex-congestion at most $O(\log n/\alpha)$ in $G$, since after $O(\log n/\alpha)$ updates of the form $x_v = (1 + \alpha)x_v$, the value $x_v > 1$,  and hence $v$ cannot be on any path $P\in \pset$ of length less than $1$.

Assume now that $|\qset|<|A|/100$. We show a near-linear algorithm to compute a cut of sparsity at most $O(\alpha)$ in $G$. Recall that, upon the termination of the algorithm, every $A'$-$B'$ path has length at least $(1 - \eps)$. So if we scale up the value $x_v$ for every regular vertex $v$ by $1/(1-\eps) \le 2$, we obtain a feasible dual solution of value at most $8|\qset|$.

Let $A''\subseteq A'$ and $B''\subseteq B$ be the sets of vertices that do not serve as endpoints for paths in $\qset$. Notice that $|A''|,|B''|>  99|A|/100$,  and for all $v\in A''\cup B''$, $x_v=0$. Consider a new graph $G''$, obtained from $G'$, after we delete all vertices of $A'\setminus A''$ and $B'\setminus B''$ from it;  unify all vertices of $A''$ into a new source $s'$; and  unify all vertices of $B''$ into a new sink $t'$. The current values $x_v$ for regular vertices $v\in V'$ now define a feasible solution to the minimum $s'$-$t'$ cut LP in this new graph $G''$. The value of this $s'$-$t'$ cut LP solution is at most $8|\qset|\leq 8 |A|/100$, since $|\qset|\leq |A|/100$. 
We can now once again use the standard random threshold rounding to recover, in  expected time $O(|V| + |E|)$, an integral $s'$-$t'$ vertex cut in $G''$ of cost at most $ |A|/10$. Let $X'$ be the set of vertices deleted in this $s'$-$t'$ cut -- note that all vertices in $X'$ are regular vertices. Since each vertex in $X'$ has capacity of $1/\alpha$, it must be that $|X'| \le  \alpha  |A|/10 $.

We now construct a vertex cut of sparsity $O(\alpha)$ in the original graph $G$.  Let $\hat A\subseteq A$ be the set of vertices of $G$ corresponding to the vertex set $A''$, that is: $\hat A=\set{a\mid a'\in A''}$, and let $\hat B$ be defined similarly for $B''$. 
By our construction of $G''$, graph $G\setminus X'$ contains no path connecting a vertex of $\hat A$ to a vertex of $\hat B$ (but it is possible that $\hat A\cap X',\hat B\cap X'\neq \emptyset$).  We let $Y$ be the union of all connected components of $G\setminus X'$ containing  vertices of $\hat A$, and we let $Z=V(G)\setminus(X'\cup Y)$. Our algorithm returns the cut $(Y,X',Z)$. We now analyze its sparsity. Recall that $|X'|\leq \alpha |A|/10$, while $|\hat A|,|\hat B|\geq 99|A|/100$. Since $\alpha\leq 1$, at least $0.8|A|$ vertices of $\hat A$ lie in $Y$, and similarly, at least $0.8|A|$ vertices of $\hat B$ lie in $Z$. Therefore, $|Y|,|Z|\geq 0.8|A|$, and the sparsity $\phi(Y,X',Z)\leq O(\alpha)$.

Before we discuss the implementation of the oracle, we analyze the running time of the algorithm so far. The running time of the primal-dual part is bounded by the number of updates to the vertex lengths $x_v$. It is easy to verify that each such variable $x_v$ is updated at most $O(\log n/\alpha)$ times, and so the total running time of this part, excluding the time needed to respond to the oracle queries, is $O(n\log n/\alpha)=O(n^2\log n)$. The final step of computing the cut via the random threshold algorithm has expected running time $O(n+|E(G)|)$. 
It now remains to show how to implement the oracle.

==> marked-vertex.tex <==
\subsection{The Marked-Vertex Model}
\label{subsec: marked-vertex model}

\mynote{we may choose to get rid of it and just use the adjacency list model.}

In some of the problems that we consider, the algorithm may not need to explore the entire input graph $G$, and in some cases, it is important that the running time of the algorithm is strictly smaller than $|E(G)|$. As an example, consider the following routing problem: we are given as input a directed graph $G$, and two disjoint sets $A$,$B$ of its vertices. The goal is to compute a largest-cardinality collection $\pset$ of paths, where each path $P\in \pset$ connects a vertex of $A$ to a vertex of $B$, the paths in $\pset$ cause low edge-congestion, and every vertex of $A\cup B$ serves as an endpoint of at most one path in $\pset$. We emphasize that vertices of $A\cup B$ may serve as inner vertices on paths in $\pset$, and it is possible that some vertex $v\in A\cup B$ serves both as an endpoint of some path in $\pset$, and as an inner vertex on several other paths. Consider now a scenario where almost all vertices of $G$ lie in $B$. In such a case, one can show that there is an optimal solution $\pset$ to the problem, such that only a small number of vertices of $B$ participate in the paths in $\pset$. In other words, in order to compute such a collection of paths, it is not necessary to explore the entire graph $G$. In such cases, we will often be ineterested in algorithms with running time roughly $O(n^{1+o(1)}\cdot (n-|B|))$, that  may be significantly smaller than $|E(G)|$, if graph $G$ is sufficiently dense. Therefore, we will need to provide the input graph $G$ to the algorithm in a way that allows it to achieve this low running time, and does not require spending $\Omega(|E(G)|)$ time in order to process the entire input. This type of issue only arises in a very specific type of routing problems that we described above, and all algorithms that we employ for such problems construct the set $\pset$ of paths gradually, by starting with $\pset=\emptyset$, and then adding one path to $\pset$ at a time. This motivates the \emph{Marked-Vertex Model} that we now define.


\begin{definition}[Marked-Vertex Model]\label{def: marked vertex}
	Suppose we are given a graph $G$, and a partition $(M,\notM)$ of its vertices into the set $M$ of \emph{marked} vertices, and the set $\notM$ of \emph{unmarked} vertices. Assume that graph $G$ serves as input to some algorithm $\alg$, and that Algorithm \alg may, at any time, turn any marked vertex $v\in M$ into an unmarked vertex (but not the other way around). We say that the input graph $G$ is given to Algorithm $\alg$ in the \emph{\MVM}, if, at the beginning of the algorithm, \alg is given the set $V(G)$ of vertices, and the initial partition $(M,\notM)$ of $V(G)$, together with all edges that are incident to the vertices of $\notM$ (including the edges between marked and unmarked vertices). If, at any time, Algorithm \alg turns a marked vertex $v\in M$, into an unmarked vertex, then it is immediately given the list of all edges that are incident to $v$ in $G$.
\end{definition}

As an example, in the routing problem described above, we initially set $M=B$ and $\notM=V(G)\setminus B$. Initially, the algorithm for this problem is given the set $V(G)$ of vertices, its partition $(M,\notM)$, and all edges that are incident to the vertices of $\notM$. Whenever the algorithm adds a new path $P$ to $\pset$, that connects a vertex $a\in A$ to a vertex $b\in B$, vertex $b$ becomes umarked, and the algorithm receives the set of all edges that are incident to $b$. This type of process will allow us to obtain running times for such routing problems roughly of the form $O(|V(G)|^{1+o(1)}\cdot (|V(G)|-|B|))$, which may be significantly lower than $\Theta(|E(G)|)$ if set $B$ contains almost all vertices of $G$, and $G$ is sufficiently dense.


==> matching-player-alg.tex <==
\subsection{Algorithm for the Matching Player -- Proof of \Cref{thm: alg for matching player}}
\label{sec: matching player alg}


As before, we call the edges of $E_G(R,L)$ \emph{special edges}, and the edges of $E_G(L,R)$ \emph{regular edges}. Notice that every vertex of $G$ may be incident to at most one special edge.

As a preprocessing step, we construct a maximum set $\qset_1$ of disjoint paths, where every path connects a distinct vertex of $A$ to a distinct vertex of $B$, and consists of a single regular edge. We do so by employing a simple greedy algorithm. We start with $\qset_1=\emptyset$. While there is a regular edge $e=(a,b)$ with $a\in A$ and $b\in B$, we add a path $Q=(e)$ to $\qset_1$, and we delete $a$ and $b$ from $A$ and $B$, respectively. Clearly, this preprocessing step can be executed in time $O(|E(G)|)$, and at the end of this step there is no regular edge in $G$ connecting a vertex of $A$ to a vertex of $B$.



Let $\hat G$ be the graph that is obtained from $G$ by replacing every edge $e$ with $d$ parallel copies. Edges that are copies of special edges in $G$ are called special edges of $\hat G$, and similarly copies of regular edges in $G$ are called regular edges of $\hat G$. 

 At the beginning of the algorithm, every special edge $e\in E(\hat G)$ is assigned a length $\ell(e)=1/d$, while every regular edge $e\in E(\hat G)$ is assigned length $0$. 
 Clearly, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq n$ holds, as there are at most $nd$ special edges in $\hat G$, each of which has length $1/d$.
 
 Over the course of the algorithm, the lengths of special edges may grow, while the lengths of regular edges remain $0$. Additionally, vertices may be deleted from sets $A$ and $B$. We will gradually construct a collection $\qset_2$ of paths in graph $\hat G$, where every path connects a distinct vertex of $A$ to a distinct vertex of $B$; the number of edges on every path is at most $d$; and the paths cause edge-congestion at most $\log n$ in $\hat G$. Initially, we set $\qset_2=\emptyset$. 
 
 
 We assume for now that we are given an oracle, that, when prompted, either returns a simple path $Q$ in the current graph $\hat G$ connecting some vertex of $A$ to some vertex of $B$, such that the length $\sum_{e\in E(Q)}\ell(e)$ of the path is at most $1$; or correctly establishes that 
such a path does not exist.

The algorithm proceeds in iterations. In every iteration, the oracle is asked to return a simple path $Q$ in the current graph $\hat G$ connecting some vertex of $A$ to some vertex of $B$, such that the length $\sum_{e\in E(Q)}\ell(e)$ of the path is at most $1$. If it successfully does so, then we add $A$ to $\qset_2$, double the length of every special edge on path $Q$, remove the endpoints of the path from sets $A$ and $B$, respectively, and continue to the next iteration. Notice that in this case, $|\qset_2|$ grows by $1$, while $\sum_{e\in E(\hat G)}\ell(e)$ increases by at most $1$.
If the oracle establishes that no such path $Q$ exists, then we terminate the algorithm.

At the end of the algorithm, we set $\qset=\qset_1\cup \qset_2$.
If $|\qset|\geq n/2-z$, then we return the collection $\qset$ of paths. It is immediate to verify that the paths in $\qset$ connect vertices of $A$ to vertices of $B$, and that their endpoints are disjoint. Moreover, since the length of every special edge in $\hat G$ is at least $\frac{1}{d}$, while the length of every path $Q\in \qset$ is at most $1$, each path in $\qset$ contains at most $d$ special edges, and at most $2d+1$ edges overall, since special and regular edges must alternate on every path. Lastly, due to the doubling of edge lengths on the paths that we add to $\qset$, every special edge of $\hat G$ may participate in at most $\log n$ paths in $\qset$, and so in total every special edge of $G$ may participate in at most $O(d\log n)$ paths in $\qset$. Moreover, if $e=(u,v)$ is a regular edge, then every path $Q\in \qset_2$ that contains $e$ must also contain either the unique special edge incident to $u$, or the unique special edge incident to $v$, while the paths in $\qset_1$ are disjoint. We conclude that the paths in $\qset$ cause congestion at most $O(d\log n)$ in $G$.

From now on we assume that, when the algorithm terminates, $|\qset|<n/2-z$ holds. Let $A'\subseteq A$, $B'\subseteq B$ be the sets of vertices that remain in $A$ and $B$, respectively at the end of the algorithm. Since the algorithm terminated, in the current graph $\hat G$, the length of the shortest path connecting a vertex of $A'$ to a vertex of $B'$ is at least $1$. Since $|\qset|<n/2-z$ and $|A'|,|B'|=n/2-|\qset|$, we get that $|A'|,|B'|\geq z$.

Recall that, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq n$ held. Over the course of the algorithm, in every iteration, $\sum_{e\in E(\hat G)}\ell(e)$ grew by at most $1$, and the number of iterations is bounded by $|A|\leq n$. Therefore,  at the end of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq 2n$ holds. 

Let $e$ be any edge of graph $G$, and let $S(e)$ be the collection of $d$ parallel edges representing $e$ in graph $\hat G$. Let $e'\in S(e)$ be the copy of $e$ with smallest current length $\ell(e')$. Notice that, if we set the lenghts of all edges in $S(e)$ to $\ell(e')$, then the length of the shortest path connecting a vertex of $A'$ to a vertex of $B'$ in $\hat G$ will remain at least $1$. Therefore, we can assume without loss of generality, that, for every edge $e\in E(G)$, the lengths of all edges in set $S(e)$ are identical; we denote this length by $\ell'(e)$.
Notice that $\sum_{e\in E(\hat G)}\ell(e)\leq 2n$ continues to hold after this transformation.

Consider now the graph $G'$ that is obtained from $G$ by
setting the length of every edge $e\in E(G)$ to $\ell'(e)$,
 unifying all vertices of $A'$ into a source vertex $s$ and all vertices of $B'$ into a destination vertex $t$. Since graph $G'$ contained $d$ parallel copies of every edge $e\in E(G)$, that all had the same length equal to $\ell'(e)$, we now have that $\sum_{e\in E(G)}\ell'(e)\leq \frac{\sum_{e\in E(\hat G)}\ell(e)}{d}\leq \frac{2n}{d}$. At the same time, since $\hat G$ did not contain an $A'$-$B'$ path of length at most $1$, we get that $\dist_{G'}(s,t)\geq 1$.
 
 Consider the following thought experiment: we choose a threshold $\rho\in (0,1)$ uniformly at random, and then define two sets $S=\set{v\in V(G')\mid \dist_{G'}(s,v)\leq \rho}$ and $T=V(G')\setminus S$ of vertices. Clearly, $s\in S$ and $t\in T$ must hold.
 By replacing $s$ with the vertices of $A'$ in $S$ and replacing $t$ with the vertices of $B'$ in $T$, we obtain a cut $(S',T')$ in graph $G$ with $|E_G(S',T')|=|E_{G'}(S,T)|$. It is easy to verify that, for every edge $e=(u,v)\in E(G')$, the probability that $u\in S$ and $v\in T$ is bounded by $\ell'(e)$. Therefore, the expected value of $|E_{G'}(S,T)|$ is bounded by $\sum_{e\in E(G)}\ell'(e)\leq \frac{2n}{d}$. By performing a BFS search from vertex $s$, we can then compute a cut $(S',T')$ in $G'$ with $|E_{G'}(S',T')|\leq \frac{2n}{d}$. Using the procedure outlined above, we can covert this cut into a cut $(S,T)$ in $G$ with $|E_G(S,T)|\leq \frac{2n}{d}$. Since $A'\subseteq S$ and $B'\subseteq T$, we are guaranteed that $|S|,|T|\geq z$. We return the cut $(S,T)$ and terminate the algorithm. In order to analyze the algorithm we need to provide an implementation of the oracle, which we do next.
 
 
 Notice that the paths in $\qset$ cause congestion at most $O(d\log n)$ in $G$, so $\sum_{Q\in \qset}|E(Q)|)\leq \tilde O(md)$. We will use this fact later.
 
 
 
 
 \paragraph{Implementing the Oracle.}
 In order to implement the oracle efficiently, we construct a new graph $H$, as follows. Initially, $H$ is obtained from $G$ by adding a source vertex $s$ that connects with an edge of length $1$ to every vertex of $A$, and a destination vertex $t$, to which every vertex of $B$ connects with an edge of length $1$.
 
 Let $q=\ceil{\log d}$.
 Additionally, for every special edge $e\in E(G)$, we replace $e$ with $q$ parallel edges $e_1,\ldots,e_q$, whose lengths are $1,2,\ldots,2^q$, respectively. The length of every regular edge is set to $0$ throughout the algorithm.
 
 Over the course of the algorithm, for every special edge $e\in E(G)$, for every index $1\leq j\leq q$, we monitor the number of copies of $e$ in graph $\hat G$, whose length is $\frac{2^j}{d}$. Once this number becomes $0$, the corresponding copy $e_j$ of $e$ is deleted from graph $H$. Additionally, whenever a vertex $a$ is deleted from set $A$, we delete edge $(s,a)$ from $H$, and whenever a vertex $b$ is deleted from set $B$, we delete edge $(b,t)$ from $H$. Therefore, the only types of updates that graph $H$ undergoes is the deletion of edges.
 
 It is now easy to verify that, throughout the algorithm, if $Q$ is an $s$-$t$ path in $H$, whose length is $\delta+2$, then the length of the corresponding path $Q'$ in $\hat G$ (where for every edge $e\in E(Q)$, we choose its cheapest copy in $\hat G$ to participate in the path) is $\frac{\delta}{d}$. Similarly, if $Q'$ is an $s$-$t$ path in graph $\hat G$, whose length is $\delta'$, then the length of the corresponding $s$-$t$ path in graph $H$ (where again for every edge $e\in E(Q')$ we use its cheapest copy available in $H$) is $\delta'\cdot d+2$.
 
 It is now enough to design an algorithm for the following problem. We are given a graph $H$, with two special vertices $s$ and $t$, and integral edge lengths, together with a parameter $d>0$. The algorithm consists of a number of iterations. In every iteration, we need to either return an $s$-$t$ path in the current graph $H$, of length at most $d+2$; or correctly establish that no such path exists. In the latter case, the algorithm terminates, while in the former case, the algorithm is given a batch of edge deletions from graph $H$, and we proceed to the next iteration.
 
 

We apply the algorithm from \Cref{thm: directed weighted ESTree} to graph $H$ and parameter $d+2$. Recall that the algorithm maintains an \EST for $H$, rooted in $s$, up to depth $d+2$. We denote the corresponding tree by $\tau$. In every iteration, we check whether vertex $t$ lies in the tree $\tau$, and if so, whether $\dist_H(s,t)\leq d+2$. If this is not the case, then we terminate the algorithm. Otherwise, we use the tree $\tau$ to compute an $s$-$t$ path $P$ of length at most $d$, in time $O(|E(P)|)$, by simply retracing the unique $s$-$t$ path in the tree $\tau$. 

It is easy to verify that the total time needed to implement the oracle is $O(|E(H)|\cdot d+\sum_{Q\in \qset}|E(Q)|)$, where $\qset$ is the set containing all paths that the algorithm ever returned. As shown already, 
$\sum_{Q\in \qset}|E(Q)|)\leq \tilde O(md)$, while it is easy to see that $|E(H)|\leq \otilde(|E(H)|)$. The total running time of the oracle is then bounded by $\otilde(md)$. 

We note that in general, the algorithm for \Cref{thm: alg for matching player} does not need to compute and maintain the graph $\hat G$ explicitly, this graph is only used for the sake of analysis. Instead, for every special edge $e\in E(G)$, for every integer $0\leq j\leq \ceil{\log d}$, we only need to keep track of the number of copies of $e$ that lie in graph $\hat G$ and have length $2^j/d$. Therefore, the total running time of the remainder of the algorithm is bounded by $O(\sum_{Q\in \qset}|E(Q)|)\leq \otilde(md)$. This includes the time required to perform a BFS in $G'$, order to compute a spase cut $(S,T)$ if needed. The total running time of the whole algorithm  for \Cref{thm: alg for matching player} is then bounded by $\otilde (md)$.





==> modified-MWU.tex <==

\newpage


\iffalse
\subsection{The \MWU Framework}

As observed by \cite{GK98, Fleischer00,AAP93}, the Multiplicative Weight Update (\MWU) framework can be adapted in order to efficiently compute approximate solutions to  various flow problems. Later, Madry \cite{madry2010faster} observed that the framework can be viewed as a reduction from a given flow problem to decremental \SSSP or \APSP, and so in order to implement the framework efficiently, it is sufficient to design an efficient algorithm for the corresponding special case of decremental \SSSP or \APSP. 
%The same approach, with slight modifications, was used in \cite{matching-old}. We further modify this approach, that we describe below.

 %Throughout this paper, we will denote by $m^*$ the smallest integral power of $2$ that is greater than $|E(G)|+2|V(G)|$.
We start by recapping a standard method for using the \MWU framework in order to solve flow problems. This method can be viewed as a slight and straightforward simplification of the algorithms of \cite{GK98, Fleischer00,AAP93}, that achieves slightly weaker approximation, but has very simple analysis. We then provide a different algorithm that modifies this framework, and is used in the remainder of this paper.


\subsubsection{The Standard \MWU Framework}

Let $G=(L,R,E)$ be the graph that serves as input to the \MBM problem, and let $m=|E|$.
Consider some maximal matching $M$ in $G$, and the residual graph $H$ of $G$ with respect to $M$. Recall that, since $M$ is a maximal matching, every $s$-$t$ path in $H$ must contain a special edge, that is, an edge connecting a vertex of $R$ to a vertex of $L$.
%We assume for simplicitly that $m=|E(H)|$ is an integral power of $2$ (otherwise we can add dummy edges that form a matching and are not connected to the rest of the graph). 
Consider the problem of computing a largest-cardinality collection  $\qset$ of edge-disjoint paths connecting $s$ to $t$ in $H$. Let $\pset^*$ denote the collection of all simple $s$-$t$ paths in $H$. Then the problem can be expressed as a linear program, where every path $P\in \pset^*$ is associated with a variable $f(P)$; we also provide a dual LP.


\begin{tabular}[t]{|l|l|}\hline &\\
	$\begin{array}{lll}
	\text{\underline{Primal}}&&\\
	\text{Max}&\sum_{P\in \pset^*} f(P)&\\
	\text{s.t.}&&\\
	%&\sum_{P\in \pset^*(a)}f(P)\leq 1&\forall a\in A'\\
	%&\sum_{P\in \pset^*(b)}f(P)\leq 1&\forall b\in B'\\
	&\sum_{\stackrel{P\in\pset^*:}{e\in E(P)}}f(P)\leq
	1&\forall e\in E(H)\\
	&f(P)\geq 0&\forall P\in \pset^*\\
	\end{array}$
	&$
	\begin{array}{lll}
	\text{\underline{Dual}}&&\\
	\text{Min}&\sum_{e\in E(H)}\ell(e)\\
	\text{s.t.}&&\\
	&\sum_{e\in E(P)}\ell(e)\geq 1&\forall P\in \pset^*\\
	&\ell(e)\geq 0&\forall e\in E(H)\\
	&&\\
	\end{array}$\\ &\\ \hline
\end{tabular}
\vspace{1cm}

In the dual LP, there is a variable $\ell(e)$ for every edge $e\in E(H)$, that we will refer as the \emph{length} of the edge. We now consider the following primal-dual algorithm, which is a simplified version of the original algorithm of \cite{GK98, Fleischer00}; this variant achieves a slightly weaker approximation, but its analysis is much simpler and the higher approximation factor does not affect our algorithm. %This is the variant of the \MWU framework that was used in \cite{matching-old}.

We start with the graph $H$, and set the length of every edge $e$ in $H$ to $\ell(e)=1/m$. We initialize $\pset=\emptyset$, and set $f(P)=0$ for all $P\in \pset^*$. Next, we perform a number of iterations. In every iteration, we compute a simple $s$-$t$ path $P$ in $H$, whose length is bounded by $1$. We then add $P$ to $\pset$, set $f(P)=1$, double the length of every edge $e\in E(P)$, and continue to the next iteration. The algorithm terminates once every $s$-$t$ path in $H$ has length greater than $1$. It is immediate to see that the final collection $\pset$ of paths is guaranteed to cause edge-congestion at most $O(\log n)$. Indeed, whenever an edge $e$ is used by a path that is being added to $\pset$, we double its length, and once the length becomes greater than $1$, the edge may no longer be used in any paths that are subsequently added to $\pset$. Since we initially set $\ell(e)=1/m$, at most $O(\log m)\leq O(\log n)$ paths in $\pset$ may use $e$. Moreover, if $\opt'$ is the cardinality of the largest collection of edge-disjoint $s$-$t$ paths in $H$, then at the end of the algorithm, $|\pset|\geq \Omega(\opt')$ holds.
This is since, at the beginning of the algorithm, the value of the dual solution is $\frac{|E(H)|}{m}\leq 1$, and the value of the primal solution is $0$. In every iteration, the value of the primal solution increases by $1$, and the value of the dual solution increases by at most $1$ (since the total length of all edges whose lengths are being doubled is at most $1$). Therefore, if we denote by $C$ the cost of the dual solution obtained at the end of the algorithm, then $C\leq 1+|\pset|\leq 2|\pset|$ holds. Since the algorithm terminates once the length of every $s$-$t$ path in $\pset^*$ is at least $1$, we obtain a valid solution to the dual LP of value $C$ at the end of the algorithm. Since the paths in $\pset$ define a valid solution to the primal LP of value $|\pset|\geq C/2\geq\opt'/2$, we get that $|\pset|\geq \opt'/2$ holds. 
 In our case, since $\opt'\geq \Delta$, we are guaranteed that $|\pset|\geq \Omega(\Delta)$. 
 
 In order to implement the above algorithm efficiently, it is sufficient to design an oracle, that, in every iteration, either computes an $s$-$t$ path $P$, whose length in the current graph $H$ is bounded by $1$, or correctly establishes that no such path exists. This problem can, in turn, be cast as a special case of decremental \SSSP: let $\hat H$ be the graph that is obtained from the original graph $H$, by replacing every edge $e\in E_H$ with $\ceil{\log n}$ parallel edges, of lengths $1/n,2/n,\ldots,1$, that we refer to as \emph{copies} of $e$. Whenever the length of edge $e$ is doubled in $H$, we delete the shortest-length copy of $e$ from $H$. We then obtain an instance of the decremental \SSSP problem on the input graph $\hat H$, and in order to design an efficient algorithm implementing the oracle, it is sufficient to design an efficient algorithm for this instance of \SSSP. We note that, however, this task appears quite challenging, since no efficient algorithms for directed \SSSP are known, and in fact there are strong conditional lower bounds suggesting that such algorithms are impossible. Even if we allow for a sufficiently large approximation factor, the best current algorithms for \SSSP have total update time that we cannot afford. \mynote{add specific bounds from \cite{SCC}}. In order to overcome this difficulty, we modify the above \MWU-based approach, keeping in mind that our goal is to reduce the problem to a variant of \SSSP that is more tractable.
 
 
 



\subsubsection{The Modified \MWU Framework}

One simple way to modify the above \MWU framework is to allow the algorithm to terminate once 
the cardinality of the largest collection of internally disjoint $s$-$t$ paths of lengths at most  $1/ {\log^{\hat c}n}$ each falls below $\frac{\Delta}{\log^{2\hat c}n}$, for some large enough constant $\hat c$. With this modification, it is now sufficient to solve the corresponding instance of \SSSP approximately (with approximation factor $O(\poly\log n)$), and moreover, we only need to be able to support approximate shortest-path queries between $s$ and $t$ as long as graph $H$ contains a large number of short $s$-$t$ paths. As we show below,  even with this relaxed stopping condition, the algorithm is still guaranteed to return a collection $\pset$ of $s$-$t$ paths that cause congestion $O(\poly\log n)$, such that
$|\pset|\geq \Omega\left(\frac{\Delta}{\poly\log n}\right )$.




We relax the above \MWU framework even more. The main intuitive motivation behind this new relaxation is to give our algorithm a greater control over which edges have their lengths doubled and when. 






At the heart of the new relaxed \MWU algorithm, is an \emph{oracle}, that we formally define next, together with the algorithm implementing the modified \MWU framework. Intuitively, the oracle, in every iteration, must either correctly establish that the current graph $H$ no longer contains a large collection of short internally disjoint $s$-$t$ paths; or it must return an $s$-$t$ path of length at most $1$ in the current graph $H$, together with some collection $\tilde E$ of special edges in $H$, whose lengths are then doubled. We place some restrictions on the collections $\tilde E$ of edges that the algorithm returns in every iteration, in order to ensure that the final collection of $s$-$t$ paths that we obtain is sufficiently large, and that the resulting paths cause a low congestion.
We now provide the formal description of our modified \MWU-based of the algorithm, and of the oracle.


Throughout the algorithm, we use a large enough constant $\hat c$, and a parameter $N=\frac{2^{12}\cdot n\log n}{\Delta}$.



Our algorithm starts by assigning, to every regular $e\in E(H)$, a length $\ell(e)=0$, and to every special edge $e'$, a length $\ell(e')= 1/N$. As the algorithm progresses, the lengths of the special edges may grow, but the lengths of all other edges remain unchanged. Whenever we talk about distances between vertices and lengths of paths, it is always with respect to the current lengths $\ell(e)$ of edges $e\in E(H)$. 
We start by defining the following property, that we refert to as a \emph{stopping condition}. If the algorithm ever discovers that this property does not hold, we will terminate it.



\begin{properties}{C}
	\item Let $\qset$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $H$, such that the paths in $\qset$ are edge-disjoint, and every path has length at most  $\frac 1 {64}$. Then $|\qset|\geq {\Delta}/{\log^{2\hat c}n}$. \label{stopping condition}
\end{properties} 


We describe the modified \MWU-based algorithm, denoted by \algmwu  in Figure \ref{alg: modified mwu}; the description excludes the implementation of the oracle. 

\program{Alg-MWU}{alg: modified mwu}{
	\begin{itemize}
		\item Start by setting $\pset=\emptyset$. For every regular edge $e\in E(H)$, set $\ell(e)=0$, and for every special edge $e'\in E(H)$, set $\ell(e')={1}/{N}$. Then iterate.
		\item In every iteration:
		
		\begin{itemize}
			\item either compute a simple $s$-$t$ path $P$  of length at most $1$ in the current graph $H$, and some collection $\tilde E_i$ of special edges in $H$; add $P$ to $\pset$; double the length of every edge in $\tilde E_i$;
			\item or correctly establish that Condition \ref{stopping condition} no longer holds and halt.
		\end{itemize}
	\end{itemize}
}



We are now ready to descibe the oracle. The oracle's execution consists of at most $\Delta$ iterations. In every iteration $i$, the oracle must either (i) correctly establish that Condition \ref{stopping condition} no longer holds in $H$; or (ii) return an $s$-$t$ path $P_i$ of length at most $1$ in the current graph $H$, together with a collection $\tilde E_i\subseteq E(H)$ of special edges. In the former case, the algorithm is terminated. In the latter case, we denote $C_i=\sum_{e\in \hat E_i}\ell(e)$, double the length of every edge in $\tilde E_i$, and continue to the next iteration.
We require that the oracle satisfies the following two conditions:

\begin{properties}{P}
	\item For all $i>0$, $\sum_{i'\leq i}C_{i'}\leq i \cdot \log^{\hat c}n$; and \label{oracle-prop: small length growth}
	\item For every special edge $e\in E_{H}(R,L)$, if $\tau$ is a consecutive collection of iterations during which the length of $e$ was never doubled, then the total number of paths that were added to $\pset$ in the iterations of $\tau$, that contained $e$, is bounded by $\log^{\hat c}n$;  \label{oracle-prop: edge congestion}
%	\item For every special edge $e\in E_{H}(R,L)$, if $e\in \hat E_i$ and $e\in \hat E_j$ for iterations $i<j$, then $e$ must belong to at least one of the paths $P_{i+1},\ldots,P_j$.\label{oracle: dont grow lengths unnecesarily}
\end{properties}

Lastly, the oracle may return ``FAIL'' at any time and terminate. The probability that the oracle ever returns ``FAIL'' must be bounded by $1/\poly(n)$. The main technical contribution of our paper is the implementation of the oracle, that is summarized in the following theorem.

\begin{theorem}\label{thm: oracle}
	There is an algorithm that implements the oracle as described above, whose running time is $O(n^{2+o(1)})$.
\end{theorem}

We note that the running time of the oracle includes both the time required to maintain its data structures (total update time), and time required to compute and output the paths $P_i$ and sets $\tilde E_i$ of edges.

We prove \Cref{thm: oracle} in the remainder of the paper, after we complete the proof of \Cref{thm: single phase} using it. Assume that we are given  a maximal matching $M$ in the input bipartite graph $G=(L,R,E)$, let $\Delta=\opt-|M|$, and let $H$ be the residual graph of $G$ with respect to $M$. We execute Algorithm \algmwu, described in  in Figure \ref{alg: modified mwu}, using the algorithm from \Cref{thm: oracle} in order to implement the oracle.
It is easy to verify that the total running time of the algorithm is dominated by the running time of the oracle, which is bounded by $O(n^{2+o(1)})$. If the oracle ever returns ``FAIL'', then we terminate our algorithm and return ``FAIL'' as well. From the definition of the oracle, this may happen with probability at most $1/\poly(n)$. Let $\pset$ be the collection of paths in graph $H$ that is obtained at the end of the algorithm. It is now enough to prove the following claim.





\begin{claim}\label{claim: appox MWU}
	Let $\pset$ be the set of paths obtained at the end of Algorithm \algmwu. Then $|\pset|\geq \Omega\left(\frac{\Delta}{\poly\log n}\right )$, and every edge of $H$ belongs to at most $O(\poly\log n)$ paths of $\pset$.
\end{claim}

\begin{proof}
	We start by proving that every special edge of $H$ belongs to at most $O(\poly\log n)$ paths of $\pset$. Consider any such special edge $e$. Recall that, at the beginning of the algorithm, we set $\ell(e)=1/N$. Let $i_1,i_2,\ldots,i_r$ denote the indices of the iterations when $\ell(e)$ was doubled. Notice that, once $\ell(e)$ grows above $1$, it may no longer be used by any paths that are added to $\pset$, so $r\leq O(\log N)\leq O(\log n)$ must hold.  Property \ref{oracle-prop: edge congestion} further ensures that, for all $1\leq j<r$, the number of paths that were added to $\pset$ between iteration $i_j$ and iteration $i_{j+1}$, that contained $e$, is bounded by $O(\poly\log n)$. Therefore, altogether $e$ may belong to at most $O(\poly\log n)$ paths in $\pset$. Consider now some regular edge $e=(u,v)$. Recall that, since matching $M$ is maximal, every $s$-$t$ path in $H$ must contain at least one special edge. It is then easy to verify that, if an $s$-$t$ path $P$ in $H$ contains the edge $e$, then it must contain either the unique special edge that is incident to $u$ (if it exists), or the unique special edge that is incident to $v$ (if it exists). Since every special edge appears in at most $O(\poly\log n)$ paths in $\pset$, so is $e$. We conclude that the paths in $\pset$ cause edge-congestion $O(\poly\log n)$ in $H$.
	
	We now turn to prove that $|\pset|\geq \Omega\left(\frac{\Delta}{\poly\log n}\right )$. %This proof slightly generalizes a similar analysis of the \MWU-based algorith of \cite{matching-old}.
	%
	%Let $H_1$ be the graph $H$ that is obtained at the end of the algorithm (where we assume that the definition of the graph includes edge lengths), and 
	Let $q$ be the total number of iterations in the algorithm, so $|\pset|=q$ holds. Recall that, at the beginning of the algorithm, $\sum_{e\in E(H)}\ell(e)\leq \frac{n}{N}=\frac{\Delta}{2^{12}\log n}$ held, since $N=
	\frac{2^{12}\cdot n\log n}{\Delta}$.
	In every iteration $i$, we double the lengths of all edges in set $\tilde E_i$, and so $\sum_{e\in E(H)}\ell(e)$ grows by (additive) $C_i$. From Property \ref{oracle-prop: small length growth} of the oracle, we are then guaranteed that, at the end of the algorithm, $\sum_{e\in E(H)}\ell(e)\leq \frac{\Delta}{2^{12}\log n}+\sum_{i=1}^qC_i\leq \frac{\Delta}{2^{12}\log n}+q\cdot \log^{\hat c}n\leq \frac{\Delta}{2^{12}\log n}+ |\pset|\cdot \log^{\hat c}n$. 
	
	

	
	Consider now the following thought experiment. We start with the set $\pset$ of paths, and the edge lengths that were obtained at the end of Algorithm \algmwu. Let $H_1$ denote the resulting graph (which is identical to $H$ but may have different edge lengths).
	
	Next, we will construct another set $\pset'$ of paths in $H_1$, as follows. Initially, we let $\pset'=\emptyset$, and we let $H_2$ be a copy of the graph $H_1$. Then we iterate, as long as there is an $s$-$t$ path in $H_2$, whose length is at most $\frac{1}{512\log n}$. In every iteration, we select an arbitrary simple $s$-$t$ path $P$ in $H_2$ of length at most  $\frac{1}{512\log n}$, add it to $\pset'$, and then double the length of every edge $e\in E(P)$ in graph $H_2$. This algorithm terminates when every $s$-$t$ path in $H_2$ has length at least $\frac{1}{512\log n}$. We denote by $H_3$ the graph $H_2$ that is obtained at the end of this algorithm (which is identical to $H$ and to $H_2$, except for the edge lengths).
In the following observation, we show that $|\pset|+|\pset'|\geq \frac{\Delta}{2048\log^{\hat c+1}n}$.

\begin{observation}\label{obs: many paths}
	 $|\pset|+|\pset'|\geq \frac{\Delta}{2048\log^{\hat c+1}n}$.
	\end{observation}
\begin{proof}
	Let $C=\sum_{e\in E(H_1)}\ell(e)$, and let $C'=\sum_{e\in E(H_3)}\ell(e)-C$. As observed already, $C\leq \frac{\Delta}{2^{12}\log n}+ |\pset|\cdot \log^{\hat c}n$. During our thought experiment, in every iteration of the algorithm, we added a single path $P$ to $\pset'$, and increased $\sum_{e\in E(H_2)}\ell(e)$ by at most (additive) $\frac{1}{512\log n}$. Therefore, the total increase in $\sum_{e\in E(H_2)}\ell(e)$ during the thought experiment is $C'\leq \frac{|\pset'|}{512\log n}$. Altogether, we get that:
	
	\[\sum_{e\in E(H_3)}\ell(e)=C+C'\leq \frac{\Delta}{2^{12}\log n}+ |\pset|\cdot \log^{\hat c}n+|\pset'|\leq \frac{\Delta}{2^{12}\log n}+(|\pset|+|\pset'|)\cdot \log^{\hat c}n.\]
	
	
Since, at the end of the algorithm, every $s$-$t$ path has length at least $\frac{1}{512\log n}$, by multiplying the length of every edge in $H_3$ by $512\log n$, we obtain a feasible solution to the dual LP (recall that graph $H_3$ is identical to $H$, except for the edge lengths). Therefore, there is a solution to the dual LP on graph $H$, whose value is $C^*=(C+C')\cdot 512\log n\leq (|\pset|+|\pset'|)\cdot 1024\log^{\hat c+1}n+\frac{\Delta}{4}$. Since the value of the optimal solution to the primal LP is at least $\Delta$, so is the value of the optimal solution to the dual LP, and so $C^*\geq \Delta$. Overall, we get that $|\pset|+\pset'|\geq \frac{\Delta}{2048\log^{\hat c+1}n}$.
\end{proof}


Lastly, we show that $|\pset|\geq \frac{\Delta}{4096\log^{\hat c+1}n}$ must hold. Indeed, assume otherwise. Then $|\pset'|\geq \frac{\Delta}{4096\log^{\hat c+1}n}$ must hold. We prove that this is impossible, by showing that, when Algorithm \algmwu was terminated, Condition \ref{stopping condition} still held, leading to a contradiction. The following observation will then finish the proof of  \Cref{claim: appox MWU}.


\begin{observation}\label{obs: few in P'}
	If $|\pset'|\geq \frac{\Delta}{4096\log^{\hat c+1}n}$, then, at the time when \algmwu terminated, Condition \ref{stopping condition} still held.
\end{observation}
\begin{proof}
Recall that each $P\in \pset'$ had length at most $\frac{1}{512\log n}$ in graph $H_2$, when it was added to $\pset'$. Since edge lengths only grow overitme, every path $P\in \pset'$ has length at most $\frac{1}{512\log n}$ in $H_1$. Consider a new graph $H^*$, that is obtained by taking the union of all edges and vertices that appear on the paths in $\pset'$. The length of every edge in $H^*$ is set to be its length in $H_1$. Denote $|\pset'|=k$. 
Since every path in $\pset'$ has length at most $\frac{1}{512\log n}$ in $H_1$, $\sum_{e\in E(H^*)}\ell(e)\leq\frac{k}{512\log n}$. 

It is easy to verify that that the paths in $\pset'$ cause edge-congestion at most $4\log n$ in $H_3$ and hence in $H^*$. 
The reason is that, for every edge $e\in E(H_2)$, its initial length is $\frac{1}{N}\geq \frac{1}{2^{12}n\log n}$. Whenever a path $P$ containing edge $e$ is added to $\pset'$, the length of $e$ is doubled; and once the lenght of $e$ reaches $1$ it can no longer be used in any paths that are subsequently added to $\pset'$. Therefore, the paths in $\pset'$ cause edge-congestion at most $4\log n$ in $H^*$.

Due to the special structure of graph $H$, the paths in $\pset'$ also cause vertex-congestion at most $4\log n$ in $H^*$. From the integrality of flow, there is a collection $\qset$ of at least $\frac{k}{4\log n}$ internally vertex-disjoint $s$-$t$ paths in $H^*$. We say that a path $Q\in \qset$ is \emph{long}, if its length is greater than $\frac{1}{64}$. Since $\sum_{e\in E(H^*)}\ell(e)\leq \frac{k}{512\log n}$, the number of long paths in $\qset$ is bounded by $\frac{k}{8\log n}$, and the remaining paths are short. But then we obtain a collection of at least $\frac{k}{8\log n}\geq \frac{\Delta}{2^{15}\log^{\hat c+2}n}\geq \frac{\Delta}{\log^{2\hat c}n}$ edge-disjoint $s$-$t$ paths of length at most $\frac{1}{64}$ each in $H_2$, so when Algorithm \algmwu terminated, Condition \ref{stopping condition} still held.
\end{proof}
\end{proof}










\subsection*{Adjustments to the Edge Lengths.}
As long as Condition \ref{stopping condition} continues to hold, graph $H$ contains a collection $\qset$ of at least $\frac{\Delta}{\log^{2\hat c}(n)}$ edge-disjoint $s$-$t$ paths of length at most $\frac 1 {256}$ each. %Recall that, due to the special structure of graph $H$, these paths are also internall vertex-disjoint. 
Let $\qset'\subseteq \qset$ be the collection of all paths that contain at most $\frac{2n\log^{2\hat c}n}{\Delta}$ special edges, and let $\qset''$ be the collection of all remaining paths. Since the paths in $\qset''$ are edge-disjoint, and since the number of special edges in $H$ is at most $n$, while every $s$-$t$ path must contain at least one special edge, we get that $|\qset''|\leq \frac{\Delta}{2\log^{2\hat c}n}$ must hold, and so $|\qset'|\geq \frac{\Delta}{2\log^{2\hat c}n}$. Consider the following condition that we will use to replace Condition \ref{stopping condition}.





\begin{properties}[1]{C}
	\item Let $\qset'$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $H$, such that the paths in $\qset'$ are edge-disjoint, every path has length at most  $\frac 1 {256}$  in the current graph, and every path contains at most  $\frac{2n\log^{2\hat c}n}{\Delta}$ special edges. Then $|\qset'|\geq \frac{\Delta}{2\log^{2\hat c}n}$ holds. \label{stopping condition2}
\end{properties} 


From the above discussion, if Condition \ref{stopping condition2} is violated in the current graph $H$, then so is condition \ref{stopping condition}. Therefore, it is sufficient for us to be able to carry out Procedure \algmwu as long as Condition \ref{stopping condition2} holds; in other words, we can replace \ref{stopping condition} with \ref{stopping condition2} in the algorithm.

Consider now the collection $\qset'$ of paths from Condition  \ref{stopping condition2}. Each such path has length at most $\frac 1 {256}$ and contains at most $\frac{2n\log^{2\hat c}n}{\Delta}$ special edges. Therefore, if we increase the length of every special edge in $H$ by adding  $\frac{\Delta}{2^{12}\cdot n\log^{2\hat c}n}$ to it, then the length of every path in $\qset'$ will still remain at most $\frac 1 {128}$. Moreover, any path $P$ whose modified length is at most $1$ has original length at most $1$. 
After this transformation, the length of every special edge in $H$ is at least $\frac{\Delta}{2^{12}\cdot n\log^{2\hat c}n}$ and at most $1$. 

Next, we multiply the length of every edge by $\frac{2^{12}\cdot n\log^{2\hat c}n}{\Delta}$, and round it up to the next integral power of $2$.
Notice that, if $\ell'(e)$ is the new length of some edge $e\in E(H)$, and $\ell(e)$ is its original lengths, before any transformations, then $\ell'(e)\geq \frac{2^{12}\cdot n\log^{2\hat c}n}{\Delta}\cdot \ell(e)$.

 Let $H^*$ denote the graph $H$ with these new edge lengths. We now get that the length of every edge in $H^*$ is an integral power of $2$ between $1$ and $\frac{2^{13}n\log^{2\hat c}n}{\Delta}$. If $P$ is a path in $H^*$ of length at most $\frac{2^{12}\cdot n\log^{2\hat c}m}{\Delta}$, then the length of $P$ in $H$ is at most $1$. Moreover, if Condition  \ref{stopping condition2} holds, then the length of every path in the corresponding set $\qset'$ in graph $H^*$ is at most $\frac{64n\log^{2\hat c}m}{\Delta}$.
For convenience, we denote $\Lambda=\frac{64n\log^{2\hat c}m}{\Delta}$.



The problem that the oracle needs to solve can now be abstracted as a modification of the directed \SSSP problem on the resulting dynamic graph $H^*$. We call this problem Modified \SSSP and define it next.

\fi

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%Leftovers from here on
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
\iffalse


We can relax the requirements from the oracle even more, and this relaxation will be crucial in reducing the running time of our algorithm. Specifically, can allow the algorithm to terminate once the following condition is violated:

\begin{properties}{C}
	\item Let $\qset$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $H$, such that the paths in $\qset$ are internally vertex-disjoint and every path has length at most  $\frac 1 8$. Then $|\qset|\geq \frac{\Delta}{256\log^2m}$. \label{stopping condition}
	\end{properties} 

The resulting algorithm, denoted by \algmwu (excluding the implementation of the oracle), appears in Figure \ref{alg: mwu}.



\program{Alg-MWU}{alg: modified mwu}{
\begin{itemize}
	\item Start by setting $\pset=\emptyset$ and for each edge $e\in E(H)$, $\ell(e)=1/m$, then interate.
	\item In every iteration:
	
	\begin{itemize}
		\item either compute a simple $s$-$t$ path $P\in \pset$ of length at most $1$; add $P$ to $\pset$; double the length of every edge on $P$;
		\item or correctly establish that Condition \ref{stopping condition} no longer holds and halt.
	\end{itemize}
\end{itemize}
}

In the following claim we show that the algorithm is indeed guaranteed to compute a large enough collection of $s$-$t$ paths.

\begin{claim}\label{claim: appox MWU}
Let $\pset$ be the set of paths obtained at the end of Algorithm \algmwu. Then $|\pset|\geq \frac{\Delta}{128\log m}$, and every edge of $H$ belongs to at most $O(\log m)$ paths of $\pset$.
\end{claim}

\begin{proof}
	It is immediate to verify that the paths in $\pset$ cause congestion $O(\log m)$, since we set the length of every edge $e$ to be $1/m$ initially, and then double it every time a path is added to $\pset$ contains $e$. Since all paths in $\pset$ have length at most $1$, once $\ell(e)>1$ holds, the edge may no longer be used by paths that are newly added to $\pset$. Therefore, the length of $e$ may be doubled at most $O(\log m)$ times, and at most $O(\log m)$ paths in $\pset$ may use $e$.
	
	Consider the following thought experiment. We start with the set $\pset$ of paths, and the edge lengths that were obtained at the end of Algorithm \algmwu. Let $H$ denote the resulting graph (which is identical to $H$ but may have different edge lengths).
	
	Next, we will construct another set $\pset'$, as follows. Initially, we let $\pset'=\emptyset$, and we let $H'$ be a copy of the graph $H$. Then we iterate, as long as there is an $s$-$t$ path in $H'$ whose length is at most $\frac{1}{32\log m}$. In every iteration, we select an arbitrary simple $s$-$t$ path $P$ in $H'$ of length at most  $\frac{1}{32\log m}$, add it to $\pset'$, and then double the length of every edge $e\in E(P)$ in graph $H'$. This algorithm terminates when every $s$-$t$ path in $H'$ has length at least $\frac{1}{32\log m}$. 
	
	We first observe that, at the end of the above algorithm, $|\pset|+|\pset'|\geq \frac{\Delta}{64\log m}$ must hold. Indeed, in every iteration of the algorithm, we added one path $P$ to $\pset\cup \pset'$, thereby increasing $|\pset|+|\pset'|$ by $1$. At the same time, we doubled the lengths of all edges in $P$, thereby increasing the value of the dual solution by at most $1$ (since the total length of all edges on $P$ before the doubling step was t most $1$). 
	
	When the algorithm starts, the value of the dual solution is $1$, and $|\pset|+|\pset'|=0$. After that, in every iteration $|\pset|+|\pset'|$ grows by $1$, while the value of the dual solution grows by at most $1$. Therefore, if we denote by $C$ the value of the dual solution at the end of the algorithm, then $C\leq |\pset|+|\pset'|+1$.
	
	Since at the end of the algorithm every $s$-$t$ path in $H'$ has length at least $\frac{1}{32\log m}$, by multiplying the lengths of the edges by $32\log m$, we obtain a feasible dual solution, whose value is $C\cdot 32\log m\leq (64\log m)(|\pset|+|\pset'|)$. Therefore, $|\pset|+|\pset'|\geq \frac{\opt'}{64\log m}\geq\frac{\Delta}{64\log m}$, where $\opt'$ is the largest number of internally disjoint $s$-$t$ paths in $H$.
	
	
	Assume now for contradiction that $|\pset|<\frac{\Delta}{128\log m}$, so that $|\pset'|\geq \frac{\Delta}{128\log m}$ holds. We will show that Condition \ref{stopping condition} must have held when Algorithm \algmwu was terminated, reaching a contradiction.
	
%	If we denote by $C$ the value of the dual solution at the end of this algorithm, then
%	We call the algorithm during which the collection $\pset$ of paths was constructed \emph{stage 1}, and we denote the graph $H$ obtained at the end of stage 1 by $H'$ (we assume that this includes edge lengths in $H'$). We then perform the second stage of the algorithm, where we continue adding paths of length at most $1$ to $\pset$ as before (while doubling the length of every edge on such a path), until the length of the shortest path in the resulting graph becomes at least $1/(32\log n)$. We denote by $\pset'$ the collection of paths that were added to $\pset$ during the first phase of the algorithm, and by $\pset''$ the collection of paths added during the second phase. Recall that we are guaranteed that $|\pset'|+|\pset''|\geq \frac{\Delta}{32\log n}$. Assume for contradiction that $|\pset|<\frac{\Delta}{64\log n}$. Then $|\pset''|>\frac{\Delta}{64\log n}$.
	
	Recall that each such path in $\pset'$ has length at most $\frac 1{32\log m}$ in graph $H'$. Consider a new graph $H^*$, that is obtained by taking the union of all edges and vertices that appear on the paths in $\pset'$. The length of every edge in $H^*$ is set to be its length in $H'$. Denote $|\pset'|=k$. 
	Since every path in $\pset'$ has length at most $\frac 1 {32\log m}$ in $H'$, $\sum_{e\in E(H^*)}\ell(e)\leq \frac{k}{32\log m}$. 
	
	Recall that the paths in $\pset'$ cause edge-congestion at most $\log m$ in $H''$ and hence in $H^*$. Due to the special structure of graph $H$, they also cause vertex-congestion at most $\log m$. From the integrality of flow, there is a collection $\qset$ of at least $\frac{k}{\log m}$ internally vertex-disjoint $s$-$t$ paths in $H^*$. We say that a path $Q\in \qset$ is \emph{long}, if its length is greater than $\frac 1 8$. Since $\sum_{e\in E(H^*)}\ell(e)\leq \frac{k}{32\log m}$, the number of long paths in $\qset$ is bounded by $\frac{k}{4\log m}$, and the remaining paths are short. But then we obtain a collection of at least $\frac{k}{2\log m}\geq \frac{\Delta}{256\log^2m}$ edge-disjoint $s$-$t$ paths of length at most $\frac 1 8$ each in $H'$, so when Algorithm \algmwu terminated, Condition \ref{stopping condition} still held, a contradiction.
\end{proof}


In order to complete the proof of \Cref{thm: one iteration main}, it is now sufficient to provide an efficient implementation of the oracle, that, in every iteration, either produces a simple $s$-$t$ path of length at most $1$ in the current graph $H$, or correctly establishes that Condition \ref{stopping condition} is violated. In order to implement the oracle, we will reduce it to a special case of the decremental \SSSP problem, called restricted \SSSP, and then provide an algorithm for that problem.  In order to do so it will be convenient for us to slightly adjust the legnths of the edges in graph $H$.

%It is easy to verify that, once this condition is met, $\pset$ must contain at least $\Delta/8$ paths. In order to see this, let us continue the same algorithm as before, and terminate it once $\dist(s,t)\geq 1/2$ holds. Let $\pset'$ be the set of paths that were added during the second part of the algorithm. On the one hand, we are guaranteed that $|\pset|+|\pset'|\ge \Delta/4$. Therefore, if $|\pset|<\Delta/8$, then $|\pset'|\geq \Delta/8$ must hold. On the other hand, the paths in $\pset'$ cause edge-congestion at most $\log n$, and so there must be a collection of at least $|\pset'|/\log n\geq \Delta/(8\log n)$ edge-disjont $s$-$t$ paths in graph $H'$, that is obtained by taking the union of the paths in $\pset'$. 
% (this is because we could continue the algorithm until $\dist(s,t)\geq 1/2$ holds, and we are guaranteed to only have added at most $\Delta/8$ paths during this second part of the algorithm. Since eventuall $|\pset|\geq \Delta/4$ must hold, during the first part of the algorithm we must have added at least $\Delta/8$ paths to $\pset$.


\paragraph{Adjustments to the Edge Lengths.}
As long as Condition \ref{stopping condition} continues to hold, graph $H$ contains a collection $\qset$ of at least $\frac{\Delta}{256\log^2m}$ internally disjoint $s$-$t$ paths of length at most $\frac 1 8$ each. Let $\qset'\subseteq \qset$ be the collection of all paths that contain at most $\frac{512n\log^2m}{\Delta}$ edges, and let $\qset''$ be the collection of all remaining paths. Since the paths in $\qset''$ are internally vertex disjoint, $|\qset''|\leq \frac{\Delta}{512\log^2m}$ must hold, and so $|\qset'|\geq \frac{\Delta}{512\log^2m}$. Consider the following condition that we will use to replace Condition \ref{stopping condition}.





\begin{properties}[1]{C}
	\item Let $\qset'$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $H$, such that the paths in $\qset'$ are internally vertex-disjoint, every path has length at most  $\frac 1 8$  in the current graph, and every path contains at most  $\frac{512n\log^2m}{\Delta}$ edges. Then $|\qset'|\geq \frac{\Delta}{512\log^2m}$ holds. \label{stopping condition2}
\end{properties} 


From the above discussion, if Condition \ref{stopping condition2} is violated in the current graph $H$, then so is condition \ref{stopping condition}. Therefore, it is sufficient for us to be able to carry out Procedure \algmwu as long as Condition \ref{stopping condition2} holds; in other words, we can replace \ref{stopping condition} with \ref{stopping condition2} in the algorithm.

Consider now the collection $\qset'$ of paths from Condition  \ref{stopping condition2}. Each such path has length at most $\frac 1 8$ and contains at most $\frac{512n\log^2m}{\Delta}$ edges. Therefore, if we increase the length of every edge in $H$ by adding  $\frac{\Delta}{2^{12}\cdot n\log^2m}$ to it, then the length of every path in $\qset'$ will still remain at most $\frac 1 4$. Moreover, any path $P$ whose modified length is at most $1$ has original length at most $1$. 
After this transformation, the length of every edge in $H$ is at least $\frac{\Delta}{2^{12}\cdot n\log^2m}$ and at most $1$. 

Next, we multiply the length of every edge by $\frac{2^{12}\cdot n\log^2m}{\Delta}$, and round it up to the next integral power of $2$. Let $H^*$ denote the graph $H$ with these new edge lengths. We now get that the length of every edge in $H^*$ is an integral power of $2$ between $1$ and $\frac{2^{13}n\log^2m}{\Delta}$. If $P$ is a path in $H^*$ of length at most $\frac{2^{12}\cdot n\log^2m}{\Delta}$, then the length of $P$ in $H$ is at most $1$. Moreover, if Condition  \ref{stopping condition2} holds, then the length of every path in the corresponding set $\qset'$ in graph $H^*$ is at most $\frac{2^{11}n\log^2m}{\Delta}$.
For convenience, we denote $\Lambda=\frac{2^{11}n\log^2m}{\Delta}$.


%For convenience, we will also round the length of every edge up to the next integral po of $2^i$ (or $2^{-i}$).

In order to implement the oracle,
it is now sufficient to solve the following instance of the \SSSP problem: we are given a graph $\hat H$ with $n$ vertices and at most $m\log m$ edges, and a parameter $\Delta$. Let $\Lambda=\frac{2^{11}n\log^2m}{\Delta}$. For every edge $e\in E(\hat H)$, we are given a length $\ell(e)$, that is an integral power of $2$ between $1$ and $2\Lambda$. 
The algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration, we need to compute a simple $s$-$t$ path in the current graph $\hat H$ of length at most $2\Lambda$, or to correctly certify that the largest-cardinality collection $\qset$ of $s$-$t$ paths in the current graph $\hat H$, such that the paths in $\qset$ are internally vertex-disjoint, every path has length at most  $\Lambda$, and every path contains at most  $\frac{512n\log^2m}{\Delta}$ edges, is less than $\frac{\Delta}{512\log^2m}$.
In the latter case, the algorithm terminates. In the former case, if $P$ is the $s$-$t$ path that the algorithm returned, we assume that for every edge $e\in E(P)$, edge $e$ is the shortest among its parallel edges in $\hat H$. The edges of $P$ are then deleted from $\hat H$ and we proceed to the next iteration.

%As the last step in this transformation, it will be convenient for us to scale all edge lengths up, so that they become integral powers of $2$ between $1$ and $\frac{32n\log n}{\Delta}$. (Each edge length needs to be scaled up by $z$-- smallest integral power of $2$ that is greater than $\frac{16n\log n}{\Delta}$).
%The paths that the algorithm computes must have lengths at most $\frac{32n\log n}{\Delta}$, and the algorithm may terminate once the following condition is violated:








To summarize, we reduced \Cref{thm: one iteration main} (and generally the \MBM problem) to the \SSSP problem in directed graphs. While the current algorithms for \SSSP in directed graphs are not so efficient, we obtain a special case of the problem with some nice additional properties that we can exploit, that include:

\begin{itemize}
	\item a special structure of the input graph $\hat H\setminus\set{s,t}$ (for every vertex, either its in-degree or its out-degree is at most $1$, if we ignore parallel edges);
	\item Throughout the algorithm, there are many short $s$-$t$ paths, and once this is not the case, we can halt;
	
	\item We only need to respond to \shortpath query between a specific pair of vertices $s$ and $t$ that is known in advance. Moreover, the only edges that are deleted from the graph are edges that appear on the paths that the algorithm returns. 
	
	\item The number of times we are required in order to respond to \shortpath queries is not too large, and we only need to bound the total time required to both maintain the data structures and respond to queries. This allows us to use a lazy approach, where, e.g. we are allowed to abort a response to a query if, as we attempt to respond to it, we discover that the data structure needs to be updated (as long as the total running time of the algorithm is suitably bounded.)
	
	\item Generally in the \SSSP problem we require that the time required to return a path in response to a \shortpath query (called \emph{query time}) is proportional to the number of the edges on the path. In our case we could afford a higher query time.
	
	\item While much work on \SSSP focuses on factor $(1-\eps)$ approximation, we can sustain a much higher approximation factor (the reduction we presented requires approximation factor $2$, but it can be easily adjusted to allow higher approximation factors, that may be as large as polynomial in $n$).
\end{itemize}

The algorithm that we present does not exploit some of the advantages listed above; this may suggest avenues for obtaining faster algorithms for \MBM via this general approach.


We abstract the special case of \SSSP problem that we need to solve, that we call \emph{restricted} \SSSP, in the following subsection.
\fi


==> modified-SSSP.tex <==

\subsection{The Modified \SSSP Problem}
\label{subsec: restricted SSSP}

The input to the Modified \SSSP problem is a bipartite $n$-vertex graph $G=(L,R,E)$, with a maximal matching $M$ in $G$, a parameter $m^*\geq |E|$, and another parameter $0<\Delta\leq n-|M|$. We let $H$ be the residual graph of $G$ with respect to $M$. As before, the edges of $E_G(R,L)$ are called \emph{special} edges, and the remaining edges of $H$ are called \emph{regular} edges. Initially, the length of every edge $e\in E(H)$ is set to $1$.

We denote $\Lambda=\frac{64n\log^{2\hat c}m}{\Delta}$, and we will use of the following as a stopping condition.





\begin{properties}[2]{C}
	\item Let $\qset$ be the largest-cardinality collection of $s$-$t$ paths in the current graph $H$, such that the paths in $\qset$ are edge-disjoint, and every path has length at most  $\Lambda$  in the current graph. Then ${|\qset|\geq \frac{\Delta}{2\log^{2\hat c}m}}$ holds. \label{stopping conditionfinal}
\end{properties} 

The algorithm for the Modified \SSSP problem consists of at most $\Delta$ iterations. In every iteration $i$, the algorithm for the Modified \SSSP problem must either:

\begin{itemize}
	\item Correctly establish that Condition \ref{stopping conditionfinal} does not hold in the current graph $H$; or
	\item Return an $s$-$t$ path $P_i$ whose length in the current graph $H$ is at most $64\Delta$, together with a collection $\hat E_i$ of special edges of $H$.
\end{itemize}

In the former case, the algorithm is terminated, while in the latter case, we denote by $\Lambda_i$ the total length of all edges in set $\hat E_i$, and we double the lengths of all edges in $\hat E_i$. We also require that the following two properties hold:



\begin{properties}{P'}
	\item For all $i>0$, $\sum_{i'\leq i}\Lambda_{i'}\leq i \cdot \frac{2^{12}\cdot n\log^{3\hat c}m^*}{\Delta}$; and \label{SSSP-prop: small length growth}
	\item For every special edge $e\in E_{H}(R,L)$, if $\tau$ is a consecutive collection of iterations during which the length of $e$ was never doubled, then the total number of paths that were added to $\pset$ in the iterations in $\tau$, that contained $e$, is bounded by $\log^{\hat c}m^*$. \label{SSSP-prop: edge congestion}
\end{properties}

The algorithm may halt and return ``FAIL'' at any time, but the probability that it ever returns ``FAIL'' must be bounded by $1/\poly(n)$. This completes the definition of the Modified \SSSP problem.


From our discussion, it is easy to verify that an algorithm for the Modified \SSSP problem immediately provides an algorithm for implementing the oracle. We simply start with the graph $H$, modify its edge lengths as defined above, and then apply the algorithm for Modified \SSSP to it. For convenience, denote the graph $H$ with the modified edge lengths by $H'$. Whenever the algorithm for the Modified \SSSP problem returns a path of length at most $64\Lambda$ in  $H'$, we are guaranteed that this path has length at most $1$ in $H$. We also double the lengths of the edges in the sets $\hat E_i$ that the algorithm returns in graph $H$. Property \ref{oracle-prop: edge congestion} immediately follows from Property \ref{SSSP-prop: edge congestion}, while Property \ref{oracle-prop: small length growth} follows from Property \ref{SSSP-prop: small length growth} and the fact that for every special edge $e\in E(H)$, it length in $H'$ is at least 




\begin{properties}{P}
	\item For all $i>0$, $\sum_{i'\leq i}\Lambda_{i'}\leq i \cdot \log^{\hat c}m^*$; and \label{oracle-prop: small length growth}
	\item For every special edge $e\in E_{H'}(R,L)$, if $\tau$ is a consecutive collection of iterations during which the length of $e$ was never doubled, then the total number of paths that were added to $\pset$ in the iterations in $\tau$, that contained $e$, is bounded by $\log^{\hat c}m^*$. \label{oracle-prop: edge congestion}
\end{properties} 




@@@


\newpage




\paragraph{Well-Structured Graphs.}
Throughout, we will work with graphs that have a special structure. Let $G$ be the given instance of the Bipartite Matching problem. All graphs that we consider are subgraphs of the residual graph of $G$ with respect to some matching $M$ (except that we may add some parallel edges). Such graph have special structural properties that we summarize in the following definition.

\begin{definition}[Well-Structured Graph]\label{def: well-structured}
Let $H$ be a directed graph, and let $m$ be a parameter. We say that $H$ is a \emph{well-structured} graph of size $m$, if $|E(H)|\leq m\log m$, and  $H$ has two special vertices $s$ and $t$. Additionally, if we denote $H'=H\setminus\set{s,t}$, then the following hold.

\begin{itemize}	
	\item $V(H')$ is partitioned into two subsets $L$ and $R$, and every edge of $H'$ has one endpoint in $L$ and another in $R$. Edges directed from vertices of $R$ to vertices of $L$ are called \emph{special edges} (they correspond to the edges of the current matching $M$), and the remaining edges of $H'$ are called \emph{regular edges}.
	
	\item Every vertex of $L\cup R$ is incident to at most $\log m$ special edges in $H'$ and all of them are parallel to each other, so the out-degree of every vertex in $R$ (ignoring parallel edges) is at most $1$, and the in-degree of every vertex in $L$ (also ignoring parallel edges) is at most $1$ in $H'$.
	
	\item In graph $H$, vertex $s$ has no incoming edges, and all edges leaving $s$ connect it to vertices of $L$.
	
	\item Similarly, in graph $H$, vertex $t$ has no outgoing edges, and all edges entering $t$ connect vertices of $R$ to it.
	
	\item Every edge of $H'$ has at most $\log m-1$ edges that are parallel to it.
\end{itemize}
\end{definition}
 (We note that strictly speaking, a residual graph corresponding to a matching may contain edges entering $s$ and/or edges leaving $t$, but since such edges will not be used in augmenting paths, we can delete them from the residual network).

Whenever an algorithm is given a well-structured graph as an input, we assume that it is also given the vertices $s$ and $t$ and the corresponding partition $(L,R)$ of $V(H')$.
We are now ready to define the restricted $\SSSP$ problem.


\begin{definition}[Restricted \SSSP problem]
The input to the restricted \SSSP problem is a well-structured graph $G$ of size $m$, where $m$ is a given parameter, together with another parameter $\Delta>0$. We denote $|V(G)|=n$ and  $\Lambda=\frac{2^{11}n\log^2m}{\Delta}$. For every edge $e\in E(G)$, we are also given a length $\ell(e)$, that is an integral power of $2$ between $1$ and $2\Lambda$. 


The algorithm consists of at most $\Delta$ iterations. At the beginning of every iteration, the algorithm must compute a simple $s$-$t$ path in the current graph $G$ of length at most $2\Lambda$ (we sometimes informally say that the algorithm responds to a \shortpath query between $s$ and $t$). We assume that for each edge $e\in E(P)$, edge $e$ is the cheapest from among its parallel copies. Every edge of $P$ is then deleted from $G$, and the iteration ends.

The algorithm is allowed, at any time, to halt and return FAIL, but it may only do so if the largest-cardinality collection $\qset$ of $s$-$t$ paths in the current graph $G$, such that the paths in $\qset$ are internally vertex-disjoint, and every path has length at most  $\Lambda$, is less than $\frac{\Delta}{512\log^2m}$. %In case the algorithm returns a path $P$, it should be done in time $\tilde O(|E(P)|)$, and this time is not counted towards the total update time of the algorithm. 
\end{definition}



One of the main technical contributions of our paper is the proof of following theorem.

\begin{theorem}\label{thm: sssp main}
	There is an algorithm for the Restricted \SSSP problem, that, given a well-structured graph $G$ with $n$ vertices and parameters $\Delta$ and $m$, has total update time $\otilde\left(\frac{n^{2.5}}{\sqrt{\Delta}}\right ) $.
	\end{theorem}

The proof of  \Cref{thm: one iteration main} immediately follows from \Cref{thm: sssp main}: we use the algorithm from \Cref{thm: sssp main} in order to implement the oracle for
\algmwu. In order to do so, we first construct a graph $\hat H$, that is obtained from $H$ by replacing each of its edges by $\log m$ parallel edges of lengths $1/m,2/m,\ldots,1$. In every iteration, we use the algorithm for the restricted \SSSP problem in order to compute a simple $s$-$t$ path $P$ in graph $\hat H$ of length at most $1$, which immediately defines a path in graph $H$ at the same length (we assume w.l.o.g. that every edge $e\in E(P)$ is the shortest among its parallel copies). The doubling of the length of every edge on $P$ is implemented by deleting the shortest copy of each such edge from graph $\hat H$. It is easy to verify that the total running time of the algorithm is bounded by $O(m\log m)$ plus the total update time of the algorithm for the restricted \SSSP problem, which is, in turn, bounded by $\otilde\left(\frac{n^{2.5}}{\sqrt{\Delta}}\right ) $. Since $\Delta\leq n$, we can bound the total running time of the algorithm by $\otilde\left(\frac{n^{2.5}}{\sqrt{\Delta}}\right ) $.


In the remainder of this paper we focus on the proof of \Cref{thm: sssp main}.
At a high level, the proof of the theorem follows the framework of \cite{SCC} for decremental \SSSP in directed graphs. But since we only need to deal with a very restricted special case of the problem we obtain a faster total update time, and also significantly simplify some of the arguments.
In the following two sections, we present the two main tools that are used in the proof of \Cref{thm: sssp main}: the \ATO framework, together with \SSSP in ``DAG-like'' graphs, and expander-based techniques. We then provide the proof of the theorem in \Cref{sec: SSSP alg}. 


==> our-techniques.tex <==
\subsection{Our Techniques}

We now provide a high-level overview of our techniques. At the heart of our approach is an observation that the problem of computing \MBM can be reduced to a restricted special case of the decremental \SSSP problem in directed graphs, which seems to be significantly easier than the general decremental directed \SSSP problem. We then adapt the approach of \cite{SCC} for solving decremental directed \SSSP to our more restricted setting. We now describe each of these parts in more detail.


It is well known that the \MBM problem can be equivalently cast as the problem of computing maximum $s$-$t$ flow in a directed graph with unit vertex capacities. One standard approach for obtaining fast algorithms for various flow problem, due to \cite{GK98, Fleischer00,AAP93}, is via the Multiplicative Weight Update (\MWU) method. It was further observed by Madry \cite{madry2010faster}  that this approach can be viewed as reducing a given flow problem to a variant of decremental \SSSP or \APSP.  However, employing this approach directly typically leads to \emph{approximate}, and not exact algorithm for the given flow problem. This is both because the \MWU method inherently leads to approximate flow solutions, and because of known lower bounds for obtaining fast exact algorithms for decremental \SSSP and \APSP (see, e.g. \cite{DorHZ00,RodittyZ11,HenzingerKNS15,abboud2022hardness,DBLP:conf/stoc/AbboudBF23}). Since our goal is to solve the \MBM problem exactly, we therefore cannot employ this method directly.

Instead, we employ an iterative algorithm. At the beginning of every iteration, we are given some matching $M$ in the input graph $G$, and the goal is to obtain a significantly larger matching. Specifically, if we denote by $\Delta=\opt-|M|$, where $\opt$ is the value of the maximum bipartite matching in $G$, then the goal of an iteration is to compute a matching $M'$ with $|M'|\geq |M|+\Omega(\Delta/\poly\log n)$. This will ensure that the number of iterations is bounded by $O(\poly\log n)$. We now focus on implementing a single iteration. 

As mentioned already, the problem of computing a maximum bipartite matching in a graph $G$ can be equivalently expressed as the problem of computing a maximum $s$-$t$ flow in a directed flow network $G'$ with unit vertex capacities. A matching $M$ in $G$ naturally defines an $s$-$t$ flow $f$ in $G'$, whose value is $|M|$. We let $H=G_f$ be the corresponding residual flow network, that we refer to as \emph{residual flow network with respect to matching $M$}. As before, all vertex capacities in $H$ are unit. It is then easy to see that $H$ must contain an integral $s$-$t$ flow of value $\Delta=\opt-|M|$. Moreover, any integral $s$-$t$ flow $f'$ in $H$ that respects vertex capacities can be transformed into a collection $\qset$ of $\val(f')$ internally disjoint $s$-$t$ paths (augmenting paths), which can then in turn  be used in order to obtain a new matching $M'$ in $G$, of cardinality at least $|M|+\val(f')$. Recall that we have established that the value of the maximum $s$-$t$ flow in $H$ is at least $\Delta=\opt-|M|$, and our goal is to ensure that $|M'|\geq |M|+\Omega(\Delta/\poly\log n)$. In other words, in order to implement a single iteration,  it is sufficient to design an algorithm for solving the maximum $s$-$t$ flow problem in directed unit-capacity graphs \emph{approximately}. Moreover, unlike the more standard setting where one seeks $(1+\eps)$-approximate flow solution, we can afford a rather high approximation factor. We can now employ the \MWU method, in order to reduce the problem of computing approximate maximum $s$-$t$ flow in the residual graph $H$ to a special case of decremental \SSSP in directed graphs.


At a high level, we follow the approach of \cite{SCC}, who designed a $(1+\eps)$-approximation algorithm for directed decremental \SSSP, with total update time $O\left (\frac{n^{2+2/3+o(1)}}{\eps}\right )$ (assuming that all edge lengths are poly-bounded). This running time is prohibitively high for our purposes, so we cannot use their algorithm directly. Instead, we observe that we only need to solve a restricted special case of directed decremental \SSSP; by adapting their algorithm to this setting, we obtain the desired faster running time. Unlike the general \SSSP problem, the special case that we need to solve has some useful properties. First, all shortest-path queries are asked between a pre-specified pair $(s,t)$ of vertices. 
Additionally, we slightly modify the \MWU method, so that the task of responding to shortest-path queries is even easier. Specifically, we can assume that we are given two parameters $d$ and $\Delta$. In response to a shortest-path query, the algorithm needs to either return an $s$-$t$ path of length at most $d$, or return ``FAIL''. The latter can only be done if the largest number of internally disjoint $s$-$t$ paths of length at most $d/2$ in the current graph is bounded by $O(\Delta/\poly\log n)$. In other words, our algorithm only needs to support shortest-path queries as long as there is a large number of short and internally disjoint $s$-$t$ paths in the current graph $H$. This property is crucially used by our algorithm to obtain a faster running time. Additionally, due to the specific setup provided by the \MWU method, the only edges that are deleted from $H$ are those appearing on the paths that the algorithm returns in response to queries. Moreover, unlike the standard setting of the dynamic \SSSP problem, where it is crucial that the time the algorithm takes to respond to each individual query is short, we only need to ensure that the total time the algorithm takes to respond to all queries is suitably bounded. We exploit all these advantages of the special case of the \SSSP problem that we obtain in order to design an algorithm for it that is significantly faster than the algorithm of \cite{SCC} for general decremental \SSSP.

We now provide aadditional details of our algorithm for restricted decremental \SSSP. We follow the high-level approach of \cite{SCC}, that consists of two parts. First, they maintain a partition $\xset$ of graph $H\setminus \set{s,t}$ into a collection of expander-like graphs; we abstract the problem of maintaining each such expander graph, that we call \maintaincluster problem, below. Second, they apply the Approximate Topological Order (\ATO) framework of \cite{evald2020decremental}, together with their algorithm for decremental \SSSP on ``almost'' DAG's to the graph $\hat H$, that is obtained from $H$ by contracting every expander $X\in \xset$ into a single vertex. We now discuss both of these components in turn, and point out similarities and differences between our algorithm and that of \cite{SCC}.

We start by defining the \maintaincluster problem, that, intuitively, is used in order to manage a single expander-like graph. We will eventually apply it to every subgraph $X\in \xset$ of $H$. The input to the problem is a subgraph $X\subseteq H\setminus \set{s,t}$, and a parameters $d\geq \poly\log n$ and $\Delta>0$. We will treat all edges of $X$ as unweighted, so the length of each edge is $1$. The algorithm consists of at most $\Delta$ iterations. In every iteration, the algorithm is given a pair $x,y\in V(X)$ of vertices, and it needs to compute a simple path $P$ of length at most $d$ connecting $x$ to $y$ in $X$. Some of the edges of $P$ may then be deleted from $H$, and the iteration ends. The algorithm can, at any time,  compute a cut $(A,B)$ in $X$, whose sparsity is at most $O\left (\frac{\poly\log n}{d}\right )$. After that, if $|A|\ge |B|$, then vertices of $B$ are deleted from $X$, and otherwise the vertices of $A$ are deleted from $X$. In either case, the algorithm must continue with the new graph $X$. Our goal is to provide an algorithm for the \maintaincluster problem, whose total running time is low. %The running time includes both the total update time and the time required to respond to all queries. 
In particular, unlike a similar problem that was considered in \cite{SCC}, we do not need to ensure that the time that the algorithm takes in order to respond to \emph{each} query is low. Instead, we only need to ensure that the total update time of the algorithm, together with the total time spent on responding to queries, is low. The seting that is considered in \cite{SCC} is more general in several other ways: there is no bound on the number of queries, and edges may be deleted from $X$ as part of update sequence\footnote{Like \cite{SCC}, we distinguish between edges that are deleted from $X$ by ``adversary'', as part of online update sequence, and edges that are deleted by the algorithm itself, when it computes a sparse cut $(A,B)$ in $X$, and deletes all vertices on the smaller side of the cut from $X$.} arbitrarily (in our setting, only edges that appear on the paths that the algorithm returns in response to queries may be deleted). The algorithm of \cite{SCC} for this more general version of the \maintaincluster problem has total update time $\ohat(|E(X)|\cdot d^2)$, and the time to respond to each query is roughly proportional to the number of edges on the path that the algorithm returns. We provide an algorithm for the \maintaincluster problem, whose total running time is bounded by $\otilde(|E(X)|\cdot d+|V(X)|^2)\cdot  \max\set{1,\frac{\Delta\cdot (d)^2}{|V(X)|}}$, which, for the setting of parameters that we employ becomes $\otilde(|E(X)|\cdot d+|V(X)|^2)$. Our algorithm uses a rather standard approach: we embed a large $\Omega(1/\poly\log n)$-expander $W$ into the graph $X$, and then use two Even-Shiloach tree (\EST) data structures in $X$, that are rooted at the vertices of $W$; in one of the resulting trees the edges are directed away to the root, and in the other they are directed towards the root. However, due to the specifics of the setting that we have described, we obtain an algorithm that is significantly simpler than that of \cite{SCC}, and other similar algorithms. For example, we use a straightforward (although somewhat slower) algorithm for the cut player in the Cut-Matching game, and our algorithm for the variant of \APSP in expanders that we obtain is quite elementary; it avoids the recursion that was used in previous work (see \cite{APSP-old,detbalanced,SCC}), and expander pruning of \cite{expander-pruning,SCC}. While some parts of our algorithm can be optimized, for example, by using the faster algorithm for the Cut Player due to \cite{SCC}, this would not affect our final running time, and we believe that the simple self-contained proofs provided in this paper are of independent interest.

We now briefly describe the second component of our algorithm -- the use of the Approximate Topological Order (\ATO) framework of  \cite{evald2020decremental}, that can be viewed as reducing the decremental \SSSP problem on general directed graphs to decremental \SSSP on ``almost DAG's''. This part is almost identical to the algorithms of \cite{evald2020decremental,SCC}. The main difference is that we save significantly on the running time of the algorithm due to the fact that we only need to support approximate shortest-path queries between $s$ and $t$, as long as graph $H$ contains many short $s$-$t$ paths. We start with the decremental graph $H$ that serves as the input to the restricted decremental \SSSP problem, and we maintain a partition $\xset$ of the vertices of $H\setminus\set{s,t}$ into subsets. At the beginning of the algorithm, we let $\xset$ contain a single set $V(H)\setminus\set{s,t}$, and, as the algorithm progresses, the only allowed updates to the collection $\xset$ of vertex subsets is a partition of a given set $X\in \xset$ into two subsets, $A$ and $B$. Intuitively, whenever a set $X$ of vertices is added to $\xset$, we view it as an instance of the \maintaincluster problem on the corresponding graph $H[X]$, with an appropriately chosen distance parameter $d_X$. We then apply the algorithm for the \maintaincluster problem to this instance. Whenever the algorithm produces a cut $(A,B)$ in $X$, we let $Z$ be the smaller-cardinality set of vertices from among $A$, $B$.   Recall that the algorithm for the \maintaincluster problem then deletes the vertices of $Z$ from $X$. We add the set $Z$ as a new vertex set to $\xset$, and initialize the algorithm for the \maintaincluster problem on it. Additinally, we update the set $X$ of vertices in $\xset$, by deleting the vertices of $Z$ from it. For convenience, we will also add to $\xset$ two additional subsets: $S=\set{s}$, $T=\set{t}$, so $\xset$ becomes a partition of the vertices of $H$ into subsets.

In order to define Approximate Topological Order (\ATO) on graph $H$, with the partition $\xset$ of the vertices of $V(H)\setminus\set{s,t}$ into subsets, we associate, with every set $X\in \xset$, a contiguous collection $I_X$ of $|X|$ integers from $\set{1,\ldots,n}$, that we refer to as an \emph{interval}. We always let $I_S=\set{1}$, $I_T=\set{n}$, and we require that all resulting intervals are mutually disjoint. Notice that the resulting collection $\set{I_X\mid X\in \xset}$ of intervals naturally defines an \emph{ordering} of the sets in $\xset$, that we denote by $\sigma$, and for convenience, we call it a \emph{left-to-right} ordering. Consider now some edge $e=(u,v)$, and let $X,Y\in \xset$ be the sets containing $u$ and $v$, respectively. Assume further that $X\neq Y$. If $X$ appears before $Y$ in the ordering $\sigma$, then we say that $e$ is a \emph{left-to-right} edge, and otherwise, we say that it is a \emph{right-to-left} edge.

Recall that, at the beginning of the algorithm, we let $\xset$ contain three vertex sets: $S=\set{s},T=\set{t}$, and $R=V(H)\setminus\set{s,t}$. We also set $I_S=\set{1}$, $I_T=\set{n}$, and $I_R=\set{2,\ldots,n-1}$. As the algorithm  progresses,
whenever a set $X$ of vertices is split into two sets $A$ and $B$, we partition the interval $I_X$ into two subintervals $I_A$ and $I_B$, of cardinalities $|A|$ and $|B|$, respectively. Recall that we only partition $X$ into sets $A$ and $B$ if $(A,B)$ defines a sparse cut in graph $H[X]$. This means that either $|E_H(A,B)|$, or $|E_H(B,A)|$ is  small relatively to $\min\set{|A|,|B|}$. In the former case, we ensure that interval $I_B$ appears before interval $I_A$, while in the latter case, we ensure that interval $I_A$ appears before interval $I_B$. This placement of intervals ensures that there are relatively few right-to-left edges.

Lastly, we consider the contracted graph $H'=H_{|\xset}$, that is obtained from $H$ by contracting every set $X\in \xset\setminus\set{S,T}$ into a single vertex. As the time progresses, graph $H'$ undergoes edge deletions and vertex-splitting updates. The letter type of updates reflects the partitioning of the sets $X\in \xset$ of vertices into smaller subsetse. At all times, the ordering $\sigma$ of the intervals in $\set{I_X\mid X\in \xset}$ that is maintained by the \ATO naturally defines an ordering of the vertices of $H'$, that we denote by $\sigma'$. Notice that, if we could ensure that no right-to-left edges are present, then graph $H'$ would be a DAG, and $\sigma'$ would define a topological ordering of its vertices. We could then use the algorithm of \cite{evald2020decremental}  for decremental \APSP in DAG's, whose total update time is $\otilde(n^2)$. In \cite{evald2020decremental} it was further observed that, if we could ensure that the number of right-to-left edges with respect to the partition $\xset$ that the \ATO structure maintains is low, and the average length of each such edge (with respect to the ordering $\sigma'$ of the vertices of $H'$) is small, one can apply an algorithm similar to that for \APSP in DAG's to the contracted graph $H'$. The total update time of the resulting algorithm depends on the number of the right-to-left edges, and on their length with respect to $\sigma'$. Exactly this approach was used in \cite{SCC} in order to obtain an algorithm for decremental \APSP in general directed graphs. We also employ the same approach, but we use the advantages of our setting, specifically, that all queries are between a pre-specified pair $s,t$ of vertices, and that we only need to support the queries as long as there are many short internally disjoint $s$-$t$ paths, in order to obtain a faster algorithm. Intuitively, since we can assume that the current graph $H$ contains $\tilde \Omega(\Delta)$ short internally disjoint $s$-$t$ paths, and since the right-to-left edges must be distributed among such paths, at least one short $s$-$t$ path must contain a very small number of right-to-left edges. It is this observation that leads to a faster running time of this part of our algorithm.

==> simple-routeandcut.tex <==
\subsubsection{A Simple and Inefficient Algorithm for the \routeandcut Problem via Basic \MWU}

\mynote{for future passes: to be consistent with what we do later it may be better to not create parallel edges in $\hat G$. Instead increase edge lengths by $(1+1/\eta)$ every time the edge is used.}
In this subsection we present a simple and not very efficient deterministic algorithm for the \routeandcut problem, that we will eventually use as the induction base. The algorithm is summarized in the following lemma, and its proof uses rather standard techinques.

\begin{lemma}\label{lem: main for route and cut basic}
	There is a deterministic algorithm for the \routeandcut problem, that, given an input $(G,A,B,\Delta,\eta,N)$, has running time  $\otilde\left(n\cdot (n-|B|)\cdot \frac{(n-|B|)\cdot \eta}{\Delta}\right)$, where $n=|V(G)|$.
\end{lemma}


\begin{proof}
Recall that we are given as input a uniform well-structured $n$-vertex graph $G=(L,R,E)$ in the adjacency-list representation, together with parameters $N\geq n$, $1\leq \Delta\leq N$ and $1\leq \eta \leq \Delta$, such that $\Delta\leq n\eta$, and two disjoint subsets $A,B$ of vertices of $G$ of with $|A|,|B|\geq \Delta$. 


Our goal is to compute a routing  $\qset$ of $A$ to $B$ in $G$ with congestion at most $4\eta\log N$, 
and a cut  $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{\Delta}{ \eta\log^4n}+\frac{|\qset|}{\eta}$, such that, if 
$A'\subseteq A, B'\subseteq B$ denote the subsets of vertices that do not serve as endpoints of the paths in $\qset$, then $A'\subseteq X$ and $B'\subseteq Y$ hold.



Throughout, we denote $m=|E|$. Recall that the edges of $E_G(R,L)$ are called special edges, and the remaining edges of $G$ are called regular edges. %The length of every special edge is $1$, and the length of every regular edge is $0$. Moreover, 
Recall also that every vertex of $G$ is incident to at most one special edge.
We partition the set $\qset^*$ of paths into two subsets: set $\qset^*_1$ contains all paths $Q\in \qset^*$ that consist of a single regular edge, and set $\qset^*_2$ contains all remaining paths. Notice that every path in $\qset^*_2$ must contain at least one special edge, and, from the definition of partial routing, the paths in $\qset^*_1$ are mutually edge- and vertex-disjoint. 

As a preprocessing step, we construct a maximal set $\qset_1$ of disjoint paths, where every path connects a distinct vertex of $A$ to a distinct vertex of $B$, and consists of a single regular edge. We do so by employing a simple greedy algorithm. We start with $\qset_1=\emptyset$. While there is a regular edge $e=(a,b)$ with $a\in A$ and $b\in B$, we add a path $Q=(e)$ to $\qset_1$, and we delete $a$ and $b$ from $A$ and $B$, respectively. Clearly, this preprocessing step can be executed in time $O(m)$, and at the end of this step there is no regular edge in $G$ connecting a vertex of $A$ to a vertex of $B$. It is easy to verify that $|\qset_1|\ge |\qset^*_1|/2$ holds. Indeed, let $H$ be the graph that is obtained from $G$ by deleting all special edges. Then the paths in $\qset^*_1$ define a matching $M^*_1\subseteq A\times B$, where each path $Q\in \qset^*_1$ contributes the unique edge $e\in E(Q)$ to the matching. Similarly, set $\qset_1$ defines a matching $M_1$ in graph $H$, and, from our construction, matching $M_1$ is maximal. Therefore $|M_1|\geq |M_1^*|/2$ and $|\qset_1|\geq |\qset^*_1|/2$ must hold.
	
	


Let $\hat G$ be the graph that is obtained from $G$ by replacing every edge $e$ with $\eta$ parallel copies. Edges that are copies of special edges in $G$ are called special edges of $\hat G$, and similarly copies of regular edges in $G$ are called regular edges of $\hat G$. Additionally, we add a source vertex $s$, that connects to every vertex of $A$ with an edge, and a destination vertex $t$, to which every vertex of $B$ connects. Edges that are incident to $s$ and $t$ are also considered regular edges.




Consider the problem of computing a largest-cardinality collection  $\qset'$ of edge-disjoint $s$-$t$ paths in graph $\hat G$.
Notice that the set $\qset^*_2$ of paths in $G$ naturally defines a solution to this problem. Let $\pset^*$ denote the collection of all simple $s$-$t$ paths  in graph $\hat G$. Then the problem can be expressed as a linear program, where every path $P\in \pset^*$ is associated with a variable $f(P)$; we also provide a dual LP.


\begin{tabular}[t]{|l|l|}\hline &\\
	$\begin{array}{lll}
	\text{\underline{Primal}}&&\\
	\text{Max}&\sum_{P\in \pset^*} f(P)&\\
	\text{s.t.}&&\\
	&\sum_{\stackrel{P\in\pset^*:}{e\in E(P)}}f(P)\leq
	1&\forall e\in E(\hat G)\\
	&f(P)\geq 0&\forall P\in \pset^*\\
	\end{array}$
	&$
	\begin{array}{lll}
	\text{\underline{Dual}}&&\\
	\text{Min}&\sum_{e\in E(\hat G)}\ell(e)\\
	\text{s.t.}&&\\
	&\sum_{e\in E(P)}\ell(e)\geq 1&\forall P\in \pset^*\\
	&\ell(e)\geq 0&\forall e\in E(\hat G)\\
	&&\\
	\end{array}$\\ &\\ \hline
\end{tabular}
\vspace{1cm}

In the dual LP, there is a variable $\ell(e)$ for every edge $e\in E(\hat G)$, that we will refer as the \emph{length} of the edge. We now consider the following primal-dual algorithm, which is a simplified version of the original algorithm of \cite{GK98, Fleischer00}; this variant achieves a slightly weaker approximation, but its analysis is much simpler and the higher approximation factor does not affect our algorithm. 





At the beginning of the algorithm, every special edge $e\in E(\hat G)$ is assigned a length $\ell(e)=\frac{\Delta}{n\eta\log^4n}$, while every regular edge $e\in E(\hat G)$ is assigned length $0$. %We also set $f(P)=0$ for every path $P\in \pset^*$.
	Clearly, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}$ holds, as there are at most $n\eta$ special edges in $\hat G$, each of which has length $\frac{\Delta}{n\eta\log^4n}$. 
	
	Over the course of the algorithm, the lengths of special edges, and the lengths of the regular edges incident to $s$ and $t$ may grow, while the lengths of all other regular edges remain $0$. Additionally, vertices may be deleted from sets $A$ and $B$, but graph $\hat G$ remains unchanged.  We will gradually construct a collection $\qset_2$ paths in graph $\hat G$, where every path connects a distinct vertex of $A$ to a distinct vertex of $B$, and the paths cause edge-congestion at most $O(\log n)$ in $\hat G$. Initially, we set $\qset_2=\emptyset$. 
	
	
	We assume for now that we are given an oracle, that, when prompted, either returns a simple path $Q$ in the current graph $\hat G$ connecting $s$ to $t$, such that the length $\sum_{e\in E(Q)}\ell(e)$ of the path is at most $1$; or correctly establishes that 
	such a path does not exist.
	
	The algorithm proceeds in iterations. In every iteration, the oracle is asked to return a simple path $Q$ in the current graph $\hat G$ connecting $s$ to $t$, such that the length $\sum_{e\in E(Q)}\ell(e)$ of the path is at most $1$. If it successfully does so, then we let $Q'$ be the path obtained from $Q$ by deleting the first and the last vertices from it. Clearly, $Q'$ connects some vertex $a\in A$ to some vertex $b\in B$. We add $Q'$ to $\qset_2$, double the length of every special edge on path $Q'$, and set the lenths of the edges $(s,a)$ and $(b,t)$ to $1$ each. We also remove $a$ from $A$ and $b$ from $B$. Notice that in this case,  $|\qset_2|$ grows by $1$, while $\sum_{e\in E(\hat G)}\ell(e)$ increases by at most $3$.
	If the oracle establishes that no $s$-$t$ path of length at most $1$ exists in $\hat G$, we terminate the algorithm. Notice that the resulting set $\qset_2$ of paths in graph $\hat G$ naturally defines a collection of paths in graph $G$, that for simplicity we also denote by $\qset_2$.
	
	At the end of the algorithm, we set $\qset=\qset_1\cup \qset_2$.
	Due to the doubling of the lengths of the special edges on the paths that we add to $\qset_2$, and since the initial length of each such edge is set to $\frac{\Delta}{n\eta\log^4n}$, every special edge of $\hat G$ may participate in at most $O\left(\log\left(\frac{n\eta\log^4n}{\Delta}\right )\right )\leq O(\log n)$ paths in $\qset$, and so in total every special edge of $G$ may participate in at most $O(\eta\log n)$ paths in $\qset$. Moreover, if $e=(u,v)$ is a regular edge, then every path $Q\in \qset_2$ that contains $e$ must also contain either the unique special edge incident to $u$, or the unique special edge incident to $v$, while the paths in $\qset_1$ are disjoint. We conclude that the paths in $\qset$ cause congestion at most $O(\eta\log n)$ in $G$.
It is also easy to see that the endpoints of the paths in $\qset$ are disjoint. Indeed, if we add a path $Q$ connecting a vertex $a\in A$ to a vertex $b\in B$ to $\qset_1$, then we delete $a$ from $A$ and we delete $b$ from $B$, so $a$ and $b$ may not serve as endpoints of paths in $\qset_2$. If we add a path $Q'$ connecting a vertex $a'\in A$ to a vertex $b'\in B$ to $\qset_2$, then we set the lengths of the edges $(s,a')$ and $(b',t)$ to $1$, so these edges may not be used in any future paths. Therefore, if $Q''$ is a path that is added to $\qset_2$ after $Q$, then the first vertex on $Q''$ must be different from $a'$, and the last vertex on $Q''$ must be different from $b'$.
Next, we prove that, if $|\qset^*|\geq \Delta$, then the collection $\qset$ of paths is sufficiently large.

\begin{observation}\label{obs: get good routing}
	If $|\qset^*|\geq \Delta$, then $|\qset|\geq \Delta/12$.
\end{observation}
\begin{proof}
	Assume that $|\qset^*|\geq \Delta$.
	Recall that we have partitioned the set $\qset^*$ of paths into $\qset_1^*$ and $\qset_2^*$. If $|\qset^*_1|\geq \Delta/2$, then we are guaranteed that $|\qset_1|\geq |\qset^*_1|/2\geq \Delta/4$. Therefore, we assume from now on that $|\qset^*_1|<\Delta/2$, and so $|\qset^*_2|\geq \Delta/2$.
	
	Set $\qset^*_2$ of paths naturally defines a solution to the primal LP of value $|\qset^*_2|\geq \Delta/2$. Recall that, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}$ holds. In every iteration, we add one path to $\qset_2$, and we increase $\sum_{e\in E(\hat G)}\ell(e)$ by at most $3$. Therefore, at the end of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}+3|\qset_2|$ holds. Moreover, at the end of the algorithm, the values $\set{\ell(e)}_{e\in E(\hat G)}$ define a feasible solution to the dual LP, and, since the value of the optimal solution to the primal and to the dual LP is at least $|\qset^*_2|\geq \Delta/2$, we get that $\sum_{e\in E(\hat G)}\ell(e)\geq \Delta/2$ must hold at the end of the algorithm. We conclude that $|\qset_2|\geq \Delta/12$ holds.
\end{proof}
	
	
	
	

Let $A'\subseteq A$, $B'\subseteq B$ be the sets of vertices that remain in $A$ and $B$, respectively at the end of the algorithm. Since the algorithm terminated, in the current graph $\hat G$, the length of the shortest path connecting a vertex of $A'$ to a vertex of $B'$ is at least $1$.

	
	Recall that, at the beginning of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}$ held. Over the course of the algorithm, in every iteration, $\sum_{e\in E(\hat G)}\ell(e)$ grew by at most $3$, and the number of iterations is bounded by $|\qset|$. Therefore,  at the end of the algorithm, $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}+3|\qset|$ holds. 
	
	Let $e$ be any edge of graph $G$, and let $S(e)$ be the collection of $d$ parallel edges representing $e$ in graph $\hat G$. Let $e'\in S(e)$ be the copy of $e$ with smallest current length $\ell(e')$. Notice that, if we set the lenghts of all edges in $S(e)$ to $\ell(e')$, then the length of the shortest path connecting a vertex of $A'$ to a vertex of $B'$ in $\hat G$ will remain at least $1$. Therefore, we can assume without loss of generality, that, for every edge $e\in E(G)$, the lengths of all edges in set $S(e)$ are identical; we denote this length by $\ell'(e)$.
	Notice that $\sum_{e\in E(\hat G)}\ell(e)\leq \frac{\Delta}{\log^4n}+3|\qset|$ continues to hold after this transformation.
	
	Consider now the graph $G'$ that is obtained from $G$ by
	setting the length of every edge $e\in E(G)$ to $\ell'(e)$,
	unifying all vertices of $A'$ into a source vertex $s$ and all vertices of $B'$ into a destination vertex $t$. Since graph $\hat G$ contained $\eta$ parallel copies of every edge $e\in E(G)$, that all had the same length equal to $\ell'(e)$, we now have that $\sum_{e\in E(G)}\ell'(e)\leq \frac{\sum_{e\in E(\hat G)}\ell(e)}{\eta}\leq \frac{\Delta}{\eta\log^4n}+\frac{3|\qset|}{\eta}$. At the same time, since $\hat G$ did not contain an $A'$-$B'$ path of length at most $1$, we get that $\dist_{G'}(s,t)\geq 1$.
	
	Consider the following thought experiment: we choose a threshold $\rho\in (0,1)$ uniformly at random, and then define two sets $S=\set{v\in V(G')\mid \dist_{G'}(s,v)\leq \rho}$ and $T=V(G')\setminus S$ of vertices. Clearly, $s\in S$ and $t\in T$ must hold.
	By replacing $s$ with the vertices of $A'$ in $S$ and replacing $t$ with the vertices of $B'$ in $T$, we obtain a cut $(S',T')$ in graph $G$ with $|E_G(S',T')|=|E_{G'}(S,T)|$. It is easy to verify that, for every edge $e=(u,v)\in E(G')$, the probability that $u\in S$ and $v\in T$ is bounded by $\ell'(e)$. Therefore, the expected value of $|E_{G'}(S,T)|$ is bounded by $\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta}{\eta\log^4n}+\frac{3|\qset|}{\eta}$. By performing a BFS search from vertex $s$, we can then compute a cut $(S',T')$ in $G'$ with $|E_{G'}(S',T')|\leq \frac{\Delta}{\eta\log^4n}+\frac{3|\qset|}{\eta}$. Using the procedure outlined above, we can covert this cut into a cut $(S,T)$ in $G$ with $|E_G(S,T)|\leq \frac{\Delta}{\eta\log^4n}+\frac{3|\qset|}{\eta}$. Clearly, $A'\subseteq S$ and $B'\subseteq T$ holds. We then return the cut $(S,T)$ and the routing $\qset$ as the output of the algorithm. In order to analyze the algorithm we need to provide an implementation of the oracle, which we do next.
	
	
	Notice that every special edge of $G$ participates in at most $\eta$ paths of $\qset_2$, and regular and special edges alternate on all paths in $\qset_2$. Therefore, $\sum_{Q\in \qset_2}|E(Q)|)\leq O(n\eta)$. It is also easy to verify that $\sum_{Q\in \qset_1}|E(Q)|)\leq O(n)$, and so $\sum_{Q\in \qset}|E(Q)|)\leq O(n\eta)$.
	We will use this fact later.
	

	
	
	
	
	\paragraph{Implementing the Oracle.}
	In order to implement the oracle efficiently, we construct a new graph $H$, as follows. Initially, $H$ is obtained from $G$ by adding a source vertex $s$ that connects with an edge to every vertex of $A$, and a destination vertex $t$, to which every vertex of $B$ connects. The edges that leave $s$ or enter $t$ are called regular edges.
	
	
	Denote $\beta=\frac{n\eta\log^4n}{\Delta}$. Recall that initially the length of every special edge in $\hat G$ is set to $1/\beta$. After that the lengths of some edges are doubled, and once the length of a special edge grows beyond $1$, it may no longer be used in any paths, and so it will no longer be doubled. Additonally, the lengths of some edges incident to $s$ and $t$ may grow from $0$ to $1$.
	
	Let $q=\ceil{\log \beta}+1$. 
	Consider any special edge $e=(u,v)\in E(G)$. We replace $e$ with $q$ parallel edges $e_1,\ldots,e_q$, whose lengths are $1,2,\ldots,2^q$, respectively. 
	Additionally, for every regular edge $e'=(x,u)$ that enters $u$, we replace $e'$ with $q$ parallel edges $e'_1,\ldots,e'_q$, whose lengths are $1,2,\ldots,2^q$, respectively (the latter transformation is also applied to the regular edge $(s,u)$, if such an edge is present). The latter step is done in order to ensure that the length of every edge in $G$ is greater than $0$, since this is a requirement in \Cref{thm: directed weighted ESTree} that we will use. 
	If $(x,y)$ is a regular edge of $G$ with $y\neq t$, such that no special edge leaves $y$, then we delete $y$ and its incident edges from $G$, since vertex $y$ does not lie on any $s$-$t$ path.
	So far we have assigned lengths to all edges of $H$, except for some edges that leave $s$, and all edges that enter $t$. Initially, we set the lengths of all these edges to $0$. We then increase the length of every edge that is incident to $s$ or $t$ by $1$, thus obtaining the final lengths of all edges in $H$.
	
	
	
	
	Over the course of the algorithm, for every special edge $e=(u,v)\in E(G)$, for every index $1\leq j\leq q$, we monitor the number of copies of $e$ in graph $\hat G$, whose length is $\frac{2^j}{\beta}$. Once this number becomes $0$, the corresponding copy $e_j$ of $e$ is deleted from graph $H$. Additionally, for every regular edge $e'=(x,u)$, we also delete the corresponding copy $e'_j$ from $H$. Lastly, whenever a vertex $a$ is deleted from set $A$, we delete edge $(s,a)$ from $H$, and whenever a vertex $b$ is deleted from set $B$, we delete edge $(b,t)$ from $H$. Therefore, the only types of updates that graph $H$ undergoes is the deletion of edges.
	
	It is now easy to verify that, throughout the algorithm, if $Q$ is an $s$-$t$ path in $H$, whose length is $\delta+2$, then the length of the corresponding path $Q'$ in $\hat G$ (where for every edge $e\in E(Q)$, we choose its cheapest copy in $\hat G$ to participate in the path) is at most $\frac{\delta}{2\beta}$. Similarly, if $Q'$ is an $s$-$t$ path in graph $\hat G$, whose length is $\delta'$, then the length of the corresponding $s$-$t$ path in graph $H$ (where again for every edge $e\in E(Q')$ we use its cheapest copy available in $H$) is $2\delta\cdot \beta+2$.
	
	It is now enough to design an algorithm for the following problem. We are given a graph $H$, with two special vertices $s$ and $t$, and integral positive edge lengths, together with a parameter $\beta>0$. The algorithm consists of a number of iterations. In every iteration, we need to either return an $s$-$t$ path in the current graph $H$, of length at most $2\beta+2$; or correctly establish that no such path exists. In the latter case, the algorithm terminates, while in the former case, the algorithm is given a batch of edge deletions from graph $H$, and we proceed to the next iteration.
	
	We apply the algorithm from \Cref{thm: directed weighted ESTree} to graph $H$ and parameter $2\beta+2$. Recall that the algorithm maintains an \EST for $H$, rooted in $s$, up to depth $2\beta+2$. We denote the corresponding tree by $T$. In every iteration, we check whether vertex $t$ lies in the tree $T$, and if so, whether $\dist_H(s,t)\leq 2\beta+2$. If this is not the case, then we terminate the algorithm. Otherwise, we use the tree $T$ to compute an $s$-$t$ path $P$ of length at most $2\beta+2$, in time $O(|E(P)|)$, by simply retracing the unique $s$-$t$ path in the tree $T$. 
	
	It is easy to verify that the total time needed to implement the oracle is $O(|E(H)|\cdot \beta+\sum_{Q\in \qset}|E(Q)|)$, where $\qset$ is the set containing all paths that the algorithm ever returned. As shown already, 
	$\sum_{Q\in \qset}|E(Q)|)\leq \tilde O(n\eta)$, while $\beta=\frac{n\eta\log^4n}{\Delta}$, and $|E(H)|\leq \otilde(m)$. The total running time of the oracle is then bounded by $\otilde\left(m\cdot \frac{n\eta}{\Delta} +n\cdot \eta\right)\leq  \otilde\left(m\cdot \frac{n\eta}{\Delta}\right)$. 
	
	We note that in general, the algorithm for \Cref{thm: alg for matching player} does not need to compute and maintain the graph $\hat G$ explicitly, this graph is only used for the sake of analysis. Instead, for every special edge $e\in E(G)$, for every integer $0\leq j\leq \ceil{\log \beta}$, we only need to keep track of the number of copies of $e$ that lie in graph $\hat G$ and have length $2^j/\beta$. Therefore, the total running time of the remainder of the algorithm is bounded by $O(m)+O(\sum_{Q\in \qset}|E(Q)|)\leq \otilde(n\eta+m)$. This includes the time required to perform a BFS in $G'$, in order to compute a spase cut $(S,T)$ if needed. The total running time of the whole algorithm  for \Cref{thm: alg for matching player} is then bounded by $\otilde\left(m\cdot \frac{n\eta}{\Delta}\right)$.
\end{proof}

==> temp-previous.tex <==
  
\begin{definition}[\routeandcut problem]\label{def: rounte and cut}
The input to the \routeandcut problem is a well-structured $n$-vertex graph $G=(L,R,E)$, that is given in the adjecency list representation, 
parameters $N\geq n$, $\Delta\geq 1$, and $1\leq \eta \leq \Delta$, and two disjoint subsets $A,B$ of vertices of $G$, with $|A|,|B|\geq \Delta$. 

The output of the problem is a (possibly partial) routing $\qset$ from $A$ to $B$, whose congestion is bounded by  $4\eta\log N$. Additionally, if $|\qset|<\Delta$, the output must contain a cut  $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{64\Delta}{ \eta\log^4n}+\frac{256|\qset|}{\eta}$, such that, if 
$A'\subseteq A, B'\subseteq B$ denote the subsets of vertices that do not serve as endpoints of the paths in $\qset$, then $A'\subseteq X$ and $B'\subseteq Y$ hold. The algorithm for the \routeandcut problem is also allowed to return ``FAIL'' without producing any output, but the probability of the algorithm doing so must be bounded by $1/2$.

We say that an instance $(G,A,B,\Delta,\eta,N)$ of the \routeandcut problem is  \emph{$r$-restricted}, for an integer $1\leq r\leq \ceil{\sqrt{\log N}}$, iff $\frac{(n-|B|)\cdot \eta}{\Delta}\leq 2^{r\cdot \sqrt{\log N}}$ holds. 
\end{definition}


======================
$\Lambda=(n-|B_1|)\cdot \frac{ \eta  \log^5n}{\Delta}$
=====================
The oracle:


\begin{definition}[Acceptable Path]\label{def: acceptable path}
	A path $P$ in the current graph $G$ is called \emph{acceptable} if $P$ is a simple path, connecting a vertex of $A_1$ to a vertex of $B_1$, the length of $P$ with respect to the current edge lengths $\ell(\cdot)$ is at most $1$, and no inner vertices of $P$ belong to $B_1$.
\end{definition}

erminates. We now define the cut-witness formally.

\begin{definition}[Cut-witness]\label{def: cut-witness}
	A \emph{cut-witness} is an assignment of lengths $\ell'(e)\geq 0$ to every edge $e\in E(G)$, such that, if  we denote by $A',B'$ the current sets $A_1,B_1$ of vertices, and by $E^*$ the set of all special edges with both endpoints in $B'$, then:		
	
	\begin{itemize}
		%		\item the length $\ell'(e)$ of every regular edge is $0$;
		\item $\sum_{e\in E(G)}\ell'(e)\leq \frac{\Delta}{2\eta\log^4n}+\sum_{e\in E(G)\setminus E^*}\ell(e)$; and
		
		\item the distance in graph $G$, with respect to edge lengths $\ell'(\cdot)$, from $A'$ to $B'$ is at least $\frac{1}{64}$. %, and moreover, the length $\ell'(e)$ of every edge $e$ connecting a pair of vertices in $B'$ is $0$.
	\end{itemize}
\end{definition}


\begin{definition}[The Oracle]\label{def: oracle}
	An oracle for the \MWU framework is an algorithm that, in every iteration, either returns an acceptable path $P$, or returns a cut-witness, or returns ``FAIL''. The probability that the oracle ever returns ``FAIL'' must be bounded by $1/2$.
\end{definition}

================================
Modified acceptable path/path witness



\begin{definition}[Modified Acceptable Path]\label{def: mod acceptable path}
	A path $P$ in the current graph $G$ is called a \emph{modified acceptable path for $G$ with respect to $A_1$ and $B_1$}, if $P$ is a simple path, connecting a vertex of $B_1$ to a vertex of $A_1$, the length of $P$ with respect to the current edge lengths $\hat \ell(\cdot)$ is at most $\Lambda$, and no inner vertices of $P$ belong to $B_1$.
\end{definition}


\begin{definition}[Modified Cut-witness]\label{def: mod cut-witness}
	A \emph{modified cut-witness} for graph $G$ with respect to $A_1$ and $B_1$ is an assignment of lengths $\ell''(e)\geq 0$ to every edge $e\in E(G)$, such that if  we denote by $A',B'$ the current sets $A_1,B_1$ of vertices, and by $E^*$ the set of all special edges with both endpoints in $B'$, then:		
	
	\begin{itemize}
		\item $\sum_{e\in E(G)}\ell''(e)\leq \frac{\Lambda\cdot \Delta}{\eta\log^4n}+\sum_{e\in E(G)\setminus E^*}\hat \ell(e)$; and
		
		\item the distance in graph $G$, with respect to edge lengths $\ell''(\cdot)$, from $B'$ to $A'$ is at least $\frac{\Lambda}{32}$. %, and moreover, the length $\ell''(e)$ of every edge $e$ connecting a pair of vertices in $B'$ is $0$.
	\end{itemize}
\end{definition}

================================
===========================================
st-SP problem:

The input to the $r$-Restricted \stSP problem is a well-structured $n$-vertex graph $G=(L,R,E)$, parameters $N\geq n$, $\Delta\ge 1$, and $1\leq \eta \leq \Delta$,  and two disjoint subsets $A,B$ of vertices of $G$, such that no regular edge of $G$ connects a vertex of $B$ to a vertex of $A$ in $G$, $\Delta\leq n-|B_1|$, and  $\frac{(n-|B_1|)\cdot \eta}{\Delta}\leq 2\cdot 2^{r\cdot \sqrt{\log N}}$ holds.
We also require that $|E|\leq O(n\cdot (n-|B|))$.

Initially, every edge $e\in E(G)$ is assigned a length $\ell(e)$ as follows: if $e$ is a regular edge then $\ell(e)=0$, and otherwise $\ell(e)=1$.
We use a parameter $\Lambda=\frac{(n-|B|) \eta \cdot \log^5n}{\Delta}$, and we initialize $\qset=\emptyset$. While the set $B$ of vertices may change over the course of the algorithm, parameter $\Lambda$ remains unchanged.

The execution of the algorithm for the $r$-restricted \stSP problem consists of at most $\Delta$ iterations. In every iteration $i$, the algorithm must do one of the following:

\begin{itemize}
	\item either return FAIL;
	\item or return a modified cut-witness for $G$ with respect to $A$ and $B$ (see \Cref{def: mod cut-witness});
	\item or return a modified acceptable path $P$ for $G$ with respect to $A$ and $B$ (see \Cref{def: mod acceptable path}).
\end{itemize}

In the former two cases, the algorithm terminates. In the last case, let $b\in B$, $a\in A$ denote the endpoints of path $P$. We remove $a$ from $A$ and $b$ from $B$ and add $P$ to $\qset$. Additionally, the lengths of some of the special edges on $P$ will be doubled; we assume that the algorithm receives a list of all such edges. 

For every special edge $e\in E(G)$, the length of $e$ is doubled once $e$ participates in exactly $\eta$ paths that the algorithm returned, since the last time the length of $e$ was doubled, or since the beginning of the algorithm -- whatever happened last.

Lastly, we require that the probability that the algorithm ever returns ``FAIL'' is bounded by $\frac{1}{2}$.


================================

Reduction thm:
====================================


\begin{theorem}\label{thm: oracle to routing} Suppose there is an algorithm for the $r$-restricted \stSP problem, that, given an input $(G,A,B,\Delta,\eta, N)$ with $|V(G)|=n$, has running time at most $n\cdot (n-|B|)\cdot T(n,\Delta,\eta,N)$. Then there is an algorithm for the $r$-restricted \routeandcut problem, that, on input $(G,A,B,\Delta,\eta, N)$ with $|V(G)|=n$, has running time at most $O\left(n\cdot (n-|B|)\cdot T(n,\Delta,\eta,N)\right)+O(n\cdot (n-|B|))$.
\end{theorem}


====================================
Induction Base:
====================================

\begin{corollary}\label{cor: ind base}
	There is a deterministic algorithm for the $r$-restricted \routeandcut problem, that, on input $(G,A,B,\Delta,\eta, N)$ with $|V(G)|=n$, has running time at most $O\left(n\cdot(n-|B|)\cdot 2^{r\cdot \sqrt{\log N}}\cdot \log N\right )$.
\end{corollary}

==================================
==================================
MaintainCluster problem:
=================================

\begin{definition}\label{def: maintaincluster problem}
	The input to the \maintaincluster problem consists of a perfect well-structured graph $G=(L,R,E)$ with a proper assignment of lengths $\ell(e)$ on its edges $e\in E$, with $|V(G)|=n$, a subset $\beta\subseteq V(G)$ of its vertices, and parameters $N\geq W^0(G)$, $1\leq \Delta\leq N$, $1\leq \eta \leq \Delta$, and $d\geq 2^{\sqrt{\log N}}$, such that $\frac{\Delta\cdot d}{\eta}\leq 2(n-\beta)$. 
	
	The algorithm consists of at most $\Delta$ iterations.
	At the beginning of every iteration $i$, the algorithm is given two vertices $x,y\in V(G)$, and it must return a simple path $P_i$ in $G$ connecting $x$ to any vertex $y'\in \beta\cup\set{y}$, such that the length of the path is at most $d$, and no inner vertices on the path lie in $\beta$. (We may sometimes say that the algorithm is given a \shortpath query between the pair $(x,y)$ of vertices, and it returns the path $P_i$ in response to the query). After that the length of some edges on path $P_i$ may be doubled, and, if $y'\in \beta$, then $y'$ may be deleted from set $\beta$. We are guaranteed that the following property holds:
	
	
	\begin{properties}{P}
		\item If $\tau'>\tau$ are two times at which the length of some edge $e\in E(G)$ is doubled, then the algorithm returned at least $\eta$ paths in response to queries during the time interval $(\tau,\tau']$ that contained $e$.
		\label{maintaincluster-prop: edge congestion}
	\end{properties}
	
	The algorithm may, at any time, produce a strongly well-structured cut $(X,Y)$ in $G$ of sparsity $\Phi_G(X,Y)\leq \phi$, where $\phi= \frac{2^{\sqrt{\log N}}}{d}$.
	If $w(X)\leq w(Y)$, then let $Z=X$ and $Z'=Y$; otherwise, let $Z=Y$ and $Z'=X$. We also let $J'\subseteq Z'$ denote the set of vertices that serve as endpoints of the edges of $E_G(X,Y)$. The vertices of $Z\cup J'$ are then deleted from $G$, and the algorithm continues with the resulting graph $G=G[Z'\setminus J']$. Note that with this modification we are guaranteed that $G$ remains a perfect well-structured graph. Once $|V(G)|\leq n/2$ holds, the algorithm terminates, even if fewer than $\Delta$ iterations have passed.
	
	The algorithm may also, at any time, return ``FAIL''. The probability that the algorithm ever returns ``FAIL'' must be bounded by $1/N^2$. 
	
	For an integer $1\leq r\leq \ceil{\sqrt{\log N}}$, we say that an instance $(G,\beta,\Delta,\eta,d,N)$ of the \maintaincluster problem is $r$-restricted, if $d\leq 2^{r\cdot\sqrt{\log N}}$.
\end{definition}

===============================
First direction
===============================

\begin{theorem}\label{thm: from maintaincluster to roundandcut}
	Suppose there exists a randomized algorithm for the $r$-restricted \maintaincluster problem, for some parameter $r\geq 1$, that, given as input  an instance
	$(G,\beta,\Delta,\eta,d,N)$ of the problem, has running time at most: 
	$c_1\cdot W^0(G)\cdot (W^0(G)-|\beta'|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$, where $\beta'$ is the set $\beta$ at the end of the algorithm. Then there is a randomized algorithm for the $(r+1)$-restricted \routeandcut problem, that, given as input
	an instance	$(G,A,B,\Delta,\eta,N)$ of the problem with $|V(G)|=n$, %either produces a valid output to the problem, or returns ``FAIL'', such that the probability that the algorithm returns ``FAIL'' is at most $1/2$, and its running time is bounded by 
	has running time at most $c_1\cdot n\cdot (n-|B|)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r+8c_2}$. 
\end{theorem}

===================================
===================================
$\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$
=====================================
The problem on H:
==================================


Throughout the algorithm, we use the parameter  $\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$.
We let $H$ be the graph that is obtained from $G$, by adding a source vertex $s$, that connects to every vertex $a\in A$ with a length-$0$ edge, and a destination vertex $t$, to which every vertex $b\in B$ connects with a length-$0$ edge. If an edge $e\in E(G)$ is a special edge for graph $G$, then $e$ remains a special edge for $H$. All other edges of $H$, including edges incident to $s$ and $t$, are called regular edges.
For every edge $e\in E(G)$, its length in $H$ remains the same as in $G$, so for convenience, we denote the length of every edge $e\in E(H)$ by $\ell(e)$.

Recall that, at the beginning  of the algorithm, for each edge $e\in E(H)$, its length $\ell(e)$ is set as follows: if $e$ is a regular edge, then $\ell(e)=0$, and if $e$ is a special edge, then $\ell(e)=1$. 
We start by setting $\qset=\emptyset$, and then perform at most $\Delta$ iterations. In every iteration, the algorithm must do one of the following:


\begin{properties}{R}
	\item either return FAIL;\label{outcome: fail}
	
	\item or return a simple $s$-$t$ path $P$ of length at most $\Lambda$ in the current graph $H$, such that $P$ contains exactly one vertex of $B$ -- the penultimate vertex on the path; \label{outcome:path}
	
	\item or compute an assignment $\ell'(e)\geq 0$ of lengths to all edges $e\in E(H)$, such that, if we denote by $E^*$ the set of all edges of $G$ with both endpoints in $B$, then $\sum_{e\in E(H)}\ell'(e)\leq \frac{\Lambda\cdot \Delta}{\eta \log^4n}+\sum_{e\in E(H)\setminus E^*}\ell(e)$; the length $\ell'(e)$ of every edge $e$ that is incident to $s$ or to $t$ is $0$; and the distance from $s$ to $t$ in $H$, with respect to edge lengths $\ell'(\cdot)$, is at least $\frac{\Lambda}{32}$;  \label{outcome: cut}
\end{properties}

Note that, if the algorithm returns assignments of lengths $\ell'(e)$ to edges $e\in E(H)$ as in Outcome \ref{outcome: cut}, then these assignments of edge lengths define a modified cut-witness for $G$ (see \Cref{def: mod cut-witness}). In this case, the algorithm terminates, and  returns the  lengths $\ell'(e)$ of all edges $e\in E(H\setminus\set{s,t})$. Slightly abusing the notation, for the sake of simplicity, we will call an assignment of lengths $\ell'(e)$ to the edges $e\in E(H)$ as  described in Outcome \ref{outcome: cut} a \emph{cut-witness}. 

If the algorithm returns an $s$-$t$ path $P$ as in Outcome \ref{outcome:path}, then $P\setminus\set{s,t}$ is a modified acceptable path for $G$ (see \Cref{def: mod acceptable path}). To simplify the notation, we say that a path $P$ described in  Outcome \ref{outcome:path} is an \emph{acceptable path}. If the algorithm returns an acceptable path $P$, then we let $P'=P\setminus\set{s,t}$, and we let $a\in A$, $b\in B$ be the endpoints of path $P'$. We remove $a$ from $A$ and $b$ from $B$, add $P'$ to $\qset$, and delete the edges $(s,a)$ and $(b,t)$ from $H$. Additionally, the lengths of some of the special edges on $P$ may be doubled; we assume that the algorithm receives the list of all such edges. 

From the problem definition, for every special edge $e\in E(H)$, the length of $e$ is doubled once $e$ participates in exactly $\eta$ paths that the algorithm returned since the last time the length of $e$ was doubled, or since the beginning of the algorithm -- whatever happened last.

Lastly, in the case of Outcome \ref{outcome: fail}, we terminate the algorithm and return ``FAIL'', but we require that the probability that the algorithm ever returns ``FAIL'' is bounded by $\frac{1}{2}$.

=====================================
 $\highlightf{N'=\max\set{N,8n\cdot \log^5n}}$. 
 ==============================
 
 Let $\tau$ be any time in the algorithm's execution, and let $H'$ be any subgraph of $H\setminus\left (\set{s,t}\right )$ that is a perfect well-structured graph. The total weight of all vertices of $H'$ must be bounded by $N'$. 
 
\begin{equation}\label{eq: bound on log n'}
\log N'\leq \log N+6\log\log N\leq \left(1+\frac{1}{64c_2r}\right)\log N,
\end{equation}

\begin{equation}
2^{\sqrt{\log N'}}\leq 2^{\sqrt{\log N}}\cdot 6\log N\leq 2^{2\sqrt{\log N}}.\label{eq: bound on N'}
\end{equation}




==> temp.tex <==
================================
Route and Cut Problem
==============================

\begin{definition}[\routeandcut problem]\label{def: rounte and cut}
	The input to the \routeandcut problem is a well-structured $n$-vertex graph $G=(L,R,E)$, that is given in the adjacency-list representation, 
	parameters $N\geq n$, $\Delta\geq 1$, and $1\leq \eta \leq \Delta$, and two disjoint subsets $A,B$ of vertices of $G$, with $|A|,|B|\geq \Delta$. 
	
	The output of the problem is a (possibly partial) routing $\qset$ from $A$ to $B$, whose congestion is bounded by  $4\eta\log N$. Additionally, if $|\qset|<\Delta$, the output must contain a cut  $(X,Y)$ in $G$ with $|E_G(X,Y)|\leq \frac{64\Delta}{ \eta\log^4n}+\frac{256|\qset|}{\eta}$, such that, if 
	$A'\subseteq A, B'\subseteq B$ denote the subsets of vertices that do not serve as endpoints of the paths in $\qset$, then $A'\subseteq X$ and $B'\subseteq Y$ hold. The algorithm for the \routeandcut problem is also allowed to return ``FAIL'' without producing any output, but the probability of the algorithm doing so must be bounded by $1/2$.
	
	We say that an instance $(G,A,B,\Delta,\eta,N)$ of the \routeandcut problem is  \emph{$r$-restricted}, for an integer $1\leq r\leq \ceil{\sqrt{\log N}}$, iff $\frac{(n-|B|)\cdot \eta}{\Delta}\leq 2^{r\cdot \sqrt{\log N}}$ holds.
\end{definition}

================================
MaintainCluster Problem
==============================

\begin{definition}\label{def: maintaincluster problem}
	The input to the \maintaincluster problem consists of a perfect well-structured graph $G=(L,R,E)$ with $|V(G)|=n$, together with a proper assignment of lengths $\ell(e)$ on its edges $e\in E$, and parameters $N\geq W^0(G)$, $1\leq \Delta\leq N$, $1\leq \eta \leq \Delta$, and $d\geq (\log N)^{64}$, such that $\frac{\Delta\cdot d}{\eta}\leq 2n$, and $N$ is greater than a sufficiently large constant. 
	
	The algorithm consists of at most $\Delta$ iterations.
	At the beginning of every iteration $i$, the algorithm is given two vertices $x,y\in V(G)$, and it must return a simple path $P_i$ in $G$ connecting $x$ to $y$ of length at most $d$. (We may sometimes say that the algorithm is given a \shortpath query between the pair $(x,y)$ of vertices, and it returns the path $P_i$ in response to the query). After that the length of some special edges on path $P_i$ may be doubled. We are guaranteed that the following property holds:
	
	
	\begin{properties}{P}
		\item If $\tau'>\tau$ are two times at which the length of some edge $e\in E(G)$ is doubled, then the algorithm returned at least $\eta$ paths in response to queries during the time interval $(\tau,\tau']$ that contained $e$.
		\label{maintaincluster-prop: edge congestion}
	\end{properties}
	
	
	The algorithm may, at any time, produce a strongly well-structured cut $(X,Y)$ in $G$ of sparsity $\Phi_G(X,Y)\leq \frac{(\log N)^{64}}{d}$.
	If $w(X)\leq w(Y)$, then let $Z=X$ and $Z'=Y$; otherwise, let $Z=Y$ and $Z'=X$. We also let $J'\subseteq Z'$ denote the set of vertices that serve as endpoints of the edges of $E_G(X,Y)$. The vertices of $Z\cup J'$ are then deleted from $G$, and the algorithm continues with the resulting graph $G=G[Z'\setminus J']$. Note that with this modification we are guaranteed that $G$ remains a perfect well-structured graph. Once $|V(G)|\leq n/2$ holds, the algorithm terminates, even if fewer than $\Delta$ iterations have passed.
	
	The algorithm may also, at any time, return ``FAIL''. The probability that the algorithm ever returns ``FAIL'' must be bounded by $1/N^4$. 
	
	For an integer $1\leq r\leq \ceil{\sqrt{\log N}}$, we say that an instance $(G,\Delta,\eta,d,N)$ of the \maintaincluster problem is $r$-restricted, if $d\leq 2^{r\cdot\sqrt{\log N}}$.
\end{definition}


=



================================
The theorem
==============================

\begin{theorem}\label{thm: from routeandcut to maintaincluster part 2}
	Suppose that, for some parameter $r\geq 1$, there exists a randomized algorithm for the $r$-restricted \routeandcut problem, that, given as an input an instance $(G,A,B,\Delta,\eta,N)$ of the problem with $|V(G)|=n$,
	has running time at most $c_1\cdot n\cdot (n-|B|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2(r-1)+8c_2}$. Then there exists a randomized algorithm for the $r$-restricted \maintaincluster problem, that, on input $(G,\Delta,\eta,d,N)$ has running time at most: $c_1\cdot  (W^0(G))^2\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2r}$.
\end{theorem}


============================
==================
=======================
Input params and inequalitites
=======================

$N\geq W^0(G)$,  
$r\leq \ceil{\sqrt{\log N}}$,
$1\leq \Delta\leq N$, 
$1\leq \eta \leq \Delta$, 
$(\log N)^{64} \leq d\leq 2^{r\cdot \sqrt{\log N}} $,  $\frac{\Delta\cdot d}{\eta}\leq 2n$.
$d\leq \frac{|V(G)\cdot \eta}{\Delta}$
$n>\Delta/\eta$.

$d_X=\min\set{\frac{|X^0|\cdot \eta}{\Delta},d}$


\begin{equation}\label{eq: bound on d} 
d\leq \frac{2n\eta}{\Delta}\leq 2n.
\end{equation}

Since $d\geq (\log N)^{64}$, we get that $(\log N)^{64}\leq 2n\leq 2N$, and so:

\begin{equation}\label{eq: comparing logs}
\log\log N\leq \log n\leq \log N.
\end{equation}


\begin{equation}\label{eq: more logs}
\log (12N)=3+\log N\leq \left(1+\frac{1}{32c_2r}\right )\log N.
\end{equation}


\begin{equation}\label{eq: even more logs}
2^{c_2\sqrt{\log(16N)}}\leq 2^{2c_2}\cdot 2^{c_2\sqrt{\log N}}\leq  2^{c_2\sqrt{\log N}}\cdot \log N,
\end{equation}


\begin{equation}\label{eq comparing other logs}
\log n-1\leq \log W\leq 4\log n.
\end{equation}

===========================
=====================


\begin{observation}\label{obs: final length of edges}
	\[ \sum_{e\in E^{\spec}}\ell^*(e)\leq 2\sum_{e\in E^{\spec}}\ell^0(e)+\frac{2d\Delta}{\eta} \leq  2\sum_{e\in E^{\spec}}\ell^0(e)+4n.  \]
\end{observation}
===========================
 $|V(H)|\leq 12W^0$ always holds.
 ============================
 
 $d'$, that is the smallest integral power of $2$ that is greater than $\frac{d}{(\log N)^{28}}$, 
 
 $\phi=\frac{4}{d'}$.
 
  as the algorithm does not terminate, $\sum_{e\in E(G)}\ell(e)\geq \frac{|V(G)|}{2}\geq \frac{n}{4}>d'$ must hold.
====================
Phases:

A phase terminates if one of the following happened: (i) the algorithm returned ``FAIL'', in which case we say that the phase is of \emph{type 1}; or (ii) at least $\frac{\hat W}{\log^{30}N}$ vertices have been deleted from graph $H$ during the current phase, where $\hat W$ is the number of vertices in $H$ at the beginning of the phase, in which case we say that the phase is of \emph{type 2}; or (iii) at least $\Delta'=\frac{\Delta}{\log^{30}N}$ queries have been responded to; in which case we say that the phase is of \emph{type 3}.

=============================
$\Delta'=\frac{\Delta}{\log^{30}N}$
===========================

Bad events:
=========================
 $\event_1$: $|T|>\frac{8\hat W}{d'}$ or $|T|<\frac{\hat W}{2d'}$

if $\event_1$ does not happen, then $\frac{\hat W}{2d'}\leq |T|\leq \frac{8\hat W}{d'}$
==============================

$\event_2$ happens if there is a weakly well-structured cut $(A,B)$ in $H$, with $|A\cap T|,|B\cap T|\geq \frac{|T|}{\log^4N}$, and $|E_H(A,B)|\leq \frac{|T|}{\log^6N}$, such that, if we denote by $E'=E_H(A,B)$, then for every canonical cut $(A',B')\in \cset'(E')$, either $|A'|\leq \frac{\hat W}{\log^{5}N}$, or $|B'|\leq \frac{\hat W}{\log^{5}N}$


since $d'\leq  \frac{8 W}{\log^{28}N}$ from Inequality \ref{eq: bound on d'}

======================================


 $\event_3$ happens if there is 
a weakly well-structured cut $(A,B)$ in $H$, with $|E_H(A,B)|\leq \frac{|T|}{\log^6N}$, such that one of the sides of the cut contains at least $\frac{\hat W} 2$ vertices of $H$ and at most $\frac{|T|}{32}$ vertices of $T$, and additionally,  if we denote by $E'=E_H(A,B)$, then for every canonical cut $(A',B')\in \cset'(E')$, either $|A'|\leq \frac{\hat W}{\log^{5}N}$, or $|B'|\leq \frac{\hat W}{\log^{5}N}$ holds.

====================================

$\event_4$, happens if there is some edge $e\in E(G)$, such that at least $16\log N$ vertices of $P^*(e)$ are in $T$.


Lastly, we let $\event$ be the bad event that either of the events $\event_1,\event_2$, $\event_3$, or $\event_4$ happened. Clearly:

\[\prob{\event}\leq 1 {16}.\]

==================================
Finalizing cuts:
=====================================

\begin{definition}\label{def: finalizing cut}
	Let $(A,B)$ be a cut in graph $H$ at any time during the execution of a phase. We say that the cut $(A,B)$ is a \emph{finalizing} cut, if the following hold:
	
	\begin{itemize}
		\item all edges in $E_H(A,B)$ are special edges; 
		\item $|E_H(A,B)|\leq \frac{|T|}{8\log^6N}$; and
		\item one of the sides of the cut $Z\in \set{A,B}$ contains at least $|V(H)|-\frac{\hat W}{32}$ vertices of $H$, and at most $|T|\cdot \left(1-\frac{7}{\log^4N}\right )$ vertices of $T$.
	\end{itemize}
\end{definition}

=======================================

\begin{claim}\label{claim: compute intermediate cut}
	There is a deterministic algorithm, that, given the graph $G_0$, the sequence of the strongly well-structured $\phi$-sparse cuts $(A_1,B_1),\ldots(A_q,B_q)$ in $G$ that the algorithm has produced during the current phase so far, the current graphs $G$ and $H$, such that all edge lengths in $G$ are bounded by $d'/2$, and the finalizing cut $(\tilde A,\tilde B)$ in the current graph $H$, computes a weakly well-structured cut $(\tilde S,\tilde S')$ in $H_0$, such that $|E_{H_0}(\tilde S,\tilde S')|\leq \frac{|T|}{\log^6N}$, and one side $\tilde Z\in \set{\tilde S,\tilde S'}$ of the cut contains all but at most $\hat W/8$ vertices of $H_0$, and at most $\left(1-\frac{2}{\log^4N}\right )\cdot |T|$ vertices of $T$. The 
	running time of the algorithm is $O(\hat W^2)$.
\end{claim}
===================================================





\begin{claim}\label{claim: finalizing cut}
	Suppose, at any time during the execution of a phase, there is a finalizing cut $(\tilde A,\tilde B)$ in the current graph $H$. Assume further that neither of the events $\event_2,\event_3$ has happened, and that every edge in the current graph $G$ has length at most $d'/2$. Then there is a strongly well-structured $\phi$-sparse cut $(A^*,B^*)$ in the current graph $G$, such that $w(A^*),w(B^*)\geq \frac{\hat W}{\log^{30}N}$. Moreover, there is a deterministic algorithm, that, given the graph $G$ at the beginning of the current phase (that we denote by $G_0$), the sequence of the strongly well-structured $\phi$-sparse cuts $(A_1,B_1),\ldots(A_q,B_q)$ in $G$ that the algorithm has produced during the current phase so far,  the current graphs $G$ and $H$, and the finalizing cut $(\tilde A,\tilde B)$ in the current graph $H$, either correctly estabishes that at least one of the events $\event_2,\event_3$ has happened,  or computes a strongly well-structured $\phi$-sparse cut $(A^*,B^*)$ in the current graph $G$, such that $w(A^*),w(B^*)\geq \frac{\hat W}{\log^{30}N}$. The running time of the algorithm is $O(\hat W^2)$.
\end{claim}
================================================
===============================================
===============================================

\begin{lemma}\label{lem: phase 1 embed expander}
	There is a randomized algorithm, that either returns ``FAIL'', or computes one of the following:
	
	\begin{itemize}
		\item either  a finalizing cut in $H$; 
		\item or a strongly well-structured $1/d'$-sparse cut $(A,B)$ in $G$ with $w(A),w(B)\geq \frac{\hat W}{(\log N)^{30}}$;
		
		\item or a graph $X^*$ with $V(X^*)=T$, such that $X^*$ has maximum vertex degree at most $24$, and it is an $\frac{\alpha_0}{81}$-expander. In the latter case, the algorithm additionally computes a set $F\subseteq E(X^*)$ of at most $\frac{\alpha_0\cdot |T|}{500}$ edges, and an embedding $\pset^*$ of $X^*\setminus F$ into $H$ via paths that have length at most $O\left (d'\cdot  (\log N)^{15}\right )$ each, that cause congestion $O\left((\log N)^{13}\right )$. 
	\end{itemize}
	
	The probability that the algorithm returns ``FAIL'' is at most $\frac{1}{N^7}$, and the running time of the algorithm is bounded by:
	
	\[O\left( c_1\cdot \hat W^{2} \cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2(r-1)+8c_2+2} \right ).\]
\end{lemma}

=================
$d''=\Theta\left (d'\cdot  (\log N)^{15}\right )$ and $\eta''=\Theta\left((\log N)^{13}\right )$
=====================
$\hat d=\frac{2^{30}\log \hat W}{\alpha_0}$. 




Failure probability:

1. event $\event$: prob $1/16$
2. algorithm for constructing expander:  \Cref{lem: phase 1 embed expander}, probl $\frac{1}{N^7}$,
3. Algorithm for connecttocenters: each has $1/N^7$ failure probability.
===================

Throughout, we use a distance parameter $\hat d=\frac{2^{30}\log \hat W}{\alpha_0}$.
Throughout the phase, we maintain an arbitrary vertex  $v\in V(X)$,
and two shortest-paths trees $\hat \tau'$ and $\hat \tau''$ rooted at $v$ in graph $X\setminus F$, where the edges in $\hat \tau'$ are directed away from $v$, and the edges in $\hat \tau''$ are directed towards $v$. In other words, for every vertex $a\in V(X)$, the unique $s$-$a$ path in $\hat \tau'$ is a shortest $s$-$a$ path in $X\setminus F$, and the unique $a$-$s$ path in $\hat \tau''$ is a shortest $a$-$s$ path in $X\setminus F$. Note that both trees can be computed in time $O(|T|)$, since $|V(X)|\leq |T|$, and maximum vertex degree in $X$ is $O(1)$. Whenever an edge or a vertex are deleted from $X$, we recompute both trees from scratch, selecting a new root vertex $v\in V(X)$ if needed. Since $|E(X)|\le O(|T|)$, the trees need to be recomputed at most $O(|T|)$ times, and so the total time spent over the course of the phase on computing the two trees is bounded by $O(|T|^2)\leq O((W^0)^2)$.



$\Lambda=(n-|B^0|)\cdot \frac{ \eta \cdot \log^5n}{\Delta}$
We have $\Delta$ iterations. So time is $(n-|B^0|)\cdot\eta\leq (n-|B^0|)\cdot \Delta$, $\Delta<n$.


$d_X=\min\set{\frac{|X^0|\cdot \eta}{\Delta}$
	So $\Delta\cdot d\leq |X^0|\cdot \eta$.
Can get $W^0\cdot \eta$
@@

==> temp2.tex <==

\begin{definition}[\connecttocenters problem]
	The input to the \connecttocenters problem consists of a perfect well-structured graph $G=(L,R,E)$ with $|V(G)|=n$, and a proper assignment $\ell(e)$ of lengths to the edges $e\in E$, that are given in the adjacency list representation, together with a subdivided graph $H$ corresponding to $G$ in the adjacency-list representation. Let $W^0$ denote the weight of all vertices in this initial graph $G$. Additionally, we are given  a parameter $N\geq \max\set{n,W^0/8}$ that is greater than a large enough constant, and parameters $d'>0$,  and $1\leq r\leq \sqrt{\log N}$, and $d'\leq\min\set{\frac{2^{r\sqrt{\log N}}}{\log^8N},\frac{n}{8}}$. Lastly, we are given a set $\beta\subseteq V(H)$ of vertices, with $|\beta|\geq \frac{W^0}{256d'}$. We denote by $\beta^0$ the initial set $\beta$.
	
	
	The algorithm consists of a number of phases, and every phase is partitioned into iterations. In every iteration, the algorithm is required to return one of the following:
	
	\begin{properties}{O}
		\item either a valid \LCDS in the current graph $G$ with the parameter  $\rho=\frac{2^{12}\cdot W^0\cdot \log^3N}{|\beta^0|}$, in which Requirement \ref{prop: routing paths} is relaxed to allow the lengths of the paths in $\bigcup_{i=1}^{\lambda-1}\qset_i$ to be bounded by $16d'\log^9N$ and $U_{\lambda}=\emptyset$; \label{outcome: LCDS}
		
		\item or a strongly well-structured $\frac{1}{d'}$-sparse cut $(A,B)$ in $G$ with $w(A)\geq 1.8|\beta\cap A|$;\label{outcome: sparse cut}
		
		\item or  a weakly well-structured cut $(A',B')$ in graph $H$, with $|A'|\geq \frac{511|V(H)|}{512}$,  $|A'\cap \beta|<\frac{2|\beta|}{\log^3N}$, and $|E_H(A',B')|\leq  \frac{|V(H)|}{d'\cdot \log^6N}$. \label{outcome: finalizing cut}
	\end{properties}
	
	In the case of Outcome \ref{outcome: finalizing cut}, the algorithm terminates. In the case of Outcome \ref{outcome: sparse cut}, the endpoints of the edges in $E_G(A,B)$ are deleted from $G$, and some additional vertices may be deleted from $\beta$. Additionally, if  $w(A)\leq w(B)$, then the vertices of $A$ are deleted from $G$, and otherwise the vertices of $B$ are deleted from $G$. In case of Outcome \ref{outcome: LCDS}, the current phase terminates, and the algorithm is given a collection of special edges of $G$, whose lengths are doubled, together with a list of vertices that are deleted from $\beta$.
	
	Once the total increase in the edge lengths becomes greater than $16n$, or at least $3/4$ of vertices in the initial set $\beta$ are deleted from $\beta$, the algorithm terminates. The algorithm may also return ``FAIL'' and terminate at any time, but we require that the probability that this ever happens is bounded by $\frac{1}{16}$.
\end{definition}



\begin{theorem}\label{thm: connecttocenters}
	Suppose that, for some parameter $r\geq 1$, there exists a randomized algorithm for the $r$-restricted \routeandcut problem, that, given as an input an instance $(G,A,B,\Delta,\eta,N)$ of the problem with $|V(G)|=n$,
	has running time at most $c_1\cdot n\cdot (n-|B|)\cdot 2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2(r-1)+8c_2}$.
	Then there is a randomized algorithm for the \connecttocenters problem, for the same value of parameter $r$, whose running time is at most:

\[	O\left(c_1\cdot W^0\cdot ( W^0-|\beta^0|+|\beta'|
	\cdot \rho +\Lambda)\cdot  2^{c_2\sqrt{\log N}}\cdot (\log N)^{16c_2(r-1)+8c_2+22}\right ),\]
	
	 where $\Lambda$ is the total increase in the edge lengths over the course of the algorithm, $\beta'$ is the set of all vertices deleted from $\beta$ over the course of the algorithm (including the vertices that are deleted from $H$ following updates to graph $G$), and $W^0$ is the total initial weight of the vertices in the input graph $G$. 
\end{theorem} 


$|\beta|\geq \frac{7|V(G)|} 8$, 
$N\geq W^0(G)$, 
$1\leq \Delta\leq \frac{|\beta|}{(\log N)^{128}}$, 
$1\leq \eta \leq \Delta$, 
 $d\geq (\log N)^{64}$, 
 
 $\frac{\Delta\cdot d}{\eta}\leq |V(G)|-|\beta|+\Delta\cdot (\log N)^{64}$. 
 
$1\leq r\leq \ceil{\sqrt{\log N}}$, 
$d\leq 2^{r\cdot\sqrt{\log N}}$.
